Distribution Estimation for Probabilistic Loops

We present an algorithmic approach to estimate the value distributions of random variables of probabilistic loops whose statistical moments are (partially) known. Based on these moments, we apply two statistical methods, Maximum Entropy and Gram-Charlier series, to estimate the distributions of the loop's random variables. We measure the accuracy of our distribution estimation by comparing the resulting distributions using exact and estimated moments of the probabilistic loop, and performing statistical tests. We evaluate our method on several probabilistic loops with polynomial updates over random variables drawing from common probability distributions, including examples implementing financial and biological models. For this, we leverage symbolic approaches to compute exact higher-order moments of loops as well as use sampling-based techniques to estimate moments from loop executions. Our experimental results provide practical evidence of the accuracy of our method for estimating distributions of probabilistic loop outputs.

==> Distribution Recovery (27)/ImplementationAndNumericalResults.tex <==
%\vspace{5mm}

\section{Experimental Evaluation}\label{section:ImplEvaluation}
In this section we report on our  experimental results towards estimating distributions of probabilistic loop variables using Algorithm~\ref{fig:algo}. We describe our benchmark set and present our practical findings using these benchmarks. {We also describe additional results on evaluating the precision of higher-order moments of loop variables. }
%\Ahmad{Here, as we dropped the table of exact moments, I revised table references and ..., I also added a paragraph to end of Sec. 4 explaining Table 2. I appreciate if you double check it: }


\begin{table}[t!]
    \centering
     \scalebox{1}{
 \begin{tabular}{c|c|c|l|l|l|l}
\toprule
          {\bf Program}   &  Var & $|S_{\text{M}}|$ & $\chi_{\me}^2$  &$\chi_{\gc}^2$ &  $D_{\me}^\ast$  & $D_{\gc}^\ast$\qquad\\\hline\hline
     StutteringP~\cite{bartocci2019automatic}& $s$ & 2 &18.6432 \cmark& 16.7943 \cmark& 0.0181 \cmark & 0.0213 \cmark \\%\hline
     %
     Square~\cite{bartocci2019automatic} & $y$ & 2 &36.9009 \xmark& 39.1309 \xmark &  0.0586 \cmark & 0.0566 \cmark\\%\hline
     %
     Binomial~\cite{Feng2017} & $x$ & 2 &27.4661 \xmark& 27.4574 \xmark&  0.0598 \cmark &  0.0597 \cmark \\%\hline
     %
   Random Walk 1D~\cite{Kura19} & $x$&  2 &18.6709 \cmark \hspace{2mm}& 18.7068 \cmark \hspace{2mm}&   0.0264 \cmark \hspace{2mm}&  0.0263 \cmark \hspace{2mm}\\%\hline
     %
    Uniform(0,1) & $u$ & 6 &16.3485 \cmark& 105.276 \xmark&  0.0214 \cmark & 0.0658 \xmark \\%\hline
    %
    Vasicek Model & $r$&  2 &17.4018 \cmark & 17.4017 \cmark & 0.0360 \cmark & 0.0360 \cmark\\
    %
     PDP Model &  $x$ & 3 & 64.4182 \cmark & 65.9500 \cmark &  0.0403 \cmark & 0.0393 \cmark \\\bottomrule
\end{tabular}
}
\vspace{2mm}
 \caption{Accuracy of the ME and GC expansion pdf estimates for  benchmarks PPs, assessed with  
 the chi-square and K-S statistical tests. \label{table:DKL-Chi2-K-SforBenchmarks}}
\end{table}



\paragraph{{\bf Benchmarks.}}%\label{section:Benchmarks}
%\subsection{Programs with Unknown Target Distribution} 
For evaluating our approach in Algorithm~\ref{fig:algo}, we use four  challenging examples of unbounded probabilistic loops from state-of-the-art approaches on quantitative analysis of PPs~\cite{Feng2017,Kura19,bartocci2019automatic}; these benchmarks are the first four entries of the first column of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}. %\lk{where is the Uniform benchmark coming from, which paper? It is not from~\cite{bartocci2019automatic,moosbrugger2021automated}} 
%\ms{I came up with the benchmark to have a conprison to an exact distribution coming from a PP  }
In addition, we also crafted three new examples, listed in the last three  entries of the first column of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}, as follows: (i) line~5 of Table~\ref{table:DKL-Chi2-K-SforBenchmarks} specifies a PP loop approximating a uniform distribution; (ii)  line~6 of Table~\ref{table:DKL-Chi2-K-SforBenchmarks} refers to the Vasicek model of Fig.~\ref{fig:vasicek-intro}; and (iii) 
the last line of Table~\ref{table:DKL-Chi2-K-SforBenchmarks} lists an example encoding a piece-wise deterministic process (PDP) modeling gene circuits based on~\cite{innocentini2018time}. In particular, the PDP model we consider 
can be used to estimate the distribution of protein $x$ and the mRNA levels $y$ in a gene; our PP encoding of this PDP model is given in Fig.~\ref{fig:PDPmodelPPandMoments}.


%{\bf StutteringP} - bartocci2019automatic
%Square - bartocci2019automatic
%Binomial- Feng2017
%{\bf Random Walk 1D} - Kura19
% {\bf Uniform} - ???
% \begin{table}[t!]
%     \centering
%     \scalebox{0.8}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & \#Mom. &  Exact Moments \\
%                          \hline
%                          \hline
%  \multirow{3}{*}{StutteringP~\cite{bartocci2019automatic}}&1& $\E(s(n)) = 3np $ \\\cline{2-3}
%     &2& $\E(s^2(n)) = 9n^2p^2 - 9np^2+32np/3$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{}$\E(s^3(n)) = 3np(9n^2p^2 - 27np^2 + 32np + 18p^2 - 32p + 14)$
%     % 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
%     %   & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
%     %   & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
%     %   & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
%     %   & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
%     \\\hline
%         \hline
% \multirow{3}{*}{Square~\cite{bartocci2019automatic}}&1& $\E(y(n)) = n^2+n$  \\\cline{2-3}
%     &2&$\E(y^2(n)) = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
%     &3&$\E(y^3(n)) = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
%         \hline
        
% \multirow{3}{*}{Binomial~\cite{Feng2017}}&1&$\E(x(n)) = np$  \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^2p^2 + np(1-p)$  \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
%         \hline 
                

% \multirow{3}{*}{Random Walk 1D~\cite{Kura19}}&1&$\E(x(n)) =  n/5$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^2/25 + 22n/75$   \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^3/125 + n^222/125 - n21/250$   \\\hline
%         \hline   

% \multirow{3}{*}{Uniform(0,1)}&1& $\E(u(n))=2^{-n}(2^n - 1)/2$ \\\cline{2-3}
%     &2&$\E(u^2(n))=2^{-3n}(2^{3n+1} + 2^n - (3)4^n)/6$  \\\cline{2-3}
%     &3&$\E(u^3(n))=2^{-3n}(-2^{2n+1} + 2^n + 8^n)/4$  \\\hline\hline
    
% \multirow{2}{*}{Vasicek Model - Fig.~\ref{fig:vasicek-intro}}& 1 & $\E(r(n)) = 2^{-n}(2^n + 9)/5$\\\cline{2-3}
% & 2& $\E(r^2(n)) = 7/75 + (18)2^{-n}/25 + (239)2^{-2n}/75$ \\\hline\hline

% \multirow{3}{*}{PDP Model for}&1& $\E(x(n)) = 1000^{-n}\big((24960)10^{3n}- (1944)300^n + (13720)500^n- (36736)800^n\big)/21$ \\
%  % & &$- (36736)800^n\big)/21$\\
%   \cline{2-3}
  
% &2&$\E(x^2(n)) = (2.62144\times 10^{27})^{-n}[-51514624000(1.048576\times 10^{27})^n $\\
%   Gene Circuits & &$+ 31603353600(1.31072\times 10^{27})^n+ 59761049600(1.6777216\times 10^{27})^n $ \\
%   Fig.~\ref{fig:PDPmodelPPandMoments}  &&$- 84619591680(2.097152\times 10^{27})^n + 30050150400  (2.62144\times 10^{27})^n $\\ 
%     & &$- 413683200 (3.93216\times 10^{26})^n+ 2326579200(6.291456\times 10^{26})^n$ \\
%     & &$- 2546790400  (6.5536\times 10^{26})^n+ 15353556480  (7.86432\times 10^{26})^n ]/20349$\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Benchmarks and their Exact Moments. \lk{Table 4 states that only 2 moments have been used for estimations in StutteringP; which is then the case?}\Ahmad{for StutteringP, Square, Binomil, and RandomWalk we used 2 moments for estimation. For Uniform 6 moments, and for Vasicek 2 momets, nd for PDP model for Gene ciruits we used 3 moments for estimation.}}
%  \label{Tab:Benchmarks}
% \end{table}


%
%The  protein ($x$) and and mRNA ($y$)  levels of the
%gene are continuous program variables. The binary variable with values 
%$s\in\{0, 1\}$ represents the promoter states (0 stands for %OFF
%and 1 stands for ON). 
%The switch between values of $s$ happens with probabilities $f$ and $h$, thus $s$ can be modelled using a Markov chain. %f from ON to OFF, h from OFF to ON
%The transcription initiation rates in states 0 and 1 are %$k_0$ and $k_1$, respectively. The translation rate is $b$, %$\rho$ is the mRNA and $a$ the protein degradation rate.
%The protein and mRNA concentrations follow the ODEs
%
%
%\begin{align}\label{PDP}
%&\frac{dy}{dt}=\begin{cases}
%k_0-\rho y & \text{if} \quad s=0\\
%k_1-\rho y &  \text{if} \quad  s=1\\
%\end{cases}\notag\\
%&\frac{dx}{dt}=by-ax
%\end{align}
 
 %We modify  the model by setting $dt=1$ in order to induce discrete-time recurrences, and translate the PDP model \eqref{PDP} for gene circuits to the prob-solvable probabilistic program in Fig.~\ref{fig:PDPmodelPPandMoments} (left).  The moments of  $x$ as functions of loop iteration calculated by Polar \cite{Moosbruggeretal2022} are given Table~\ref{Table:Benchmarks} in Appendix~\ref{Appendix}. A histogram of sampled data, as well as the ME and GC estimated pdfs using the first 3 moments, are drawn in Fig.~\ref{fig:PDPmodelPPandMoments} (right).

\begin{singlespace}
\begin{figure}[t!]
    \centering
    %\scalebox{0.6}{
    \begin{minipage}{0.41\textwidth}
\begin{algorithmic}
    \STATE $k_1:=4$, $k_2:=40$, $y:=0$
    % \STATE $k_2:=40$
    %  \STATE $y:=0$%, $x:=0$
    % \STATE $x:=0$
    % % \STATE $a:=0.2$
    % \STATE $a:=0.2$ 
    \STATE $x:=0$, $a:=0.2$, $b:=4$, $s:=0$
    \STATE  $h:=0.6$, $f:=0.1$, $\rho:=0.5$
    %\STATE $\rho:=0.5$
    % \STATE $f:=0.1$
    % \STATE $h:=0.6$
    % % %\STATE $p:=0.5$
    % % \STATE $f:=0.1$, $h:=0.6$
    %   \STATE  $\rho:=0.5$
    % % %\STATE $\epsilon:=0.5$
    \WHILE{$true$}
        %\STATE $k:= k_1 \;[\;p\;] \;k_2$
        \IF{$s=0$}
            \STATE $s = 1 \;[\;f\;]\; 0$
        \ELSE
            \STATE $s = 0 \;[\;h\;]\; 1$
        \ENDIF
        \STATE $k:= k_2 * s + k_1 * (1-s)$
        % \STATE s:= 1 \;[\;p\;]\; 0
        % \STATE if s= 0 
        % \STATE    k=k0
        % \STATE else
        % \STATE    k=k1
        % \STATE end\\\notag
        \STATE $y:=(1-\rho)y+k$
        \STATE $x:=(1-a)x+by$
    \ENDWHILE
\end{algorithmic}
\end{minipage}
\begin{minipage}{0.58\textwidth}
\includegraphics[width=\textwidth]{Figures/HistogramMEGCPDPmodelnew1.eps}
\end{minipage}
%\vspace{5mm}
\caption{A PDP model for gene circuits, modeled as a PP in the left,  representing a 
gene  controlled by a two-valued, probabilistically updated variable $s\in\{0,1\}$. 
%(representing OFF/ON activation), where the 
%switch between values of $s$ comes with a probabilistic update. 
We respectively denote with $k_0$ and $k_1$ the gene transcription  rates  in states $s=0$ and $s=1$, and let $b$ the translation rate of protein $x$ production in the gene. Further, $\rho$ controls the mRNA level $y$ and $a$ denotes the protein degradation rate.
The (normalized) histogram  of sampled data of the resulting PP, with execution time/sample size $e=1000$ and loop iteration $n=100$ is given on the right, together with the  ME and GC expansion  estimates of the pdf of $x$ using  the first 3 moments of $x$.} 
\label{fig:PDPmodelPPandMoments}
%}
\end{figure}
\end{singlespace}
%%%%%%%%%%%%%%%%



%\lk{Further details on our examples can be found in  Appendix~\ref{Appendix}. }


\paragraph{{\bf Experimental Setup.}}
All our seven examples in Table~\ref{table:DKL-Chi2-K-SforBenchmarks} implement polynomial loop updates and fall in the class of probabilistic loops supported by~\cite{moosbrugger2021automated}. As such, for each example of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}, exact higher-order moments of random loop variables can be computed using the algorithmic approach of~\cite{moosbrugger2021automated}. In our work, we use the Polar tool of~\cite{moosbrugger2021automated} to derive a {\it finite} set $M$ of exact higher-order moments for each PP of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}, and we set $S_M = M$ to be further used in Algorithm~\ref{fig:algo}.
%, as described in Algorithm~\ref{fig:algo}.
% , whereas the third column of Table~\ref{table:DKL-Chi2-K-SforBenchmarks} lists the exact moments $M$ for a PP variable. 
% For each PP of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}, we use the set $|S_{\text M}|$ of moments to  estimate distributions of PP variables, as described in Algorithm~\ref{fig:algo}. 
Further, we 
%
%\paragraph{Evaluation setup.} 
%We compute moments for program variables using 
%Mora and its successor 
%Polar\footnote{\url{https://github.com/probing-lab/polar}}\cite{Moosbruggeretal2022}.
%\cite{bartocci2020mora,Moosbruggeretal2022}.
% for all benchmarks except the model of \eqref{eq:SDE2}.
generate our sampled data ($Sample_{Data}$)  by executing each PP $e=1000$ times and  for loop iteration $n=100$. %  and collecting random variable values at  loop
%iteration $n=100$.
For assessing the adequacy of estimated distributions, we set $\alpha = 0.05$ as a statistical significance level for the chi-square and K-S tests. Moreover,   we use $k=15$ bins for chi-square tests. As such, the critical test values for the chi-square  and  K-S tests are respectively  $CV_{\chi^2}=23.685$ and  $CV_{\text{K-S}}=0.0608$. All our numerical computations are conducted in Matlab. 
%Matlab is used for computations, and  the \texttt{ksdensity}\footnote{\url{https://mathworks.com/help/stats/ksdensity.html}} function for kernel density estimation.


% \Ahmad{I dropped the Kulback Leibler, but suggest to keep Precision of Higher Moments.}
% Sections \ref{section:MaximumEntropyMethod} and \ref{section:GramCharlierExpansion} 
% including {\bf StutteringP}, {\bf Square}, {\bf Binomial}, {\bf Random Walk 1D}, and {\bf Uniform}. We refer to Table~\ref{table:BenchmarkPrograms} in Appendix~\ref{Appendix} for their description. 

%We estimate the distributions of the random variables in these probabilistic programs  using their exact moments. The selected benchmarks are prob-solvable loops and their  exact moments can be calculated  via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora} without executing the programs. They are reported, % exact moments of the output  random variable for selected benchmarks,  
%as functions of loop iteration $n$,  in Table~\ref{Table:Benchmarks} in Appendix~\ref{Appendix}.


%We also formulate, for the first time, 
%a gene circuit  model in biology as a probabilistic program. Furthermore, the resulting PP is prob-solvable so that  Mora/Polar can calculate the exact moments of the generated random variables. They are then used to estimate the distribution of protein and mRNA levels  of a gene, the random variables of this model.  


%\paragraph{A Piecewise-deterministic process (PDP) Model for Gene  Circuits: }
%As another real life  example, we present, for the first time, a piecewise-deterministic process (PDP) model  in biology as a prob-solvable probabilistic program. 
 %   This  model is used to represent gene networks. 
%    We consider the simple model of
%    a single constitutive gene controlled by a two state (ON/OFF) promoter (see \cite{innocentini2018time}).


%\newpage
%Our approach for distribution estimation using moments is not limited to prob-solvable loops. Once  moments of a  probabilistic program, either exact or approximated, are available, we can estimate the distribution of any random variable. As an example of a probabilistic program that is not prob-solvable, we next represent a stochastic differential equation (SDE) as a PP and estimate the distribution of its random variable. 

% \lk{I removed the SDE example, as it does not bring much. It is now at the end of the paper. If we put it back, we need to update benchmark tables and all further tables.} \Ahmad{As we have page limit of 16 pages, I put the SDE example in the Appendix, but I suggest we keep a paragraph here which says that our method of estimation are not limited to only prob-solvable loops, but general loops can be handled provided that moments are given - \lk{but this is what Algorithm 1 states, we never mention that we are using only Prob-solvable loops. We can use arbitrary PPs, only our 7 examples are Prob-solvable}}
% \Ahmad{OK. Shall I keep this SDE example in Appendix? As it is now?}
% \lk{keep it for now, and we decide tomorrow. I am not sure we need an appendix at all, but we can discuss tomorrow}
% %\newpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Evaluation}\label{section:Evaluation}
%
%We evaluate the accuracy of our two approaches for the estimation  of distributions in  probabilistic programs (and probabilistic loops in particular) using  given exact moments.


%\paragraph{KL Divergence.} 

\paragraph{{\bf Experimental Results on  Distribution Estimation.}} 
Table~\ref{table:DKL-Chi2-K-SforBenchmarks}  summarizes our experimental results on  estimating the distributions of our benchmark programs. 
The first column of  Table~\ref{table:DKL-Chi2-K-SforBenchmarks} lists the name of the benchmark. 
The se\-cond column of
Table~\ref{table:DKL-Chi2-K-SforBenchmarks} specifies the random variable of the benchmark for which $|S_M|$ moments are derived, in order to estimate the distribution of the respective variable. The number $|S_M|$ of moments used for estimating distributions are given in column~3 of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}.
Columns~4--5 of 
Table~\ref{table:DKL-Chi2-K-SforBenchmarks}
respectively give the resulting chi-square test values for the ME and GC expansion estimations of the pdf of the respective PP variable of the benchmark. % the respective PP; to this end, we used the PP output variable as  the one for which exact moments are comuted by Mora/Polar \cite{bartocci2020mora,Moosbruggeretal2022}.
%listed in column~3 of Table~\ref{Tab:Benchmarks}. 
In addition to the chi-square test values, columns~4--5 also indicate the adequacy  of our estimated distribution (as in lines~10--11 of Algorithm~\ref{fig:algo}): we use
\cmark{} to specify that the estimated pdf is an accurate estimate of the true distribution, and write  \xmark{} otherwise. 
The results reported in columns 6--7 of Table~\ref{table:DKL-Chi2-K-SforBenchmarks} are as in columns 4--5, yet by using the K-S test instead of the  chi-square test. 






%
%a also reports the   $D^\ast$ statistic values  for the K-S test, as well as the $\chi^2$ statistics for the chi-square goodness-of-fit tests. 
%
%In the K-S test, we reject the null hypothesis that sampled data follow the estimated distribution, if $D^\ast$ is greater than $CV_{\text{K-S}}=0.0608$. For the chi-square test, we reject the same null if  $\chi^2$ is greater than  $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$.

 

% , we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of  probabilistic programs  follow the  distributions estimated using moments. 



% In order to assess the our estimations, we set the number of loop in the StutteringP program to be 100 and we take 1000 sample for the output $s$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments.   To perform the $\chi^2$ goodness-of-fit test for the StutteringP benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the maximum entropy estimated distribution  is $\chi^2=15.1544$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program StutteringP follow the  distribution estimated using  moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 


% %%%% Square Chi2 Evaluation 
% In order to assess the our estimations, we fix the number of loop in the Square program to be 1000 and we take 1000 sample for the output, i.e. the variable $y$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments (cumulants).   To perform the $\chi^2$ goodness-of-fit test for the Square benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the Gram-Charlier estimated distribution  is $\chi^2=9.9100$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program Square  follow the  distribution estimated using  moments (cumulants) calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 




% \bigskip
% \bigskip




% \begin{table}[tpbh!]
%     \centering
%      \scalebox{0.8}{
%  \begin{tabular}{c|l|l|l|l|l|l}
% \hline
%           {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & $D^\ast$ (ME) & $D^\ast$ (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline\hline
%      StutteringP& 0.005858 & 0.005831& 0.0181 \cmark & 0.0213 \cmark & 18.6432 \cmark& 16.7943 \cmark\\%\hline
%      Square & 0.005116 & 0.007204 & 0.0586 \cmark & 0.0566 \cmark& 36.9009 \xmark& 39.1309 \xmark \\%\hline
%      Binomial & 0.003779 & 0.003844 & 0.0598 \cmark &  0.0597 \cmark & 27.4661 \xmark& 27.4574 \xmark\\%\hline
%      \hspace{2mm} Random Walk 1D \hspace{2mm}& 0.006410 \hspace{2mm} & 0.006710 \hspace{2mm}&  0.0264 \cmark \hspace{2mm}&  0.0263 \cmark \hspace{2mm}& 18.6709 \cmark \hspace{2mm}& 18.7068 \cmark \hspace{2mm}\\%\hline
%     Uniform (Cont.) & 0.062240 & 0.007650 & 0.0214 \cmark & 0.0658 \xmark & 16.3485 \cmark& 105.276 \xmark\\%\hline
%      PDP Model & 0.006180 & 0.009348 & 0.0403 \cmark & 0.0393 \cmark & 64.4182 \cmark $^{\ast\ast}$& 65.9500 \cmark $^{\ast\ast}$\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler distance, $D^\ast$  (Kolmogorov–Smirnov statistics) and $\chi^2$ (chi-square statistics) for the benchmark probabilistic programs.  \xmark \; means that the null hypothesis of the underlying test is rejected while \cmark states that we can not reject the null hypothesis which means there is no evidence against null hypothesis. \\
% $^{\ast\ast}$ The chi-square test accepts the null hypothesis when the number of bins $k$ is at least 50, for which $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,49}=66.339$. }
%  \label{table:DKL-Chi2-K-SforBenchmarks}
% \end{table}


% \lk{changed the notation $\chi_{ME}^2$, ..., in Table 2, as in  Alg1; we need to be consistent}

 Table~\ref{table:DKL-Chi2-K-SforBenchmarks} indicates that our approach in Algorithm~\ref{fig:algo}, based on GC expansion and ME, for distribution estimation  yields accurate estimates for pdfs of   continuous random variables, as assessed by either the chi-square test or the K-S test; the benchmarks of {\sc StutteringP}, {\sc Random Walk 1D}, {\sc Vasicek Model}, and {\sc PDP Model} fall in this category. 
 %which is the case of the benchmarks of. Both goodness of fit tests cannot reject  the null hypothesis that the sampled data follow the estimated distributions. 
 For estimating the pdf of discrete random variables, as in the {\sc Square} and {\sc Binomial} programs, the K-S test infers our method to be accurate, but the chi-square test does not. 
 %\lk{what about {\sc Uniform}? ME pdf passes with both tets, whereas the GC pdf is rejected by both test. Any explanation/intuition why?}
 The  GC expansion (see Section~\ref{ssec:reconstructing-distribution}) expresses a distribution as a series in terms of the normal distribution. When estimating pdfs of random variables whose distributions are markedly different from the normal, this GC expansion is not adequate. This occurs in the  {\sc Uniform} example, where the PP implements a uniform distribution. In contrast, the ME based  pdf estimation is accurate, as concluded by  both the chi-square and the K-S test. 
 %
%However, the latter is sensitive to the choice of bins. In the PDP model, the test rejects the null hypothesis for  $\alpha=0.05$ and  $k=15$. Increasing the number of bins to $k=50$, the chi-square test no longer rejects the null hypothesis as the test statistics $\chi^2$ for both ME and GC estimates are below the critical value  $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,49}=66.339$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{PrecisionOfHigherMoments}


==> Distribution Recovery (27)/OldVersion.tex <==



% \section{Introduction}

% \textcolor{red}{To do: 
%  \bigskip 
% \begin{itemize}
%     \item Finding several benchmarks in PPs for which we should do distribution recovery.
%     \mm{Check out Github of polar and the paper draft for the polar tool. Also related work cited in the polar paper draft.}
%     \bigskip 
%     \item What is the gain of this distribution recovery. In particular, what we can do having this estimated distribution that we can not do without it (in the context of verification and program analysis)? Sensitivity Analysis? Add some reasoning and justification.
%     \mm{I would say answer questions of the form $\mathbb{P}(a \leq x \leq b)$: What's the probability that some program variable of interest is in some interval.}
%      \Ahmad{We take advantage of the reconstructed pdf  for different queries, such as to compute the probability of assertions and to answer questions of the form $\mathbb{P}(a \leq x \leq b)$: What's the probability that some program variable of interest is in some interval. Calculating  expectations, performing inference,  quantifying the loss of precision would be the other advantages of the distribution recovery for probabilistic programs with the help of their moments and without executing of the programs themselves (which is of essential premises in the field of  program analysis and verification).}
%         \bigskip 
%      \item How good are our distribution estimations? If we have the true distribution (for example in Square)? and If we do not have the true distribution? For latter, we do sampling and assess our estimated distribution and sampled one. For this, we have done with statistical tests (Chi-squared and Kolmogorov-Smirnov goodness of fit test) and using Kullback-Leibler Divergence in Section~\ref{Section:Implementation and Benchmark Problems}.
%      \ms{There should be quite a few known distributions we can encode as loops and compare exactly (there may be a bias, and the performance would be, potentially, better than for arbitrary distribution). %something to mention in the evaluation section
%      Another way, potentially, would be to only use some moments for reconstruction and a few more to test. E.g. use first 6 moments to get an approximate distribution and compare it's 7th, 8th moments to 7th and 8th precise moments (computed by Polar). }
%       \bigskip 
%       \item Writing what we have and we have done in a proper story. Adding a section on Prob-solvable programs that we can calculate exact moments. Then,...?, Adding from Polar? 
%       \ms{We can differentiate between \textit{moment computation} and \textit{distribution recovery}, both being somewhat separate problems in a wider problem of analysing probabilistic programs/loops.}
% \end{itemize}
% }

% Probabilistic programs are ordinary programs whose execution is based  on the outcome of
% random experiments.  Running a probabilistic program (repeatedly) on a \efi{single
% input} generally produces probability distributions over outputs.

% Almost all machine or statistical learning involves probabilistic algorithms
% (programs) for representing and updating the beliefs of an artificially intelligent system about the world in
% light of data; i.e., inferring plausible models to explain observed data. We aim to derive the probability
% distribution of the random variables generated by a PP. Quantifying and modelling the uncertainty in probabilistic programs
% will bring together computer programming, statistics and machine learning. 



% Computing invariant properties is of importance in probabilistic programs analysis as they summarize loop behaviors. \cite{bartocci2019automatic} presented fully automated approaches  to generate invariants over higher-order moments of program variables, without any user guidance. In the way to recover the full probabilistic program behavior, in this paper, we present numerical methods to reconstruct distributions of program variables using their moments. This procedure would help us to efficiently estimate posterior distributions of different variable directly without any use of sampling or running of the program itself, which is an essential requirement  in the verification of computer programs. 



% In this paper, we go through several approaches to reconstruct distributions for different variables involving in the probabilistic programs: characterization of distributions associated with prob-solvable probabilistic programs,  reconstruction of distribution from the scratch using numerical methods, and extracting properties of distribution using concentration inequalities. Our reconstruction methods will be tested on benchmarks. 


% \bigskip
% \bigskip


% % \section{Characterization of  Distributions Associated with Prob-Solvable Probabilistic Programs}
% % % \deleted{ The outcome values of a probabilistic program are
% % % realizations of random variables representing program expressions that are not deterministic. }

% % % \mm{"outcome values" is not a common terminology. "non-determinism" is very common but in CS means something different than probabilistic. Suggestion: The result of a PP is not a single value but rather different values with different probabilities according to the distribution the PP encodes.} \ahmad{Done!}

% % { The result of a PP is not a single value but rather different values with different probabilities according to the distribution the PP encodes. }
% % Different paths in a
% % PP are typically selected by draws from commonly used distributions such as the uniform or the normal, whose
% % properties and features have been extensively studied in probability and statistics. Yet, since a PP’s output values
% % are the result of multiple operations, their distributions are most often non common ones.
% % %Most developments in the analysis of PPs focus on the derivation of the first moment of the outcome values,
% % %[3, 16, 20, 33], 
% % %which provides a limited account of the distribution of the random variables arising from a
% % %PP. 
% % %Bouissou et al. (2016) \cite{bouissou2016uncertainty} considered the problem of answering queries on probabilities of assertions over program variables and
% % %their moments; that is, of assessing the likelihood of program variables and their moments producing outputs in a
% % %specified range. Their approach consists of approximating program random variables with affine forms under the
% % %assumption that they have bounded support and all their moments are finite.

% % The study of distributions and their characteristics is a much explored topic in statistics. Many distributions are fully characterized by their moments. Many of well known known distributions fall in this category. For example, the normal, the Poisson, the uniform, etc. 
% % % In particular, if
% % % a random variable has bounded support, then the sequence of all its moments uniquely
% % % determines its distribution \cite{billingsley2013convergence}. Nevertheless, knowledge of all
% % % the moments of a random variable does not necessarily uniquely characterize its distribution.

% % \begin{definition}\cite{casella2021statistical}\label{momentgeneratingfunction}
% % Let $X$ be a random variable with cdf $F_X$. The moment generating function (mgf)
% %  of $X$, denoted by $M_X(t)$, is 
% %  \begin{align}
% %      M_X(t)=E(e^{tX}),
% %  \end{align}
% % provided that the expectation exists for $t$ in some neighborhood of $0$. That is, there is an $h>0$ such that, for all $t\in(-h,h)$, $E(e^{tX})$ exists. If the expectation does not exists in a neighborhood of $0$, we say that moment generating function does not exist.  
% % \end{definition}

% % If the moment generating function exists, it characterizes all moments, but characterizing the set of moments is not enough to determine a distribution uniquely as  two distinct random variables can have the same moments (see e.g.  Example~2.3.10 in \cite{casella2021statistical}). If the random variable has bounded compact support, then the infinite sequence of moments  uniquely determines its distribution (\cite{billingsley1995probability} Section~30). More generally, if the moment generating function exists in a neighborhood of $0$, then the distribution is uniquely determined. Existence of all moments is not equivalent to existence of the moment generating function. 


% % % \efi{this has to do with the definition and existence of the moment generating function. See for example Casella and Berger's book}.  

% % % %The main approaches for characterizing distributions rely on moments of order statistics or conditional expectations \cite{bairamov2007characterization,su2000characterizations}.

% % % \efi{These paragraphs try to say what wrt our problem???}

% % % \textcolor{blue}{Carleman's condition guarantees that a probability distribution is uniquely determined by its moments.
% % % Let $\{\mu_k\}$ be the moment sequence of random variable $X \geq 0$, and let
% % % $$\sum_{k=1}^{\infty}\mu_k^{-1/(2k)}=\infty \qquad \text{(Carleman’s condition)},$$
% % % then   the  cumulative distribution function (cdf) $X$ is uniquely determined by the moments
% % % $\{\mu_k\}$. \cite{yarovaya2020conditions} study the relationship between the well-known Carleman's condition and some easily checkable conditions on the rate of growth of the moments. In the Stieltjes problem of moments, the pdf of a non-negative  random variable $X$ is determinable depends on the rate of growth of the moments. Let the moments $\{\mu_k\}$ follow a quadratic rate of growth, that is, 
% % % $$\frac{\mu_{k+1}}{\mu_k} = {\mathcal{O}}\big((k+1)^2\big) \quad as \quad k\rightarrow \infty.$$
% % % Then the random variable $X$ is uniquely determined by the moments \cite{lin2015moment}.
% % % As an extension, assume that
% % % $$\frac{\mu_{k+1}}{\mu_k} = {\mathcal{O}}\big((k+1)^2q^2(k+1)\big) \quad  as  \quad k\rightarrow \infty$$
% % % for the moment sequence $\{\mu_k\}$ of the random variable  $X$, where $q(k) > 0, n = 1,2,\dots$, is a function satisfying the condition 
% % % $$\sum_{k=1}^{\infty}\frac{1}{kq(k)}=\infty.$$
% % % \cite{yarovaya2020conditions} show that the moments $\{\mu_k\}$ satisfy Carleman’s condition, and these
% % % moments uniquely determine the random variable $X$.}




% % % %Also, if the moment generating function of a random variable $X$,
% % %$M_X(t)=E(e^{tX})$, exists in an open neighborhood of 0, then its distribution is uniquely determined %regardless of
% % %its support \cite{casella2021statistical}. Unfortunately, ascertaining this condition requires prior knowledge of the
% % %distribution of $X$.
% % %The main approaches for characterizing distributions rely on moments of order statistics or conditional expectations \cite{bairamov2007characterization,su2000characterizations}.
% % %Conditional moments of order statistics are extensively used in characterizing the parent probability distribution. 

% % %[51] obtained the explicit expression of the cumulative distribution function F(x) of a random variable
% % %X starting from $E(X|x\leq X\leq y) =
% % %\int_{x}^{y}tdF (t)/(F(y)-F(x))$ and define the relationship with order
% % %statistics as
% % %
% % %$$...$$





% % % \begin{comment}
% % % \bigskip
% % % \bigskip
% % % \textit{
% % % ... We have to  identify the class of PPs that admit closed form solutions for the distributions and those
% % % 	that do not. For the latter, the probability distributions will be approximated via simulations.}


% % % \bigskip
% % % \bigskip
% % % \textit{
% % % ... We should  identify the class of PPs that admit closed-form distribution(s)
% % % of the underlying random variables and characterize their distributions via higher order moments. When PPs do not
% % % generate variables whose distribution is characterized by moments, we will explore other statistical approaches,
% % % such as those based on order statistics \cite{balakrishnan1988recurrence} and conditional expectations, for distribution characterization.}

% % % \bigskip
% % % \bigskip

% % % \textit{
% % % ...We will characterize the distributions of
% % % continuous random variables in Prob-solvable and non Prob-solvable programs using distribution theory and results
% % % on moments of order statistics and/or conditional expectations. We will explore computer algebra packages
% % % that support the symbolic computation of probability and cumulative density functions for continuous random
% % % variables.}
% % % \end{comment}






% \section{Distribution Reconstruction via Their Moments and Cumulants}
% The reconstruction  of a probability density function (PDF) from  a finite number of its moments is
% known as the finite-moment problem which  arises in different  applications, such as physics, engineering, computer science, verification and cyber-physical systems \cite{gavriliadis2009moment, john2007techniques}. 

% Generally, the finite-moment problem is ill-posed and  there is no well-established algorithm available to solve this problem \cite{de2010reconstruction}. Depending on the specific problem and underlying field of study, 
%  several methods  add constraints on the domain and
% on the range of density function due to the underlying physics of the
% application, and try to reconstruct distributions from available finite number of moments. A typical example in the literature  is the reconstruction of particle
% size distributions (PSD) when considering particulate processes
% like crystallization in chemical engineering. Among existing  methods for physic-based finite-moment problem are for example: A kernel density estimation method \cite{athanassoulis2002truncated}, spline-based methods \cite{john2007techniques,de2010reconstruction}, and  Maximum Entropy \cite{biswas2010function, lebaz2016reconstruction} to reconstruct distributions from moments. 
% % We focus on nonparametric density estimation (e.g. kernel-based or spline-based methods) and Maximum Entropy. 
% Kernel density estimation together with a constrained minimization problem  is proposed by  \cite{athanassoulis2002truncated} for the Hausdorff moment problem and is extended in \cite{gavriliadis2009moment} for the Stieltjes moment problem.  In this method, the target pdf at a point is approximated by a sum of weights. The weight is typically modeled by a symmetric density, such as the standard normal. The optimal weights are computed through  minimizing the distance between the set of given moments and those estimated via the kernel density estimator. However, this nonparametric estimation method requires constant tuning  of the bandwidth parameters which increase with the number of moments and is seen to often perform poorly \cite{lebaz2016reconstruction}.


% The spline-based nonparametric density estimation (see, e.g., \cite{john2007techniques}) uses a piecewise polynomial function to recover  the target distribution.  This method is improved by \cite{de2010reconstruction} to be an adaptive algorithm to have better performance in non-smooth and multi-modal distributions.  As shown in \cite{mortier2014comparison,lebaz2016reconstruction}, the spline-based algorithm is highly sensitive to the negative tolerances leading to different reconstructions for the same target probability density function. This method assumes a smooth transition at the boundaries of sub-intervals and these conditions need to be changed during the reconstruction process.   

% Maximum Entropy is based on the maximization of the Shannon entropy (\cite{mead1984maximum}, \cite{tagliani1999hausdorff,tagliani2001numerical}, \cite{biswas2010function}). Its main advantage is the low computational cost  
% %there is no need to {\it a priori} information on the shape of target distribution and  
% (\cite{lebaz2016reconstruction}: Tables~2, 3) and has received increasing interest over the last two decades.

% Recovery of (posterior) distribution given some evidences is a common task in probabilistic inference. Existing  approaches for probabilistic inference  include: 
% \textit{exact symbolic} approaches (see e.g. \cite{sanner2012symbolic,bhat2013deriving,gehr2016psi}) and \textit{approximate symbolic} approaches (\cite{?, ?, ?}).  
% In \cite{gehr2016psi}, a symbolic
% analysis system, called \textit{PSI (Probabilistic Symbolic Inference)}, is presented  for automating exact inference in PPs via program analysis. PSI  automatically  computes the exact pdf of the random variable(s) of interest represented by that program. 
% As exact inference is theoretically expensive,  
% probabilistic inference systems may exploit  approximate
%   techniques and implement algorithms that calculate numerical approximations \cite{?,?,?,?}. 
% % These methods trade precision for better performance \cite{gehr2016psi}.

% Distribution recovery from moments  has not been much explored in the context of probabilistic programs, verification and cyber-physical systems.
% Note that non of above-mentioned works (nor existing symbolic-based methods, neither approximation-based methods) recover an unknown distribution form its moments. A quantitative analysis of PPs is presented in \cite{sankaranarayanan2020quantitative} using only expectation and concentration inequalities, but recovering distribution numerically using higher order moments in the context of (prob-solvable) probabilistic programs has not been well studied so far. Since exact inference is theoretically expensive, we exploit approximate
% inference techniques for  probabilistic inference. 
% % Although there is no accuracy guarantee in approximation approaches, they still worth to focus on them ad they  provide us with an  insight on the problem.   



% \addnote[id=ahmad]{Are you aware of any work in this context, Marcel and Miroslav?}
% \mm{A relevant work could be the tool PSI (from ETH) (https://psisolver.org/). The can reconstruct the exact distribution for some (loop-free) PPs. PSI could also serve as a comparison. For programs PSI can recover the distribution approximate it with some moments and compare it to the exact distribution given by PSI.}
% \todo{Effie: a description and comparison, or at the very least, why it is not directly comparable, should be given.}

% %\efi{Previous attempts to estimate distributions from their moments in the context ??? of PP are KDE and splines???, maximum entropy etc}

% % Here we focus on maximum entropy because there is no need to {\it a priori} information on the shape of target distribution and  the computational cost is low (\cite{lebaz2016reconstruction}).


% % \subsection{Spline-based Methods}
% % Splines can be applied for the reconstruction of a function for which a finite number of moments is given. Let $x_1 <x_2 <x_3 <\cdots
% % <x_{n+1}$ be discrete points on the $x$-axis. A spline  $s(x)$ is a piecewise polynomial of degree $q$. When $q= 1, 2$, or 3, the spline is called linear, quadratic, or cubic, respectively. Here, we use the cubic splines and  generate a linear system of equations. Let $[a, b]$ be a given
% % interval and $a=x_1 <x_2 <x_3 <\cdots
% % <x_{n+1}=b$. The ansatz is
% % $$s_i(x) =
% % \sum_{j=0}^3
% % s_{ij} (x-x_i)^j, \qquad x\in[x_i, x_{i+1}],\quad i= 1,\dots,n.$$
% % There are $4n$ unknown coefficients $s_{ij}$ to determine. The function $f(x)$ which should be reconstructed is a probability
% % density function. We assume that $f(x)$ vanishes everywhere
% % outside $[x_1, x_{n+1}]$ and   the transition
% % at the boundaries of the interval is smooth.
% % This means for the left boundary 
% % $$s_1(x_1) = 0, \quad s'_1(x_1) = 0, \quad s''_1 (x_1) = 0.$$ 
% % Inserting these conditions into the ansatz gives the following
% % three equations:
% % $$s_1(x_1) = s_{10} = 0, \quad  s'_1(x_1) = s_{11} = 0, \quad s''_1 (x_1) = 2s_{12}= 0.$$
% % Analogously, the right boundary corresponds to
% % $$s_n(x_{n+1}) = 0, \quad s'_n(x_{n+1}) = 0, \quad s''_n (x_{n+1}) = 0.$$ 
% % which gives the following three equations:
% % \begin{equation*}
% % \begin{pmatrix}
% % 1&x_{n+1}-x_n &(x_{n+1}-x_n)^2 &(x_{n+1}-x_n)^2 \\
% % 0 &1     &  2(x_{n+1}-x_n)  &  3(x_{n+1}-x_n)^2\\
% % 0 & 0     & 2     &  6(x_{n+1}-x_n)
% % \end{pmatrix}
% % \begin{pmatrix}
% % 	s_{n0}\\
% % 	s_{n1}\\
% % 	s_{n2}\\
% % 	s_{n3}
% % \end{pmatrix}
% % =
% % \begin{pmatrix}
% % 0\\
% % 0\\
% % 0
% % \end{pmatrix}
% % \end{equation*}
% % For continuity of the estimator at $x_{i+1} \;\;  (i=1,\dots,n-1)$ we include $s_i(x_{i+1})=s_{i+1}(x_{i+1})$ which give us $n-1$ equations of the form 
% % \begin{equation*}
% % 	\begin{pmatrix}
% % 		1&x_{i+1}-x_i &(x_{i+1}-x_n)^2 &(x_{i+1}-x_i)^2 & -1
% % 	\end{pmatrix}
% % 	\begin{pmatrix}
% % 		s_{i0}\\
% % 		s_{i1}\\
% % 		s_{i2}\\
% % 		s_{i3}\\
% % 		s_{(i+1)0}
% % 	\end{pmatrix}
% % 	= 0.
% % \end{equation*}
% % For smoothness of the spline estimator, we include the continuity of the first derivative of cubic spline. To this end, we set $s'_i(x_{i+1})=s'_{i+1}(x_{i+1})$ for all $i=1,\dots,n-1$. This leads to $n-1$ equations of the form 
% % \begin{equation*}
% % 	\begin{pmatrix}
% % 		1&2(x_{i+1}-x_i) &3(x_{i+1}-x_i)^2  & -1
% % 	\end{pmatrix}
% % 	\begin{pmatrix}
% % 		s_{i1}\\
% % 		s_{i2}\\
% % 		s_{i3}\\
% % 		s_{(i+1)1}
% % 	\end{pmatrix}
% % 	= 0.
% % \end{equation*}
% % Also we should include the continuity of the second derivative of the cubic spline at $x_{i+1} \;\;  (i=1,\dots,n-1)$,  $s''_i(x_{i+1})=s''_{i+1}(x_{i+1})$ which add $n-1$ equations of following form to our system:  
% % \begin{equation*}
% % 	\begin{pmatrix}
% % 		2 &6(x_{i+1}-x_i)  & -1
% % 	\end{pmatrix}
% % 	\begin{pmatrix}
% % 		s_{i2}\\
% % 		s_{i3}\\
% % 		s_{(i+1)2}
% % 	\end{pmatrix}
% % 	= 0.
% % \end{equation*}
% % We need $n-3$ more equations for the system of equations to be solvable. These equations derive from the known moments. The $k$th moment of the cubic spline $s(x)$, $k\in\mathbb{N}$,
% % \begin{align*}
% % 	\mu_k=\int_{a}^{b}x^k s(x) dx = \sum_{i=1}^{n}\int_{x_i}^{x_{i+1}}x^k s_i(x)dx=\sum_{i=1}^{n}\sum_{j=0}^{3}s_{ij}\int_{x_i}^{x_{i+1}} x^k (x-x_i)^jdx. 
% % \end{align*}
% % The straightforward calculations and setting 
% % \begin{align*}
% % I_1=\frac{x_{i+1}^{k+1}-x_i^{k+1}}{k+1}, \qquad I_2=\frac{x_{i+i}^{k+2}-x_i^{k+2}}{k+2}, \qquad I_3=\frac{x_{i+i}^{k+3}-x_i^{k+3}}{k+3},  \qquad I_4=\frac{x_{i+i}^{k+4}-x_i^{k+4}}{k+4},
% % \end{align*}
% % leads to 
% % \begin{align*}
% % 	\mu_k&=\int_{a}^{b}x^k s(x) dx \\
% % 	&= \sum_{i=1}^{n} \big[I_1s_{i0} + (I_2-x_iI_1)s_{i1} + (I_3-2x_iI_2+x_i^2I_1)s_{i2} + (I_4 - 3x_iI_3 + 3x_i^2I_2 -x_i^3I_1)s_{i3}\big]. 
% % \end{align*}
% % Now, a $4n\times4n$ linear system of equations has been obtained
% % and can be solved. The simplifications corresponding to linear
% % and quadratic splines are straightforward. 

% % Figure~\ref{fig:SplinemomentsQuad} shows numerical results of implementation of quadratic spline for two different examples.  A finite number of  moments for each distribution are given. In the first example,the true distribution is assumed to be \begin{align}\label{pdf1}
% %  f_X(x)&=\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}  
% % \end{align} whose  support in $[0,1]$. The first 6 moments of  $f$ are calculated separately and are used to approximate the pdf $f$ via quadratic spline method.  The same strategy is applied for the second example with probability density function 
% % \begin{align}\label{pdf2}
% %  g_X(x)&=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}.
% % \end{align} 

% % \efi{Recompute the right panel of  Figure~\ref{fig:SplinemomentsQuad} and verify \eqref{pdf2} is a proper density}

% % You should approximate the following distributions
% % \begin{itemize}
% %     \item Normal mixture: $f(x)=\alpha N(\mu_1,\sigma_1)+(1-\alpha) N(\mu_2,\sigma_2)$, $\alpha \in (0,1)$.
% %     \item check distributions from \url{https://en.wikipedia.org/wiki/List_of_probability_distributions}. Specifically, the Cauchy, truncated normal, gamma, the Gompertz distribution, the half-normal distribution, Hotelling's T-squared distribution, F-distribution, Weibull, Gumbel, Generalized extreme value distribution.
% % \end{itemize}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	%	\includegraphics{Figures/reconstME6Moments.pdf}
% % 	\includegraphics[height=5cm]{Figures/reconstSpline6moments.eps}
% % 	\includegraphics[height=5cm]{Figures/SplineQsecondExample.eps}
% % 	%\includegraphics[height=3.7cm]{Figures/recostSpline7moments.eps}
% % 	%\includegraphics[height=3.7cm]{Figures/reconst1Spline.eps}
% % 	\caption{Quadratic Spline Method with 6 moments: Example 1 (left), Example 2 (right).}
% % 	\label{fig:SplinemomentsQuad}
% % \end{figure}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % %\begin{figure}[tpbh!]
% % %	\centering
% % %	%	\includegraphics{Figures/reconstME6Moments.pdf}
% % %	\includegraphics[height=3.7cm]{Figures/SplineQsecondExample.eps}
% % %	\caption{Quadratic Spline Method Example 2 with 5 moments }
% % %	\label{fig:Splinemoments}
% % %\end{figure}
% % %\newpage

% % %\newpage
% %\newpage

% \todo{Effie: no discussion about cumulant-based methods in this preamble. Needs to be added.}

% In this paper, the Maximum Entropy and Gram-Charlier expansion methods will be used. 

% \iffalse

% \subsection{Maximum Entropy}\label{section:MaximumEntropyMethod}

% The Maximum Entropy (ME) method is based on the maximization of the Shannon entropy  from information theory. In order to estimate the unknown distribution $f$, we  maximize $H[f]$ given by \cite{bernardo2009bayesian,o2004kendall}
% \begin{align}
%   H[f]=-\int_{a}^{b} f(x) \ln(f(x))dx,  
% \end{align}
% subject to its given moments $\mu_i=\int x^if(x)dx$. The explicit representation of the ME approximation $f_M(x)$ of the target PDF takes the form
% \begin{align}
% f_M(x)=\exp\Big[-\sum_{j=0}^N\xi_jx^j\Big],    
% \end{align}
% where the Lagrange's multipliers $\xi_j\;\; j=0,1,\dots,N$ can be obtained from given moments. To this end, the following system of $N+1$ nonlinear equations is solved,
% \begin{align}\label{eq:nonlinearSystemME}
% \int_a^b x^i\exp\Big[-\sum_{j=0}^N\xi_jx^j\Big]dx=\mu_i.   
% \end{align}
% For more details on the maximum entropy method for distribution recovery, we refer to \cite{buchen1996maximum}. Numerically, iterative methods are used to solve the nonlinear system of equations \cite{mead1984maximum,lebaz2016reconstruction}.  Here, we use a numerical minimization algorithm, called  Levenberg–Marquardt which was developed  to solve
% nonlinear least squares problems \cite{levenberg1944method, marquardt1963algorithm}. This algorithm is an iterative procedure  (a combination of   gradient descent and
% Gauss-Newton) with an initial choice of the Lagrange's multipliers $\xi_j$ in \eqref{eq:nonlinearSystemME} and
% a given tolerance of $10^{-6}$ for stopping the iterative process. 

% Before we move to distribution recovery in probabilistic programs where we have no information about the target PDF, we present  two  examples in which the following bimodal and tri-modal functions on the interval $[0,1]$ are recovered via ME.  
% \begin{itemize}
%     \item Example 1, $f_X(x)=\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}$,
%     \item Example 2, $g_X(x)=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}$. 
% \end{itemize}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/reconst6moments.eps}
% 		\includegraphics[width=4.2cm]{Figures/MEsecondExample.eps}
% 	\caption{Maximum Entropy Method with 6 moments: Example 1 (left), Example 2 (right).}
% 	\label{fig:MaxEntropy6Moments}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figure~\ref{fig:MaxEntropy6Moments} shows reconstructed distributions compared to the given ones in Example 1 and 2. 
% We compare the accuracy of the reconstruction using the Kullback–Leibler divergence. The  Kullback-Leibler divergence, or simply, KL
% divergence is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% Assuming that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% \begin{align}\label{Kullback-LeiblerDivergence}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.

% A quantitative comparison of the distributions (target and reconstructed) is also carried out. The Kullback–Leibler divergence values for the ME estimates of both functions are given in  Table~\ref{table:Kullback-LeiblerDivergence11}. 
% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|}
% \hline
%               & Example 1 & Example 2\\
%                           \hline
%      Maximum Entropy & 0.0328 & 0.0139\\\hline
%     \end{tabular}
% \vspace{5mm}
%  \caption{Kullback-Leibler divergence ($D_{KL}$ of sampled and ME estimated  distributions).}
%       \label{table:Kullback-LeiblerDivergence11} 
%  \end{table}


% % We compare the accuracy of the reconstruction using the Kullback–Leibler divergence. The  Kullback-Leibler divergence, or simply, KL
% % divergence is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% % Assuming that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% % \begin{align}
% %     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% % \end{align}
% % $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.

% % A quantitative comparison of the distributions (target and reconstructed) is also carried out. The Kullback–Leibler divergence values for the ME estimates of both functions are given in  Table~\ref{table:Kullback-LeiblerDivergence11}. 
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %               & Example 1 & Example 2\\
% %                           \hline
% %      Maximum Entropy & 0.0328 & 0.0139\\\hline
% %     \end{tabular}
% % \vspace{5mm}
% %  \caption{Kullback-Leibler divergence ($D_{KL}$ of sampled and ME estimated  distributions).}
% %       \label{table:Kullback-LeiblerDivergence11} 
% %  \end{table}
 
% % \mm{Would be nice to see this method for a concrete PP here: (1) Get precise moments via Polar. (2) approximate distribution with Maximum Entropy.}
% % \ahmad{Done for Random Walk 1D!}

% Next, we apply  Maximum Entropy to estimate distributions of a random variable generated in the probabilistic program  \textit{Random Walk 1D} using its calculated moments via moment-based invariant generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. The target distribution is unknown and  only moments of the random variable of interest, expressed as a function of loop iteration, are available (Equations~(\ref{eq:ExactmomentsofRandomWalk1}-\ref{eq:ExactmomentsofRandomWalk3})). \textcolor{blue}{In order to reconstruct the distribution of random variable $x$ in the probabilistic program Random Walk 1D, we fix the loop iteration to be $n=100$ and use the first three exact moments of $x$, i.e. $E[x(100)], E[x^2(100)]$ and $E[x^3(100)]$. Applying ME method to the given moments, we recover the pdf and the cdf of $x$ which is shown with red color in Figure~\ref{fig:pdfRandomwalk1DME1} (Middle and Right).}  
 







% In order to assess accuracy of distribution estimation, we carry out a Monte Carlo ``experiment'' by executing  the PP a \textit{large} number of times (here, large=1000), and  compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test. Results (see Figure~\ref{fig:pdfRandomwalk1DME1}) show visually the agreement of the estimated pdf and cdf with the sampled data (indeed, with the KS density approximation of the sampled data). Details and numerical result of the accuracy evaluation will be presented in Section~\ref{section:Evaluation}.

% % Here, we apply the Maximum Entropy method  to estimate distributions of a random variable of probabilistic program  Random Walk 1D  using its calculated moments via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. Note that the target distribution is unknown and we have only moments of the random variable of interest presented as a function of loop iteration. With the help of  statistical tools, we also confirm the agreement of our estimated distributions with the ones generated during the execution of these probabilistic programs. 


% \todo{The following is not a correct statement: We assess the agreement or accuracy  of the estimated distributions with the ones generated during the execution of the probabilistic programs.}

% What you do is the following: 

% \begin{enumerate}
%     \item You estimate the distribution using ME and the exact moments provided by the recurrence-based algorithm in \cite{bartocci2020mora,bartocci2019automatic}
%     \item Assess accuracy of ME estimation of moments and the true moments with plots only (so far)!
%     \item To assess accuracy of distribution estimation, you carry out a monte carlo ``experiment,'' as follows: You repeat the PP a \textit{large} number of times (here, large=1000), and then compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test.   
% \end{enumerate}

% \fi



 
% % \bigskip

% % \noindent{\bf Random Walk 1D} 
% % \begin{align}
% % &v:=0\\\notag
% % &x:=0\\\notag
% % &\text{while true:}\\\notag
% % &\quad v:=\text{uniform}(0,1)\\\notag
% % &\quad x:=x+v\;\;[7/10]\;\;x-v
% % \end{align}
% % Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~1 of  \cite{bartocci2019automatic}: 
% % \begin{align}\label{eq:ExactmomentsofRandomWalk1}
% % &E[x(n)] = n/5\\\label{eq:ExactmomentsofRandomWalk2}
% % &E[x^2(n)] = n^2/25 + 22n/75\\\label{eq:ExactmomentsofRandomWalk3}
% % &E[x^3(n)] = n^3/125 + n^222/125 - n21/250
% % \end{align}
% % Figure~\ref{fig:SampledEXforRandomWalk1Sample1000loop1} show the agreement of sampled data and exact expected value of random variable $x$ per each loop iteration. One easily can see that the uncertainty propagates through probabilistic loop and remains around the exact expected value of the variable $x$. Figure~\ref{fig:SampledEXforRandomWalk1000Sample1000loop1} shows that the mean value and the second moment for a sample of size 1000 agrees the exact expected values for each loop iteration $n$. This shows the strength  of the moment-based invariant generator in which on can calculate moments of random variables of a PP without running the program.  
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% % % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% % 	\caption{$x$-axis: iteration, $y$-axis: sampled values of the random variable. In red is the Mora generated $E(x)$, and in blue are the sampled values of the random variable in \textit{Random Walk 1D}.}
% % 	\label{fig:SampledEXforRandomWalk1Sample1000loop1}
% % \end{figure}

% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1000loop1000Sample.eps}
% % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ $E(x)$ and $E(x^2)$ for Random Walk 1D using 1000 sample for each iteration of loop.}
% % 	\label{fig:SampledEXforRandomWalk1000Sample1000loop1}
% % \end{figure}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=10cm]{Figures/absoluteErrorExRandomWalk1D.eps}\\
% % 	\includegraphics[width=10cm]{Figures/relativeErrorExRandomWalk1D.eps}
% % 	\caption{ Absolute and relative errors $E(x)$ and $E(x^2)$ for Random Walk 1D: \\
% % 	Absolute Error of $E(x)= |{E(x)}_{sample}-{E(x)}_{exact}|$\\
% % 	Absolute Error of $E(x^2)= |{E(x^2)}_{sample}-{E(x^2)}_{exact}|$\\
% %     Relative Error=$\frac{\text{Absolute Error}}{\text{Exact Value}}$}
% % 	\label{fig:AbsoluteandRelativeErrorsRandomWalk1D}
% % \end{figure}








% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=3.8cm]{Figures/histogramRandomwalk1D.eps}
% % 	\includegraphics[width=3.8cm]{Figures/pdfRandomwalk1DME.eps}
% % 	\includegraphics[width=3.8cm]{Figures/cdfRandomwalk1DME.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Random Walk 1D. Estimation of Distribution using Maximum Entropy method with 3 moments.}
% % 	\label{fig:pdfRandomwalk1DME1}
% % \end{figure}

 
 
% %  In order to evaluate our estimation, as there is no pdf and nor cdf of the target distribution available, we assess it via sampling strategy. Running the program itself and stopping at the fixed loop iteration (here, $n=100$), we apply Chi-Square Goodness-of-Fit Test to see if  our sampled data came from a population with the ME estimated distribution. To this end,  we consider following hypothesis:

% % \bigskip

% % \hspace{10mm} $\text{H}_0$:	The data follow the estimated distribution.

% % \hspace{10mm} $\text{H}_a$:	The data do not follow the estimated distribution.

% % \bigskip	

% % For the chi-square goodness-of-fit computation, we divide the data  into $k$ bins and define the test statistic as
% % \begin{equation}
% %     \chi^2=\sum\limits_{i=1}^k(O_i-E_i)^2/E_i,
% % \end{equation}
% % where $O_i$ is the observed frequency for bin $i$ and $E_i$ is the expected frequency (with respect to the estimated distribution) for bin $i$. The expected frequency is calculated by
% % $$
% % E_i=N(F(Y_u)-F(Y_l)),
% % $$
% % where $F$ is the estimated cumulative distribution function with maximum entropy, $Y_u$ is the upper limit for bin $i$, $Y_l$ is the lower limit for class $i$, and $N$ is the sample size.
% % The $\text{H}_0$ hypothesis (the data are from a population with the estimated distribution) is rejected if
% % \begin{equation}
% %     \chi^2 > \chi^2_{1-\alpha,k-1}
% % \end{equation}
% % where $\chi^2_{1-\alpha,k-1}$ is the chi-square critical value with $k-1$ degrees of freedom and significance level $\alpha$. Here, we set $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and our estimated distribution using maximum entropy method  is $\chi^2=11.3721$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we can not reject the null hypothesis which means the sampled data obtained through running the prob-solvable program Random Walk 1D  follow the  distribution estimated using  3 first moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 
% % % We have the same $\chi^2$ goodness-of-fit test result for the same sampled data and estimated distribution using Gram-Charlier expansion in which the test statistic $\chi^2=11.5346$.

% % % \bigskip


% % % Another goodness-of-fit test is the Kolmogorov-Smirnov which is  used for continuous distributions. The two-sample Kolmogorov-Smirnov test is a  hypothesis test that evaluates the difference between the cdfs of the distributions of the two sample data vectors over the range of $x$ in each data set. The test uses the maximum absolute difference between the cdfs of the distributions of the two data vectors. The test statistic is 
% % %  $$D^\ast=\max_x(|{G}(x)-{F}(x)|),$$
% % % where ${G}(x)$ is the empirical cdf (of the sampled data obtained by running of prob-solvable programs) and F(x) is the cdf of the hypothesized distribution (estimated distribution by moments).

% % % Here we reject the null hypothesis by comparing the $p$-value $p$ with the significance level $\alpha=0.05$, If the $p$-value is very small ($p\text{-value} <\alpha$), then either the null hypothesis is false or something unlikely has occurred.

% % % \begin{table}[tpbh!]
% % %     \centering
% % %  \begin{tabular}{|c|c|c|}
% % % \hline
% % %           {\bf Random Walk 1D}   & $D_{KL}$ &  p-value (KS) \qquad\\
% % %                          \hline
% % %      Maximum Entropy&0.0045 &0.6418\\\hline
% % %      Gram-Charlier& 0.0045&0.6423\\\hline
% % % \end{tabular}
% % %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Random Walk 1D probabilistic program.}
% % %     \label{tableRandomwalk}
        
% % % \end{table}

% % % Table~\ref{tableRandomwalk} shows the  Kullback-Leibler distances between sampled distribution and the estimated distribution  (using 3 first moments by maximum entropy and Gram-Charlier expansion) and also p-values for Kolmogorov–Smirnov goodness-of-fit test for Random Walk 1D probabilistic program. As $p$-values are not smaller than the significance level $\alpha=0.05$, we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of prob-solvable probabilistic program Random Walk 1D follow the  distributions estimated using moments. 




% \iffalse 

% \subsection{Gram-Charlier Expansion}\label{section:GramCharlierExpansion}
% The Gram–Charlier A series  approximates a probability distribution in terms of its cumulants \cite{hald2000early,brenn2017revisit}.  Cumulants $\kappa_n$  (an alternative to the moments) of the distribution are defined using the {\it{cumulant-generating function}} $K(t)=\ln(\text{E}[e^{itX}])$, i.e. the natural logarithm of the characteristic function. The relationship between the  moments and cumulants can be obtained 
% by extracting coefficients from the expansion. The first cumulant, $\kappa_1$, is the mean, $\mu_1$, the second cumulant, $\kappa_2$ is the variance, $\sigma^2$, and the third cumulant is the same as the third central moment. But fourth and higher-order cumulants are not equal to central moments. \todo{Effie: Define central moments $\mu_i$--before they first show up in the paper.}
% The $n$th cumulant can be expressed in terms of the first $n$ moments in a closed form via the determinant of following matrix \cite{broca2004cumulant},
% \begin{align}\label{eq:CumulantMomentRelation}
%     \kappa_n=(-1)^{n+1}\det
%     \begin{pmatrix}
%     \mu_1& 1 & 0 & 0 & 0 & 0 & \dots & 0\\
%     \mu_2& \mu_1 & 1 & 0 & 0 & 0 & \dots & 0\\
%     \mu_3& \mu_2 & \binom{2}{1}\mu_1 & 1 & 0 & 0 & \dots & 0\\
%     \mu_4& \mu_3 & \binom{3}{1}\mu_2 & \binom{3}{2}\mu_1 & 1 & 0 & \dots & 0\\
%     \mu_5& \mu_4 & \binom{4}{1}\mu_3 & \binom{4}{2}\mu_2 &
%     \binom{4}{3}\mu_1 & 1 & \dots & 0\\
%     \vdots& \vdots & \vdots & \vdots & \vdots & \ddots & \ddots & \vdots\\
%     \mu_{n-1}& \mu_{n-2} & \dots & \dots & \dots & \dots & \ddots & 1\\
%     \mu_{n}& \mu_{n-1} & \dots & \dots & \dots & \dots & \dots & \binom{n-1}{n-2}\mu_1 \\
%     \end{pmatrix}
% \end{align}
% Gram-Charlier is similar to the Edgeworth expansion (see, e.g., \cite{Kolassa2006}). Both write the characteristic function of the distribution whose probability density function $f$ is to be approximated in terms of the characteristic function of a known distribution, and recover $f$ through the inverse Fourier transform. They differ as to the arrangement of terms, which may affect the accuracy of truncating the series. As in  the cases we consider here, both perform roughly the same, we focus on the Gram-Charlier expansion. 

% Assume that $f$ is an unknown pdf and we would like to expand $f$ using its cumulants $\kappa_r$ in terms of a known distribution $\psi$. We denote the characteristic function of $f$ by $\hat{f}$ and assume $\hat{\psi}$ and $\gamma_r$ to be the characteristic function and cumulants of the known distribution $\psi$, respectively. Following \cite{wallace1958asymptotic}, 
% \begin{align}
% \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}\kappa_r\frac{(it)^r}{r!}\Big] \quad \text{and} \quad \hat{\psi}(t)=\exp\Big[\sum_{r=1}^{\infty}\gamma_r\frac{(it)^r}{r!}\Big],    
% \end{align}
% which leads to the identity 
% \begin{align}
%  \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(it)^r}{r!}\Big]\hat{\psi}(t).    
% \end{align}
% The term $(it)^r\hat{\psi}(t)$ is exactly the Fourier transform of the term  $(-1)^r[D^r(\psi)(-x)]$, where $D$ is the differential operator with respect to $x$. Thus, the expansion of $f$ in terms of the known distribution $\psi$ is
% \begin{align}
%   {f}(x)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\psi}(x).  
% \end{align}
% Suppose $\psi(x)$ is the normal  density with  mean $\mu=\kappa_1$, variance $\sigma^2=\kappa_2$, and pdf
% \begin{align}
%   \psi(x)=\phi(x)=\frac{1}{\sqrt{2\pi}}\exp\Big[-\frac{(x-\mu)^2}{2\sigma^2}\Big], 
% \end{align}
% Since for all $r>2$, the  higher cumulants $\gamma_r$ of the normal distribution are zero, we obtain the expansion
% \begin{align}
% 	{f}(x)&=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\phi}(x)
% 	= \exp\Big[\sum_{r=3}^{\infty}\kappa_r\frac{(-D)^r}{r!}\Big]{\phi}(x). 
% \end{align}
% Expanding the exponential term using Bell polynomials, we find the \textit{Gram-Charlier A series}, which can be written as
% \begin{align}
%     {f}(x)=\sum_{n=0}^{\infty}B_n(0,0,\kappa_3,\dots,\kappa_n)\frac{(-D)^n}{n!}{\phi}(x),
% \end{align}
% where the $n$-th derivative of the Gaussian function can be presented using Hermite polynomials\footnote{$He_n \left(x\right)$ stands for  the probabilist's Hermite polynomials \cite{johnson2005univariate} which is defined by $He_n \left(x\right)= (-1)^ne^{\frac{x^2}{2}}\frac{d^n}{dx^n}e^{-\frac{x^2}{2}}$}  and the function $\phi$ itself, 
% \begin{align}
%   D^n\phi(x)=\phi^{(n)}(x)=\frac{(-1)^n}{\sigma^n} He_n(\frac{x-\mu}{\sigma}) \phi(x). 
% \end{align}
% The  Gram-Charlier A expansion of the unknown probability density $f$ using its cumulants is
% \begin{align}\label{pdfGC}	{f}(x)={\phi}(x) \sum_{n=0}^{\infty}\frac{1}{n!\sigma^n}B_n(0,0,\kappa_3,\dots,\kappa_n) He_n \left(\frac{x-\mu}{\sigma}\right).
% \end{align}
% %\addnote{\efi{give the formula for $He_n \left(x\right)$} Done!}
% % The cumulative distribution function (CDF) is
% % \begin{align}
% % {F}(x)&=\int_{-\infty}^{x}f(u)du\\\notag
% % &={\Phi}(x)-{\phi}(x) \sum_{n=3}^{\infty}\frac{1}{n!\sigma^{n-1}}B_n(0,0,\kappa_3,\dots,\kappa_n) He_{n-1} \Big(\frac{x-\mu}{\sigma}\Big),    
% % \end{align}
% \begin{figure}[tpbh!]
% 	\centering
% 	%	\includegraphics{Figures/reconstME6Moments.pdf}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier1.eps}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier8Cumulants.eps}\\
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier4CumulantsSecondExample.eps}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier8CumulantsExample2.eps}
% %	\includegraphics[height=5.5cm]{Figures/recostSpline7moments.eps}
% %	\includegraphics[height=5.5cm]{Figures/reconst1Spline.eps}
% 	\caption{Estimation of distribution using Gram-Charlier expansion  with the use of 4 cumulants (left), 8 cumulants (right). Top: $f_X(x)=\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}$. \\Bottom: $g_X(x)=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}$.}
% 	\label{fig:Splinemoments}
% \end{figure}

% In practice, the summation in \eqref{pdfGC} goes up to the order of the cumulant needed to be computed from the corresponding first moments via the cumulants-moments relation \eqref{eq:CumulantMomentRelation}. Discretizing the support of target PDF, we are able to implement our distribution reconstruction methods numerically.   To this end, we consider $a=x_0 < x_1 <x_2 <x_3 <\cdots <x_{n}=b$, discrete points on the $x$-axis and evaluate the Hermite and Bell polynomials and  $\phi(x)$ at these points. 

% \fi








% % Figure~\ref{fig:Splinemoments} shows the estimated distributions for Examples 1 and 2 using 4 and 8 cumulants. The accuracy of the estimation is measured with  the Kullback-Leibler distance (see Equation~\eqref{Kullback-LeiblerDivergence}), shown in Table~\ref{table:Kullback-LeiblerDivergence1}. Examples of estimating known distributions using ME and GC are given in  Appendix A. 

% % % Implementation and numerical results for prob-solvable probabilistic programs will be presented in Section~\ref{Section:Implementation and Benchmark Problems} and estimation of known distribution are investigated in Appendix A.
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %               &  GC &GC\\
% %               &  (4 cumul.)&(8 cumul.)\\
% %               \hline
% %      Example 1&  0.1002 &0.0148\\\hline
% %      Example 2& 0.1373 & 0.0360\\\hline
% % \end{tabular}
% % \vspace{2mm}
% %  \caption{Kullback-Leibler divergence ($D_{KL}$ of true and estimated  distributions with  Gram-Charlier (GC)).}
% %       \label{table:Kullback-LeiblerDivergence1} 
% %  \end{table}

% %%% Moved to the Evaluation Section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % For probabilistic program Random Walk 1D, we have almost the same $\chi^2$ goodness-of-fit test result for the same sampled data and estimated distribution using Gram-Charlier expansion in which the test statistic $\chi^2=11.5346$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ which shows  
% % the sampled data follow the estimated distribution.  

% % Another goodness-of-fit test is the Kolmogorov-Smirnov which is  used for continuous distributions. The two-sample Kolmogorov-Smirnov test is a  hypothesis test that evaluates the difference between the cdfs of the distributions of the two sample data vectors over the range of $x$ in each data set. The test uses the maximum absolute difference between the cdfs of the distributions of the two data vectors. The test statistic is 
% %  $$D^\ast=\max_x(|{G}(x)-{F}(x)|),$$
% % where ${G}(x)$ is the empirical cdf (of the sampled data obtained by running of prob-solvable programs) and F(x) is the cdf of the hypothesized distribution (estimated distribution by moments).
% % %%% Here we reject the null hypothesis by comparing the $p$-value $p$ with the %%%significance level $\alpha=0.05$, If the $p$-value is very small ($p\text{-value} %%%<\alpha$), then either the null hypothesis is false or something unlikely has occurred.
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Random Walk 1D}   & $D_{KL}$ &  p-value (KS) \qquad\\
% %                          \hline
% %      Maximum Entropy&0.0045 &0.6418\\\hline
% %      Gram-Charlier& 0.0045&0.6423\\\hline
% % \end{tabular}
% % \vspace{2mm}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Random Walk 1D probabilistic program.}
% %  \label{tableRandomwalk}
      
% % \end{table}

% % Table~\ref{tableRandomwalk} shows the  Kullback-Leibler distances between sampled distribution and the estimated distribution  (using 3 first moments by maximum entropy and Gram-Charlier expansion) and also p-values for Kolmogorov–Smirnov goodness-of-fit test for Random Walk 1D probabilistic program. As $p$-values are not smaller than the significance level $\alpha=0.05$, we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of prob-solvable probabilistic program Random Walk 1D follow the  distributions estimated using moments. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % \newpage
% % \ahmad{I am going to ignore this sub-section because I did not use it for the simulations.} {\bf The Edgeworth Series:}  Similar to Gram-Charlier expansion, Edgeworth series \cite{hall2013bootstrap} is also used to  approximate a probability distribution in terms of its cumulants. The series are the
% % same but, they differ in the ordering of their terms \cite{benhamou2018gram}. Let $Z_i$ be a sequence of i.i.d. random variables with mean $\mu$ and variance $\sigma^2$, and let $X_n$ be their standardized sums
% % $$X_n=\frac{1}{\sqrt{n}}\sum_{i=1}^{n}\frac{Z_i-\mu}{\sigma}.$$
% % Using the central limit theorem \cite{fischer2010history}, one can see that  the normalized sum $X_n$ tends toward a normal distribution. That is, if $F_n$ be the cumulative distributions of $X_n$, then 
% % $$\lim_{n\rightarrow\infty}F_n(x)=\Phi(x)\equiv\int_{-\infty}^{x}\frac{1}{\sqrt{2\pi}}e^{-\frac{1}{2}q^2}dq$$ 
% % for every $x$, as long as the mean and variance are finite. Assume that random variables $Z_i$ have also higher cumulants $\kappa_r$. Cumulants of $X_n$ can be calculated in terms of cumulants of $Z_i$
% % $$\kappa_r^{F_n}=\frac{n\kappa_r}{\sigma^rn^{r/2}} = \frac{\lambda_r}{n^{r/2-1}} \quad \text{where} \quad \lambda_r=\frac{\kappa_r}{\sigma^r} \quad \text{and}\quad r\geq2.$$
% % The Gram-Charlier A series for the density function $X_n$ would change to 
% % $$	{f}_n(x)={\phi}(x) \sum_{r=0}^{\infty}\frac{1}{r!}B_r\Big(0,0,\frac{\lambda_3}{n^{1/2}},\dots,\frac{\lambda_r}{n^{r/2-1}}\Big) He_r(x).$$
% % In the Edgeworth series the terms are collected according to powers of $n$. To this end, the coefficient of $n^{-m/2}$ term is obtained by collecting monomials of the Bell polynomials corresponding to the integer parts of $m$. Therefore, the characteristic function of unknown distribution would be as
% % $$\hat{f}_n(t)=\Big[1+\sum_{j=1}^{\infty}\frac{P_j(it)}{n^{j/2}}\Big]\exp(-t^2/2), $$
% % where $P_j(x)$ is a polynomial of degree $3j$ with coefficients depending on the cumulants of orders $3$ to $j+2$. Inverse Fourier transform leads us to the pdf  $f_n$ as follows \cite{wallace1958asymptotic} 
% % $${f}_n(x)=\phi(x)+\sum_{j=1}^{\infty}\frac{P_j(-D)}{n^{j/2}}\phi(x). $$ 
% % The first few terms of the Edgeworth expansion are 
% % $${f}_n(x)=\phi(x)-\frac{\lambda_3\phi^{(3)}(x)}{6\sqrt{n}} + \frac{1}{n}\Big(\frac{\lambda_4\phi^{(4)}(x)}{24} + \frac{\lambda_3^2\phi^{(6)}(x)}{72}\Big) + \cdots.$$ 
% % \cite{cramer1928composition} proved that such a series is valid uniformly in $x$. 

% % \efi{What is the connection between Edgeworth and G-C? Since the results look the same?}


% %\subsection{Polynomial Chaos Expansion} 
% %Polynomial Chaos Expansion (PCE) provides a way to represent a random variable $Y$ with finite variance  as a function of an $M$-dimensional random vector $X$, using a polynomial basis that is orthogonal to the distribution of this random vector. 




% % \bigskip
% % \bigskip

% % \newpage
% % \section{Numerical Inversion of Characteristic Functions}

% % For a univariate random variable $X$, with cumulative  distribution
% % function $F$, the characteristic function $\varphi:\mathbb{R}\rightarrow\mathbb{C}$ is defined
% % by
% % $$\varphi(\omega) := E\Big[e^{i\omega X}\Big]= \int_{-\infty}^{\infty} e^{i\omega x} dF(x), $$
% % which is the Fourier transform of the probability distribution function. For any random variable, the characteristic function always
% % exists and it uniquely determines the distribution.  
% % If $F(x)$
% % has a density $f(x)$ then $\varphi(\omega)$ can be written in terms of $f$
% % $$\varphi(\omega) = \int_{-\infty}^{\infty} e^{i\omega x} f(x)dx. $$
% % If we have the characteristic function $\varphi(\omega)$, we can obtain $F(x)$ and $f(x)$ using inversion \cite{bohman1975numerical,mccullagh1994does,waller1995does,waller1995obtaining, witkovsky2016numerical,witkovsky2017computing}. 

% % Having moments (or cumulants) of an unknown distribution, the idea for reconstruction is that we approximate characteristic function of the unknown distribution using function approximation methods, then we will apply numerical inversion of characteristic function to recover PDF and/or CDF of the distribution of interest. Bohman \cite{bohman1975numerical} presented an approximation for inversion of characteristic function to obtsin cumulative distribution function where $E(x)=0$ and $\text{var}(x)=1$ as follows,
% % $$F_X(x)=\frac{1}{2}+\frac{\eta x}{2\pi} - \sum_{\nu=1-H}^{H-1} \frac{\varphi(\eta\nu)}{2\pi i \nu}e^{-i\eta\nu x} \qquad {\nu\neq0},$$
% % where $\eta$ and $H$ are parameters. Waller \cite{waller1995does} showed that even though two random variables have quite similar moments, the characteristic functions are distinct enough to numerically approximate two different cdf's. He applied McCullagh's example \cite{mccullagh1994does} to illustrate how characteristic function can distinguish distribution functions while the moment generating functions are very similar. More details and discussion on Bohman's inversion method are presented in \cite{waller1995obtaining}.
% % %Witkovsky \cite{witkovsky2016numerical,witkovsky2001computing} presented numerical methods to derive PDF/CDF from characteristic function.
% % \bigskip
% % \bigskip

% % \todo{to do /////}
% % \newpage
% % \section{Uncertainty Propagation in Prob-Solvable Probabilistic Programs}
% % Concentration of measure is a well-studied phenomenon with a wealth of results that under suitable conditions
% % provide an upper bound on the probability of deviations from the expected value of a random
% % quantity. References for concentration inequalities for distribution recovery \cite{bouissou2016uncertainty,sankaranarayanan2020quantitative,chakarov2013probabilistic}.

% % Let $X_1,\dots,X_n$ be independent random variables bounded by the interval $[0,1]$. The empirical mean of these variables is defined by
% % $$ {\overline {X}}={\frac{1}{n}}(X_{1}+\cdots +X_{n}).$$
% % Hoefding's inequality states that 
% % $$P\Big(\overline{X}-E\Big[\overline{X}\Big]\geq \delta \Big)\leq e^{-2n\delta^2},$$
% % where $\delta\geq0$.
% % As a  generalization of the Hoeffding's inequality is  that when $X_i$ are strictly bounded by the intervals $[a_i, b_i]$:
% % $$P\Big(\Big|\overline{X}-E\Big[\overline{X}\Big]\Big|\geq \delta \Big)\leq 2\exp{\Big(-\frac{2n\delta^2}{\sum_{i=1}^n (b_i-a_i)^2}\Big)}.$$
% % $E\Big[\overline{X}\Big]$ is the expected value of $\overline{X}.$

% % Here, we would like to analyse the uncertainty propagation through prob-solvable probabilistic programs. We would like to find an upper  bound  on  the  probability  of deviation of a random variable   from  its expected  value that we are able to compute symbolically using Mora tool. We are not going to run the program itself to see what happens to a random variable, say $X$, after a fixed number of loop iterations being executed, but using calculated $E(X)$  by Mora, we are able to quantify how far a realization of $X$ could be from $E(X)$ before we run the loop.  Consider  Random Walk 1D probabilistic program:  
% % \begin{align*}
% % &v:=0\\
% % &x:=0\\
% % &\text{while true:}\\
% % &\quad v:=\text{uniform}(0,1)\\
% % &\quad x:=x+v\;\;[7/10]\;\;x-v
% % \end{align*}  
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% % % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% % 	\caption{Mora generated $E(x)$ compared to the sampled $x$  in  Random Walk 1D stopping at each iteration of loop.}
% % 	%\label{fig:SampledEXforRandomWalk1Sample1000loop}
% % \end{figure}
% % Without running the program, Mora computes moments of random variable $X$ for each iteration of loop as $E(X)=\frac{n}{5}$ and $E(X^2)=\frac{n^2}{25} + \frac{22n}{75}$ where $n$ is the number of loop iteration.  
% % Applying the generalization of the Hoefding's inequality, 
% % $$P\Big({X}-E\Big[{X}\Big]\geq \delta \Big)\leq \exp{\Big(-\frac{2\delta^2}{(b-a)^2}\Big)}.$$
% % where $a=-n$ and $b= n$ are lower and upper bounds for $X$, respectively,  with $P(a\leq X\leq b)=1$. If we take $n$ number of loop iterations to be, for example 1000, then the probability of being bigger than  $E(X)=200$ as $\delta$ is at maximum $\exp(-\frac{2\delta^2}{2000^2})$.
% % %\begin{figure}[tpbh!]
% % %	\centering
% % %	\includegraphics[height=5.5cm]{Figures/ConcentrationIneqBounds.eps}
% % %		\caption{Hoefding's and Bernstein's Upper Bounds for Random Walk 1D.}
% % %	\label{fig:ConcentrationIneqBounds}
% % %\end{figure}
    


% % Bernstein inequality is another concentration inequality  that provides
% % sharper bounds on distances between a realization  and the expectation of the random variable. If $P(|X_i|\leq c)=1$ and $E(X_i)=\mu$ then, for any $\delta>0$, 
% % $$P\Big(\Big|{\overline{X}}-\mu\Big|\geq \delta \Big)\leq 2\exp{\Big(-\frac{n\delta^2}{2\sigma^2 + 2c\delta/3}\Big)},$$
% % where $\sigma^2=\frac{1}{n}\sum_{i=1}^{n}\text{Var}(X_i).$


% \subsection{PPs with Prob-solvable loops}

% Prob-solvable programs are generalization of $P$-solvable programs  allowing probabilistic 
% assignments over random variables and distributions.
% %\begin{definition}\cite{bartocci2019automatic}
%     Let $m\in\mathbb{N}$ and $x_1,\dots,x_m$ denote real-valued program variables.
% Prob-solvable loops  with $x_1,\dots,x_m$ variables are programs of the following form \cite{bartocci2019automatic}:
% \begin{align}
%     I; \text{ while (true) } \{U\},
% \end{align}
% where $I$ is a sequence of initial assignments over $x_1,\dots,x_m$ (i.e. $x_1:=c_1,x_2:= c_2,\dots,x_m:=c_m$, with $c_i\in \mathbb{R}$ representing a real number
% drawn from a known distribution). $U$ is a sequence of $m$ random updates as the loop body. Each update is of the form:
% \begin{align}\label{poly-assgmt}
%  x_i := a_ix_i + P_i(x_1,\dots,x_{i-1})\; [p_i] \; b_ix_i + Q_i(x_1,\dots,x_{i-1}),   
% \end{align}
% where $a_i, b_i\in\mathbb{R}$ are constants and $P_i, Q_i  \in \mathbb{R}[x_1,\dots,x_{i-1}]$ are polynomials
% over program variables $x_1,\dots,x_{i-1}$ and  $p_i \in [0, 1]$  is the probability
% of updating $x_i$ to $a_ix_i + P_i(x_1,\dots,x_{i-1})$, whereas the probability to update $x_i$ to
% $b_ix_i + Q_i(x_1,\dots,x_{i-1})$  is $1-p_i$.
% %\end{definition}

% Considering a Prob-solvable
% program with $n\in \mathbb{N}$ denoting the loop iteration counter, \cite{bartocci2019automatic} show that variable
% updates of Prob-solvable programs lead to  special recurrences in $n$, so-called moment-based
% recurrences. Assume that the sequences
% $x_1(n),\dots,x_m(n)$  describe relations between values of $x_i$ at
%  loop iteration $n$. Then Prob-Solvable updates are expressed as 
%  \begin{align}
% &  x_i(n+1) := a_ix_i(n)\\\notag
% & + P_i(x_1(n),\dots,x_{i-1}(n))\; [p_i] \; b_ix_i(n) + Q_i(x_1(n),\dots,x_{i-1}(n)).   
%  \end{align}
 
%  PPs with Prob-solvable loops: Bartocci et al. (2019) \cite{bartocci2019automatic, bartocci2020mora} calculate all moments of all generated random variables via recurrence
% relations when assignments are of a specific form (see \eqref{poly-assgmt}). We focus on random variables generated in Prob-solvable loops. Our aim is to recover their distribution from their moments. 

% This can be easily answered when the distributions of the random variables produced by a PP are among the known and
% well studied distributions in Statistics. %One approach is to study recurrence relations that characterize variable updates that result in known distributions.
% When distributions are not recognized as known, the task is more difficult and is the focus of this paper.
% %we should use or adapt the approaches based on conditional expectation  to analyze the discrete and/or continuous random variables produced by prob-solvable PPs \cite{kotz1980some,su2000characterizations,zoroa1990characterization}. 


% % We investigate  recurrence relations that characterize variable updates that result in known distributions. We should identify the class of PPs that admit closed-form distribution(s) of the underlying random variables and reconstruct  their distributions via higher order moments.

% \mm{This is a bit outdated with Polar. Important is that under some conditions moments can be obtained precisely. And given precise moments we can start reconstructing the distribution. It doesn't really matter where this moments came from (as discussed in our last meeting).}


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %\newpage
% \section{Implementation and Benchmark Problems: Distribution Reconstruction in Probabilistic Programs}\label{Section:Implementation and Benchmark Problems}
% In this section, we apply the approaches in Sections \ref{section:MaximumEntropyMethod} and \ref{section:GramCharlierExpansion} to estimate distributions of the random variables of probabilistic programs in \cite{bartocci2019automatic} using their calculated moments via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora} without executing programs. With the help of  statistical tools, we also confirm the agreement of our estimated distributions with the ones generated during the execution of these probabilistic programs. We refer to Section~\ref{section:Evaluation} for evaluation of estimations for the benchmark programs.  We  do our assessment for the Random Walk 1D and the  selected probabilistic programs (see Table~\ref{table:BenchmarkPrograms}) for which the exact calculated moments are available on in Table~\ref{Table:Benchmarks}. 

% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|clc|clc|clc|}
% \hline
%       \multirow{3}{*}{} 
%       &&&&& &&&\\
% \hspace{2mm}&{\bf StutteringP}&\hspace{2mm}&\hspace{3mm}& {\bf Square} & \hspace{2mm}&\hspace{3mm}&  {\bf Binomial($p$)} \hspace{10mm} & \hspace{2mm}\\
% &&&&&&&&\\
% &$f:=0$&&& $x:=0$ &&& $x:=0$ &\\
% &$x:=-1$&&& $y:=1$ &&&$\text{while true:}$&\\
% &$y:=1$&&& $\text{while true:}$ &&&$\quad x:=x+1\;\;[\;p\;]\;\;x$ &\\
% &$s:=0$&&& $\quad x:=x+2\;\;[1/2]\;\;x$  &&&&\\
% &$\text{while true:}$&&& $\quad y:=x^2$ &&&&\\
% &$\quad f:=1\;\;[\;{ p }\;]\;\;0$&&&  &&&&\\
% &$\quad x:=x+f*\text{uniform}(0,2)$&&&  &&&&\\
% &$\quad y:=y+f*\text{uniform}(0,4)$&&&  &&&&\\
% &$\quad s:=x+y$&&&&  &&&\\
% &&&&&  &&&\\
%                          \hline
                         
% &&&&& &&&\\
% \hspace{2mm}&{\bf Sum Rand. Series}  &\hspace{2mm}&\hspace{3mm}& {\bf Prod. Dep. Vars.}  & \hspace{2mm}&\hspace{3mm}& {\bf Bimodal}  & \hspace{2mm}\\
% &&&&& &&&\\
% &$n:=0$&&& $f:=0$ &&& $....$ &\\
% &$x:=0$&&& $x:=0$ &&& $....$ &\\
% &$\text{while true:}$&&& $y:=0$ &&& $....$ &\\
% &$\quad n:= n + 1$&&& $p:=0$ &&& $....$ &\\
% &$\quad x:=x+n\;\;[1/2]\;\;x$&&& $\text{while true:}$ &&& $....$ &\\
% &  &&& $\quad f:=0\;\;[1/2]\;\;1$ &&& $....$ &\\
% &  &&& $\quad x:=x+f$ &&& $....$ &\\
% &  &&& $\quad y:=y+1-f$ &&& $....$ &\\
% &  &&& $\quad p:=x \ast y$ &&& $....$ &\\
% &&&&& &&&\\
%                          \hline
                         
%                          &&&&& &&&\\
% \hspace{2mm}&{\bf ..... }&\hspace{2mm}&\hspace{3mm}& {\bf ..... } & \hspace{2mm}&\hspace{3mm}& {\bf .... } & \hspace{2mm}\\
% &&&&& &&&\\

% &&&&& &&&\\
%                          \hline
    
% \end{tabular}
% \vspace{2mm}
%  \caption{Benchmark Programs.}
%     \label{table:BenchmarkPrograms}
        
% \end{table}



% % \addnote{Explain why I did choose these 3 programs. Any other suggestion Marcel and Miroslav?}
% \mm{See my comment above. Also you could again take (loop-free) programs from PSI and try to approximate the distribution with just the moments.}




% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|l|}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
 
 
%  \multirow{3}{*}{StutteringP}&1& $E[s(n)] = 3np $ \\\cline{2-3}
%     &2& $E[s^2(n)] = 9n^2p^2 - 9np^2+\frac{32}{3}np$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{} $E[s^3(n)] = 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
%       & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
%       & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
%       & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
%       & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
%     \\\hline
%         \hline
   
% \multirow{3}{*}{Square}&1& $E[y(n)] = n^2+n$  \\\cline{2-3}
%     &2&$E[y^2(n)] = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
%     &3&$E[y^3(n)] = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
%         \hline
        
% \multirow{3}{*}{Binomial($p$)}&1&$E[x(n)] = np$  \\\cline{2-3}
%     &2& $E[x^2(n)] = n^2p^2 + np(1-p)$  \\\cline{2-3}
%     &3&$E[x^3(n)] = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
%         \hline        

% \multirow{3}{*}{Sum Rand. Series}&1&$E[x(n)] = n^2/4 + n/4$  \\\cline{2-3}
%     &2& $E[x^2(n)] = n^4/16 + 5n^3/24 + 3n^2/16 + n/24$  \\\cline{2-3}
%     &3&$E[x^3(n)] = n^6/64 + 7n^5/64 + 13n^4/64 + 9n^3/64 + n^2/32$    \\\hline
%         \hline        
 
% \multirow{3}{*}{Prod. Dep. Var.}&1&$E[p(n)] = n^2/4 - n/4$  \\\cline{2-3}
%     &2& $E[p^2(n)] = n^4/16 - n^3/8 + 3n^2/16 - n/8$  \\\cline{2-3}
%     &3& \multirow{3}{*}{}$E[x^3(n)] = n^6/64 - 3n^5/64 + 9n^4/64 - 21n^3/64$ \\
%     & &+ $15n^2/32 -n/4$    \\\hline
%         \hline        
        
% \multirow{3}{*}{Bimodal}&1& .  \\\cline{2-3}
%     &2&.  \\\cline{2-3}
%     &3&.   \\\hline
%         \hline   
        
% \multirow{3}{*}{Loop free PPs}&1& .  \\\cline{2-3}
%     &2&.  \\\cline{2-3}
%     &3&.   \\\hline
%         \hline   
% \end{tabular}
% \vspace{2mm}
%  \caption{Benchmarks}
%  \label{Table:Benchmarks}
% \end{table}



% % \subsection{Random Walk 1D} 

% % \begin{align}
% % &v:=0\\\notag
% % &x:=0\\\notag
% % &\text{while true:}\\\notag
% % &\quad v:=\text{uniform}(0,1)\\\notag
% % &\quad x:=x+v\;\;[7/10]\;\;x-v
% % \end{align}
% % Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~1 of  \cite{bartocci2019automatic}: 
% % \begin{align}
% % &E[x(n)] = n/5\\
% % &E[x^2(n)] = n^2/25 + 22n/75\\
% % &E[x^3(n)] = n^3/125 + n^222/125 - n21/250
% % \end{align}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% % % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% % 	\caption{Mora generated $E(x)$ compared to the sampled $x$  in  Random Walk 1D stopping at each iteration of loop.}
% % 	\label{fig:SampledEXforRandomWalk1Sample1000loop}
% % \end{figure}

% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1000loop1000Sample.eps}
% % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ $E(x)$ and $E(x^2)$ for Random Walk 1D using 1000 sample for each iteration of loop.}
% % 	\label{fig:SampledEXforRandomWalk1000Sample1000loop}
% % \end{figure}


% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=3.8cm]{Figures/histogramRandomwalk1D.eps}
% % 	\includegraphics[width=3.8cm]{Figures/pdfRandomwalk1DME.eps}
% % 	\includegraphics[width=3.8cm]{Figures/cdfRandomwalk1DME.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Random Walk 1D. Estimation of Distribution using Maximum Entropy method with 3 moments.}
% % 	\label{fig:pdfRandomwalk1DME}
% % \end{figure}


% % We apply Chi-Square Goodness-of-Fit Test to see if  our sampled data came from a population with the estimated distribution. To this end,  we consider following hypothesis:

% % \bigskip

% % \hspace{10mm} $\text{H}_0$:	The data follow the estimated distribution.

% % \hspace{10mm} $\text{H}_a$:	The data do not follow the estimated distribution.

% % \bigskip	

% % For the chi-square goodness-of-fit computation, we divide the data  into $k$ bins and define the test statistic as
% % \begin{equation}
% %     \chi^2=\sum\limits_{i=1}^k(O_i-E_i)^2/E_i,
% % \end{equation}
% % where $O_i$ is the observed frequency for bin $i$ and $E_i$ is the expected frequency (with respect to the estimated distribution) for bin $i$. The expected frequency is calculated by
% % $$
% % E_i=N(F(Y_u)-F(Y_l)),
% % $$
% % where $F$ is the estimated cumulative distribution function with maximum entropy, $Y_u$ is the upper limit for bin $i$, $Y_l$ is the lower limit for class $i$, and $N$ is the sample size.
% % The $\text{H}_0$ hypothesis (the data are from a population with the estimated distribution) is rejected if
% % \begin{equation}
% %     \chi^2 > \chi^2_{1-\alpha,k-1}
% % \end{equation}
% % where $\chi^2_{1-\alpha,k-1}$ is the chi-square critical value with $k-1$ degrees of freedom and significance level $\alpha$. Here, we set $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and our estimated distribution using maximum entropy method  is $\chi^2=11.3721$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we can not reject the null hypothesis which means the sampled data obtained through running the prob-solvable program Random Walk 1D  follow the  distribution estimated using  3 first moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 
% % We have the same $\chi^2$ goodness-of-fit test result for the same sampled data and estimated distribution using Gram-Charlier expansion in which the test statistic $\chi^2=11.5346$.

% % \bigskip


% % Another goodness-of-fit test is the Kolmogorov-Smirnov which is  used for continuous distributions. The two-sample Kolmogorov-Smirnov test is a  hypothesis test that evaluates the difference between the cdfs of the distributions of the two sample data vectors over the range of $x$ in each data set. The test uses the maximum absolute difference between the cdfs of the distributions of the two data vectors. The test statistic is 
% %  $$D^\ast=\max_x(|{G}(x)-{F}(x)|),$$
% % where ${G}(x)$ is the empirical cdf (of the sampled data obtained by running of prob-solvable programs) and F(x) is the cdf of the hypothesized distribution (estimated distribution by moments).

% % Here we reject the null hypothesis by comparing the $p$-value $p$ with the significance level $\alpha=0.05$, If the $p$-value is very small ($p\text{-value} <\alpha$), then either the null hypothesis is false or something unlikely has occurred.

% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Random Walk 1D}   & $D_{KL}$ &  p-value (KS) \qquad\\
% %                          \hline
% %      Maximum Entropy&0.0045 &0.6418\\\hline
% %      Gram-Charlier& 0.0045&0.6423\\\hline
% % \end{tabular}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Random Walk 1D probabilistic program.}
% %     \label{tableRandomwalk}
        
% % \end{table}

% % Table~\ref{tableRandomwalk} shows the  Kullback-Leibler distances between sampled distribution and the estimated distribution  (using 3 first moments by maximum entropy and Gram-Charlier expansion) and also p-values for Kolmogorov–Smirnov goodness-of-fit test for Random Walk 1D probabilistic program. As $p$-values are not smaller than the significance level $\alpha=0.05$, we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of prob-solvable probabilistic program Random Walk 1D follow the  distributions estimated using moments. 





% % % %\newpage
% % \subsection{StutteringP}\label{subsectionStutteringP} 

% % \begin{align*}
% % &f:=0\\
% % &x:=-1\\
% % &y:=1\\
% % &s:=0\\
% % &\text{while true:}\\
% % &\quad f:=1\;\;[\text{ p }]\;\;0\\
% % &\quad x:=x+f*\text{uniform}(0,2)\\
% % &\quad y:=y+f*\text{uniform}(0,4)\\
% % &\quad s:=x+y\\
% % \end{align*}

% Exact moments of the output  random variable of each probabilistic program are computed as functions of $n$, iteration of the loop are available in Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}: Table~1)\footnote{The second moment $E[s^2(n)]$ here differs from the one mentioned in \cite{bartocci2019automatic} as it did not agree with the simulations. The Calculations are presented in Appendix B.}. 
% % \begin{align}
% % &E[s(n)] = 3np \label{1st}\\
% % &E[s^2(n)] = 9n^2p^2 - 9np^2+\frac{32}{3}np\label{2nd}\\
% % &E[s^3(n)] = 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3) \notag\\
% % &+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)\notag\\ &+3np(4p^2-3p+3)+3np(8p^2-12p+9) \notag \\
% % &+ np(p^2-3p(-p-1)-3p+2)/2\notag \\
% % &+2np(2p^2 -6p(-p+2)-6p+13) +6 \label{3rd}
% % \end{align}

% % % \newpage
% % % \includepdf[pages=-]{deriveSecondmoment.pdf}

% % In order to assess the our estimations, we set the number of loop in the StutteringP program to be 100 and we take 1000 sample for the output $s$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments.   To perform the $\chi^2$ goodness-of-fit test for the StutteringP benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the maximum entropy estimated distribution  is $\chi^2=15.1544$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program StutteringP follow the  distribution estimated using  moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 


% % For the Kolmogorov-Smirnov goodness-of-fit test, we set again the significance level $\alpha=0.05$.  The test result is reported in Table~\ref{tableStutteringP}. In this test $p$-value is greater than the significance level $\alpha$, therefore we can not reject the $\text{H}_0$.

% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Square}   & $D_{KL}$ &  p-value (KS) \qquad\\
% %                          \hline
% %      Maximum Entropy& 0.00425 & 0.4494\\\hline
% % \end{tabular}
% % \vspace{2mm}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for the StutteringP probabilistic program. As p-value is greater than the  significance  level $\alpha=0.05$, the $\text{H}_0$ is not rejected which states that the sampled data obtained by the StutteringP program follow the maximum entropy estimated distribution. }
% %  \label{tableStutteringP}
% % \end{table}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/ExSampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex2SampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex3SampledandMora1000sample1000loopSttuteringP.eps}
% 	\caption{ $E(S)$, $E(S^2)$ and $E(S^2)$ for Stuttering P using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora1000loop1000sampleStutteringP}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/histogramStutteringP100loop1000sample.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfStutteringP100loop1000sampleME.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfStutteringP100loop1000SampleME.eps}
% 	\caption{ Left: histogram of sampled data by executing the StutteringP program (number of samples is 1000 and number of loop iteration in SutteringP is 100). Middle: pdf of sampled (kernel density estimation) and maximum entropy estimated Distribution for SutteringP. Right: cdf of sampled distribution and Maximum Entropy Estimation  for random varible $S$ in SutteringP.  }
% 	\label{fig:StutteringP100loop1000sample}
% \end{figure}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[height=5.5cm]{Figures/MEforStutterinP.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled and Estimated Distribution for Stuttering P. Estimation of Distribution using Maximum Entropy with 2 cumulants.}
% % 	\label{fig:MEforStutterinP}
% % \end{figure}

% %\newpage
% % \subsection{The Square Probabilistic Program} 
% % Square is a prob-solvable probabilistic program with polynomial assignment \cite{bartocci2019automatic}. The exact moments are available in Table~\ref{Table:Benchmarks}.
% % \begin{align*}
% % &x:=0\\
% % &y:=1\\
% % &\text{while true:}\\
% % &\quad x:=x+2\;\;[1/2]\;\;x\\
% % &\quad y:=x^2\\
% % \end{align*}
% % Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop (\cite{bartocci2019automatic}: Table~1): 
% % \begin{align*}
% % &E[y(n)] = n^2+n\\
% % &E[y^2(n)] = n^4+6n^3+3n^2-2n\\
% % &E[y^3(n)] = n^6+15n^5+45n^4-15n^3-30n^2+16n
% % \end{align*}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4.2cm]{Figures/ExSampledandMora100loop1sampleSquare.eps}
% % % 	\includegraphics[width=4.2cm]{Figures/Ex2SampledandMora100loop1sampleSquare1.eps}
% % 	\caption{Mora generated  $E(Y)$ compared to the sampled $y$ in  Square probabilistic program stopped at each iteration of loop.}
% % 	\label{fig:ExSampledandMora100loop1sampleSquare}
% % \end{figure}
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/ExSampledandMora100loop1000sampleSquare.eps}
% 	\includegraphics[width=4.2cm]{Figures/Ex2SampledandMora100loop1000sampleSquare.eps}
% 	\caption{ $E(Y)$ and $E(Y^2)$ for Square using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora100loop1000sampleSquare}
% \end{figure}

% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[height=5.5cm]{Figures/pdfSampledandMoraSquare.eps}
% % 	\includegraphics[height=5.5cm]{Figures/cdfSampledandMoraSquare.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled (kernel density estimation) and Gram-Charlier Estimated Distribution for Square. Estimation of Distribution using Gram-Charlier Expansion with 3 cumulants.}
% % 	\label{fig:GramCharlierforSquare}
% % \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/HistogramSquare1000Sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfSquare1000sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfSquare1000sample1000loop.eps}
% 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% 	\caption{Left: histogram of sampled data by executing the Square program (number of samples is 1000 and number of loop iteration in Square is 1000). Middle: pdf of sampled (kernel density estimation) and Gram-Charlier Estimated Distribution for Square. Estimation of Distribution using Gram-Charlier Expansion with 3 cumulants. Right: cdf of sampled distribution and Gram-Charlier estimation.}
% 	\label{fig:GramCharlierforSquare}
% \end{figure}



% \todo{explain about figures}



% {\bf Programs with Known Distribution:} Variable $x$ and $y$ in the Square program are inherently discrete random variables. Consider a Bernoulli process as a sequence of independent random variables $t_1, t_2, t_3 , \dots$ such that for each $i=1,2,3,\dots$, the variable $t_i$ is 0 or 1, and for all $i$, $P(t_i=1)=p$. In our special case, $p=1/2$. Using Bernoulli process we can rewrite the Square program as follows:
% \begin{align*}
% &x:=0\\
% &y:=1\\
% &\text{while true:}\\
% &\quad t:=1\;\;[ p ]\;\;0\\
% &\quad x:=x+2*t\\
% &\quad y:=x^2\\
% \end{align*}
% Note that $x$ and $y$ are somehow sum of Bernoulli variables which have Binomial distributions. In a more general case, we can use $x:=x+f(t)$ to update variable $x$, where  $f:\{0,1\}\rightarrow \mathbb{R}$ is a function for which $f(0)\neq f(1)$. In this case again we have Binomial distribution.   



% \bigskip
% \bigskip
% \bigskip



% % In order to assess the our estimations, we fix the number of loop in the Square program to be 1000 and we take 1000 sample for the output, i.e. the variable $y$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments (cumulants).   To perform the $\chi^2$ goodness-of-fit test for the Square benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the Gram-Charlier estimated distribution  is $\chi^2=9.9100$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program Square  follow the  distribution estimated using  moments (cumulants) calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 

% % Table~\ref{tableSquare} shows the result for the Kolmogorov–Smirnov goodness-of-fit test as well as the Kullback-Leibler between sampled and estimated distributions. As $p$-value is greater than the  significance  level $\alpha=0.05$, the $\text{H}_0$ is not rejected which states that the sampled data obtained by Square program follow the Gram-Charlier estimated distribution.

% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Square}   & $D_{KL}$ &  p-value (Kolmogorov–Smirnov) \qquad\\
% %                          \hline
% %      Gram-Charlier& 0.0025 & 0.0886\\\hline
% % \end{tabular}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Square probabilistic program.  }
% %   \label{tableSquare}
% % \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \newpage
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  \multirow{3}{*}{Random Walk 1D}&1& 20 & $9.20\times 10^{-2}$  &$2.37 \times 10^{-5}$&$1.88\times 10^{-6}$\\\cline{2-6}
% %     &2& $4.2933 \times 10^2 $ &  $4.23 \times 10^{0}$ &$5.25\times 10^{-4}$& $6.63 \times 10^{-5}$\\\cline{2-6}
% %     &3& $9.7516 \times 10^3$  & $1.45 \times 10^{2} $ &$1.04\times 10^{-2}$& $3.56 \times 10^{-3}$\\\cline{2-6}
% %     &4&   & &   &  \\\cline{2-6}
% %     &5&   & &   &  \\\cline{2-6}
% %     &6&   & &   &  \\\cline{2-6}
% %     &7&   & &   &  \\\cline{2-6}
% %     &8&   & &   &  
% %     \\\hline
% %         \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In Table~\ref{table:AbsoluteandRelativeErrors}, we compare  errors of sample moments and estimated ones. Here, we first use 3 exact moments of each benchmark program and estimate the target distribution using these moments. Having the distribution for the variable of interest, we compute moments of order 4 to 10 and we call them estimated moments. Comparing first 10 moments of the underlying variable yields absolute estimate errors as \textit{absolute error of }$E(x^i)= |{E(x^i)}_{estimate}-{E(x^i)}_{exact}|$. Normalizing obtained errors with the exact moments we reach the \textit{relative estimate errors}. The same process is done for the \textit{absolute and relative sample errors}, but instead of estimated moments we compare  sample moments to the exact ones. Comparing two columns of sample error and estimate error shows the importance of the distribution recovery as the errors (absolute and relative) of moments obtained by estimated distribution are less than the errors of moments calculated by sampled data. 
% \begin{table}[tpbh!]\label{table:AbsoluteandRelativeErrors}
%     \centering
%  \begin{tabular}{|c|c|c|c|c|}
% \hline
%   {\bf Program}   & Moment &   Exact Value$^{1}$  & Absol. sample error$^{2}$   &Absol. estimate error$^{3}$  \\
%     &  & & (relative error$^\ast$)&  (relative error$^\ast$) \\
%                          \hline
%                          \hline
 
%  \multirow{3}{*}{RandomWalk1D}&1& 20 & $9.20\times 10^{-2} (0.5\%)$  &$1.88\times 10^{-6} (0.00001\%)$\\\cline{2-5}
%     &2& $4.2933 \times 10^2 $ &  $4.23 \times 10^{0} (1.0\%)$& $6.63 \times 10^{-5} (0.000015\%)$\\\cline{2-5}
%     &3& $9.7516 \times 10^3$  & $1.45 \times 10^{2} (1.5\%) $& $3.56 \times 10^{-3} (0.000037\%)$\\\cline{2-5}
%     &4&   & &     \\\cline{2-5}
%     &5&   & &    \\\cline{2-5}
%     &6&   & &    \\\cline{2-5}
%     &7&   & &    \\\cline{2-5}
%     &8&   & &    
%     \\\hline
%         \hline

%  \multirow{3}{*}{StutteringP}&1& 210 & $2.29\times 10^{-1} (0.1\%)$  &$8.11\times 10^{-5} (0.000038\%)$\\\cline{2-5}
%     &2& $4.4405 \times 10^4 $ &  $8.16 \times 10^{1} (0.2\%)$& $1.76 \times 10^{-2} (0.000039\%)$\\\cline{2-5}
%     &3& $9.3823 \times 10^6$  & $5.01 \times 10^{4} (0.5\%) $& $7.12 \times 10^{4} (0.75\%)$\\\cline{2-5}
%     &4&   & &     \\\cline{2-5}
%     &5&   & &    \\\cline{2-5}
%     &6&   & &    \\\cline{2-5}
%     &7&   & &    \\\cline{2-5}
%     &8&   & &    
%     \\\hline
%         \hline

%  \multirow{3}{*}{Square}&1& 10100 & $1.024\times 10^1 (0.1\%)$  &  $1.1063\times 10^{0} (0.01\%)$   \\\cline{2-5}
%     &2& $1.060298 \times 10^8$ & $6.78\times 10^5 (0.6\%)$ & $2.3037\times 10^3 (0.002\%)$    \\\cline{2-5}
%     &3& $1.1545\times 10^{12}$  &$1.93\times 10^{10} (1.7\%)$  &  $1.2681\times 10^7 (0.001\%)$  \\\cline{2-5}
%     &4&   & &     \\\cline{2-5}
%     &5&   & &     \\\cline{2-5}
%     &6&   & &     \\\cline{2-5}
%     &7&   & &     \\\cline{2-5}
%     &8&   & &     
         
%     \\\hline
%         \hline



% %  \multirow{3}{*}{StutteringP}&1& $E[s(n)] = 3np $ \\\cline{2-3}
% %     &2& $E[s^2(n)] = 9n^2p^2 - 9np^2+\frac{32}{3}np$  \\\cline{2-3}
% %     &3&  \multirow{3}{*}{} $E[s^3(n)] = 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
% %       & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
% %       & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
% %       & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
% %       & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
% %     \\\hline
% %         \hline
   
% % \multirow{3}{*}{Square}&1& $E[y(n)] = n^2+n$  \\\cline{2-3}
% %     &2&$E[y^2(n)] = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
% %     &3&$E[y^3(n)] = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
% %         \hline
        
% % \multirow{3}{*}{Binomial(p)}&1&$E[x(n)] = np$  \\\cline{2-3}
% %     &2& $E[x^2(n)] = n^2p^2 + np(1-p)$  \\\cline{2-3}
% %     &3&$E[x^3(n)] = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
% %         \hline        

% % \multirow{3}{*}{Sum Rand. Series}&1&$E[x(n)] = n^2/4 + n/4$  \\\cline{2-3}
% %     &2& $E[x^2(n)] = n^4/16 + 5n^3/24 + 3n^2/16 + n/24$  \\\cline{2-3}
% %     &3&$E[x^3(n)] = n^6/64 + 7n^5/64 + 13n^4/64 + 9n^3/64 + n^2/32$    \\\hline
% %         \hline        
 
% % \multirow{3}{*}{Prod. Dep. Var.}&1&$E[p(n)] = n^2/4 - n/4$  \\\cline{2-3}
% %     &2& $E[p^2(n)] = n^4/16 - n^3/8 + 3n^2/16 - n/8$  \\\cline{2-3}
% %     &3&$E[x^3(n)] = n^6/64 - 3n^5/64 + 9n^4/64 - 21n^3/64 + 15n^2/32 -n/4$    \\\hline
% %         \hline        
        
% % \multirow{3}{*}{Bimodal}&1& .  \\\cline{2-3}
% %     &2&.  \\\cline{2-3}
% %     &3&.   \\\hline
% %         \hline   
        
% % \multirow{3}{*}{Loop free PPs}&1& .  \\\cline{2-3}
% %     &2&.  \\\cline{2-3}
% %     &3&.   \\\hline
% %         \hline   
% \end{tabular}
% \vspace{2mm} 
%  \caption{Error for Benchmarks:\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Table ~\ref{Table:Benchmarks})\\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$}
%  \label{Table:ErrorforBenchmarks}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \bibliographystyle{splncs04}
% \bibliography{refs1}
%
% \begin{thebibliography}{8}
% \bibitem{ref_article1}
% Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

% \bibitem{ref_lncs1}
% Author, F., Author, S.: Title of a proceedings paper. In: Editor,
% F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
% Springer, Heidelberg (2016). \doi{10.10007/1234567890}

% \bibitem{ref_book1}
% Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
% Location (1999)

% \bibitem{ref_proc1}
% Author, A.-B.: Contribution title. In: 9th International Proceedings
% on Proceedings, pp. 1--2. Publisher, Location (2010)

% \bibitem{ref_url1}
% LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
% Oct 2017
% \end{thebibliography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \newpage

% \section{Appendix A: Estimation of Known Distributions}

% % \subsection{Cauchy Distribution}

% % \todo{explain more!!!}


% % The Cauchy distribution has the probability density function 
% % \begin{align*}
% %     f(x)=\frac{1}{\pi\gamma\Big[1+\Big(\frac{x-x_0}{\gamma}\Big)^2\Big]}
% % \end{align*}
% % where $x_0$   is the location parameter specifies location of the peak of the distribution, and  the scale parameter $\gamma$   specifies half the width of the PDF at half the maximum height.

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4.2cm]{Figures/MEforCauchyDist6moments.eps}
% % 	\caption{Maximum Entropy with 6 moments: Standard Cauchy Distribution.}
% % 	\label{fig:MEforChauchyDist6moments}
% % \end{figure}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4.2cm]{Figures/GramCharlierCauchyDist4Cumulants.eps}
% % 	\includegraphics[width=4.2cm]{Figures/GramCharlierCauchyDist8Cumulants.eps}
% % 	\caption{Gram-Charlier for Standard Cauchy Distribution: with 4 cumulants (left), with 8 cumulants (right)}
% % 	\label{fig:GramCharlierforChauchyDist6moments}
% % \end{figure}

% % \bigskip
% % %\newpage
% \subsection{Normal Mixture Distribution}

% \addnote{explain more!!!}

% Normal mixture: $f(x)=\alpha N(\mu_1,\sigma_1)+(1-\alpha) N(\mu_2,\sigma_2)$, $\alpha \in (0,1)$.
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/MEforNormalMixture.eps}
% 	\includegraphics[width=3.8cm]{Figures/MEforNormalMixturealph05.eps}
% 	\includegraphics[width=3.8cm]{Figures/MEforNormalMixturealpha018.eps}
% 	\caption{Maximum Entropy for Normal Mixture with $\mu_1=-2, \sigma_1=1, \mu_2=1, \sigma_2=1$:   $\alpha=0.85$ (left),  $\alpha=0.5$ (middle), $\alpha=0.19$ (right).}
% 	\label{fig:MEforNormalMixtureDist6moments}
% \end{figure}


% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture4cumulantsalpha085.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture4cumulantsalpha05.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture4cumulantsalpha019.eps}\\
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture8cumulantsalpha0850.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture8cumulantsalpha05.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture8cumulantsalpha019.eps}
% 	\caption{Maximum Entropy for Normal Mixture with $\mu_1=-2, \sigma_1=1, \mu_2=1, \sigma_2=1$: (top: 4 cumulants, bottom: 8 cumulants);  $\alpha=0.85$ (left),  $\alpha=0.5$ (middle), $\alpha=0.19$ (right).}
% 	\label{fig:GramCharlierforNormalMixtureDist}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \bigskip
% % \newpage
% % \subsection{Gamma Distribution}

% % \subsection{Gompertz Distribution}
% % .
% % \bigskip
% \subsection{Weibull Distribution}

% \addnote{explain more!!!}

% The PDF of Weibull random variable is 
% \begin{align*}
%     f(x;\lambda,k)=\Big\{
%     \begin{matrix}
%          \frac{k}{\lambda}(\frac{x}{\lambda})^{k-1}e^{-(x/\lambda)^k}& & x\geq 0, \\
%           0& &  x<0,\\
%     \end{matrix}
% \end{align*}
% where $k>0$ is the shape parameter and $\lambda>0$ is the scale parameter of the distribution.
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/MEforWeibull.eps}
% 		\caption{Maximum Entropy for Weibull Distribution  with $k=1.5, \lambda=1$.}
% 	\label{fig:MEforWeibull6moments}
% \end{figure}


% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/GramCharlierforWeibull4cumulants05.eps}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlierforWeibull8cumulants05.eps}
% 	\caption{Gram-Charlier for Weibull Distribution  with $k=1.5, \lambda=1$:   4 cumulants (left),  8 cumulants (right).}
% 	\label{fig:GramCharlierforWeibull}
% \end{figure}

% % \subsection{Hotelling's T-squared Distribution}

% % \subsection{Truncated Normal Distribution}

% % \subsection{Half-normal Distribution}

% % \subsection{F-distribution}

% % \subsection{Generalized Extreme Value Distribution}

% % \subsection{Gumbel Distribution}
% %\newpage

% \subsection{Numerical Results}
% % \begin{itemize}
% % \item The {\bf Hellinger Distance} is used to quantify the similarity between two probability distributions.  Let $p(x)$ and $q(x)$ are pdfs of true and estimated distributions, respectively.  The square of the Hellinger distance is defined as follows: 
% % \begin{align*}
% %     H^2(P,Q)&=\frac{1}{2}\int\Big(\sqrt{p(x)} - \sqrt{q(x)}\Big)^2dx \\
% %     &= 1-\int\sqrt{p(x)q(x)} dx.
% % \end{align*}
% % Note that $0\leq H(P,Q) \leq 1$.

% % \item 
% {\bf Kullback–Leibler Divergence},  $D_{\text{KL}}$ quantifies how much one probability distribution differs from another probability distribution.
% To measure the difference between two probability distributions over the same
% variable $X$,  the Kullback-Leibler divergence, or simply, the KL
% divergence, has been popularly used in the data mining literature and it is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$. Here we assume that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$.  The continuous version of KL divergence is 
% \begin{align}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.


% %\end{itemize}

% \bigskip
% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|c|}
% \hline
%               & ME& GC &GC\\
%               & (6 mom.)& (4 cumul.)&(8 cumul.)\\
%               \hline
%     %  Example 1& 0.0328& 0.1002 &0.0148\\\hline
%     %  Example 2& 0.0139&0.1373 & 0.0360\\\hline
%      Cauchy & 0.8516& 0.3684& 0.2990\\\hline
%      Normal Mixture& 0.0236 & 0.0399 &0.0012\\\hline
%      Weibull& 0.0105 & 0.0614 & 0.0407\\\hline
     
% \end{tabular}
%  \caption{Kullback-Leibler divergence ($D_{KL}$ of true and estimated  distributions with Maximum Entropy (ME) and Gram-Charlier (GC)).}
%      \label{table:Kullback-LeiblerDivergence} 
        
% \end{table}

% %\todo{to do /////}


% \bigskip
% \bigskip



% \newpage
% \section{Appendix B: Second Moment of StutteringP}

% \addnote{Type the calculation!}

% With a closer look at the StutteringP probabilistic program in Table~\ref{table:BenchmarkPrograms} we can see that \begin{align}
%     & E[f(n+1)]= p E[1] + (1-p) E[0],\\
%     & E[x(n+1)]= E[x(n)+ f(n+1)\cdot rand(0,2)],\label{eq:firstmomentStutteringPCalculations-1}\\
%     & E[y(n+1)]= E[y(n)+ f(n+1)\cdot rand(0,4)],\label{eq:firstmomentStutteringPCalculations-2}\\
%     &  E[s(n+1)]= E[x(n+1)+ y(n+1)].
% \end{align}
% which leads to 
% \begin{align}
%     & E[f(n+1)]= p,\\
%     & E[x(n+1)]= E[x(n)]+ E[f(n+1)]\cdot E[rand(0,2)],\\
%     & E[y(n+1)]= E[y(n)]+ E[f(n+1)]\cdot E[rand(0,4)],\\
%     &  E[s(n+1)]= E[x(n+1)]+E[y(n+1)].
% \end{align}
% Then we can write the recurrence relations. Solving this recurrences leads us to the close form of first moments, i.e. expectation, of each involved variables. 
% \begin{align}
%     & E[f(n)]= p,\label{eq:firstmomentStutteringPCalculations1}\\
%     & E[x(n+1)]= E[x(n)]+ p \;\Longrightarrow \; E[x(n)]=np-1 \; \text{ as } \; x(0)=-1,\label{eq:firstmomentStutteringPCalculations2}\\
%     & E[y(n+1)]= E[y(n)]+ 2p \;\Longrightarrow \; E[y(n)]=2np+1 \; \text{ as } \; y(0)=1,\label{eq:firstmomentStutteringPCalculations3}\\
%     &  E[s(n)]= E[x(n)]+E[y(n)]= np-1+2np+1 \;\Longrightarrow \; E[s(n)]=3np. 
% \end{align}

% Now we calculate recurrences and closed forms for the second moments of involved variables. As  $E[f(n+1)^2]=p E[1^2] + (1-p) E[0^2] = p$, we conclude that 
% \begin{align}
%     E[f(n)^2]=p.
% \end{align}
% For other variables
% \begin{align}
%   E[x(n+1)^2] & = E[\big(x(n)+ f(n+1)\cdot rand(0,2)\big)^2]\notag\\
%              & = E[x(n)^2]+ 2E[x(n)] E[f(n+1)]E[rand(0,2)] \notag\\
%              & \hspace{2.8cm}+ E[f(n+1)^2] E[rand(0,2)^2]\notag\\
%              & = E[x(n)^2]+ 2E[x(n)] E[f(n+1)] + E[f(n+1)^2] \frac{4}{3}\notag\\
%              & = E[x(n)^2]+ 2E[x(n)] E[f(n+1)] + E[f(n+1)^2] \frac{4}{3}
% \end{align}
% Considering Equations~\eqref{eq:firstmomentStutteringPCalculations1} and \eqref{eq:firstmomentStutteringPCalculations2} we have following recurrence for the second moment of random variable $x$:
% \begin{align}
%   E[x(n+1)^2] = E[x(n)^2]+ 2(np-1)p +  \frac{4}{3}p.
% \end{align}
% To solve this recurrence we have
% \begin{align*}
%   E[x(n)^2] &= E[x(0)^2]+ \sum_{i=0}^{n-1}\Big(2(ip-1)p +  \frac{4}{3}p\Big)\\
%   & = E[x(0)^2]+ 2p^2\Big(\sum_{i=0}^{n-1} i\Big)+ n(-2p+\frac{4}{3}p)\\
%   &=1+ 2p^2\Big(\frac{(n-1)(n)}{2}-\frac{2np}{3},
% \end{align*}
% which leads us to the closed form for second moment of $x$ in StutteringP:
% \begin{align}
%   E[x(n)^2] &= n^2p^2 - np^2 -\frac{2}{3}np+1.
% \end{align}
% The same calculations and considering Equations ~\eqref{eq:firstmomentStutteringPCalculations1} and \eqref{eq:firstmomentStutteringPCalculations3}, we reach 
% \begin{align}
%   E[y(n)^2] &= 4n^2p^2 - 4np^2 -\frac{28}{3}np+1.
% \end{align}
% To obtain recurrence relation for random variable $s$ we consider 
% \begin{align*}
%   E[s(n+1)^2]&=E[\Big(x(n+1)+y(n+1)\Big)^2]\\
%               &= E[x(n+1)^2] + 2E[(xy)(n+1)]  + E[y(n+1)^2] 
% \end{align*}
% in which $E[(xy)(n+1)]$ can be represented as a recurrence by multiplication of recurrences of $E[x(n+1)]$ and $E[y(n+1)]$ in \eqref{eq:firstmomentStutteringPCalculations-1} and \ref{eq:firstmomentStutteringPCalculations-2}:
% \begin{align*}
%   E[(xy)(n+1)]&= E[(xy)(n)] + 2 E[x(n)] E[f(n+1)] + E[y(n)] E[f(n+1)]+ 2E[f(n+1)^2] \\
%   &= E[(xy)(n)] + 2(np-1)p + (2np+1)p +2p
% \end{align*}
% Solving this recurrence we obtain
% \begin{align*}
%   E[(xy)(n)]&= E[(xy)(0)] + \sum_{i=0}^{n-1}\Big(2ip^2-2p+2ip^2+p+2p\Big)\\
%   &=2n^2p^2 -2np^2+np-1.
% \end{align*}
% Finally we obtain a closed form  for the second moment of random variable $s$:
% \begin{align*}
%   E[s(n)^2]&=E[\big(x(n)+y(n)\big)^2]\\
%               &= E[x(n)^2] + 2E[(xy)(n)]  + E[y(n)^2]\\
%               &=(n^2p^2 - np^2 -\frac{2}{3}np+1)+2(2n^2p^2 -2np^2+np-1)+(4n^2p^2 - 4np^2 -\frac{28}{3}np+1)\\
%               & = 9n^2p^2 - 9np^2+ 32np.
% \end{align*}




==> Distribution Recovery (27)/PrecisionOfHigherMoments.tex <==
%\lk{precision of moments, moved from Sect.3}
%----------------------------------
%\newpage
%moved from Section 3



\paragraph{{\bf Precision Evaluation of Higher-Order Moments of PP Variables.}}
In addition to effectively estimating distributions of a  PP variable $x$, in our experiments we were also interested to compare the higher-order moments of the estimated pdfs of $x$ against the exact moments of $x$. That is, we were interested to see how the estimated moments that we compute  from  the $|S_M|$ exact moments of $x$ differ from their respective, exact higher-order moments. 

For this evaluation setting, we use the loop iteration $n=100$ as before and apply the following setting: we compute the higher-order moments $M'_{\me}$ and $M'_{\gc}$ of the  estimated distributions $f_{\me}$ and $f_{\gc}$, and  compare 
them with the set $S_M$ of exact moments of $x$. In the sequel, we let  
$\E(x^i)_{\me}$ and  $\E(x^i)_{\gc}$
denote the $i$th estimated moment of $x$ computed from $f_{\me}$ and $f_{\gc}$,
and write ${\E(x^i)}$ for the $i$th exact moment of $x$ from $S_M$ (as in Algorithm~\ref{fig:algo}). 
For comparing moments, we compute  the \textit{absolute estimate error} for the $i$th moment of $x$ as the difference between the respective  estimated (either from $M'_{\me}$ or $M'_{\gc}$) and exact moments (from $S_M$), i.e. 
\begin{equation}\label{AbsoluteEstimateErrorDef}
\begin{array}{l}
  \text{AE}_{\me}=|{\E(x^i)}_{\me}-{\E(x^i)}|,\\
  \text{AE}_{\gc}=|{\E(x^i)}_{\gc}-{\E(x^i)}|.\\
  \end{array}
\end{equation}
In addition, we also compare the exact moments of $x$ against its respective moments obtained from sampling the PP (from $Sample_{Data}$ in Algorithm~\ref{fig:algo}). We write ${\E(x^i)}_{Sample}$ to denote the $i$th higher-order moment of $x$ obtained from $Sample_{Data}$. {As such, the    
 \textit{absolute sample error} between the sampled and exact moments of $x$ is derived by
\begin{equation}\label{AbsoluteSampleErrorDef}
  \text{AE}_{Sample}=|{\E(x^i)}_{Sample}-{\E(x^i)}|. 
\end{equation} 
The respective 
{\it relative errors} $\text{RE}_{\me}$ and $\text{RE}_{\gc}$ of the ME and GC estimation, as well as the relative error  $\text{RE}_{Sample}$ based on sampled data, are computed as 
\begin{equation}\label{eq:RE}
\begin{array}{l}
    \text{RE}_{\me}=\frac{\left|{\E(x^i)}_{\me}-{\E(x^i)}\right|}{\E(x^i)},\\ 
    \text{RE}_{\gc}=\frac{\left|{\E(x^i)}_{\gc}-{\E(x^i)}\right|}{\E(x^i)},\\ 
    \text{RE}_{Sample}=\frac{\left|{\E(x^i)}_{Sample}-{\E(x^i)}\right|}{\E(x^i)}.
\end{array}
\end{equation}
 }  
%nd \textit{relative sample error} as the ratio of  absolute sample error and exact moments.
%\Ahmad{We should add a paragraph (as another method of evaluation) here that we compute the higher moments using our estimations and we represent the error of moments (sample moment - exact moment) and (estimate moment - exact moment). This shows, once we have a few (for example 2) moments for our PP, then using our ME/GC estimated distribution we are able to compute higher moments with a high accuracy. This procedure is much faster that calculating all higher exact moments using symbolic computations.}
%We further investigate the precision of higher moments.  As  in \ref{ssec:methods-of-evaluation},  we start by using the first two exact moments of each benchmark program to estimate the target distribution. Using the latter, we then compute higher moments (of order three to eight), which we call  estimated moments. 
Table~\ref{table:AbsoluteandRelativeErrors} summarizes our experiments on evaluating the precision of sampled and estimated moments against exact moments, for each PP in Table~\ref{table:DKL-Chi2-K-SforBenchmarks}. 
Columns~1--3 of Table~\ref{table:AbsoluteandRelativeErrors} correspond to columns~1--3 of Table~\ref{table:DKL-Chi2-K-SforBenchmarks}. 
Column~4 lists the the order of the moment of the random variable in column~2: for each $i$th moment, we give its exact value (column~5), as well as its absolute~\eqref{AbsoluteEstimateErrorDef} and relative estimate errors~\eqref{eq:RE} (in parentheses) using $Sample_{Data}$ (column~6), ME (column~7) and GC expansion (column~8). 


%\lk{this table needs a description in relation to the moments of Table~\ref{Tab:Benchmarks} , refinement; the Vasicek model should also appear in it.  Don't we use eqs (12) and (13)?-  the table caption indicate relative errors, which is not the same as in (12) and (13). }
%\Ahmad{Done! I dropped the table that we discussed, we use eqn. (12)-(16), therefore, I dropped the caption detail in Table 2.}
%absolute  (and relative) sample errors defined in \eqref{AbsoluteSampleErrorDef}, absolute (and relative) estimate errors (defined by \eqref{AbsoluteEstimateErrorDef}) for the ME and GC based estimates. The results provide evidence of the high accuracy of our methods for estimating distributions of probabilistic loop outputs.  Comparing  the columns of sample error and estimate error shows the importance of the distribution recovery as the errors (absolute and relative) of moments obtained by the estimated distribution are smaller than the errors of moments calculated using sampled data. However, the Gram-Charlier method fails to estimate the uniform distribution as the relative estimate errors for this method are rather high compared to the sample and ME estimate errors.
%Maximum Entropy estimates the Uniform distribution with high accuracy.


\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
 \begin{tabular}{c|c|c|c|l|l|l|l}
\toprule
  {\bf Program}  & Var &$|S_{\text{M}}|$ & Moment &   Exact Moment   & AE$_{Sample}$ (RE$_{Sample}$)  & AE$_{\me}$ (RE$_{\me}$) & AE$_{\gc}$ (RE$_{\gc}$)  \\
                         \midrule
 \multirow{3}{*}{StutteringP}& & &1& 210 & $5.69\times 10^{-2} (0.027\%)$  &$8.08\times 10^{-5} (0.00003\%)$&$4.71\times 10^{-5} (0.00002\%)$\\%\cline{2-6}
    & $s$&2&2& $4.4405 \times 10^4 $ &  $2.39 \times 10^{1} (0.053\%)$& $1.75 \times 10^{-2} (0.00003\%)$&$1.75 \times 10^{-2} (0.00003\%)$\\%\cline{2-6}
    &&&3& $9.4536\times 10^6$  & $6.78 \times 10^{3} (0.0.072\%)$ & $9.21 \times 10^{1} (0.000974\%)$ & $9.25 \times 10^{1} (0.000978\%)$\\%\cline{2-6}
    &&&4& $2.0260\times 10^9$  & $1.48 \times 10^{6} (0.073\%)$& $7.38 \times 10^{4} (0.00364\%)$   & $7.42 \times 10^{4} (0.00366\%)$\\%\cline{2-6}
    &&&5& $4.3705\times 10^{11}$  & $2.17 \times 10^{8} (0.050\%)$ & $3.82 \times 10^{7} (0.00873\%)$ & $3.83 \times 10^{7} (0.00876\%)$ \\%\cline{2-6}
    &&&6&  $9.4884\times 10^{13}$ & $5.51 \times 10^{9} (0.0058\%)$ & $1.60 \times 10^{10} (0.0168\%)$  & $1.60 \times 10^{10} (0.0168\%)$\\%\cline{2-6}
    &&&7& $2.0729\times 10^{16}$  & $2.10 \times 10^{13} (0.101\%)$& $5.88 \times 10^{12} (0.0284\%)$  & $5.90 \times 10^{12} (0.0285\%)$\\%\cline{2-6}
    &&&8& $4.5570\times 10^{18}$  &$1.12 \times 10^{16} (0.245\%)$ &  $1.99 \times 10^{15} (0.0438\%)$  & $2.00 \times 10^{15} (0.0439\%)$
    \\\midrule
 \multirow{3}{*}{Square}&&&1& 10100 & $1.66\times 10^1 (0.16\%)$  &  $1.11\times 10^{0} (0.011\%)$  & $7.97\times 10^{-3} (0.00007\%)$ \\%\cline{2-6}
    &$y$&2&2& $1.0602 \times 10^8$ & $2.31\times 10^5 (0.22\%)$ & $2.30\times 10^3 (0.00217\%)$   & $1.64\times 10^{2} (0.00015\%)$ \\%\cline{2-6}
    &&&3& $1.1544\times 10^{12}$  &$1.27\times 10^{9} (0.11\%)$  &  $1.26\times 10^7 (0.0011\%)$  &$2.39\times 10^{9} (0.2072\%)$\\%\cline{2-6}
    &&&4& $1.3012\times 10^{16}$  & $2.98\times 10^{13} (0.23\%)$& $1.99\times 10^{12} (0.0153\%)$   &$9.79\times 10^{13} (0.7581\%)$ \\%\cline{2-6}
    &&&5& $1.5157\times 10^{20}$  & $1.32\times 10^{18} (0.87\%)$& $8.83\times 10^{16} (0.0583\%)$    &$2.61\times 10^{18} (1.7505\%)$
    \\\midrule
\multirow{3}{*}{Binomial}&&&1& 50 & $2.95\times 10^{-1} (0.59\%)$  &  $5.19\times 10^{-5} (0.000051\%)$ & $3.16\times 10^{-3} (0.0063\%)$\\%\cline{2-6}
    &$x$&2&2&   2525  & $2.82\times 10^{1} (1.12\%)$ & $2.74\times 10^{-3} (0.000108\%)$  & $1.87\times 10^{-1} (0.0074\%)$ \\%\cline{2-6}
    &&&3& 128750  & $2.04\times 10^{3} (1.59\%)$ & $1.43\times 10^{-1} (0.000111\%)$  & $1.22\times 10^{1} (0.0095\%)$ \\%\cline{2-6}
    &&&4&  $6.6268\times 10^{6}$  &$1.32\times 10^{5} (2.00\%)$ & $3.66\times 10^{0} (0.000055\%)$  & $8.22\times 10^{2} (0.0125\%)$ \\%\cline{2-6}
    &&&5&  $3.4421\times 10^{8}$ &$8.08\times 10^{6} (2.35\%)$ &  $5.52\times 10^{2} (0.000160\%)$ & $5.53\times 10^{4} (0.0161\%)$ \\%\cline{2-6}
    &&&6& $1.8038\times 10^{10}$ & $4.67\times 10^{8} (2.64\%)$& $1.20\times 10^{5} (0.000664\%)$   & $3.66\times 10^{6} (0.0203\%)$\\%\cline{2-6}
    &&&7&  $9.5354\times 10^{11}$ &$2.74\times 10^{10} (2.87\%)$ &  $1.51\times 10^{7} (0.001587\%)$  & $2.38\times 10^{8} (0.0250\%)$\\%\cline{2-6}
    &&&8&  $5.0830\times 10^{13}$ &$1.54\times 10^{12} (3.04\%)$ &  $1.54\times 10^{9} (0.0030363\%)$   & $1.51\times 10^{10} (0.0298\%)$
         \\\midrule
 \multirow{3}{*}{RandomWalk1D}&&&1& 20 & $1.57\times 10^{-1} (0.79\%)$  &$1.83\times 10^{-6} (0.000009\%)$ & $4.44\times 10^{-3} (0.022\%)$\\%\cline{2-6}
    &$x$&2&2& $4.2933\times 10^{2} $ &  $6.78 \times 10^{0} (1.58\%)$& $6.76 \times 10^{-5} (0.00001\%)$ & $1.90\times 10^{-1} (0.0044\%)$\\%\cline{2-6}
    &&&3& $9.7516\times 10^{3}$  & $2.45 \times 10^{2} (2.51\%) $& $8.40 \times 10^{0} (0.09\%)$  & $5.61\times 10^{-1} (0.0057\%)$\\%\cline{2-6}
    &&&4&  $2.3230\times 10^{5}$ & $8.38\times 10^{3} (3.61\%)$&  $6.48\times 10^{2} (0.28\%)$  & $3.54\times 10^{2} (0.15\%)$\\%\cline{2-6}
    &&&5& $5.7681\times 10^{6}$  & $2.79\times 10^{5} (4.48\%)$&  $3.37\times 10^{4} (0.58\%)$ &$2.32\times 10^{4} (0.40\%)$ \\%\cline{2-6}
    &&&6&  $1.4858\times 10^{8}$ & $9.19\times 10^{6} (6.19\%)$&  $1.48\times 10^{6} (0.98\%)$ & $1.12\times 10^{6} (0.75\%)$ \\%\cline{2-6}
    &&&7& $3.9565\times 10^{9}$  & $3.03\times 10^{8} (7.66\%)$& $5.94\times 10^{7} (1.48\%)$  & $4.72\times 10^{7} (1.18\%)$ \\%\cline{2-6}
    &&&8& $1.0857\times 10^{11}$  & $1.01\times 10^{10} (9.26\%)$&  $2.26\times 10^{9} (2.04\%)$  & $1.85\times 10^{9} (1.67\%)$
    \\\midrule
 \multirow{3}{*}{Uniform(0,1)}&&&1& 0.5 & $5.92\times 10^{-3} (1.18\%)$  & $1.47\times 10^{-9} (3\times 10^{-7}\%)$ & $3.28\times 10^{-2} (7.03\%)$\\%\cline{2-6}
    &$u$&6&2& 0.333333 & $4.94\times 10^{-3} (1.48\%)$ &   $1.66\times 10^{-5} (0.00499\%)$& $3.40\times 10^{-2} (11.36\%)$\\%\cline{2-6}
    &&&3& 0.25  & $4.57\times 10^{-3} (1.83\%)$ & $2.50\times 10^{-5} (0.00998\%)$  & $3.46\times 10^{-2} (16.06\%)$ \\%\cline{2-6}
    &&&4&  0.20  &$4.57\times 10^{-3} (2.28\%)$ &  $3.33\times 10^{-5} (0.0166\%)$  & $3.43\times 10^{-2} (20.69\%)$\\%\cline{2-6}
    &&&5&  0.166667  & $4.66\times 10^{-3} (2.80\%)$&   $4.18\times 10^{-5} (0.0249\%)$ &$3.35\times 10^{-2} (25.18\%)$ \\%\cline{2-6}
    &&&6&  0.142857 &$4.74\times 10^{-3} (3.32\%)$ &   $4.99\times 10^{-5} (0.0349\%)$ & $3.25\times 10^{-2} (29.51\%)$\\%\cline{2-6}
    &&&7&  0.125 &$4.76\times 10^{-3} (3.81\%)$ &     $5.82\times 10^{-5} (0.00465\%)$ &$3.15\times 10^{-2} (33.65\%)$\\%\cline{2-6}
    &&&8&  0.1111111 &$4.73\times 10^{-3} (4.25\%)$ &  $6.66\times 10^{-5} (0.00599\%)$ &  $3.04\times 10^{-2} (37.60\%)$\\\midrule
\multirow{3}{*}{Vasicek Model}&&&1& 0.20 & $2.16\times 10^{-3} (1.08\%)$  &$6.63\times 10^{-11} (3.32\times 10^{-8}\%)$ &$1.40 \times 10^{-8} (7.00\times 10^{-6}\%)$\\%\cline{2-6}
     &$r$&2& 2& $0.0933$ &  $5.91 \times 10^{-3} (6.33\%)$& $9.67\times 10^{-11} (1.04\times 10^{-7}\%)$ &$2.15 \times 10^{-8} (2.31\times 10^{-5}\%)$ \\%\cline{2-6}
     
    &&&3& $0.0400$  & $3.13 \times 10^{-3} (7.83\%)$& $2.00 \times 10^{-8} (5.00\times 10^{-5}\%)$& $3.32 \times 10^{-8} (8.30\times 10^{-5}\%)$\\%\cline{2-6}
    
    &&&4& 0.0229 & $ 2.54\times 10^{-3} (11.09\%) $ &   $4.02 \times 10^{-8} (1.75\times 10^{-4}\%)$ & $5.11\times 10^{-8} (2.23\times 10^{-4}\%)$ \\%\cline{2-6}
    &&&5& 0.0131  & $ 1.83\times 10^{-3} (13.93\%) $ &   $7.11 \times 10^{-8} (5.42\times 10^{-4}\%)$ & $7.89\times 10^{-8} (6.01\times 10^{-4}\%)$\\%\cline{2-6}
    &&&6& 0.0087& $ 1.61\times 10^{-3} (18.46\%) $&  $1.15 \times 10^{-7} (1.32\times 10^{-3}\%)$ & $1.22\times 10^{-7} (1.39\times 10^{-3}\%)$\\%\cline{2-6}
    &&&7& 0.0059  &$ 1.40\times 10^{-3} (23.49\%) $ &   $1.83 \times 10^{-7} (3.07\times 10^{-3}\%)$ & $1.88\times 10^{-7} (3.16\times 10^{-3}\%)$\\%\cline{2-6}
    &&&8&  0.0044 & $ 1.33\times 10^{-3} (29.86\%) $&   $2.86 \times 10^{-7} (6.43\times 10^{-3}\%)$ & $2.91\times 10^{-7} (6.53\times 10^{-3}\%)$
    \\\midrule
 \multirow{3}{*}{PDP Model}&&&1& $1.1885\times 10^{3}$ & $1.60\times 10^{1}  (1.35\%)$  &$2.84\times 10^{-1}  (0.024\%)$ &$5.74\times 10^{0}  (0.48\%)$ \\%\cline{2-6}
    &$x$&3&2& $1.4767\times 10^{6}$ &  $3.93\times 10^{4} (2.66\%)$& $3.95\times 10^{2} (0.027\%)$ &$1.16\times 10^{4} (0.78\%)$ \\%\cline{2-6}
    &&&3& $1.8981\times 10^{9}$  & $7.37 \times 10^{7} (3.88\%)$& $3.19\times 10^{6}(0.168\%)$ & $2.35\times 10^{7} (1.23\%)$\\%\cline{2-6}
     &&&4& $2.5058\times 10^{12}$ & $1.28\times 10^{11}(5.01\%)$ &  $1.64\times 10^{10}$ (0.650\%)  & $4.85\times 10^{10} (1.90\%)$\\%\cline{2-6}
     &&&5& $3.3804\times 10^{15}$  &$2.04\times 10^{14}(6.03\%)$  & $ 4.97\times 10^{13} (1.450\%)$ & $1.00\times 10^{14} (2.87\%)$\\%\cline{2-6}
%      &&6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\%\cline{2-6}
%      &&7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\%\cline{2-6}
%      &&8& $1.19415322490998\times 10^{24}$
%   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
%     & $2.95\times 10^{22} (2.4119\%)$\\\hline
        \bottomrule
\end{tabular}
}
\vspace{2mm} 
 \caption{Precision evaluation of higher-order moments  using $|S_M|$ exact moments.  %\textcolor{blue}{$|S_{\text{M}}|$ is the number of moments that are used for the estimation.}  
 %\lk{again, we should only use the moments from Table 1, consistently}
%  :\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Appendix~\ref{Appendix}: Table ~\ref{Table:Benchmarks})\\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$\\
 %\\$^{\ast\ast}$Moments of order above 5  could not be computed within ~30 minutes
 }
%  \label{Table:ErrorforBenchmarks}
\label{table:AbsoluteandRelativeErrors}
\end{table}

%\lk{todo later - mention maybe 30s eval, bound of 5 moments fo KS}



% As shown in the Tables~\ref{table:DKL-Chi2-K-SforBenchmarks} and \ref{table:AbsoluteandRelativeErrors}, the relative estimate errors for Gram-Charlier method are rather high comparing to the sample errors and ME estimate errors. Therefore, Gram-Charlier method fail to estimate Uniform distribution using its moments while Maximum Entropy estimates the distribution in a high accuracy level. 
 


% Comparing first 8 moments of the underlying variable yields absolute estimate errors as \textit{absolute error of }$\E(x^i)= |{\E(x^i)}_{estimate}-{\E(x^i)}_{exact}|$. Normalizing obtained errors with the exact moments we reach the \textit{relative estimate errors}\footnote{Moments above 5 for the Square benchmark could not be computed within ~30 minutes.}. The same process is done for the \textit{absolute} and \textit{relative sample errors}, but instead of estimated moments we compare  sample moments to the exact ones. 

%\Ahmad{We should revise and decide if we keep it or not???}\\
%\textcolor{blue}
{ 
Table~\ref{table:AbsoluteandRelativeErrors} gives practical  evidence of the accuracy of estimating the pdf, and hence moments, using Algorithm~\ref{fig:algo}. The absolute and relative errors listed in Table~\ref{table:AbsoluteandRelativeErrors}  show  that
we gain higher precision when computing moments from the estimated pdfs using ME and/or GC expansion when compared to the moments  calculated
using sampled data.  
%However, the Gram-Charlier method fails to estimate the
%Uniform distribution as the relative estimate errors for this method are rather
%high compared to the sample errors and ME estimate errors. Maximum Entropy
%estimates the Uniform distribution with high %accuracy.\\
The accuracy of moments calculated from sampled data depends on the quality of the sampling process, which in turn  depends on the number of samples ($e$) and number of loop iterations ($n$). Our results in Table~\ref{table:AbsoluteandRelativeErrors} indicate that computing  moments from estimated pdfs provides a more  accurate and time-efficient alternative to estimating moments by sampling. 
%
%In complex PPs, calculating exact higher moments is (time) expensive. For example, for the \textit{Square} probabilistic program and PDP model for gene circuits, calculating moments higher than the fifth is not possible within $\sim30$ minutes. Using our  estimation methods, we can approximate higher moments of complex PPs much faster as the estimation only requires the first few moments, whose computation  only takes few seconds.  
}



==> Distribution Recovery (27)/Precision_Vasicek.tex <==

\begin{example}
    %We have previously estimated the distribution  using ME and GC  from the first two moments of $r$. 
We  compute the first 8 exact moments of $r$ of the Vasicek model using Mora/Polar. We also compute these moments for the ME/GC estimated distributions and for $Sample_{Data}$. Resulting errors, absolute and relative, are listed in  Table~\ref{Table:ErrorforBenchmarksVasicek}. 
The error rates of the  ME and GC estimated pdfs are much smaller than the errors from sampling. Furthermore, ME performs marginally better than GC. Running times for distribution reconstruction using different number of moments for the Vasicek PP are shown in Table~\ref{table:TimeVasicekTable}. The running time for both methods increases with the number of higher moments used for estimation, with  ME being faster than GC.
    %The results show that, in this case, error for the moments from samples are a few orders of magnitude larger than in the case of estimating the distribution using ME or GC method.  \mm{MM: The last sentence is a bit hard to parse.}
\end{example}

%\vspace{5mm}


\begin{table}[tpbh!]\label{table:AbsoluteandRelativeErrorsVasicek}
\centering
\scalebox{0.8}{
\begin{tabular}{c|c|c|c|c}
\hline
  Moment & \;\;  Exact \;\;  & Absol. sample error$^{2}$   &Absol. ME estimate error$^{3}$  &Absol. GC estimate error$^{3}$ \\
    &Value$^{1}$ & (relative error$^\ast$)&  (relative error$^\ast$)&  (relative error$^\ast$) \\
                         \hline
                         \hline
 
1& 0.20 & $2.16\times 10^{-3} (1.08\%)$  &$6.63\times 10^{-11} (3.32\times 10^{-8}\%)$ &$1.40 \times 10^{-8} (7.00\times 10^{-6}\%)$\\%\cline{2-6}
    2& $0.0933$ &  $5.91 \times 10^{-3} (6.33\%)$& $9.67\times 10^{-11} (1.04\times 10^{-7}\%)$ &$2.15 \times 10^{-8} (2.31\times 10^{-5}\%)$ \\%\cline{2-6}
    3& 0.0400  & $3.13 \times 10^{-3} (7.83\%) $& $2.00 \times 10^{-8} (5.00\times 10^{-5}\%)$& $3.32 \times 10^{-8} (8.30\times 10^{-5}\%)$\\%\cline{2-6}
    4& 0.0229 & $ 2.54\times 10^{-3} (11.09\%) $ &   $4.02 \times 10^{-8} (1.75\times 10^{-4}\%)$ & $5.11\times 10^{-8} (2.23\times 10^{-4}\%)$ \\%\cline{2-6}
    5& 0.0131  & $ 1.83\times 10^{-3} (13.93\%) $ &   $7.11 \times 10^{-8} (5.42\times 10^{-4}\%)$ & $7.89\times 10^{-8} (6.01\times 10^{-4}\%)$\\%\cline{2-6}
    6& 0.0087& $ 1.61\times 10^{-3} (18.46\%) $&  $1.15 \times 10^{-7} (1.32\times 10^{-3}\%)$ & $1.22\times 10^{-7} (1.39\times 10^{-3}\%)$\\%\cline{2-6}
    7& 0.0059  &$ 1.40\times 10^{-3} (23.49\%) $ &   $1.83 \times 10^{-7} (3.07\times 10^{-3}\%)$ & $1.88\times 10^{-7} (3.16\times 10^{-3}\%)$\\%\cline{2-6}
    8&  0.0044 & $ 1.33\times 10^{-3} (29.86\%) $&   $2.86 \times 10^{-7} (6.43\times 10^{-3}\%)$ & $2.91\times 10^{-7} (6.53\times 10^{-3}\%)$
    \\\hline
      %  \hline
\end{tabular}
}
\vspace{2mm}
\caption{Error of moments (sample error and estimate error) for Vasicek model:\\
 $^{1}$ Exact value of moments at the iteration loop $n=100$ \\
 $^{2}$ Error of exact moments and sample moments\\
 $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
 $^\ast$ Relative error ($\%$)=$100 \times (\text{Absolute Error}/\text{Exact Value})$}
 \label{Table:ErrorforBenchmarksVasicek}
\end{table}
%\vspace{-15mm}

\begin{table}[tpbh!]
\centering
     %\scalebox{0.95}{
 %\footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength\abovecaptionskip{8pt}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}ccccccc@{}}
 %\begin{tabular}{c|c|c|c|c|c|c}
\toprule
& & \multicolumn{5}{c}{\# moments for estimation}\\
   & & 2 & 3 & 4 & 5 & 6 \\
  \cline{3-7}
  \multirow{2}{*}{Time $(s)$ }& Gram-Charlier & 1.55 & 1.73 & 1.88 & 2.11 & 2.28 \\
 % &&&&&&\\
  %\cline{2-7}
   %&&&&&&\\
   & Maximum Entropy & 0.63 & 0.71 & 0.89 & 1.14 & 1.67\\
  %&&&&&&\\
    \bottomrule
\end{tabular}
%}
%\vspace{2mm}
 \caption{Running times for distribution reconstruction vs. number of moments used for the Vasicek PP.
 %\ms{Maybe only address computation times in the to Evaluation section?}\Ahmad{All results of Vasicek are presented here. I think we keep this table here as well.}
 }
 \label{table:TimeVasicekTable}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%


==> Distribution Recovery (27)/benchmarks.tex <==
%!TEX root = samplepaper.tex
%\newpage
\section{Benchmarks}\label{section:Benchmarks}
%\subsection{Programs with Unknown Target Distribution} 
We evaluate our approach in Section~\ref{section:Evaluation}
% Sections \ref{section:MaximumEntropyMethod} and \ref{section:GramCharlierExpansion} 
on several benchmarks selected from \cite{bartocci2019automatic,Moosbruggeretal2022}. These benchmarks include {\bf StutteringP}, {\bf Square}, {\bf Binomial}, {\bf Random Walk 1D}, and {\bf Uniform}. We refer to Table~\ref{table:BenchmarkPrograms} in Appendix~\ref{Appendix} for the description of benchmarks.  We estimate the distributions of the random variables in these probabilistic programs  using their exact moments. The selected benchmarks are prob-solvable loops and their  exact moments can be calculated  via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora} without executing the programs. Exact moments of the output  random variable for selected benchmarks  are available,  as functions of loop iteration $n$, in Appendix~\ref{Appendix}: Table~\ref{Table:Benchmarks}.

\efi{what is this???  are available in Appendix~\ref{Appendix}:  Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}).}



% We  do our assessment for different probabilistic programs (see Table~\ref{table:BenchmarkPrograms}) for which the exact calculated moments are available on in Table~\ref{Table:Benchmarks}. Exact moments of the output  random variable of each probabilistic program are computed as functions of $n$, iteration of the loop are available in Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}:






% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.6}{
%  \begin{tabular}{|clc|clc|clc|clc|}
% \hline
%       \multirow{3}{*}{} 
%       &&&&& &&&& &&\\
% \hspace{2mm}&{\bf StutteringP}&\hspace{2mm}&\hspace{3mm}& {\bf Square} & \hspace{2mm}&\hspace{3mm}&  {\bf Binomial($p$)} \hspace{10mm} & \hspace{2mm}&\hspace{3mm}& {\bf Random Walk 1D } & \hspace{2mm}\\
% &&&&&&&&&&&\\
% &$f:=0$&&& $x:=0$ &&& $x:=0$ && & $v:=0$&\\
% &$x:=-1$&&& $y:=1$ &&&$\text{while true:}$&& & $x:=0$&\\
% &$y:=1$&&& $\text{while true:}$ &&&$\quad x:=x+1\;\;[\;p\;]\;\;x$ && & $\text{while true:}$&\\
% &$s:=0$&&& $\quad x:=x+2\;\;[1/2]\;\;x$  &&&&& &$\quad v:=\text{uniform}(0,1)$&\\
% &$\text{while true:}$&&& $\quad y:=x^2$ &&&&& &$\quad x:=x+v\;\;[7/10]\;\;x-v$&\\
% &$\quad f:=1\;\;[\;{ p }\;]\;\;0$&&&  &&&&& &&\\
% &$\quad x:=x+f*\text{uniform}(0,2)$&&&  &&&&& &&\\
% &$\quad y:=y+f*\text{uniform}(0,4)$&&&  &&&&& &&\\
% &$\quad s:=x+y$&&&&  &&&& &&\\
% &&&&&  &&&& &&\\
%                          \hline
% &&&&& &&&& &&\\
% \hspace{2mm}&{\bf Sum Rand. Series}  &\hspace{2mm}&\hspace{3mm}& {\bf Prod. Dep. Vars.}  & \hspace{2mm}&\hspace{3mm}& {\bf Bimodal}  & \hspace{2mm}&  &{\bf Uniform}&\hspace{2mm}\\
% &&&&& &&&& &&\\
% &$n:=0$&&& $f:=0$ &&& $x := 0$ && &$x := 1/2$&\\
% &$x:=0$&&& $x:=0$ &&& $xlow := 0$ && &$u := 0$ &\\
% &$\text{while true:}$&&& $y:=0$ &&& $xup := 0$ && &$\text{while true:}$&\\
% &$\quad n:= n + 1$&&& $p:=0$ &&& $\text{while true:}$ && &$\quad u:=u\;\;[1/2]\;\;u+x$&\\
% &$\quad x:=x+n\;\;[1/2]\;\;x$&&& $\text{while true:}$ &&& $\quad d := \text{Bernoulli}(1/3)$ && &$\quad  x := x/2$ &\\
% &  &&& $\quad f:=0\;\;[1/2]\;\;1$ &&& $\quad \text{if } d :== 0:$ && &&\\
% &  &&& $\quad x:=x+f$ &&& $\quad \quad step := \text{Normal}(3/4, 1)$ && &&\\
% &  &&& $\quad y:=y+1-f$ &&& $\quad \quad xlow := xlow - step$ && &&\\
% &  &&& $\quad p:=x \ast y$ &&& $\quad \quad x := xlow$ && &&\\
% &&&&& &&$\quad \text{else:}$&& &&\\
% &&&&& &&$\quad \quad step := \text{Normal}(3/4, 1)$&& &&\\
% &&&&& &&$\quad \quad xup := xup + step$&& &&\\
% &&&&& &&$\quad \quad x := xup$&& &&\\
% &&&&& && $\quad \text{end}$&& &&\\
% &&&&& &&&& &&\\
%                          \hline
% %                         &&&&& &&&& &&\\
% % \hspace{2mm}&{\bf Random Walk 1D }&\hspace{2mm}&\hspace{3mm}& {\bf Uniform } & \hspace{2mm}&\hspace{3mm}& {\bf .... } & \hspace{2mm}\\
% % &&&&  &&&&\\
% % &$v:=0$&&& $x := 1/2$ &&&&\\
% % &$x:=0$&&& $u := 0$ &&&&\\
% % &$\text{while true:}$&&& $\text{while true:}$  &&&&\\
% % &$\quad v:=\text{uniform}(0,1)$&&& $\quad u:=u\;\;[1/2]\;\;u+x$&&&&\\
% % &$\quad x:=x+v\;\;[7/10]\;\;x-v$&&& $\quad  x := x/2$ &&&&\\
% % &&&&& &&&\\
% %                         \hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Benchmark Programs.}
%     \label{table:BenchmarkPrograms}
% \end{table}
% % \addnote{Explain why I did choose these 3 programs. Any other suggestion Marcel and Miroslav?}
% % \mm{See my comment above. Also you could again take (loop-free) programs from PSI and try to approximate the distribution with just the moments.}
% \end{singlespace}
% \begin{singlespace}
% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.7}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
%  \multirow{3}{*}{StutteringP}&1& $\E(s(n)) = 3np $ \\\cline{2-3}
%     &2& $\E(s^2(n)) = 9n^2p^2 - 9np^2+\frac{32}{3}np$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{} $\E(s^3(n)) = 3np(9n^2p^2 - 27np^2 + 32np + 18p^2 - 32p + 14)$
%     % 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
%     %   & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
%     %   & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
%     %   & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
%     %   & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
%     \\\hline
%         \hline
   
% \multirow{3}{*}{Square}&1& $\E(y(n)) = n^2+n$  \\\cline{2-3}
%     &2&$\E(y^2(n)) = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
%     &3&$\E(y^3(n)) = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
%         \hline
        
% \multirow{3}{*}{Binomial($p$)}&1&$\E(x(n)) = np$  \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^2p^2 + np(1-p)$  \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
%         \hline 
                
% \multirow{3}{*}{Random Walk 1D}&1&$\E(x(n)) =  n/5$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^2/25 + 22n/75$   \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^3/125 + n^222/125 - n21/250$   \\\hline
%         \hline   

% \multirow{3}{*}{Uniform(0,1)}&1& $\E(u(n))=2^{-n}(2^n - 1)/2$ \\\cline{2-3}
%     &2&$\E(u^2(n))=2^{-3n}(2^{3n+1} + 2^n - (3)4^n)/6$  \\\cline{2-3}
%     &3&$\E(u^3(n))=2^{-3n}(-2^{2n+1} + 2^n + 8^n)/4$  \\\hline
%   %      \hline           
% % \multirow{3}{*}{Loop free PPs}&1& .  \\\cline{2-3}
% %     &2&.  \\\cline{2-3}
% %     &3&.   \\\hline
% %         \hline   
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Exact moments of Benchmarks calculated by Mora/Polar.}
%  \label{Table:Benchmarks}
% \end{table}
% \end{singlespace}
% Exact moments of the output  random variable of each probabilistic program are computed as functions of $n$, iteration of the loop are available in Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}: Table~1).%\footnote{The second moment $\E(s^2(n))$ here differs from the one mentioned in \cite{bartocci2019automatic} as it did not agree with the simulations. Calculations are presented in Appendix B.}. 

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/ExSampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex2SampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex3SampledandMora1000sample1000loopSttuteringP.eps}
% 	\caption{ $E(S)$, $E(S^2)$ and $E(S^2)$ for Stuttering P using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora1000loop1000sampleStutteringP}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/histogramStutteringP100loop1000sample.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfStutteringP100loop1000sampleME.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfStutteringP100loop1000SampleME.eps}
% 	\caption{ Left: histogram of sampled data by executing the StutteringP program (number of samples is 1000 and number of loop iteration in SutteringP is 100). Middle: pdf of sampled (kernel density estimation) and maximum entropy estimated Distribution for SutteringP. Right: cdf of sampled distribution and Maximum Entropy Estimation  for random varible $S$ in SutteringP.  }
% 	\label{fig:StutteringP100loop1000sample}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/ExSampledandMora100loop1000sampleSquare.eps}
% 	\includegraphics[width=4.2cm]{Figures/Ex2SampledandMora100loop1000sampleSquare.eps}
% 	\caption{ $E(Y)$ and $E(Y^2)$ for Square using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora100loop1000sampleSquare}
% \end{figure}



% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/HistogramSquare1000Sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfSquare1000sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfSquare1000sample1000loop.eps}
% 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% 	\caption{Left: histogram of sampled data by executing the Square program (number of samples is 1000 and number of loop iteration in Square is 1000). Middle: pdf of sampled (kernel density estimation) and Gram-Charlier Estimated Distribution for Square. Estimation of Distribution using Gram-Charlier Expansion with 3 cumulants. Right: cdf of sampled distribution and Gram-Charlier estimation.}
% 	\label{fig:GramCharlierforSquare}
% \end{figure}






% \newpage
% \subsection{Programs with Known Distribution} 
% Variable $x$ and $y$ in the Square program are inherently discrete random variables. Consider a Bernoulli process as a sequence of independent random variables $t_1, t_2, t_3 , \dots$ such that for each $i=1,2,3,\dots$, the variable $t_i$ is 0 or 1, and for all $i$, $P(t_i=1)=p$. In our special case, $p=1/2$. Using Bernoulli process we can rewrite the Square program as follows:
% \begin{align*}
% &x:=0\\
% &y:=1\\
% &\text{while true:}\\
% &\quad t:=1\;\;[ p ]\;\;0\\
% &\quad x:=x+2*t\\
% &\quad y:=x^2
% \end{align*}
% Note that $x$ and $y$ are somehow sum of Bernoulli variables which have Binomial distributions. In a more general case, we can use $x:=x+f(t)$ to update variable $x$, where  $f:\{0,1\}\rightarrow \mathbb{R}$ is a function for which $f(0)\neq f(1)$. In this case again we have Binomial distribution.  

% For a fixed loop iteration, say $n$, a trajectory of random variable $\{y(i)\}_{i=0}^{n}$ could be a sequence of $\{x(i)^2\}$ where $x(i)=2b(i)$. In other word, $\{y(i)\}$ is the sequence of \textit{even-squared} numbers between 0 and $(2n)^2$. Here $b(i)=i$ where $i=0,1,2,\dots,n$. Random variable $b$ has  binomial distribution.    

% \begin{align}
%   P\Big[y=\text{even-squared}(i)\Big]&=p\Big[y=(2b(i))^2\Big]\notag\\
%   &=p\Big[x=2b(i)\Big]\notag\\
%   &=p\Big[b=i\Big]={n \choose
% i} p^i(1-p)^n-i \qquad i=0,1,2,\dots,n  
% \end{align}




% \newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \multirow{3}{*}{Random Walk 1D}&1& 20 & $9.20\times 10^{-2}$  &$2.37 \times 10^{-5}$&$1.88\times 10^{-6}$\\\cline{2-6}
%     &2& $4.2933 \times 10^2 $ &  $4.23 \times 10^{0}$ &$5.25\times 10^{-4}$& $6.63 \times 10^{-5}$\\\cline{2-6}
%     &3& $9.7516 \times 10^3$  & $1.45 \times 10^{2} $ &$1.04\times 10^{-2}$& $3.56 \times 10^{-3}$\\\cline{2-6}
%     &4&   & &   &  \\\cline{2-6}
%     &5&   & &   &  \\\cline{2-6}
%     &6&   & &   &  \\\cline{2-6}
%     &7&   & &   &  \\\cline{2-6}
%     &8&   & &   &  
%     \\\hline
%         \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%\subsection{A Real-life Application}


% {\bf Vasicek Model in Finance:}
% In finance, the Vasicek model is a mathematical model describing the evolution of interest rates. 
% %It is a type of one-factor short-rate model as it describes interest rate movements as driven by only one source of market risk.
% Following stochastic differential equation describes the Vasicek model: 
% \begin{align}
%  dr_{t}=a(b-r_{t})\,dt+\sigma \,dW_{t}   
% \end{align}
% where $W_t$ is a Wiener process under  modeling the continuous inflow of randomness into the system. $\sigma$ is the standard deviation factor which shows the amplitude of the instantaneous randomness inflow. $b$ is the long term mean level which paths  will evolve around it in a long term. $a$ is the speed of reversion specifying  the velocity at which such trajectories will regroup around $b$ in time.

% \bigskip
% \bigskip

% The Vasicek model of interest rate can be represented as a prob-solvable  probabilistic program as follows:
% \iffalse
% \begin{align}
% &a:=0.5\\\notag
% &b:=0.2\\\notag
% &\sigma:=0.2\\\notag
% &w:=0\\\notag
% %&dt:=1\\\notag
% &r:=2\\\notag
% &\text{while true:}\\\notag
% &\quad w:=\text{Normal}(0,1)\\\notag
% &\quad r:=(1-a)r + a\ast b + \sigma\ast w
% \end{align}
% \fi
% \begin{algorithmic}
%     \STATE $a:=0.5$
%     \STATE $b:=0.2$
%     \STATE $\sigma:=0.2$
%     \STATE $w:=0$
%     \STATE $r:=2$
%     \WHILE{true} 
%         \STATE $w:=\text{Normal}(0,1)$
%         \STATE $r:=(1-a)\ast r + a\ast b + \sigma\ast w$
%     \ENDWHILE
% \end{algorithmic}

% \bigskip

% % The expected value and variance of the random variable $r(t)$ given $r(0)$ are:
% % \begin{align}\label{eq:firstmomentVasicek}
% % &E\big(r(t)\big) = r(0) e^{-at}\,+\, b\big(1-e^{-at}\big)\\\label{eq:secondmomentVasicek}
% % &Var\big(r(t)\big) =\frac{\sigma^2}{2a} \big(1-e^{-2at}\big)
% % \end{align}



% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|l|}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
 
 
%  \multirow{3}{*}{Vasicek}&1& $\E(r(n)) = 2^{-n}(2^n + 9)/5 $ \\\cline{2-3}
%     &2& $\E(r^2(n)) = 7/75 + (18)2^{-n}/25 + (239)2^{-2*n}/75$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{}$\E(r^3(n)) = 8^{-n}((239)2^n + (63)4^n + (5)8^n + 693)/125 $
%     \\\hline
%         \hline
% \end{tabular}
% \vspace{2mm}
%  \caption{Moments for Vasicek Model calculated by Polar\cite{}}
%  \label{Table:VasicekMomentsfromPolar}
% \end{table}

% %\newpage

% \begin{figure}[tpbh!]
% 	\centering
% % 	\includegraphics[width=10cm,  height=6cm]{Figures/AbsoluteErrorVasicek1000loop1000sample.eps}\\
% % 	\includegraphics[width=10cm,  height=6cm]{Figures/RelativeErrorVasicek.eps}\\
% \includegraphics[width=10cm,  height=6cm]{Figures/abserrorvasicekmodeln100sigma02.eps}\\
% 	\includegraphics[width=10cm,  height=6cm]{Figures/relerrorvasicekmodeln100sigma02.eps}\\
% 	\caption{Absolute and relative error of $E(r)$ and $E(r^2)$ in  \textit{Vasicek} model of interest rate.}
% 	\label{fig:AbsoluteandRelativeErrorsVasicekModel}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% % 	\includegraphics[width=3.9cm]{Figures/HistogramVasicek100loop1000sample.eps}
% % 	\includegraphics[width=3.9cm]{Figures/pdfVasicekME.eps}
% %      \includegraphics[width=3.9cm]{Figures/cdfVasicekModelME.eps}
% \includegraphics[width=3.9cm]{Figures/histogramvasicekmodeln100sigma02.eps}
% 	\includegraphics[width=3.9cm]{Figures/pdfvasicekmodeln100sigma02.eps}
%      \includegraphics[width=3.9cm]{Figures/cdfvasicekmodeln100sigma02.eps}
% 	\caption{Left: histogram of sampled data of random variable $r$ in Vasicek PP (sample size=1000 and loop iteration=100). Middle: PDF of ME estimate distribution in comparison with the K-S density of sampled data. Right: CDF (ME estimate and the K-S density).}
% 	\label{fig:HistogramPDFCDFofVasicekME}
% \end{figure}

% \begin{table}[tpbh!]
%     \centering
%   \scalebox{0.9}{
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & p-value (ME) & p-value (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline
%     \hspace{2mm} Vasicek \hspace{2mm}&\hspace{2mm} 0.0027 \hspace{2mm} & \hspace{2mm} 0.002685\hspace{2mm} & \hspace{2mm}0.15  \hspace{2mm} & 0.1456& \hspace{2mm} 17.4018 \hspace{2mm}& \hspace{2mm} 17.4017 \hspace{2mm}\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence of ME estimated distribution and sampled one), p-value (Kolmogorov–Smirnov), $\chi^2$ statistics for the Vasicek  probabilistic programs.}
%  \label{table:VasicekTable}
      
% \end{table}

% \begin{table}[tpbh!]\label{table:AbsoluteandRelativeErrorsVasicek}
%     \centering
%      \scalebox{0.7}{
%  \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%   {\bf Program}   & Moment &   Exact Value$^{1}$  & Absol. sample error$^{2}$   &Absol. ME estimate error$^{3}$  &Absol. GC estimate error$^{3}$ \\
%     &  & & (relative error$^\ast$)&  (relative error$^\ast$)&  (relative error$^\ast$) \\
%                          \hline
%                          \hline
 
%  \multirow{3}{*}{Vasicek}&1& 0.200000000000000 & $2.16\times 10^{-3} (1.08\%)$  &$6.63\times 10^{-11} (3.32\times 10^{-8}\%)$ &$1.40 \times 10^{-8} (7.00\times 10^{-6}\%)$\\\cline{2-6}
%     &2& $0.093333333333333$ &  $5.91 \times 10^{-3} (6.33\%)$& $9.67\times 10^{-11} (1.04\times 10^{-7}\%)$ &$2.15 \times 10^{-8} (2.31\times 10^{-5}\%)$ \\\cline{2-6}
%     &3& 0.0400000000000000  & $3.13 \times 10^{-3} (7.83\%) $& $2.00 \times 10^{-8} (5.00\times 10^{-5}\%)$& $3.32 \times 10^{-8} (8.30\times 10^{-5}\%)$\\\cline{2-6}
%     &4& 0.0229333333333333  & $ 2.54\times 10^{-3} (11.09\%) $ &   $4.02 \times 10^{-8} (1.75\times 10^{-4}\%)$ & $5.11\times 10^{-8} (2.23\times 10^{-4}\%)$ \\\cline{2-6}
%     &5& 0.0131200000000000  & $ 1.83\times 10^{-3} (13.93\%) $ &   $7.11 \times 10^{-8} (5.42\times 10^{-4}\%)$ & $7.89\times 10^{-8} (6.01\times 10^{-4}\%)$\\\cline{2-6}
%     &6& 0.00873955555555556  & $ 1.61\times 10^{-3} (18.46\%) $&  $1.15 \times 10^{-7} (1.32\times 10^{-3}\%)$ & $1.22\times 10^{-7} (1.39\times 10^{-3}\%)$\\\cline{2-6}
%     &7& 0.00594631111111111  &$ 1.40\times 10^{-3} (23.49\%) $ &   $1.83 \times 10^{-7} (3.07\times 10^{-3}\%)$ & $1.88\times 10^{-7} (3.16\times 10^{-3}\%)$\\\cline{2-6}
%     &8&  0.00445202962962963 & $ 1.33\times 10^{-3} (29.86\%) $&   $2.86 \times 10^{-7} (6.43\times 10^{-3}\%)$ & $2.91\times 10^{-7} (6.53\times 10^{-3}\%)$
%     \\\hline
%         \hline
 
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Error of moments (sample error and estimate error):\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ \\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$}
%  \label{Table:ErrorforBenchmarksVasicek}
% \end{table}


% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \hspace{2mm}{Vasicek}\hspace{2mm} & \# moments for estimation  & 2 & 3 & 4 & 5 & 6 \\
%                          \hline
%                           &&&&&&\\
%   \multirow{3}{*}{\hspace{2mm}Time \hspace{2mm}}& \hspace{2mm}Gram-Charlier\hspace{2mm} & 1.55 & 1.73 & 1.88 & 2.11 & 2.28 \\
%   &&&&&&\\\cline{2-7}
%   &&&&&&\\
%   $([s])$ & \hspace{2mm}Maximum Entropy \hspace{2mm}& \hspace{2mm}0.63\hspace{2mm} &\hspace{2mm} 0.71\hspace{2mm} &\hspace{2mm} 0.89\hspace{2mm} &\hspace{2mm} 1.14\hspace{2mm} &\hspace{2mm} 1.67 \hspace{2mm}\\
%   &&&&&&\\
%     \hline
% \end{tabular}
% \vspace{2mm}
%  \caption{Time of distribution reconstruction vs. number of moments applied for the reconstruction for Vasicek probabilistic program.}
%  \label{table:TimeVasicekTable}
      
% \end{table}

% \bigskip
% \bigskip
%\newpage

We also present, for the first time, 
a gene circuit  model in biology as a probabilistic program. As the resulting PP is prob-solvable, Mora/Polar calculate exact moments which are used to estimate the distribution of protein and mRNA levels  of a gene, the random variables of this model.  


\paragraph{A Piecewise-deterministic process (PDP) Model for Gene  Circuits: }
%As another real life  example, we present, for the first time, a piecewise-deterministic process (PDP) model  in biology as a prob-solvable probabilistic program. 
This  model is used to represent gene networks. 
We consider the simple model of
a single constitutive gene controlled by a two state (ON/OFF) promoter (see \cite{innocentini2018time}).

The continuous
variables are the protein ($x$) and and mRNA ($y$)  levels of the
gene. The discrete variable is a two-value variable
$s\in\{0, 1\}$ representing the promoter states (0 stands for OFF
and 1 stands for ON). 
The transition rates between ON and OFF are $f$ and $h$, thus $s$ can be modelled using a Markov chain. %f from ON to OFF, h from OFF to ON
The transcription initiation rates in states 0 and 1 are $k_0$ and $k_1$, respectively. The translation rate is $b$, $\rho$ is the mRNA and $a$ the protein degradation rate.
The protein and mRNA concentrations follow the ODEs
\begin{align}\label{PDP}
&\frac{dy}{dt}=\begin{cases}
k_0-\rho y & \text{if} \quad s=0\\
k_1-\rho y &  \text{if} \quad  s=1\\
\end{cases}\notag\\
&\frac{dx}{dt}=by-ax
\end{align}
We modify  the model by setting $dt=1$ in order to induce discrete-time recurrences, and translate the PDP model \eqref{PDP} for gene circuits to the prob-solvable probabilistic program in Figure~\ref{table:PDPmodelPPandMoments} (left).  The first- and second-order moments of the random variable $x$ as functions of loop iteration calculated by Polar \cite{Moosbruggeretal2022} are available in Appendix~\ref{Appendix}: Table~\ref{Table:Benchmarks}.
\begin{singlespace}
\begin{table}[tpbh!]
    \centering
    %\scalebox{0.6}{
    \begin{minipage}{0.48\textwidth}
\begin{algorithmic}
    \STATE $k_1:=4$, $k_2:=40$, $y:=0$
    % \STATE $k_2:=40$
    %  \STATE $y:=0$%, $x:=0$
    % \STATE $x:=0$
    % % \STATE $a:=0.2$
    % \STATE $a:=0.2$ 
    \STATE $x:=0$, $a:=0.2$, $b:=4$ 
    \STATE $s:=0$, $h:=0.6$, $f:=0.1$
    \STATE $\rho:=0.5$
    % \STATE $f:=0.1$
    % \STATE $h:=0.6$
    % % %\STATE $p:=0.5$
    % % \STATE $f:=0.1$, $h:=0.6$
    %   \STATE  $\rho:=0.5$
    % % %\STATE $\epsilon:=0.5$
    \WHILE{$true$}
        %\STATE $k:= k_1 \;[\;p\;] \;k_2$
        \IF{$s=0$}
            \STATE $s = 1 \;[\;f\;]\; 0$
        \ELSE
            \STATE $s = 0 \;[\;h\;]\; 1$
        \ENDIF
        \STATE $k:= k_2 * s + k_1 * (1-s)$
        % \STATE s:= 1 \;[\;p\;]\; 0
        % \STATE if s= 0 
        % \STATE    k=k0
        % \STATE else
        % \STATE    k=k1
        % \STATE end\\\notag
        \STATE $y:=(1-\rho)y+k$
        \STATE $x:=(1-a)x+by$
    \ENDWHILE
\end{algorithmic}
\end{minipage}
\begin{minipage}{0.58\textwidth}

\end{minipage}
\vspace{5mm}
\caption{The Prob-solvable loop expressing the PDP model \eqref{PDP} for gene circuits (left).} 
\label{table:PDPmodelPPandMoments}
%}
\end{table}
\end{singlespace}
% \begin{table}%[tpbh!]
%      \scalebox{0.7}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
%  \multirow{4}{*}{PDPModel} \hspace{2mm} &1& $\E(x(n)) = 1000^{-n}\big((24960)10^{3n} - (1944)300^n + (13720)500^n - (36736)800^n\big)/21$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = (2.62144\times 10^{27})^{-n}\big(-51514624000*(1.048576\times 10^{27})^n $\\
%     &&$+ 31603353600*(1.31072\times 10^{27})^n   + 59761049600(1.6777216\times 10^{27})^n  $\\
%     &&$- 84619591680(2.097152\times 10^{27})^n  + 30050150400*  (2.62144\times 10^{27})^n $\\ 
%     &&$- 413683200*  (3.93216\times 10^{26})^n  + 2326579200* (6.291456\times 10^{26})^n $\\
%     &&$- 2546790400*  (6.5536\times 10^{26})^n  + 15353556480*  (7.86432\times 10^{26})^n \big)/20349$ \\
%     \hline
%      %   \hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Moments for PDP  Model for Gene Circuits calculated by Polar \cite{polar}}
%  \label{Table:PDPModel}
% \end{table}


% \begin{algorithmic}
%     \STATE $k_1:=4$  
%     \STATE $k_2:=40$
%     \STATE $y:=0$
%     \STATE $x:=0$
%     \STATE $a:=0.2$
%     \STATE $b:=4$
%     \STATE $f:=0.1$
%     \STATE $h:=0.6$
%     %\STATE $p:=0.5$
%     \STATE $\rho:=0.5$
%     %\STATE $\epsilon:=0.5$
%     \WHILE{$true$}
%         %\STATE $k:= k_1 \;[\;p\;] \;k_2$
%         \IF{$s=0$}
%             \STATE $s = 1 \;[\;f\;]\; 0$
%         \ELSE
%             \STATE $s = 0 \;[\;h\;]\; 1$
%         \ENDIF
%         \STATE $k:= k_2 * s + k_1 * (1-s)$
%         % \STATE s:= 1 \;[\;p\;]\; 0
%         % \STATE if s= 0 
%         % \STATE    k=k0
%         % \STATE else
%         % \STATE    k=k1
%         % \STATE end\\\notag
%         \STATE $y:=(1-\rho)y+k$
%         \STATE $x:=(1-a)x+by$
%     \ENDWHILE
% \end{algorithmic}
% \ms{I updated the $s$ in the PDP to come form a MC. To do: update results in Tab 10-12 and Fig 14, 15, if necessary}
% \Ahmad{I need first 10 moments as functions of loop iteration (also evaluated in n=100), I appreciate it if I can have them to update the results.}

% \begin{table}[tpbh!]
%     \centering
%      \scalebox{0.7}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
 
 
%  \multirow{4}{*}{PDPModel} \hspace{2mm} &1& $\E(x(n)) = -4400(4/5)^n/3 + 880 + (1760)2^{-n}/3$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = 17920000(16/25)^n/9 - 13760000(2/5)^n/9$ \\
%     & & $- 7744000(4/5)^n/3 + 819200 + (2406400)4^{-n}/9$ \\
%     & & $+ (3097600)2^{-n}/3$ 
%     % \\
%     % \cline{2-3}
%     % &3&  \multirow{3}{*}{}$\E(x^3(n)) = 15769600000(16/25)^n/3 $\\
%     % &&$- 12108800000(2/5)^n/3 - 3604480000(4/5)^n $\\
%     % &&$- 66176000000(64/125)^n/27 + 23936000000(8/25)^n/9 $\\
%     % &&$+ 799744000 + (1802240000)8^{-n}/27 - (7546880000)5^{-n}/9 $\\
%     % &&$+ (2117632000)4^{-n}/3 + (1441792000)2^{-n}$
%     \\\hline
%      %   \hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Moments for PDP  Model for Gene Circuits calculated by Polar \cite{polar}}
%  \label{Table:PDPModel}
% \end{table}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=10cm,  height=4cm]{Figures/absErrorPDPmodeln100simoltain.eps}\\
% 	\includegraphics[width=10cm,  height=4cm]{Figures/relErrorPDPmodeln100simoltain.eps}\\
% % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% 	\caption{Absolute and relative error of $\E(x)$ and $\E(x^2)$ in  {PDP} model for Gene Circuits.}
% 	\label{fig:AbsoluteandRelativeErrorsPDPModeln10}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.3cm]{Figures/histogramPDPmodeln100simoltain.eps}
% 	\includegraphics[width=3.3cm]{Figures/pdfPDPmodeln100simoltain.eps}
%     %  \includegraphics[width=3.9cm]{Figures/cdfPDPmodeln100simoltain.eps}
% 	\caption{Left: histogram of sampled data of random variable $x$ in the PDP model for Gene Circuits  (sample size=1000 and loop iteration=100). Right: PDF of ME estimate distribution in comparison with the kernel smoothing density approximation  of sampled data. %Right: CDF (ME estimate and the K-S density).
% 	}
% 	\label{fig:HistogramPDFCDFofPDPmodeln10ME}
% \end{figure}

%\Ahmad{Results moved to the Evaluation section. }
% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.8}{
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & $D^\ast$ (ME) & $D^\ast$ (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline
%     \hspace{2mm} PDP Model \hspace{2mm}&\hspace{2mm} 0.00439 \hspace{2mm} & \hspace{2mm}0.00415 \hspace{2mm} & \hspace{2mm}- \hspace{2mm}& - &16.4081   & 14.7861\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence of ME estimated distribution and sampled one), $D^\ast$ statistics (Kolmogorov–Smirnov test), $\chi^2$ statistics (Chi-Square test) for the PDP model for Gene Circuits (maximum loop iteration $n=100$).}
%  \label{table:PDPmodeln10}
      
% \end{table}

% \begin{table}[tpbh!]
%     \centering
%      \scalebox{0.7}{
%  \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%   {\bf Program}   & Moment &   Exact Value$^{1}$  & Absol. sample error$^{2}$   &Absol. ME estimate error$^{3}$ & Absol. GC estimate error$^{3}$ \\
%     &  & & (relative error$^\ast$)&  (relative error$^\ast$) &  (relative error$^\ast$)\\
%                          \hline
%                          \hline
 
%  \multirow{3}{*}{PDP Model}&1& 879.999999701235 & $3.89 \; (0.44\%)$  &$3.42 (0.39\%)$  &$0.012 (0.0014\%)$ \\\cline{2-6}
%     &2& 819199.999474173 &  $8.95\times 10^{3} (1.09\%)$& $3.61\times 10^{3} (0.44\%)$ &$2.362\times 10^{1} (0.0029\%)$ \\\cline{2-6}
%     &3& 799743999.265754  & $1.63 \times 10^{7} (2.04\%)$& $1.70\times 10^{6}(0.21\%)$ & $4.35\times 10^{4} (0.0054\%)$\\\cline{2-6}
%      &4& 813327753935.119 & $2.70\times 10^{10}(3.32\%)$ &  $2.40\times 10^{9}$ (0.29\%)  & $4.67\times 10^{8} (0.0573\%)$\\\cline{2-6}
%      &5& 857115541104823  &$4.22\times 10^{13}(4.92\%)$  & $ 9.61\times 10^{12}$ (1.11\%) & $2.26\times 10^{12} (0.2630\%)$\\\cline{2-6}
%      &6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\\cline{2-6}
%      &7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\\cline{2-6}
%      &8& $1.19415322490998\times 10^{24}$
%   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
%     & $2.95\times 10^{22} (2.4119\%)$\\\hline
%         \hline
 
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Error of moments (sample error and estimate error):\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ \\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$}
%  \label{Table:ErrorforBenchmarksPDPmodeln100}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
Our approach for distribution estimation using moments is not limited to prob-solvable loops. Once  moments of a  probabilistic program, either exact or approximated, are available, we can estimate the distribution of any random variable. As an example, we also represent a stochastic differential equation (SDE) as a probabilistic program that is not prob-solvable next, and estimate the distribution of its random variable. 


%\newpage
\paragraph{General Loops in Probabilistic Programs: }

We consider the  stochastic differential equation,
\begin{align}\label{eq:SDE2}
    dX(t)= -\frac{1}{4}X^3(t) dt -\frac{1}{2}X^2(t) dW(t) \qquad \text{with} \qquad X(0)=2,
\end{align}
where $W$ denotes the Wiener process (standard Brownian motion) \cite{morters2010brownian}. Eqn. \eqref{eq:SDE2} can be represented as a probabilistic program which is shown  in Figure~\ref{fig:HistogramPDFCDFofGeneralLoopEx1}.
\begin{figure}[tpbh!]
	\centering
	\begin{minipage}{0.42\textwidth}
	\begin{align*}
&x:=2\\\notag
&w:=0\\\notag
&dt:=1\\\notag
&\sigma:=0.1\\\notag
&\text{\bf while } true \text{ \bf do}\\\notag
&\quad w:=\text{Normal}(0,1)\\\notag
&\quad x:=x-\frac{1}{4}x^3\ast dt -\frac{1}{2}x^2\ast \sigma\ast w\\
& \text{\bf end while }
\end{align*}
	\end{minipage}
	\begin{minipage}{0.56\textwidth}
	\includegraphics[width=\textwidth]{Figures/pdfGeneralSDEusingGC.eps}
% 	\includegraphics[width=5.5cm,height=3cm]{Figures/HistogramGeneralLoopExample1Loop1000Sample1000.eps}\\
% 	\includegraphics[width=5.5cm,height=3cm]{Figures/PDFGeneralLoopExample1.eps}
    %  \includegraphics[width=3.9cm]{Figures/CDFGeneralLoopExample1.eps}
	\end{minipage}
	\caption{Left: Probabilistic program of the SDE in \eqref{eq:SDE2} (left).  Sampled data from $x$ from executing the PP (sample size=1000 and loop iteration=1000) and the GC estimate of underlying distribution compared to the kernel density estimate of the sampled data (right). The first 6 empirical moments are used for estimation. %Right: CDF (GC estimate and the sampled distribution).
	}
	\label{fig:HistogramPDFCDFofGeneralLoopEx1}
\end{figure}



% \begin{align}
% &x:=2\\\notag
% &w:=0\\\notag
% &dt:=1\\\notag
% &\sigma:=0.1\\\notag
% &\text{while true:}\\\notag
% &\quad w:=\text{Normal}(0,1)\\\notag
% &\quad x:=x-\frac{1}{4}x^3\ast dt -\frac{1}{2}x^2\ast \sigma\ast w
% \end{align}
Currently,  we are not able to theoretically compute moments of the probabilistic program. We can, nevertheless, approximate them by carrying out a Monte-Carlo experiment (i.e. running the program   and stopping at a fix loop iteration) in order to obtain empirical moments from sampled data. For  the specific value  of  $\sigma=0.1$,
% \Ahmad{parameter $\sigma=0.1$} \efi{which parameters?}, 
the program generates data whose histogram in the left panel of Figure \ref{fig:HistogramPDFCDFofGeneralLoopEx1} indicates the distribution for the output random variable $x$ is bimodal. Here we use the first 6 (empirical) moments  and apply the Gram-Charlier expansion  to reconstruct the target distribution. The estimated pdf as well as the sampled data and their kernel density estimate are presented in Figure~\ref{eq:SDE2} (right panel). 


\efi{what does this sentence say? With the help of  statistical tools, we  evaluate   our estimations to see if  the probabilistic programs generate data with the estimated distributions. We refer to Section~\ref{section:Evaluation} for evaluation of estimations for the benchmark programs.}  













% \multirow{3}{*}{Sum Rand. Series}&1&$\E(x(n)) = n^2/4 + n/4$  \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^4/16 + 5n^3/24 + 3n^2/16 + n/24$  \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^6/64 + 7n^5/64 + 13n^4/64 + 9n^3/64 + n^2/32$    \\\hline
%         \hline        
 
% \multirow{3}{*}{Prod. Dep. Var.}&1&$\E(p(n)) = n^2/4 - n/4$  \\\cline{2-3}
%     &2& $\E(p^2(n)) = n^4/16 - n^3/8 + 3n^2/16 - n/8$  \\\cline{2-3}
%     &3& \multirow{3}{*}{}$\E(p^3(n)) = n^6/64 - 3n^5/64 + 9n^4/64 - 21n^3/64$ \\
%     & &+ $15n^2/32 -n/4$    \\\hline
%         \hline        
        
% \multirow{3}{*}{Bimodal}&1&$\E(x(n)) =  - n/4$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = 3n^2/16 + 67n/72 + 4/9$   \\\cline{2-3}
%     &3&$\E(x^3(n)) = -5n^3/64 - 37n^2/48 - 3n/8 + 1/3$   \\\hline
%         \hline   

        

==> Distribution Recovery (27)/conclusion.tex <==
%!TEX root = samplepaper.tex
\section{Conclusion}\label{section:Conclusion}
We present an algorithmic approach to  estimate the distribution of the random variables of a PP using a finite number of its moments.   Our estimates are based on Maximum Entropy and Gram-Charlier expansion. The accuracy of our estimation is assessed with the  chi-square and Kolmogorov-Smirnov  statistical tests. Our evaluation combines static analysis methods for the  computation of exact moments of a PP random variable $x$ with the aforementioned statistical techniques to produce estimates of the distribution of $x$. 
%using stati symbolic ap
%estomato approximate the program variables'
%Methods from program analysis allowed us to compute exact higher moments of program variables parameterized by the loop iteration without sampling the program.
%Given a finite number of these moments, we utilized two approaches based on Maximum Entropy and Gram-Charlier expansion to approximate the program variables' distributions.
%Our  evaluations demonstrate that both approaches are capable of accurately estimating the program variable's distributions from finitely many moments.
Extending our approach %to estimate values of random loop variables,  % $x$ at an arbitrary loop iteration $n$  has values $x_n$ in an interval $[a,b]$, $\mathbb{P}\left(x_n \in [a,b]\right)$, where $a,b$ are real constants.  % $\mathbb{P}(x_n \in [a,b])$ for an arbitrary loop iteration $n \in \mathbb{N}$.
% expectations, 
to support probabilistic inference  and quantify the loss of precision in the estimation are  future research directions. 
%can also benefit from our work on distribution estimation. We are not aware of other automated approaches addressing such and similar questions for PPs with unbounded loops.

==> Distribution Recovery (27)/data/Vasicek2.tex <==


a := 0.5
b := 0.2
σ := 0.2
w := 0
r := 2
while true:
  w := Normal(0, 1)
  r := (1 − a)r + a*b + σ*w


-------------------
- Analysis Result -
-------------------

E(r) = 2; 2**(-n)*(2**n + 9)/5
Solution is exact
E(r | n=100) = 253530120045645880299340641077/1267650600228229401496703205376 ≅ 0.200000000000000

E(r**2) = 4; 7/75 + 18*2**(-n)/25 + 239*2**(-2*n)/75
Solution is exact
E(r**2 | n=100) = 149980884130839092383916461952754551334236604588804957602669/1606938044258990275541962092341162602522202993782792835301376 ≅ 0.0933333333333333

E(r**3) = 8; 8**(-n)*(239*2**n + 63*4**n + 5*8**n + 693)/125
Solution is exact
E(r**3 | n=100) = 81481439053379443450737827537185023216365266845510598919987987673794078674015657532856473/2037035976334486086268445688409378161051468393665936250636140449354381299763336706183397376 ≅ 0.0400000000000000

E(r**4) = 16; 2**(-4*n)*(43*2**(4*n) + 540*2**(3*n) + 3346*2**(2*n) + 8316*2**n + 17755)/1875
Solution is exact
E(r**4 | n=100) = 59219597204126436989442413011855738679145584841728838252514556454886256672408394853108933389625452502820767086708240601/2582249878086908589655919172003011874329705792829223512830659356540647622016841194629645353280137831435903171972747493376 ≅ 0.0229333333333333

E(r**5) = 32; 2**(-5*n)*(123*2**(5*n) + 1935*2**(4*n) + 11950*2**(3*n) + 48510*2**(2*n) + 88775*2**n + 148707)/9375
Solution is exact
E(r**5 | n=100) = 42946884775597381334573048822911077251919481576989991755124800942140761042733912071887585838142022029768983929394608421699637813635503080332355671357/3273390607896141870013189696827599152216642046043064789483291368096133796404674554883270092325904157150886684127560071009217256545885393053328527589376 ≅ 0.0131200000000000

E(r**6) = 64; 2**(-6*n)*(1229*2**(6*n) + 19926*2**(5*n) + 154155*2**(4*n) + 623700*2**(3*n) + 1864275*2**(2*n) + 2676726*2**n + 3659989)/140625
Solution is exact
E(r**6 | n=100) = 36264921842878153571639105881185156521580337367664624127957672288901956281099069362776500776899554565851166879332188330544999827221389308132321888632909870492299823163071732165189/4149515568880992958512407863691161151012446232242436899995657329690652811412908146399707048947103794288197886611300789182395151075411775307886874834113963687061181803401509523685376 ≅ 0.00873955555555556

E(r**7) = 128; 2**(-7*n)*(4181*2**(7*n) + 77427*2**(6*n) + 617337*2**(5*n) + 3128895*2**(4*n) + 9321375*2**(3*n) + 21859929*2**(2*n) + 25619923*2**n + 29370933)/703125
Solution is exact
E(r**7 | n=100) = 31278404557331555034701623040914634656167423086083456156766362702659579153171254629832650079870748091303698134448546411992295494282693334866367516710555464058758582123882604560113739560579007664916682138937633/5260135901548373507240989882880128665550339802823173859498280903068732154297080822113666536277588451226982968856178217713019432250183803863127814770651880849955223671128444598191663757884322717271293251735781376 ≅ 0.00594631111111111

E(r**8) = 256; 2**(-8*n)*(46955*2**(8*n) + 903096*2**(7*n) + 8224468*2**(6*n) + 42960456*2**(5*n) + 160327650*2**(4*n) + 374741640*2**(3*n) + 717357844*2**(2*n) + 704902392*2**n + 690535499)/10546875
Solution is exact
E(r**8 | n=100) = 29686197825979122483144954390572284923930250139993009936185830000520152338839023081641180484786642282433946112372019741643745567514422084630227190246209822387957001403434044596220966652898047036100720692016431132255698829984912102724515761/6668014432879854274079851790721257797144758322315908160396257811764037237817632071521432200871554290742929910593433240445888801654119365080363356052330830046095157579514014558463078285911814024728965016135886601981690748037476461291163877376 ≅ 0.00445202962962963

E(r**9) = 512; 2**(-9*n)*(20083*2**(9*n) + 422595*2**(8*n) + 3997036*2**(7*n) + 23847516*2**(6*n) + 91722330*2**(5*n) + 268564842*2**(4*n) + 512398460*2**(3*n) + 822386124*2**(2*n) + 690535499*2**n + 586105515)/5859375
Solution is exact
E(r**9 | n=100) = 28971660817196551215770391622053942220586843408638230430695122534651023736937175953318538441972273492466562962635319988358915515574566103043159448389609991936435689058349888480144827004813194240325030545689885603381082801013465370689821514002448419952380726545067749957/8452712498170643941637436558664265704301557216577944354047371344426782440907597751590676094202515006314790319892114058862117560952042968596008623655407033230534186943984081346699704282822823056848387726531379014466368452684024987821414350380272583623832617294363807973376 ≅ 0.00342749866666667

E(r**10) = 1024; 2**(-10*n)*(248069*2**(10*n) + 5422410*2**(9*n) + 56111225*2**(8*n) + 347691960*2**(7*n) + 1527462650*2**(6*n) + 4609322172*2**(5*n) + 11016566890*2**(4*n) + 17622559800*2**(3*n) + 24168742465*2**(2*n) + 17583165450*2**n + 13062706909)/87890625
Solution is exact
E(r**10 | n=100) = 30243051369368479065924818887093930259555860295286037811428443049326984815308826250630029488486876242907115877511165375938365244482659680813374744284381961810350034679590221740546855862357410930250928086911333845150303793313754208581573881355989648252003025109644410242401807502359866531233537969949/10715086071862673209484250490600018105614048117055336074437503883703510511249361224931983788156958581275946729175531468251871452856923140435984577574698574803934567774824230985421074605062371141877954182153046474983581941267398767559165543946077062914571196477686542167660429831652624386837205668069376 ≅ 0.00282247395555556





==> Distribution Recovery (27)/evaluation.tex <==
%!TEX root = samplepaper.tex


%vs exact, psi, sampling; some moms; (measure: #moms b4 close match?)
%exact - limited complexity, arbitrary iteration
%psi - more complex, limited # iterations
%sampling - not precise,
%witheld moms - 'ability to generalize' within the class of distributions (PP encodable) 
%\newpage
\section{Evaluation}\label{section:Evaluation}

We evaluate how well do the two approaches estimate distributions of random variables involved in  probabilistic programs (and probabilistic loops in particular) using their given exact moments.

% We evaluate against a few sets of benchmarks:
% (1) against loops encoding a known distribution; 
% (2) against loop-free programs, with fully characterized distributions; %PSI
% (3a) against complex programs encoding a distribution that cannot be easily characterized - using sampling;
% (3b) against complex programs encoding a distribution that cannot be easily characterized - against exact moments. %only use subset of computed moments to approximate a distribution, use the remaining moments to check accuracy
% For each set of benchmarks we also give a detailed case study of one of the benchmarks - we discuss the underlying probabilistic program, distribution it encodes, how we measure the goodness of fit. 



%\paragraph{KL Divergence.} 
Table~\ref{table:DKL-Chi2-K-SforBenchmarks} provides us with the Kulback-Leibler distance for benchmark programs in which $D_{KL}$ is the distance between sampled distributions (as the target distribution are not known) and the estimated ones using either ME or GC methods. For the benchmark programs, Table~\ref{table:DKL-Chi2-K-SforBenchmarks}  also includes  $D^\ast$ statistics  for Kolmogorov–Smirnov goodness-of-fit test as well as $\chi^2$ statistics for Chi-Square goodness-of-fit test. In Kolmogorov-Smirnov test, We reject the null hypothesis, that sampled data follow the estimated distribution, if $D^\ast$ is greater than $CV_{\text{K-S}}=0.0608$, the critical value with respect to the significance level $\alpha=0.05$ and sample size 1000. For Chi-Square test: we reject the null hypothesis, that the sampled data follow the estimated distribution, if  $\chi^2$ is greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$, where $k=15$ is the number of bins that the sample data belongs to, and  $\alpha=0.05$ is the significance level. 

 

% , we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of  probabilistic programs  follow the  distributions estimated using moments. 



% In order to assess the our estimations, we set the number of loop in the StutteringP program to be 100 and we take 1000 sample for the output $s$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments.   To perform the $\chi^2$ goodness-of-fit test for the StutteringP benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the maximum entropy estimated distribution  is $\chi^2=15.1544$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program StutteringP follow the  distribution estimated using  moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 


% %%%% Square Chi2 Evaluation 
% In order to assess the our estimations, we fix the number of loop in the Square program to be 1000 and we take 1000 sample for the output, i.e. the variable $y$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments (cumulants).   To perform the $\chi^2$ goodness-of-fit test for the Square benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the Gram-Charlier estimated distribution  is $\chi^2=9.9100$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program Square  follow the  distribution estimated using  moments (cumulants) calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 




% \bigskip
% \bigskip




\begin{table}[tpbh!]
    \centering
     \scalebox{0.8}{
 \begin{tabular}{c|l|l|l|l|l|l}
\hline
          {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & $D^\ast$ (ME) & $D^\ast$ (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
                         \hline\hline
     StutteringP& 0.005858 & 0.005831& 0.0181 \cmark & 0.0213 \cmark & 18.6432 \cmark& 16.7943 \cmark\\%\hline
     Square & 0.005116 & 0.007204 & 0.0586 \cmark & 0.0566 \cmark& 36.9009 \xmark& 39.1309 \xmark \\%\hline
     Binomial & 0.003779 & 0.003844 & 0.0598 \cmark &  0.0597 \cmark & 27.4661 \xmark& 27.4574 \xmark\\%\hline
     \hspace{2mm} Random Walk 1D \hspace{2mm}& 0.006410 \hspace{2mm} & 0.006710 \hspace{2mm}&  0.0264 \cmark \hspace{2mm}&  0.0263 \cmark \hspace{2mm}& 18.6709 \cmark \hspace{2mm}& 18.7068 \cmark \hspace{2mm}\\%\hline
    Uniform (Cont.) & 0.062240 & 0.007650 & 0.0214 \cmark & 0.0658 \xmark & 16.3485 \cmark& 105.276 \xmark\\%\hline
     PDP Model & 0.006180 & 0.009348 & 0.0403 \cmark & 0.0393 \cmark & 64.4182 \cmark $^{\ast\ast}$& 65.9500 \cmark $^{\ast\ast}$\\\hline
\end{tabular}
}
\vspace{2mm}
 \caption{Kullback-Leibler distance, $D^\ast$  (Kolmogorov–Smirnov statistics) and $\chi^2$ (Chi-Square statistics) for the benchmark probabilistic programs.  \xmark \; means that the null hypothesis of the underlying test is rejected while \cmark states that we can not reject the null hypothesis which means there is no evidence against null hypothesis. \\
 $^{\ast\ast}$ Chi-Square test accepts null hypothesis when the number of bins $k$ is at least 50, for which $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,49}=66.339$. }
 \label{table:DKL-Chi2-K-SforBenchmarks}
      
\end{table}
Based on Table~\ref{table:DKL-Chi2-K-SforBenchmarks}, one can see that our distribution estimation methods work very well for continuous random variables and goodness of fit tests accept the null hypothesis that sampled data (generated by executing of PP) follow the estimated distributions. For discrete random variables (e.g. in Square and Binomial PPs), Chi-Square goodness of fit test rejects the null hypothesis while Kolmogorov-Smirnov accepts it.

We note that  Chi-Square test is sensitive to the choice of bins while Kolmogorov–Smirnov is independent of this issue. In PDP model The test rejects the null hypothesis for the $\alpha=0.05$ and  $k=15$, while Kolmogorov–Smirnov accept the null hypothesis. Increasing the number of bins to $k=50$, Chi-Square test accepts the null hypothesis as the test statistics $\chi^2$ for both ME and GC methods are below $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,49}=66.339$. 

\bigskip



%%%%%%%%%%%%%%%%%%%%%%
We further investigate the precision of higher moments.  As explained in \ref{ssec:methods-of-evaluation},  we first use 2 exact moments of each benchmark program and estimate the target distribution using these moments. Having the distribution for the variable of interest, we compute moments of order 3 to 8 and we call them estimated moments.  Table~\ref{table:AbsoluteandRelativeErrors}, shows absolute  (and relative) sample errors, absolute (and relative) estimate errors for Maximum Entropy method, as well as  absolute (and relative) estimate errors for Gram-Charlier method. Results expose practical evidence of the high accuracy of our methods for estimating distributions of probabilistic loop outputs.  Comparing  columns of sample error and estimate error shows the importance of the distribution recovery as the errors (absolute and relative) of moments obtained by estimated distribution are less than the errors of moments calculated by sampled data. However, Gram-Charlier method fail to estimate Uniform distribution as the relative estimate errors for this method are rather high comparing to the sample errors and ME estimate errors.
Maximum Entropy estimates the Uniform distribution in a high accuracy level.



% As shown in the Tables~\ref{table:DKL-Chi2-K-SforBenchmarks} and \ref{table:AbsoluteandRelativeErrors}, the relative estimate errors for Gram-Charlier method are rather high comparing to the sample errors and ME estimate errors. Therefore, Gram-Charlier method fail to estimate Uniform distribution using its moments while Maximum Entropy estimates the distribution in a high accuracy level. 
 


% Comparing first 8 moments of the underlying variable yields absolute estimate errors as \textit{absolute error of }$\E(x^i)= |{\E(x^i)}_{estimate}-{\E(x^i)}_{exact}|$. Normalizing obtained errors with the exact moments we reach the \textit{relative estimate errors}\footnote{Moments above 5 for the Square benchmark could not be computed within ~30 minutes.}. The same process is done for the \textit{absolute} and \textit{relative sample errors}, but instead of estimated moments we compare  sample moments to the exact ones. 

In complex PPs, calculating exact higher moments is (time) expensive. For example, for Square probabilistic program and PDP model for gene circuits, calculating moments higher than fifth order is not possible within $\sim30$ minutes. Using our methods of estimation one can approximate higher moments of complex PPs much faster as it only needs to estimate distribution using the first few moments (which takes few seconds).  
 
\begin{table}[tpbh!]
    \centering
    \scalebox{0.7}{
 \begin{tabular}{c|c|c|l|l|l|l}
\hline
  {\bf Program}  &\#Mom. & Moment &   Exact Value$^{1}$  &Absol. sample error$^{2}$   & Absol. ME est. error$^{3}$ & Absol. GC est. error$^{3}$  \\
    & for est.& & & (relative error$^\ast$)&  (relative error$^\ast$) &  (relative error$^\ast$)\\
                         \hline
                         \hline
 


 \multirow{3}{*}{StutteringP}&&1& 210 & $5.69\times 10^{-2} (0.027\%)$  &$8.08\times 10^{-5} (0.00003\%)$&$4.71\times 10^{-5} (0.00002\%)$\\%\cline{2-6}
    &2&2& $4.4405 \times 10^4 $ &  $2.39 \times 10^{1} (0.053\%)$& $1.75 \times 10^{-2} (0.00003\%)$&$1.75 \times 10^{-2} (0.00003\%)$\\%\cline{2-6}
    &&3& $9.4536\times 10^6$  & $6.78 \times 10^{3} (0.0.072\%)$ & $9.21 \times 10^{1} (0.000974\%)$ & $9.25 \times 10^{1} (0.000978\%)$\\%\cline{2-6}
    &&4& $2.0260\times 10^9$  & $1.48 \times 10^{6} (0.073\%)$& $7.38 \times 10^{4} (0.00364\%)$   & $7.42 \times 10^{4} (0.00366\%)$\\%\cline{2-6}
    &&5& $4.3705\times 10^{11}$  & $2.17 \times 10^{8} (0.050\%)$ & $3.82 \times 10^{7} (0.00873\%)$ & $3.83 \times 10^{7} (0.00876\%)$ \\%\cline{2-6}
    &&6&  $9.4884\times 10^{13}$ & $5.51 \times 10^{9} (0.0058\%)$ & $1.60 \times 10^{10} (0.0168\%)$  & $1.60 \times 10^{10} (0.0168\%)$\\%\cline{2-6}
    &&7& $2.0729\times 10^{16}$  & $2.10 \times 10^{13} (0.101\%)$& $5.88 \times 10^{12} (0.0284\%)$  & $5.90 \times 10^{12} (0.0285\%)$\\%\cline{2-6}
    &&8& $4.5570\times 10^{18}$  &$1.12 \times 10^{16} (0.245\%)$ &  $1.99 \times 10^{15} (0.0438\%)$  & $2.00 \times 10^{15} (0.0439\%)$
    \\\hline
        \hline

 \multirow{3}{*}{Square$^{\ast\ast}$}&&1& 10100 & $1.66\times 10^1 (0.16\%)$  &  $1.11\times 10^{0} (0.011\%)$  & $7.97\times 10^{-3} (0.00007\%)$ \\%\cline{2-6}
    &2&2& $1.0602 \times 10^8$ & $2.31\times 10^5 (0.22\%)$ & $2.30\times 10^3 (0.00217\%)$   & $1.64\times 10^{2} (0.00015\%)$ \\%\cline{2-6}
    &&3& $1.1544\times 10^{12}$  &$1.27\times 10^{9} (0.11\%)$  &  $1.26\times 10^7 (0.0011\%)$  &$2.39\times 10^{9} (0.2072\%)$\\%\cline{2-6}
    &&4& $1.3012\times 10^{16}$  & $2.98\times 10^{13} (0.23\%)$& $1.99\times 10^{12} (0.0153\%)$   &$9.79\times 10^{13} (0.7581\%)$ \\%\cline{2-6}
    &&5& $1.5157\times 10^{20}$  & $1.32\times 10^{18} (0.87\%)$& $8.83\times 10^{16} (0.0583\%)$    &$2.61\times 10^{18} (1.7505\%)$
    \\\hline
        \hline

\multirow{3}{*}{Binomial}&&1& 50 & $2.95\times 10^{-1} (0.59\%)$  &  $5.19\times 10^{-5} (0.000051\%)$ & $3.16\times 10^{-3} (0.0063\%)$\\%\cline{2-6}
    &2&2&   2525  & $2.82\times 10^{1} (1.12\%)$ & $2.74\times 10^{-3} (0.000108\%)$  & $1.87\times 10^{-1} (0.0074\%)$ \\%\cline{2-6}
    &&3& 128750  & $2.04\times 10^{3} (1.59\%)$ & $1.43\times 10^{-1} (0.000111\%)$  & $1.22\times 10^{1} (0.0095\%)$ \\%\cline{2-6}
    &&4&  $6.6268\times 10^{6}$  &$1.32\times 10^{5} (2.00\%)$ & $3.66\times 10^{0} (0.000055\%)$  & $8.22\times 10^{2} (0.0125\%)$ \\%\cline{2-6}
    &&5&  $3.4421\times 10^{8}$ &$8.08\times 10^{6} (2.35\%)$ &  $5.52\times 10^{2} (0.000160\%)$ & $5.53\times 10^{4} (0.0161\%)$ \\%\cline{2-6}
    &&6& $1.8038\times 10^{10}$ & $4.67\times 10^{8} (2.64\%)$& $1.20\times 10^{5} (0.000664\%)$   & $3.66\times 10^{6} (0.0203\%)$\\%\cline{2-6}
    &&7&  $9.5354\times 10^{11}$ &$2.74\times 10^{10} (2.87\%)$ &  $1.51\times 10^{7} (0.001587\%)$  & $2.38\times 10^{8} (0.0250\%)$\\%\cline{2-6}
    &&8&  $5.0830\times 10^{13}$ &$1.54\times 10^{12} (3.04\%)$ &  $1.54\times 10^{9} (0.0030363\%)$   & $1.51\times 10^{10} (0.0298\%)$
         \\\hline
        \hline



 \multirow{3}{*}{RandomWalk1D}&&1& 20 & $1.57\times 10^{-1} (0.79\%)$  &$1.83\times 10^{-6} (0.000009\%)$ & $4.44\times 10^{-3} (0.022\%)$\\%\cline{2-6}
    &2&2& $4.2933\times 10^{2} $ &  $6.78 \times 10^{0} (1.58\%)$& $6.76 \times 10^{-5} (0.00001\%)$ & $1.90\times 10^{-1} (0.0044\%)$\\%\cline{2-6}
    &&3& $9.7516\times 10^{3}$  & $2.45 \times 10^{2} (2.51\%) $& $8.40 \times 10^{0} (0.09\%)$  & $5.61\times 10^{-1} (0.0057\%)$\\%\cline{2-6}
    &&4&  $2.3230\times 10^{5}$ & $8.38\times 10^{3} (3.61\%)$&  $6.48\times 10^{2} (0.28\%)$  & $3.54\times 10^{2} (0.15\%)$\\%\cline{2-6}
    &&5& $5.7681\times 10^{6}$  & $2.79\times 10^{5} (4.48\%)$&  $3.37\times 10^{4} (0.58\%)$ &$2.32\times 10^{4} (0.40\%)$ \\%\cline{2-6}
    &&6&  $1.4858\times 10^{8}$ & $9.19\times 10^{6} (6.19\%)$&  $1.48\times 10^{6} (0.98\%)$ & $1.12\times 10^{6} (0.75\%)$ \\%\cline{2-6}
    &&7& $3.9565\times 10^{9}$  & $3.03\times 10^{8} (7.66\%)$& $5.94\times 10^{7} (1.48\%)$  & $4.72\times 10^{7} (1.18\%)$ \\%\cline{2-6}
    &&8& $1.0857\times 10^{11}$  & $1.01\times 10^{10} (9.26\%)$&  $2.26\times 10^{9} (2.04\%)$  & $1.85\times 10^{9} (1.67\%)$
    \\\hline
        \hline

 \multirow{3}{*}{Uniform (Cont.)}&&1& 0.5 & $5.92\times 10^{-3} (1.18\%)$  & $1.47\times 10^{-9} (3\times 10^{-7}\%)$ & $3.28\times 10^{-2} (7.03\%)$\\%\cline{2-6}
    &6&2& 0.333333 & $4.94\times 10^{-3} (1.48\%)$ &   $1.66\times 10^{-5} (0.00499\%)$& $3.40\times 10^{-2} (11.36\%)$\\%\cline{2-6}
    &&3& 0.25  & $4.57\times 10^{-3} (1.83\%)$ & $2.50\times 10^{-5} (0.00998\%)$  & $3.46\times 10^{-2} (16.06\%)$ \\%\cline{2-6}
    &&4&  0.20  &$4.57\times 10^{-3} (2.28\%)$ &  $3.33\times 10^{-5} (0.0166\%)$  & $3.43\times 10^{-2} (20.69\%)$\\%\cline{2-6}
    &&5&  0.166667  & $4.66\times 10^{-3} (2.80\%)$&   $4.18\times 10^{-5} (0.0249\%)$ &$3.35\times 10^{-2} (25.18\%)$ \\%\cline{2-6}
    &&6&  0.142857 &$4.74\times 10^{-3} (3.32\%)$ &   $4.99\times 10^{-5} (0.0349\%)$ & $3.25\times 10^{-2} (29.51\%)$\\%\cline{2-6}
    &&7&  0.125 &$4.76\times 10^{-3} (3.81\%)$ &     $5.82\times 10^{-5} (0.00465\%)$ &$3.15\times 10^{-2} (33.65\%)$\\%\cline{2-6}
    &&8&  0.1111111 &$4.73\times 10^{-3} (4.25\%)$ &  $6.66\times 10^{-5} (0.00599\%)$ &  $3.04\times 10^{-2} (37.60\%)$
         
    \\\hline
        \hline

 
 \multirow{3}{*}{PDP Model$^{\ast\ast}$}&&1& $1.1885\times 10^{3}$ & $1.60\times 10^{1}  (1.35\%)$  &$2.84\times 10^{-1}  (0.024\%)$ &$5.74\times 10^{0}  (0.48\%)$ \\%\cline{2-6}
    &3&2& $1.4767\times 10^{6}$ &  $3.93\times 10^{4} (2.66\%)$& $3.95\times 10^{2} (0.027\%)$ &$1.16\times 10^{4} (0.78\%)$ \\%\cline{2-6}
    &&3& $1.8981\times 10^{9}$  & $7.37 \times 10^{7} (3.88\%)$& $3.19\times 10^{6}(0.168\%)$ & $2.35\times 10^{7} (1.23\%)$\\%\cline{2-6}
     &&4& $2.5058\times 10^{12}$ & $1.28\times 10^{11}(5.01\%)$ &  $1.64\times 10^{10}$ (0.650\%)  & $4.85\times 10^{10} (1.90\%)$\\%\cline{2-6}
     &&5& $3.3804\times 10^{15}$  &$2.04\times 10^{14}(6.03\%)$  & $ 4.97\times 10^{13}$ (1.450\%) & $1.00\times 10^{14} (2.87\%)$\\%\cline{2-6}
%      &&6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\%\cline{2-6}
%      &&7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\%\cline{2-6}
%      &&8& $1.19415322490998\times 10^{24}$
%   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
%     & $2.95\times 10^{22} (2.4119\%)$\\\hline
        \hline


\end{tabular}
}
\vspace{2mm} 
 \caption{Error for Benchmarks:\\
 $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Appendix~\ref{Appendix}: Table ~\ref{Table:Benchmarks})\\
 $^{2}$ Error of exact moments and sample moments\\
 $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
 $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$\\
 $^{\ast\ast}$Moments of order above 5  could not be computed within ~30 minutes
 }
%  \label{Table:ErrorforBenchmarks}
\label{table:AbsoluteandRelativeErrors}
\end{table}



















%%%%backup last version

% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.7}{
%  \begin{tabular}{c|c|c|l|l|l|l}
% \hline
%   {\bf Program}  &\#Mom. & Moment &   Exact Value$^{1}$  &Absol. sample error$^{2}$   & Absol. ME est. error$^{3}$ & Absol. GC est. error$^{3}$  \\
%     & for est.& & & (relative error$^\ast$)&  (relative error$^\ast$) &  (relative error$^\ast$)\\
%                          \hline
%                          \hline
 


%  \multirow{3}{*}{StutteringP}&&1& 210 & $5.69\times 10^{-2} (0.027\%)$  &$8.08\times 10^{-5} (0.00003\%)$&$4.71\times 10^{-5} (0.00002\%)$\\%\cline{2-6}
%     &2&2& $4.4405 \times 10^4 $ &  $2.39 \times 10^{1} (0.053\%)$& $1.75 \times 10^{-2} (0.00003\%)$&$1.75 \times 10^{-2} (0.00003\%)$\\%\cline{2-6}
%     &&3& $9.453658199999997\times 10^6$  & $6.78 \times 10^{3} (0.0.072\%)$ & $9.21 \times 10^{1} (0.000974\%)$ & $9.25 \times 10^{1} (0.000978\%)$\\%\cline{2-6}
%     &&4& $2.026042602406666\times 10^9$  & $1.48 \times 10^{6} (0.073\%)$& $7.38 \times 10^{4} (0.00364\%)$   & $7.42 \times 10^{4} (0.00366\%)$\\%\cline{2-6}
%     &&5& $4.370501248066238\times 10^{11}$  & $2.17 \times 10^{8} (0.050\%)$ & $3.82 \times 10^{7} (0.00873\%)$ & $3.83 \times 10^{7} (0.00876\%)$ \\%\cline{2-6}
%     &&6&  $9.488480678476714\times 10^{13}$ & $5.51 \times 10^{9} (0.0058\%)$ & $1.60 \times 10^{10} (0.0168\%)$  & $1.60 \times 10^{10} (0.0168\%)$\\%\cline{2-6}
%     &&7& $2.072981561969703\times 10^{16}$  & $2.10 \times 10^{13} (0.101\%)$& $5.88 \times 10^{12} (0.0284\%)$  & $5.90 \times 10^{12} (0.0285\%)$\\%\cline{2-6}
%     &&8& $4.557008480549055\times 10^{18}$  &$1.12 \times 10^{16} (0.245\%)$ &  $1.99 \times 10^{15} (0.0438\%)$  & $2.00 \times 10^{15} (0.0439\%)$
%     \\\hline
%         \hline

%  \multirow{3}{*}{Square}&&1& 10100 & $1.66\times 10^1 (0.16\%)$  &  $1.11\times 10^{0} (0.011\%)$  & $7.97\times 10^{-3} (0.000078\%)$ \\%\cline{2-6}
%     &2&2& $1.060298 \times 10^8$ & $2.31\times 10^5 (0.22\%)$ & $2.30\times 10^3 (0.00217\%)$   & $1.64\times 10^{2} (0.000155\%)$ \\%\cline{2-6}
%     &&3& $1.1544847016\times 10^{12}$  &$1.27\times 10^{9} (0.11\%)$  &  $1.26\times 10^7 (0.0011\%)$  &$2.39\times 10^{9} (0.2072\%)$\\%\cline{2-6}
%     &&4& $1.301272653385280\times 10^{16}$  & $2.98\times 10^{13} (0.23\%)$& $1.99\times 10^{12} (0.0153\%)$   &$9.79\times 10^{13} (0.7581\%)$ \\%\cline{2-6}
%     &&5& $1.515712810699512\times 10^{20}$  & $1.32\times 10^{18} (0.87\%)$& $8.83\times 10^{16} (0.0583\%)$    &$2.61\times 10^{18} (1.7505\%)$
%     \\\hline
%         \hline

% \multirow{3}{*}{Binomial}&&1& 50 & $2.95\times 10^{-1} (0.59\%)$  &  $5.19\times 10^{-5} (0.000051\%)$ & $3.16\times 10^{-3} (0.0063\%)$\\%\cline{2-6}
%     &2&2&   2525  & $2.82\times 10^{1} (1.12\%)$ & $2.74\times 10^{-3} (0.000108\%)$  & $1.87\times 10^{-1} (0.0074\%)$ \\%\cline{2-6}
%     &&3& 128750  & $2.04\times 10^{3} (1.59\%)$ & $1.43\times 10^{-1} (0.000111\%)$  & $1.22\times 10^{1} (0.0095\%)$ \\%\cline{2-6}
%     &&4&  $6.6268625\times 10^{6}$  &$1.32\times 10^{5} (2.00\%)$ & $3.66\times 10^{0} (0.000055\%)$  & $8.22\times 10^{2} (0.0125\%)$ \\%\cline{2-6}
%     &&5&  $3.44215625\times 10^{8}$ &$8.08\times 10^{6} (2.35\%)$ &  $5.52\times 10^{2} (0.000160\%)$ & $5.53\times 10^{4} (0.0161\%)$ \\%\cline{2-6}
%     &&6& $1.803882346250000\times 10^{10}$ & $4.67\times 10^{8} (2.64\%)$& $1.20\times 10^{5} (0.000664\%)$   & $3.66\times 10^{6} (0.0203\%)$\\%\cline{2-6}
%     &&7&  $9.535413368750000\times 10^{11}$ &$2.74\times 10^{10} (2.87\%)$ &  $1.51\times 10^{7} (0.001587\%)$  & $2.38\times 10^{8} (0.0250\%)$\\%\cline{2-6}
%     &&8&  $5.083096302286250\times 10^{13}$ &$1.54\times 10^{12} (3.04\%)$ &  $1.54\times 10^{9} (0.0030363\%)$   & $1.51\times 10^{10} (0.0298\%)$
%          \\\hline
%         \hline



%  \multirow{3}{*}{RandomWalk1D}&&1& 20 & $1.57\times 10^{-1} (0.79\%)$  &$1.83\times 10^{-6} (0.000009\%)$ & $4.44\times 10^{-3} (0.022\%)$\\%\cline{2-6}
%     &2&2& $429.333333333333 $ &  $6.78 \times 10^{0} (1.58\%)$& $6.76 \times 10^{-5} (0.00001\%)$ & $1.90\times 10^{-1} (0.0044\%)$\\%\cline{2-6}
%     &&3& $9751.60000000000$  & $2.45 \times 10^{2} (2.51\%) $& $8.40 \times 10^{0} (0.09\%)$  & $5.61\times 10^{-1} (0.0057\%)$\\%\cline{2-6}
%     &&4&  232303.040000000 & $8.38\times 10^{3} (3.61\%)$&  $6.48\times 10^{2} (0.28\%)$  & $3.54\times 10^{2} (0.15\%)$\\%\cline{2-6}
%     &&5& 5768119.43466667  & $2.79\times 10^{5} (4.48\%)$&  $3.37\times 10^{4} (0.58\%)$ &$2.32\times 10^{4} (0.40\%)$ \\%\cline{2-6}
%     &&6&  148588624.477714 & $9.19\times 10^{6} (6.19\%)$&  $1.48\times 10^{6} (0.98\%)$ & $1.12\times 10^{6} (0.75\%)$ \\%\cline{2-6}
%     &&7& 3956546143.08960  & $3.03\times 10^{8} (7.66\%)$& $5.94\times 10^{7} (1.48\%)$  & $4.72\times 10^{7} (1.18\%)$ \\%\cline{2-6}
%     &&8& 108576810406.772  & $1.01\times 10^{10} (9.26\%)$&  $2.26\times 10^{9} (2.04\%)$  & $1.85\times 10^{9} (1.67\%)$
%     \\\hline
%         \hline

%  \multirow{3}{*}{Uniform (Cont.)$^{\ast\ast}$}&&1& 0.5 & $5.92\times 10^{-3} (1.18\%)$  & $1.47\times 10^{-9} (3\times 10^{-7}\%)$ & $3.28\times 10^{-2} (7.03\%)$\\%\cline{2-6}
%     &6&2& 0.333333 & $4.94\times 10^{-3} (1.48\%)$ &   $1.66\times 10^{-5} (0.00499\%)$& $3.40\times 10^{-2} (11.36\%)$\\%\cline{2-6}
%     &&3& 0.25  & $4.57\times 10^{-3} (1.83\%)$ & $2.50\times 10^{-5} (0.00998\%)$  & $3.46\times 10^{-2} (16.06\%)$ \\%\cline{2-6}
%     &&4&  0.20  &$4.57\times 10^{-3} (2.28\%)$ &  $3.33\times 10^{-5} (0.0166\%)$  & $3.43\times 10^{-2} (20.69\%)$\\%\cline{2-6}
%     &&5&  0.166667  & $4.66\times 10^{-3} (2.80\%)$&   $4.18\times 10^{-5} (0.0249\%)$ &$3.35\times 10^{-2} (25.18\%)$ \\%\cline{2-6}
%     &&6&  0.142857 &$4.74\times 10^{-3} (3.32\%)$ &   $4.99\times 10^{-5} (0.0349\%)$ & $3.25\times 10^{-2} (29.51\%)$\\%\cline{2-6}
%     &&7&  0.125 &$4.76\times 10^{-3} (3.81\%)$ &     $5.82\times 10^{-5} (0.00465\%)$ &$3.15\times 10^{-2} (33.65\%)$\\%\cline{2-6}
%     &&8&  0.1111111 &$4.73\times 10^{-3} (4.25\%)$ &  $6.66\times 10^{-5} (0.00599\%)$ &  $3.04\times 10^{-2} (37.60\%)$
         
%     \\\hline
%         \hline

 
%  \multirow{3}{*}{PDP Model$^{\ast\ast\ast}$}&&1& $1.18857142821508\times 10^{3}$ & $1.60\times 10^{1}  (1.35\%)$  &$2.84\times 10^{-1}  (0.024\%)$ &$0.012 (0.0014\%)$ \\%\cline{2-6}
%     &3&2& $1.47673843347401\times 10^{6}$ &  $3.93\times 10^{4} (2.66\%)$& $3.95\times 10^{2} (0.027\%)$ &$2.362\times 10^{1} (0.0029\%)$ \\%\cline{2-6}
%     &&3& $1.89812214743201\times 10^{9}$  & $7.37 \times 10^{7} (3.88\%)$& $3.19\times 10^{6}(0.168\%)$ & $4.35\times 10^{4} (0.0054\%)$\\%\cline{2-6}
%      &&4& $2.50589193271731\times 10^{12}$ & $1.28\times 10^{11}(5.01\%)$ &  $1.64\times 10^{10}$ (0.650\%)  & $4.67\times 10^{8} (0.0573\%)$\\%\cline{2-6}
%      &&5& $3.38043447836444\times 10^{15}$  &$2.04\times 10^{14}(6.03\%)$  & $ 4.97\times 10^{13}$ (1.450\%) & $2.26\times 10^{12} (0.2630\%)$\\%\cline{2-6}
% %      &&6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\%\cline{2-6}
% %      &&7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\%\cline{2-6}
% %      &&8& $1.19415322490998\times 10^{24}$
% %   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
% %     & $2.95\times 10^{22} (2.4119\%)$\\\hline
%         \hline


% \end{tabular}
% }
% \vspace{2mm} 
%  \caption{Error for Benchmarks:\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Table ~\ref{Table:Benchmarks})\\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$\\
%  $^{\ast\ast}$ Distributions are estimated using 6 moments.
%  }
% %  \label{Table:ErrorforBenchmarks}
% \label{table:AbsoluteandRelativeErrors}
% \end{table}







 %  Sum Rand. Series & -- & -- & & & & \\\hline
    %  Prod. Rand. Var. & -- & -- & & & & \\\hline
    % Bimodal & -- & -- & & & & \\\hline

% \multirow{3}{*}{Sum Rand. Series}&&1& 0.5 &   &   &\\\cline{2-6}
%     &&2&     &  &   & \\\cline{2-6}
%     &&3&   &  &   & \\\cline{2-6}
%     &&4&    & &    & \\\cline{2-6}
%     &&5&    & &    & \\\cline{2-6}
%     &&6&   & &    & \\\cline{2-6}
%     &&7&   & &    & \\\cline{2-6}
%     &&8&   & &     &
         
%     \\\hline
%         \hline
        
%         \multirow{3}{*}{Prod. Rand. Var}&&1& 0.5 &   &   &\\\cline{2-6}
%     &&2&     &  &   & \\\cline{2-6}
%     &&3&   &  &   & \\\cline{2-6}
%     &&4&    & &    & \\\cline{2-6}
%     &&5&    & &    & \\\cline{2-6}
%     &&6&   & &    & \\\cline{2-6}
%     &&7&   & &    & \\\cline{2-6}
%     &&8&   & &    & 
         
%     \\\hline
%         \hline
        
%         \multirow{3}{*}{Bimodal}&1& 0.5 &   &  & \\\cline{2-6}
%     &&2&     &  &   & \\\cline{2-6}
%     &&3&   &  &   & \\\cline{2-6}
%     &&4&    & &    & \\\cline{2-6}
%     &&5&    & &    & \\\cline{2-6}
%     &&6&   & &    & \\\cline{2-6}
%     &&7&   & &    & \\\cline{2-6}
%     &&8&   & &     &
         
%     \\\hline
%         \hline



% , however, $D_{KL}$ is a small number in these cases. Therefore,  Kullback-Leibler distance would not be a proper tool to decide on the quality of  estimations in probabilistic programs. 

==> Distribution Recovery (27)/introduction.tex <==
%!TEX root = samplepaper.tex

\section{Introduction}\label{section:Introduction}




%\paragraph{Related work}
% For PPs: PSI solver (great but only for loop-free programs/loops with a small, bounded number of iterations), ...
% Other distribution recovery methods (not from moments) - sampling, 
% Truncated moment problem - 
% Discrete <- Polar
%\paragraph{Main contributions}

Probabilistic programs (PPs) are programs %extended 
with primitives to draw from probability distributions.
As such, PPs do not produce a single output but rather a probability distribution over outputs. In consequence, PPs provide a powerful framework to model system behavior  involving 
uncertainties. 

Many machine and statistical learning techniques leverage PPs for representing and updating data-driven AI systems~\cite{Ghahramani2015}. %As such, quantifying and modelling  distributions arising from PPs bring together computer programming, statistics and machine learning.
Quantifying and modelling  distributions arising from PPs, and thus formally capturing PP behavior, is challenging. In this work, we address this challenge and provide an algorithmic approach to effectively estimate the probability distributions of  random variables generated by PPs, focusing on PPs with unbounded loops. 


While sampling-based techniques are standard statistical approaches to approximate probability distributions in PPs, see e.g.~\cite{Hastings1970}, they cannot be applied to infinite-state PPs with potentially unbounded loops. More recently, static program analysis was combined with statistical techniques to infer  higher-order statistical moments of random program variables in PPs with restricted  loops and polynomial updates~\cite{bartocci2019automatic,Moosbruggeretal2022}. Our work complements these techniques with an algorithmic approach to compute the  distributions of random variables in PPs with unbounded loops for which (some)  higher-order moments are known (see Algorithm~\ref{fig:algo}). 
Moreover, we assess the quality of our estimation via formal statistical tests.

%
%moments, $\E(x^p_n)$ for $p \in \mathbb{N}$, of any program variable $x$ parameterized by the loop iteration $n \in \mathbb{N}$.
%These techniques are exact, fully automated, and do not rely on user guidance. Nevertheless, they apply only to PPs with polynomial updates. 
%Nevertheless, moments provide only partial information regarding the underlying distributions.

Our method can be applied to any PP for which some moments are known. We provide an algorithmic solution to the so-called finite-moment problem~\cite{gavriliadis2009moment,john2007techniques}, as follows: {\it using a finite number of statistical moments of a PP random variable,  compute  the probability density function (pdf) of the variable to  capture the probability of the random variable falling within a particular range of values}. 
In full generality, the finite-moment problem is ill-posed and  there is no single best technique available to solve it~\cite{DeSouzaetal2010}. In our approach, we tackle the finite-moment problem for PPs by focusing on two particular statistical methods, the
Gram-Charlier expansion~\cite{hald2000early} and Maximum Entropy~\cite{biswas2010function,lebaz2016reconstruction},  to estimate the distribution of PP variables. Our approach is further complemented by statistical goodness-of-fit tests for assessing the accuracy of our estimated pdfs, such as the chi-square~\cite{ross2020introduction} and Kolmogorov-Smirnov~\cite{massey1951kolmogorov} tests.


%, to estimate the distributions arising from PPs with loops (Section~\ref{section:Methodology}).  %We demonstrate the applicability of our approach over PPs with polynomial updates for which (higher) moments of program variables can be computed in closed form  using~\cite{bartocci2020mora,Moosbruggeretal2022} (Section~\ref{section:Evaluation}). 
%\sout{In order to characterize the distributions arising from PPs, we use recent results in exact moment analysis} \efi{what does this mean? and established statistical methods to reconstruct distributions of program variables using their exact moments.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\lk{TODO: we should use the same axis/scale on Fig.1 and Fig.3, and it should be consistent with $e=1000$}
%
%
%\Ahmad{I normalized the histogram like this: the height of each bin divided by sum of areas of bins. With this, in the resulting normalized histogram,  we have the sum of all bins to be 1. Matlab function ``histogram(Sampled$_{Data}$,nbins,'Normalization','pdf')'' does this. If we want to plot histogram together with estimated pdfs, we should normalize such way.  x-axis and scale of each pdf depends on the support of pdf. For Vasicek model is [-1,1] while for PDP model is [0,2000]. depending on the x-axis, the y-axis are also different. I can not plot all pdfs of different problems in a same scale. }
%
%
%LK: OK, I added "normalized" to the caption of Figure 1, as Effie suggested

\paragraph{\bf Motivating Example.} %We motivate our work  using a stochastic process implementing 
The Vasicek model in finance~\cite{vasicek1977equilibrium} describes the evolution of interest rates and serves to motivate our work. This model is defined by the stochastic differential equation, 
\begin{equation}
 dr_{t}=a(b-r_{t})\,dt+\sigma \,dW_{t}   \label{vasicek}
\end{equation}
where $W_t$ is a Wiener process (standard Brownian motion) \cite{morters2010brownian} modeling the continuous inflow of randomness into the system, $\sigma$ is the standard deviation representing the amplitude of the randomness inflow, $b$ is the long term mean level around which paths evolve  in the long term, $a$ is the speed of reversion specifying the velocity at which such trajectories will regroup around $b$ in time.
We encode~\eqref{vasicek} as a PP in Fig.~\ref{fig:vasicek-intro}, using program constants $a,b,\sigma$, as described above and variables $r,w$ to respectively capture the randomness ($r_t$) and Wiener process ($W_t$) of the Vasicek model. The PP of Fig.~\ref{fig:vasicek-intro} has polynomial loop  updates over random variables $r,w$ drawn from a  normal  distribution with 
zero mean and unit variance. This PP satisfies the programming model of~\cite{bartocci2019automatic,Moosbruggeretal2022}, and as such higher-order moments of this PP %in Fig.~\ref{fig:vasicek-intro} 
can be computed using~\cite{bartocci2019automatic,Moosbruggeretal2022}. Based on the first- and second-order 
%\lk{add: the first- and second-order (???how many???)} \Ahmad{we use only two moments for estimations and compare estimated moments (of order 2-8) to the exact one } 
moments of $r$ in the Vasicek model PP, %, Fig.~\ref{fig:vasicek-intro} (left panel), 
we estimate the distribution of the random variable $r$ using 
 Maximum Entropy  and Gram-Charlier expansion (see Section~\ref{ssec:reconstructing-distribution}). Data generated by executing the PP repeatedly, at loop iteration 100, are summarized in the histogram in the right panel of Fig.~\ref{fig:vasicek-intro}, giving a rough estimate  of the distribution of $r$. The black and red lines are kernel density estimates~\cite{Silverman1998} of the pdf of $r$ using 
Maximum Entropy and Gram-Charlier expansion, respectively. Both pdf estimates  closely track the histogram, a proxy for the true distribution of $r$. 
The close match between our estimated pdfs and the true distribution of $r$ is also supported by the chi-square and Kolmogorov-Smirnov test results (see Section~\ref{ssec:methods-of-evaluation}).
%
%These estimates provide a basis for different validation/verification queries over the PP. 
%\lk{we need to add an interpretation of the figure. Once the methodology section is ready, double-check and explain the use of Kernel Smoothing, as it is not yet mentioned in the intro} \Ahmad{I have updated the figure to show ME and GC estimated distributions and histogram of sampled data. We use Kernel Smoothing only for calculating Kullback-Leibler distance, which I added the detail of Kernel Smoothing there (3rd paragraph of Methods of Evaluation).}
\begin{figure}[t]
    \centering
    \begin{minipage}{0.4\textwidth}
    \begin{algorithmic}
        \STATE $a:=0.5$
        \STATE $b:=0.2$
        \STATE $\sigma:=0.2$
        \STATE $w:=0$
        \STATE $r:=2$
        \WHILE{true} 
            \STATE $w:=\text{Normal}(0,1)$
            \STATE $r:=(1-a) r + a b + \sigma w$
        \ENDWHILE
    \end{algorithmic}
    \end{minipage}
    \begin{minipage}{0.58\textwidth}
        \includegraphics[width=6.5cm]{Figures/HistogramGCMEforVasicekmodel.eps}
    \end{minipage}
%   % \begin{minipage}
%     \begin{table}
%     \begin{align*}
%         f_{GC}(r)=
%         \frac{\alpha\; \exp\big(-\frac{\big(r - {(2^n + 9)}/{(5*2^n)}\big)^2}{((36/25)2^{-n}) 
%         - ((2/2^{2n})(2^n + 9)^2)/25 + (478/2^{2n})/75 + 14/75)}\big)}{\beta\; \big((18/25)2^{-n} 
%         - ((1/2^{2n})(2^n + 9)^2)/25 + (239/2^{2n})/75 + 7/75\big)^{1/2}}
%     \end{align*}
%     \end{table}
%     %\end{minipage}
    \caption{The Vasicek model~\eqref{vasicek} describing the evolution of interest rates, modeled as a PP in the left panel. 
    The estimated distributions  of $r$ are plotted in the right panel. The (normalized) histogram plots the 1000 sampled  $x$-values generated by running the PP 1000 times at iteration $n=100$. The kernel density estimates of the  Maximum Entropy (black dash-dotted line) and 
    Gram-Charlier (red solid line) pdf estimations follow closely the sampled data based histogram, showcasing that both estimates are  effectively estimating the true (sampled) distributions of $r$ (blue histogram). 
 %
 %
 %and \efi{normalized ?} \Ahmad{height of each bin divided by sum of areas of bins, with this we have the sum of all bins to be 1.} histogram of sampled data together with the  Gram-Charlier (red solid line) and  Maximum Entropy (black dash-dotted line) based pdf estimates, smoothed using kernel density estimation, at iteration $n{=}100$. %where $\alpha=2251799813685248$ and $\beta=5644425081792261$.
    % \efi{what is the Difference between the GC and ME estimated pdfs is plotted in (right-bottom)?}. 
    % \lk{why Kernel Smoothing and not Gran-Charlier? \Ahmad{I have updated the figure.} We need to explain the figure, what is the gain, what is the message?}.
    }
    \label{fig:vasicek-intro}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\paragraph{\bf Related Works.} Kernel density estimation is combined with a constrained minimization problem for an (Hausdorff) instance of the  finite-moment problem in~\cite{athanassoulis2002truncated}. This approach is further extended in~\cite{gavriliadis2009moment}. % for the Stieltjes moment problem.
%In this method, the target pdf at a point is approximated by a sum of weights.
%The latter are typically modelled by a symmetric density, such as the standard normal. The optimal weights are computed through minimizing the distance between the set of given moments and those estimated via the kernel density estimator.
However, this nonparametric estimation method requires constant tuning of the bandwidth parameters, which increase with the number of moments, and is seen to often perform poorly~\cite{lebaz2016reconstruction}.
Along similar lines, the approach of~\cite{john2007techniques} employs spline-based non-parametric density estimation using piecewise polynomial functions to recover  target distributions. This method is  improved in~\cite{DeSouzaetal2010} to an adaptive algorithm dealing with non-equidistant grids. 
This method, though, assumes a smooth transition at the boundaries of sub-intervals that needs to be checked repeatedly during the reconstruction process \cite{lebaz2016reconstruction}. 
Our work complements these approaches by a tailored algorithmic method to effectively  estimate distributions arising from PPs that  uses higher-order moments of these PPs in combination with Maximum Entropy  and Gram-Charlier expansion.
To the best of our knowledge, 
%\lk{anything else wrt mentioned lines, that they do/we do not do, or vice versa}
these statistical methods  have not yet been used and evaluated in the setting of probabilistic loops.


%As shown in \cite{mortier2014comparison,lebaz2016reconstruction}, the spline-based algorithm is highly sensitive to negative tolerances leading to different reconstructions for the same target probability density function\footnote{Negative tolerance is a variable used in adaptive spline-based methods that authors of \cite{mortier2014comparison,DeSouzaetal2010} recommended to set $tol_{neg}$ at a very small negative value instead of 0 in their algorithm.}.
%This method assumes a smooth transition at the boundaries of sub-intervals and these conditions need to be changed during the reconstruction process.
%Maximum Entropy is based on the maximization of the Shannon entropy \cite{tagliani1999hausdorff,tagliani2001numerical,mead1984maximum,biswas2010function}.
%Its main advantage is the low computational cost \cite{lebaz2016reconstruction} and has received increasing interest over the last two decades.

Our work is related to emerging efforts in estimating probabilistic distributions/densities in PP, as addressed by the works~\cite{gehr2016psi,gehr2020lpsi,HuangDM21,HoltzenBM20}.
The provided automation, supported by the tools ($\lambda$)PSI \cite{gehr2016psi,gehr2020lpsi}, AQUA~\cite{HuangDM21}, and DICE~\cite{HoltzenBM20}, yield  symbolic frameworks to  compute exact (posterior) densities for PPs with {bounded loops}. Also focusing on bounded loops,  sampling-based techniques to approximate the distributions resulting from PPs are exploited in~\cite{CaretteS16,NarayananCRSZ16,Carpenter2017StanAP,BhatBGR17}.
In contrast, our approach is not restricted to bounded loops but focuses on density estimation for PPs with unbounded loops.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \todo{Effie: a description and comparison, or at the very least, why it is not directly comparable, should be given.}
% \Ahmad{I have added this paragraph to above:
% Recovery of (posterior) distribution given some evidences is a common task in probabilistic inference. Existing  approaches for probabilistic inference  include: 
% \textit{exact symbolic} approaches (see e.g. \cite{sanner2012symbolic,bhat2013deriving,gehr2016psi}) and \textit{approximate symbolic} approaches (\cite{?, ?, ?}).  
% In \cite{gehr2016psi}, a symbolic
% analysis system, called \textit{PSI (Probabilistic Symbolic Inference)}, is presented  for automating exact inference in PPs via program analysis. PSI  automatically  computes the exact pdf of the random variable(s) of interest represented by that program. 
% As exact inference is theoretically expensive,  
% probabilistic inference systems may exploit  approximate
%   techniques and implement algorithms that calculate numerical approximations \cite{?,?,?,?}. 
% % These methods trade precision for better performance \cite{gehr2016psi}.
% Distribution recovery from moments  has not been much explored in the context of probabilistic programs, verification and cyber-physical systems.
% Note that non of above-mentioned works (nor existing symbolic-based methods, neither approximation-based methods) recover an unknown distribution form its moments.}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{\bf Our Contributions.}
The  main contribution of this paper is the development of  an {\it algorithmic  approach to effectively estimate distributions arising from PPs with unbounded loops (Algorithm~\ref{fig:algo})}. We employ two formal techniques from mathematical statistics, Maximum Entropy (ME) and Gram-Charlier (GC) expansion, to estimate distributions of PP variables (Section~\ref{ssec:reconstructing-distribution}).  We use symbolic approaches to compute exact moments of loop variables as symbolic expressions parameterized by the loop counter.
Further, we apply statistical tests to assess the adequacy of the estimated distributions of PP variables (Section~\ref{ssec:methods-of-evaluation}). We evaluate our approach on a number of benchmarks and demonstrate the accuracy of our proposed estimation approach (Section~\ref{section:ImplEvaluation}).



% $n \in \mathbb{N}$. 
%\textcolor{blue}{Our ME method overcomes the reconstruction numerically via an optimization procedure while our GC method  estimates the target distribution symbolically in terms of loop iteration $n$ and parameterized (unknown) variables}. We  use statistical approaches to evaluate our approach on a number of benchmarks and demonstrate the accuracy of our work (Section~\ref{section:ImplEvaluation}). 

\paragraph{\bf Paper Outline.} The rest of the paper is organized as follows.  Section~\ref{section:Preliminaries} introduces the necessary prerequisites from probability theory, statistics, and probabilistic programs.
In Section~\ref{section:Methodology}, we introduce the (adjusted) methods we use to estimate the distributions of program variables from their moments.
%We also present the methods we use to evaluate their accuracy in estimating distributions. 
We report on our practical findings in Section~\ref{section:ImplEvaluation}, and conclude the paper in Section~\ref{section:Conclusion}. %, by first 
%introducing  our benchmark suite  in Section~\ref{section:Benchmarks} and then describing our experimental evaluation in  Section~\ref{section:Evaluation}. There, we  demonstrate the applicability of our approach over PPs with polynomial updates for which (higher) moments of program variables can be computed in closed form  using~\cite{bartocci2020mora,Moosbruggeretal2022}. %(Section~\ref{section:Evaluation}). %
%We conclude in Section~\ref{section:Conclusion}.


==> Distribution Recovery (27)/methodology.tex <==
%!TEX root = samplepaper.tex
\section{Methodology}\label{section:Methodology}
Maximum Entropy is applied to estimate the distribution of the random variable generated in the probabilistic program  \textit{Random Walk 1D} using its calculated moments via moment-based invariant generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. The target distribution is unknown and  only moments of the random variable of interest, expressed as a function of loop iteration, are available (Equations~(\ref{eq:ExactmomentsofRandomWalk1}-\ref{eq:ExactmomentsofRandomWalk3})). 

In order to reconstruct the distribution of random variable $x$ in the probabilistic program Random Walk 1D, we fix the loop iteration to be $n=100$ and use the first three exact moments of $x$, i.e. $E[x(100)], E[x^2(100)]$ and $E[x^3(100)]$. Applying ME method to the given moments, we recover the pdf and the cdf of $x$ which is shown with red color in Figure~\ref{fig:pdfRandomwalk1DME1} (Middle and Right).  


In order to assess accuracy of distribution estimation, we carry out a Monte Carlo ``experiment'' by executing  the PP a \textit{large} number of times (here, large=1000), and  compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test. Results (see Figure~\ref{fig:pdfRandomwalk1DME1}) show visually the agreement of the estimated pdf and cdf with the sampled data (indeed, with the KS density approximation of the sampled data). Details and numerical result of the accuracy evaluation will be presented in Section~\ref{section:Evaluation}.

% Here, we apply the Maximum Entropy method  to estimate distributions of a random variable of probabilistic program  Random Walk 1D  using its calculated moments via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. Note that the target distribution is unknown and we have only moments of the random variable of interest presented as a function of loop iteration. With the help of  statistical tools, we also confirm the agreement of our estimated distributions with the ones generated during the execution of these probabilistic programs. 


% \todo{The following is not a correct statement: We assess the agreement or accuracy  of the estimated distributions with the ones generated during the execution of the probabilistic programs.}

% What you do is the following: 

% \begin{enumerate}
%     \item You estimate the distribution using ME and the exact moments provided by the recurrence-based algorithm in \cite{bartocci2020mora,bartocci2019automatic}
%     \item Assess accuracy of ME estimation of moments and the true moments with plots only (so far)!
%     \item To assess accuracy of distribution estimation, you carry out a monte carlo ``experiment,'' as follows: You repeat the PP a \textit{large} number of times (here, large=1000), and then compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test.   
% \end{enumerate}

\efi{What about multivariate distribution approximation? That is, in a Prob PP, multiple random variables can be generated that are dependent so they have a joint distribution. I believe ME applies also in multivariate distribution estimation.}


\bigskip

\noindent{\bf Random Walk 1D} 
\begin{align}
&v:=0\\\notag
&x:=0\\\notag
&\text{while true:}\\\notag
&\quad v:=\text{uniform}(0,1)\\\notag
&\quad x:=x+v\;\;[7/10]\;\;x-v
\end{align}
Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~1 of  \cite{bartocci2019automatic}: 
\begin{align}\label{eq:ExactmomentsofRandomWalk1}
&E[x(n)] = n/5\\\label{eq:ExactmomentsofRandomWalk2}
&E[x^2(n)] = n^2/25 + 22n/75\\\label{eq:ExactmomentsofRandomWalk3}
&E[x^3(n)] = n^3/125 + n^222/125 - n21/250
\end{align}
Figure~\ref{fig:SampledEXforRandomWalk1Sample1000loop1} shows the agreement of sampled data and exact expected value of random variable $x$ per each loop iteration. One easily can see that the uncertainty propagates through probabilistic loop and remains around the exact expected value of the variable $x$. Figure~\ref{fig:SampledEXforRandomWalk1000Sample1000loop1} shows that the mean value and the second moment for a sample of size 1000 agrees the exact expected values for each loop iteration $n$. This shows the strength  of the moment-based invariant generator in which on can calculate moments of random variables of a PP without running the program.  
\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
	\caption{$x$-axis: iteration, $y$-axis: sampled values of the random variable. In red is the Mora generated $E(x)$, and in blue are the sampled values of the random variable in \textit{Random Walk 1D}.}
	\label{fig:SampledEXforRandomWalk1Sample1000loop1}
\end{figure}

\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=4cm]{Figures/ExSampledandMora1000loop1000Sample.eps}
	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
	\caption{ $E(x)$ and $E(x^2)$ for Random Walk 1D using 1000 sample for each iteration of loop.}
	\label{fig:SampledEXforRandomWalk1000Sample1000loop1}
\end{figure}
\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=10cm,height=6cm]{Figures/absoluteErrorExRandomWalk1D.eps}\\
	\includegraphics[width=10cm,height=6cm]{Figures/relativeErrorExRandomWalk1D.eps}
	\caption{ Absolute and relative errors $E(x)$ and $E(x^2)$ for Random Walk 1D: \\
	Absolute Error of $E(x)= |{E(x)}_{sample}-{E(x)}_{exact}|$\\
	Absolute Error of $E(x^2)= |{E(x^2)}_{sample}-{E(x^2)}_{exact}|$\\
    Relative Error=$\frac{\text{Absolute Error}}{\text{Exact Value}}$}
	\label{fig:AbsoluteandRelativeErrorsRandomWalk1D}
\end{figure}








\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=3.8cm]{Figures/histogramRandomwalk1D.eps}
	\includegraphics[width=3.8cm]{Figures/pdfRandomwalk1DME.eps}
	\includegraphics[width=3.8cm]{Figures/cdfRandomwalk1DME.eps}
	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Random Walk 1D. Estimation of Distribution using Maximum Entropy method with 3 moments.}
	\label{fig:pdfRandomwalk1DME1}
\end{figure}

 








==> Distribution Recovery (27)/methodologynew.tex <==
%!TEX root = samplepaper.tex
%\newpage
\section{Effective Estimation of Distributions for Probabilistic Loops}\label{section:Methodology}
%We now present our approach to  estimate the distributions  of (random) variables of probabilistic loops, while also assessing the quality of the estimated distributions.
%
%summarizes our main steps in this respect  (Section~\ref{ssec:reconstructing-distribution}), including an effective framework for evaluating the quality/accuracy of our estimated distributions  (Section~\ref{ssec:methods-of-evaluation}).

We present our estimation approach for the pdf of a random variable $x$ 
in a probabilistic loop $\mathcal{P}$, provided the first $M$ statistical moments of $x$ are known. We use 
Maximum entropy (ME) and Gram-Charlier A (GC)  expansion (lines~{1--4} of Algorithm~\ref{fig:algo}). 
We  assess the accuracy of our pdf estimates by conducting statistical tests over our distribution estimates (lines~5--14 of  Algorithm~\ref{fig:algo}). 
Our approach is summarized in Algorithm~\ref{fig:algo} and detailed next. 



\begin{algorithm}[t!]
   %\SetKwInOut{Params}{Params}
%    \Params{My params}
%\Params{Object}
\begin{algorithmic}[1]
    \REQUIRE Probabilistic loop $\mathcal{P}$ with program variable(s) $x$;\\ 
    \qquad set $M$ of exact  moments of~$x$ for loop iteration $n$ of $\mathcal{P}$\\% computed by Mora/Polar \cite{bartocci2020mora,Moosbruggeretal2022}
    \ENSURE Estimated distributions  $f_{\me}$ and $f_{\gc}$ of $x$,  with respective {accuracy} $\mathcal{A}_{\me}$ and $\mathcal{A}_{\gc}$
    \\
    \hspace*{-1.7em}{\bf Parameters:} Loop iteration $n\in\mathbb{N}$; number of executions $e\in \mathbb{N}$  of $\mathcal{P}$\\
    \vspace{0.5em} \textbf{Initialization:}\\
    %\STATE If not given, compute exact moments $M$ of a program variable $x$ of $\mathcal{P}$\\
    \STATE Choose a subset of exact moments $S_{\text{M}}=\{\E(x),\E(x^2),\dots,\E(x^{|S_{\text{M}}|})\} \subset M$ 
    \STATE Collect ${Sample_{Data}}$ by sampling $e$ many $\mathcal{P}$ variable values at the $n$th loop iteration \\
    \vspace{0.5em}
    \textbf{Distribution Estimation:}\\
    \STATE Compute $f_{\me}$ using $S_{\text{M}}$ and ME as in~\eqref{eq:pdf:ME}\\
    \STATE Compute $f_{\gc}$ using  $S_{\text{M}}$ and GC as in~\eqref{pdfGC}\\

    
    % \vspace{0.5em} \textbf{KL Divergence:}\\
    % \STATE Compute KL Divergence for $f_{\me}$ and $f_{\gc}$ using ${Sample_{Data}}$, as in~\eqref{eq:KL:ME}--\eqref{eq:KL:GC} \\
    \vspace{0.5em}
    \textbf{$\boldsymbol\chi^2$ Test:}\\
    \STATE Split ${Sample_{Data}}$ into bins and compute observed frequencies $O_i$\\
    \STATE Calculate expected frequencies $E_{\me, i}$ and $E_{\gc, i}$ from $f_{\me}$ and $f_{\gc}$, as in~\eqref{eq:ChiSquare:EFreqs}\\
    \STATE Compute $\chi^2$ test statistics for $f_{\me}$ and $f_{\gc}$ as in~\eqref{eq:ChiSquare:Tests} and compare them to the critical value $CV_{\chi^2}$\\%=\chi^2_{0.95,\#\text{bins}-1}$\\
    %
    \vspace{0.5em} \textbf{K-S Test:}\\
    \STATE Calculate the empirical cdf $F_{Sample}$ of $Sample_{Data}$ and cdfs $F_{\me}$, $F_{\gc}$ using $f_{\me}$ and $f_{\gc}$\\
    \STATE Compute K-S test statistics $D_{\me}^\ast$, $D_{\gc}^\ast$ of  $f_{\me}$ and $f_{\gc}$ as in~\eqref{eq:KSTest} and compare to the critical value $CV_{\texttt{K-S}}$\\
    
    %\vspace{0.5em}
   %\textcolor{blue}{  \textbf{Higher Moments Precision:}\\
    %\STATE Calculate approximated moments  $M_{\me}, M_{\gc}, M_{Sample}$ of size of  $M$ using pdfs  $f_{\me}$, $f_{\gc}$, and $Sample_{Data}$\\
    %\STATE Calculate absolute and relative errors of approximated moments  $M_{\me}, M_{\gc}, M_{Sample}$, compared to the exact moments $M$
    %}
    
    \vspace{0.5em} \textbf{Pdf Accuracy Evaluation:}\\
    \STATE If $\chi_{\me}^2<CV_{\chi^2}$ or $D_{\me}^\ast<CV_{\texttt{K-S}}$ then $\mathcal{A}_{\me}\leftarrow NOT\; REJECTED$ \\
    \qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad else $\mathcal{A}_{\me}\leftarrow REJECTED$
    \STATE If $\chi_{\gc}^2<CV_{\chi^2}$ or $D_{\gc}^\ast<CV_{\texttt{K-S}}$ then $\mathcal{A}_{\gc}\leftarrow NOT\; REJECTED$ \\
    \qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad else $\mathcal{A_{\gc}}\leftarrow REJECTED$
\end{algorithmic}
\caption{Effective Distribution Estimation}
\label{fig:algo}
\end{algorithm}




\subsection{Distribution Estimation}\label{ssec:reconstructing-distribution}

Given a variable $x$ of a probabilistic loop $\mathcal{P}$, we use a subset $S_{\text{M}}\subset M$  of its exact moments for estimating the  distribution of $x$  through ME and GC expansion. 
%For each probabilistic loop we compute moments using Mora/Polar\footnote{\url{https://github.com/probing-lab/polar}}\cite{bartocci2020mora,Moosbruggeretal2022}, and then approximate the distributions in two different ways: through Maximum entropy (ME) and the Gram-Charlier (GC) expansion.
For this, 
we  adjust ME and GC expansion  
%\eqref{pdfGC} and adjust~\eqref{eq:pdf:ME} 
to compute the  estimated distributions $f_{\gc}$ and $f_{\me}$ of $f$, the pdf of $x$, respectively. 
For doing so, we use the set $S_{\text{M}}=\{\E(x),\E(x^2),\dots,\E(x^{|S_{\text{M}}|})\}$ of exact moments of $x$. 
For ME, we derive the Lagrange multipliers $\xi_j$, for $j=0, 1, \ldots, |S_{\text{M}}|$ in the ME approximation~\eqref{eq:pdf:ME}, where $|S_{\text{M}}|$ denotes the cardinality of $S_M$.  %
%
%In the setting of GC expansion,  we truncate 
%
%use the normal/Gaussian distribution  as the known distribution $\psi$, with mean $\mu$ and variance $\sigma^2$, in the GC expansion. We thus have %To this end, we set %
%We use the normal/Gaussian distribution  as the known distribution $\psi$ in the Gram-Charlier expansion with
%mean $\mu$ and variance $\sigma^2$. Thus, %~\eqref{pdfGCGeneral};
%$\kappa_1=\mu$, $\kappa_2=\sigma^2$, and  $\psi(x)=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$. %in~\eqref{pdfGCGeneral}.  
%We also exploit the property that GC expansion can be expressed in terms of Hermite- and Bell-polynomials~\cite{brenn2017revisit}. 
For GC expansion, we truncate the GC expansion~\eqref{pdfGCGeneralC} based on $|S_M|$ moments, and we use the $f_{\gc}(x)$  to estimate the pdf of $x$ as
\begin{align}\label{pdfGC}	f_{\gc}(x) = 
 %{\psi}(x) \sum_{m=0}^{\infty}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right),
%  {f}(x)=\sum_{m=0}^{\infty}B_m(0,0,\kappa_3,\dots,\kappa_m)\frac{(-D)^m}{m!}{\psi}(x),
{\psi}(x) \sum_{m=0}^{|S_{\text{M}}|}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right).
\end{align} 
%where $B_m$ are the Bell polynomials
%and $He_m$ are the Hermite polynomials. 
The cumulants $\kappa_m$ of the pdf of $x$ in \eqref{pdfGC} are computed from the  moments in  $S_{\text{M}}$. 
%We provide the details of the derivation of \eqref{pdfGC} in the Appendix.

The $f_{\gc}(x)$ estimate of the pdf of a PP variable~$x$ can be computed % approximation~\eqref{pdfGC}, 
even when the moments of~$x$ are parametric; i.e., their closed-form functional representations depend on the loop iteration~$n$ and/or other symbolic values. This is especially useful in the analysis of (probabilistic) loops, as it allows us to encompass {\it all} loop iterations in a single symbolic estimate using GC expansion. 
\iffalse
Our $f_{\me}(x)$ and $f_{\gc}(x)$ estimates of the pdf of a PP variable $x$ can be computed % approximation~\eqref{pdfGC}, 
even when the moments of $x$ are parametric; i.e., their closed-form functional representations depend on the  loop iteration $n$ and/or other symbolic values. This is especially useful in the analysis of (probabilistic) loops, as it allows us to encompass {\it all} loop iterations in a single symbolic estimate using ME and/or GC expansion. 
\fi


%Further,  we use the normal/Gaussian distribution  as the known distribution $\psi$ in the Gram-Charlier expansion~\eqref{pdfGCGeneral}; hence, we have the mean $\mu=\kappa_1$, variance $\sigma^2=\kappa_2$, and pdf  $\psi(x)=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$ in~\eqref{pdfGCGeneral}. In addition, the cumulants $\kappa_m$ of the pdf of $x$ are computed from the moments $S_{\text{M}}$. As such, the adjusted Gram-Charlier A expansion $f_{GC}(x)$ approximating the pdf of $x$ in our setting is
%\begin{align}\label{pdfGC}	f_{GC}(x) = 
 %{\psi}(x) \sum_{m=0}^{\infty}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right),
%  {f}(x)=\sum_{m=0}^{\infty}B_m(0,0,\kappa_3,\dots,\kappa_m)\frac{(-D)^m}{m!}{\psi}(x),
%{\psi}(x) \sum_{m=0}^{|S_{\text{M}}|}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right),
%\end{align} 
%where $B_m$ are the Bell polynomials
%and $He_m$ are the Hermite polynomials~\cite{brenn2017revisit}.

%\lk{check the text above and whether~\eqref{pdfGC} is indeed the correct equation for our work. Do we really have $m$ in ~\eqref{pdfGC} ranging from 0 to $\infty$?}\Ahmad{I have updated the formulas, now they are correct.} LK: OK!

% \Ahmad{for me to follow notation to be consistent: $S_{\text{M}}$ is a set of moments and $|S_{\text{M}}|$ is its cardinal. Am I right?} \lk{YsES}

%\Ahmad{$\mu=\kappa_1$ and $\sigma^2=\kappa_2$. The formula \ref{pdfGC} with Bell  and Hermite ploynomials is only derivable if we assume our known distribution is normal. Otherwise we can not write Gram-Charlier expansion using Bell and Hermite polynomials }




\begin{example}\label{exactmomentsVasicek} We use the PP in Fig.~\ref{fig:vasicek-intro} to illustrate our approach.
The set $M$ in Algorithm~\ref{fig:algo} contains the exact first two moments of $r$ for an arbitrary loop iteration $n$. These two moments can be expressed as functions of loop iteration~$n$ of the PP (see Sec.~\ref{section:ImplEvaluation}), 
    \begin{equation}\label{eq:Vasicek:R:2Moments}
        \begin{split}
            &\E(r(n)) = 2^{-n}(2^n + 9)/5,\\
            &\E(r^2(n)) = 7/75 + (18)2^{-n}/25 + (239)2^{-2n}/75.
            %\\&\E(r^3(n)) = 8^{-n}((239)2^n + (63)4^n + (5)8^n + 693)/125
        \end{split}
    \end{equation}
   As a result, we set $S_{\text{M}}=M=\{\E(r(n)),\E(r^2(n))\}$ for loop iteration $n$ (line~1 of Algorithm~\ref{fig:algo}). These functions yield exact moments of  $r$ for concrete values of the loop iteration $n$, by only instantiating the above expressions with the respective values of~$n$. For example, at 
    loop iteration $n=100$, the two exact moments of $r$ are $\E(r(100)) = 0.20 $ and $\E(r^2(100)) = 0.093\bar{3} $.
    
 
  
%We next  estimate the pdf of $r$ using ME computation and GC expansion (line~3--4 of Algorithm~\ref{fig:algo}).   
%For example , at loop iteration $n=100$, the moments are $\E(r) = 0.20 $ and $\E(r^2) = 0.093\bar{3} $.
    % \mm{MM: TODO add the moments at iteration $100$.}\Ahmad{done!}



\paragraph{ME estimation of the pdf of $r$.} 
%We fix the iteration number $n$. 
Given~\eqref{eq:Vasicek:R:2Moments}, %the exact moments $\E(r(n))$ and $\E(r^2(n))$, 
we solve the  system~\eqref{eq:nonlinearSystemME}
of nonlinear equations to obtain the respective  Lagrange multipliers $\xi_j$, $j = 0,1,2$. 
For solving~\eqref{eq:nonlinearSystemME}, %we exploit numerical approaches where iterative methods are used to solve the nonlinear system of equations \cite{mead1984maximum,lebaz2016reconstruction}.  Here, 
we assume that the support of  the target pdf of $r$ is a subset of $[l,u]$, where $l$ and $u$ are known scalars and apply the Levenberg–Marquardt numerical minimization algorithm~\cite{levenberg1944method,marquardt1963algorithm}. %as an iterative procedure that combines gradient descent and
%Gauss-Newton, with an initial choice of the $\xi_j$'s in \eqref{eq:nonlinearSystemME} and
%a tolerance of $10^{-6}$ for stopping the iterative process.
Once the optimal multipliers for~\eqref{eq:nonlinearSystemME} are computed, the ME estimate is $f_{\me}(r)=\exp\left[-(\xi_0+\xi_1r+\xi_2r^2)\right]$. 
%\lk{changed  $f_{ME}(x)$ to $f_{ME}(r)$, that is $r$ instead of $x$}
%\lk{do we need to mention  support here? Maybe this is relevant only for Sect4}\Ahmad{for implementation, we need an upper and a lower bound for the support of the random variable. otherwise, we are not able to compute integrals in the eqn. \eqref{eq:nonlinearSystemME} during the ME reconstruction.}
%\Ahmad{No, they are different than parameters $a$ and $b$ in the PP of Vasicek. The interval $[a,b]$ is a superset of support of random variable and   depends on the problem, for Vasicek I set a=-1.5 and b=1.5, we can consider the interval [a,b] as wide as to be sure the support of the distribution is a subset of [l,u] }
%and compute the  integrals in \eqref{eq:nonlinearSystemME} numerically.  
%We use Matlab for our implementation.  
Specifically, $f_{ME}(r)= \exp[0.171658 + 3.749999 \,r + 9.374997\, r^2]$ at loop iteration $n=100$. As seen from Fig.~\ref{fig:vasicek-intro}, this estimate is closely approximating the true (sampled) distribution of $r$.


%We use ... \ms{matlab? what are the key intermediate states and how we compute everything?} \Ahmad{a paragraph  was added.} \ms{The computation was done I'm matlab, right? could any other engine be used, or was any matlab-specific function used (such as the kernel smoothing later)? same question for GC.}

% In order to reconstruct the distribution of random variable $r$ in the probabilistic program Vasicek Model, we fix the loop iteration to be $n=100$ and use the first two exact moments of $r$, i.e. $\E(r(100))$ and $\E(r^2(100))$. 
% \begin{example}
%     \ms{TODO: PDF of the ME-based estimation.}
% \end{example}




\paragraph{GC estimation of the pdf of $r$.}  Given the first two exact moments of $r$ in \eqref{eq:Vasicek:R:2Moments}, we apply ~\eqref{eq:CumulantMomentRelation} in order to compute the corresponding cumulants.  
% We again assume that the support of the pdf of $r$ is a subset of $[l,u]$, where $l$ and $u$ are known scalars \lk{again, what are a, b?} \Ahmad{interval [l,u] for Vasicek model is [-1.5,1.5] which is a superset for the support of random variable $r$.}.
Using the normal distribution  with mean $\mu=\kappa_1=\E(r)$ and variance $\sigma^2=\kappa_2=\E(r^2)-\E^2(r)$ in~\eqref{pdfGC}, 
the GC estimate of the pdf  of $r$ is $f_{\gc}(r)=({1}/{\sqrt{2\pi\kappa_2}})\exp\big[-{(r-\kappa_1)^2}/{2\kappa_2}\big]$. %\lk{complete: we need $f_{GC}(r)$ in the setting we consider, which is with two moments. } 
% \Ahmad{if we use only two moment $\E(x)$ and $\E(x^2)$ (or cumulants $\kappa_1$ and $\kappa_2$), then all terms in the  sum \eqref{pdfGC} is 0 except for the first term which is 1. In this case, the  resulting pdf is only $\psi(x)$ which is a normal distribution with the mean $\kappa_1$ and variance $\kappa_2$. If we go up to have estimation with 3 moments (3 cumulants), then the pdf will be more complicated, I can compute it but for a symbolic representation (see below) it would be quite long that would be hard to mention it it here, to show we have a symbolic estimation of pdf w.r.t loop iteration. (Ezio asked for this symbolic estimation in our last meeting) }
%\Ahmad{Yes, Gram-Charlier formula using symbolic moments w.r.t loop iteration $n$. It works for every loop iteration $n$.}
By expressing  $\kappa_1$ and $\kappa_2$ in terms of exact moments,  $\kappa_1=\E(r)$ and $\kappa_2=\E(r^2)-\E^2(r)$, and using~\eqref{eq:Vasicek:R:2Moments}, 
the GC estimate is further expressed as a function of $n$: 
% \begin{align*}
%         f_{\gc}(r(n))=
%         &\frac{\eta\; \exp\left[-\frac{\left(r - \frac{2^n + 9}{5 \cdot  2^n}\right)^2}{\frac{36 \cdot 2^{-n}}{25} 
%         - \frac{2 \cdot (2^n + 9)^2}{2^{2n} \cdot 25} + \frac{478}{2^{2n} \cdot 75} + \frac{14}{75}}\right]}{\beta\; \left(\frac{18 \cdot2^{-n}}{25}
%         - ((1/2^{2n})(2^n + 9)^2)/25 + (239/2^{2n})/75 + 7/75\right)^{1/2}}
%     \end{align*}
%\ezio
{\begin{align*}
        f_{\gc}(r(n))=
        &\frac{\eta\; \exp\left[-\frac{\left(r(n) - \frac{2^n + 9}{5 \cdot  2^n}\right)^2}{\frac{36 \cdot 2^{-n}}{25} 
        - \frac{2 \cdot (2^n + 9)^2}{2^{2n} \cdot 25} + \frac{478}{2^{2n} \cdot 75} + \frac{14}{75}}\right]}{\beta\; \left(\frac{18 \cdot2^{-n}}{25}
        - \frac{2^{-2n}(2^n + 9)^2}{25} + \frac{239 \cdot 2^{-2n}}{75} + \frac{7}{75}\right)^{1/2}}~,
    \end{align*}}
%\efi{we agreed that the numerator should read like the denominator--please fix
% \begin{align*}
%         f_{\gc}(r)=
%         &\frac{\eta\; \exp\left[-{\Big(r - {(2^n + 9)}/{((5)2^n)}\Big)^2}/{\Big(((36/25)2^{-n})
%         - ((2/2^{2n})(2^n + 9)^2)/25 + (478/2^{2n})/75 + 14/75\Big)}\right]}{\beta\; \Big((18/25)2^{-n} 
%         - ((1/2^{2n})(2^n + 9)^2)/25 + (239/2^{2n})/75 + 7/75\Big)^{1/2}}
%     \end{align*}}
   % \Ahmad{Done! Is that ok now? Please check and let me know if this is ok. Thanks. Last version are commented below and above. }
% \begin{align*}
    %     f_{\gc}(r)=
    %     &\frac{\eta\; \exp\left[-\frac{\big(r - {(2^n + 9)}/{((5)2^n)}\big)^2}{((36/25)2^{-n}) 
    %     - ((2/2^{2n})(2^n + 9)^2)/25 + (478/2^{2n})/75 + 14/75}\right]}{\beta\; \Big((18/25)2^{-n} 
    %     - ((1/2^{2n})(2^n + 9)^2)/25 + (239/2^{2n})/75 + 7/75\Big)^{1/2}}
    % \end{align*}
\noindent where $\eta=2251799813685248$ and $\beta=5644425081792261$. 
In particular, for loop iteration $n=100$, the obtained  $f_{\gc}(r)=1.7275\exp[-9.3750(r - 0.2)^2]$  closely approximates the true (sampled) distributed of $r$, as evidenced in Fig.~\ref{fig:vasicek-intro}. 





   % {which further simplifies~\eqref{pdfGC} to 
% \begin{equation}\label{eqn:pdfGCnormal}
%     {f}(x)={\psi}(x) \sum_{m=0}^{\infty}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right),
% \end{equation}
% where $He_m$ are the Hermite polynomials~\cite{brenn2017revisit}.}
%We use Eqn~\eqref{pdfGC} to obtain the GC estimated pdf. 
%In practice, the summation in~\eqref{pdfGC} goes up to the order of the cumulant needed (2 for the Vasicek model). %In.  %to be computed from the corresponding  moments via the cumulants-moments relation \eqref{eq:CumulantMomentRelation}. 
%We implement the method numerically by ``discretizing'' $[a,b]$.   We consider $a=r_0 < r_1 <r_2 <r_3 <\cdots <r_{n}=b$, discrete points on the $x$-axis, and evaluate the Hermite and Bell polynomials and  the normal pdf $\phi(x)$ at these points. 

% \begin{example}
%     \ms{TODO: PDF of the GC-based estimation.} 
% \end{example}



\end{example}

%\begin{example}
%    Applying the ME and GC methods to the first two given moments, we recover the pdf of $r$ as shown in Figure~\ref{fig:vasicek-intro}. The ME estimated pdf  in loop iteration $n=100$ is $f_{ME}(r)= \exp(0.171658 + 3.749999 \,r + 9.374997\, r^2)$. Gram-Charlier estimates the target pdf symbolically in terms of loop iteration $n$ by
%    \begin{align*}
%        f_{GC}(r)=
%        &\frac{\alpha\; \exp\left(-\frac{\left(r - \frac{2^n + 9}{5 \cdot  2^n}\right)^2}{\frac{36 \cdot 2^{-n}}{25} 
%        - \frac{2 \cdot (2^n + 9)^2}{2^{2n} \cdot 25} + %\frac{478}{2^{2n} \cdot 75} + \frac{14}{75}}\right)}{\beta\; %\left(\frac{18 \cdot2^{-n}}{25}
%        - ((1/2^{2n})(2^n + 9)^2)/25 + (239/2^{2n})/75 + 7/75\right)^{1/2}}
%    \end{align*}
%    where $\alpha=2251799813685248$ and $\beta=5644425081792261$. 
    % \ms{TODO: If there is a nice/compact way to describe the equations for the pdfs, we can give them here.}\Ahmad{Done!}
%\end{example}

% \begin{align*}
%         f_{GC}(r)&=\\
%         &\frac{\Big(\alpha\; exp\big(-\frac{(r - {(2^n + 9)}/{(5*2^n)})^2}{(36/(25*2^n) 
%         - (2/2^{2n}*(2^n + 9)^2)/25 + (478/2^{2n})/75 + 14/75)}\big)\Big)}{\Big(\beta\; (18/(25*2^n) 
%         - (1/2^{2n}*(2^n + 9)^2)/25 + (239/2^{2n})/75 + 7/75)^{1/2}\Big)}
%     \end{align*}

% \begin{figure}[tpbh]
% 	\centering
% 	\includegraphics[width=5.4cm]{Figures/pdfVasicekME.eps}
% 	\caption{
%     \ms{TODO: update the figure to show distributions estimated using ME and GC methods, together with samples/histogram. alternatively, refer to the figure in intro, which will have the estimated distributions. } \Ahmad{I updated the figure in intro and I refer to that figure}}
% 	\label{fig:Vasicek-ME-GC}
% 	% maybe also show the moments(100)
% \end{figure}



% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=6cm]{Figures/SampledxVasicekModeln1000loop100sigma02.eps}
% 	\caption{$x$-axis: iteration, $y$-axis: sampled values of the random variable. In red is the Polar generated $E(x)$, and in blue are the sampled values of the random variable in \textit{Vasicek Model}.}
% 	\label{fig:SampledEXforRandomWalk1Sample1000loop1}
% \end{figure}


% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=6cm]{Figures/SampledExVasicekModeln1000loop100sigma02.eps}
% 	\includegraphics[width=6cm]{Figures/SampledEx2VasicekModeln1000loop100sigma02.eps}
% 	\caption{ $E(x)$ and $E(x^2)$ for Vasicek Model using 1000 sample for each iteration of loop.}
% 	\label{fig:SampledEXforRandomWalk1000Sample1000loop1}
% \end{figure}

% Figure~\ref{fig:SampledEXforRandomWalk1Sample1000loop1} shows the agreement of sampled data and exact expected value of random variable $x$ per each loop iteration. One easily can see that the uncertainty propagates through probabilistic loop and remains around the exact expected value of the variable $x$. Figure~\ref{fig:SampledEXforRandomWalk1000Sample1000loop1} shows that the mean value and the second moment for a sample of size 1000 agrees the exact expected values for each loop iteration $n$. This shows the strength  of the moment-based invariant generator in which on can calculate moments of random variables of a PP without running the program.  
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=10cm,height=6cm]{Figures/abserrorvasicekmodeln100sigma02.eps}\\
% 	\includegraphics[width=10cm,height=6cm]{Figures/relerrorvasicekmodeln100sigma02.eps}
% 	\caption{ Absolute and relative errors $E(x)$ and $E(x^2)$ for Vasicek Model: \\
% 	Absolute Error of $\E(x)= |{\E(x)}_{sample}-{\E(x)}_{exact}|$\\
% 	Absolute Error of $\E(x^2)= |{\E(x^2)}_{sample}-{\E(x^2)}_{exact}|$\\
%     Relative Error=$\frac{\text{Absolute Error}}{\text{Exact Value}}$}
% 	\label{fig:AbsoluteandRelativeErrorsRandomWalk1D}
% \end{figure}


  


% In order to assess accuracy of distribution estimation, we carry out a Monte-Carlo ``experiment'' by executing  the PP a \textit{large} number of times (here, large=1000), and  compare the agreement of \textcolor{blue}{the sampled data} with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test. Results (see Figure~\ref{fig:histogram-pdf-cdf-VasicekModel}) show visually the agreement of the estimated pdf with the sampled data (indeed, with the KS density approximation of the sampled data). Details and numerical result of the accuracy evaluation will be presented in Section~\ref{section:Evaluation}.

% \efi{What about multivariate distribution approximation? That is, in a Prob PP, multiple random variables can be generated that are dependent so they have a joint distribution. I believe ME applies also in multivariate distribution estimation.}
% \Ahmad{We can not do it in such short time before deadline.}

% \bigskip

% {\bf Vasicek Model in Finance:}
% This is a mathematical model describing the evolution of interest rates. 
% %It is a type of one-factor short-rate model as it describes interest rate movements as driven by only one source of market risk.
% The Vasicek model is described by the  stochastic differential equation, 
% \begin{align}
%  dr_{t}=a(b-r_{t})\,dt+\sigma \,dW_{t}   
% \end{align}
% where $W_t$ is a Wiener process under  modeling the continuous inflow of randomness into the system. $\sigma$ is the standard deviation factor which shows the amplitude of the instantaneous randomness inflow. $b$ is the long term mean level which paths  will evolve around it in a long term. $a$ is the speed of reversion specifying  the velocity at which such trajectories will regroup around $b$ in time.

% % \bigskip
% % %\bigskip
% 
% The Vasicek model of interest rate can be represented as a prob-solvable  probabilistic program as follows:
% \begin{align}
% &a:=0.5\\\notag
% &b:=0.2\\\notag
% &\sigma:=0.2\\\notag
% &w:=0\\\notag
% %&dt:=1\\\notag
% &r:=2\\\notag
% &\text{while true:}\\\notag
% &\quad w:=\text{Normal}(0,1)\\\notag
% &\quad r:=(1-a)r + a\ast b + \sigma\ast w
% \end{align}

% \bigskip

% Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~\ref{table:ExactmomentsofVasicelModel}.


% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/histogramvasicekmodeln100sigma02.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfvasicekmodeln100sigma02.eps}
% %	\includegraphics[width=3.8cm]{Figures/cdfvasicekmodeln100sigma02.eps}
% 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% 	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Vasicek Model.}
% 	\label{fig:histogram-pdf-cdf-VasicekModel}
% \end{figure}

 

\subsection{Assessing Accuracy of Estimated Distributions}\label{ssec:methods-of-evaluation}

To evaluate the accuracy of the estimated pdfs $f_{\me}$ and $f_{\gc}$ of the PP variable~$x$, we would, ideally, compare them to the true underlying pdf of~$x$. This comparison, however, is not possible in general, as the true distribution of $x$ arising from an (unbounded) probabilistic loop is complex and unknown. To overcome this obstacle, we 
execute the  probabilistic loop $e$ times to  
sample the distribution of~$x$ and use the such collected $Sample_{Data}$ as proxy of the underlying probability distribution of $x$ (line~2 of Algorithm~\ref{fig:algo}). For this, we carry out a Monte-Carlo ``experiment''~\cite{Hastings1970},  by executing $\mathcal{P}$ a large number of times ($e$) and collect the value of $x$ at loop iteration $n$ in $Sample_{Data}$\footnote{in our experiments, we use $e=1000$ and $n=100$, see Section~\ref{section:ImplEvaluation}}. %We call the resulting sample \textcolor{blue}{\textit{sampled data}}.
% we use $1000$ samples by running the programs for $100$ iterations. (or \Ahmad{we carry out a Monte-Carlo “experiment” by executing the PP (stopping at the fixed loop iteration (here, $n=100$)) a large number of times (here, large=1000), which is called  \textcolor{blue}{\textit{sampled data}}}). 
%
Based on $Sample_{Data}$, we  evaluate the accuracy of our ME and GC expansion estimations using {two} statistical tests, namely the 
chi-square ($\chi^2$)~\cite{ross2020introduction} and the Kolmogorov-Smirnov~\cite{massey1951kolmogorov} goodness-of-fit tests, as described next. 
%we use the chi-square ($\chi^2$)
%goodness-of-fit~\cite{ross2020introduction} and the  Kolmogorov-Smirnov tests~\cite{massey1951kolmogorov}.


%\lk{do we really need four, and not only two methods. Why do we need KL and/or precision of higher moments? If we drop, Alg1 should be updated and line references revised in text} 
% \Ahmad{We evaluate our estimation using different tools to show that our distributions are close to the true target (sample) distribution or data generated by the PP follow the estimated distribution. With this estimated distributions, then we calculate higher moments to see and be sure that our estimated distribution generate very accurate higher moments (in few seconds) instead of maybe over ~30 minute for exact moments. We can also report higher moments computed by estimated pdfs as output of Alg 1. 
% If we drop something, I believe all paper line by line should be revised again.}

%  To evaluate the accuracy of an approximation we use statistical tools that  measure the distance of the target distribution and the estimates. 
%In order to evaluate the accuracy of estimation, as there is no pdf and nor cdf of the target distribution available for the underlying random variable of a probabilistic program, we assess it via sampling strategy. We carry out a Monte-Carlo “experiment” by executing the PP (and stopping at the fixed loop iteration (here, $n=100$)) a large number of times (here, large=1000), and compare the agreement of the \textcolor{blue}{sampled data} with the estimated distribution via statistical tools (as explained below). 

% \begin{remark}
% In our evaluations, as there is no true target pdf available to compare with, we need to have a pdf approximated by the sampled data (we call it, here,  \textit{sampled distribution}). To this end, we use kernel smoothing density approximation  of the sampled data which is calculated by the  predefined Matlab function \textit{ksdensity}\footnote{\url{https://de.mathworks.com/help/stats/ksdensity.html}} with the  default bandwidth that is the optimal for normal densities. This approximation is based on normal kernel function. 
% \end{remark}

%\efi{I think the Kullblack-Leibler adds nothing of essence and we should drop it} \Ahmad{done!}

% \Ahmad{We evaluate our estimation using different tools to show that our distributions are close to the true target (sample) distribution or data generated by the PP follow the estimated distribution. With this estimated distributions, then we calculate higher moments to see and be sure that our estimated distribution generate very accurate higher moments (in few seconds) instead of maybe over ~30 minute for exact moments. We can also report higher moments computed by estimated pdfs as output of Alg 1. 
% If we drop something, I believe all paper line by line should be revised again.}


% \paragraph{{\bf Kullback-Leibler (KL) Divergence.}} The
% Kullback-Leibler (KL) divergence is a  distance measure between two distributions \cite{Kullback1959}, and can be used to assess closeness, with smaller values indicating closer match. We use   KL divergence to compare $f_{\me}$ and $f_{\gc}$ to the true distribution of $x$ (line~5 of Algorithm~\ref{fig:algo}), as follows. 
% Since the true underlying distribution of a probabilistic loop variable $x$ is, in general, unknown, we use the sampled distribution of $x$ based on $Sample_{Data}$  as its ``true'' distribution. We next compute the kernel density estimate~\cite{Silverman1998} of the pdf $f_{Sample}$ of $Sample_{Data}$.% in Matlab with the function \texttt{ksdensity}\footnote{\url{https://mathworks.com/help/stats/ksdensity.html}} and the default bandwidth that is optimal for normal densities.
% The KL divergence~\cite{KullbackLeibler1951,hershey2007approximating} between $f_{Sample}$ and $f_{\me}$ is
% \begin{equation}\label{eq:KL:ME}
% D_{KL}(f_{Sample}||f_{\me}) = \int f_{Sample}(x)\log (f_{Sample}(x)/f_{\me}(x))dx.
% \end{equation}
% Similarly, the KL divergence between $f_{Sample}$ and $f_{\gc}$ is  
% \begin{equation}\label{eq:KL:GC}
% D_{KL}(f_{Sample}||f_{\gc}) = \int f_{Sample}(x)\log (f_{Sample}(x)/f_{\gc}(x))dx.
% \end{equation}


% \begin{example}\label{example:VasicekModel-KL}
% For the PP corresponding to the Vasicek model of Fig.~\ref{fig:vasicek-intro}, the  KL divergences  
% between  $f_{Sample}$ and $f_{\me}$, as well as between $f_{Sample}$ and $f_{\me}$, are both $0.0026851753$. Both values are very small, pointing to little difference between the  estimated and true distributions of $r$~\cite{KullbackLeibler1951,hershey2007approximating}. 
% However, from the KL divergence alone, we cannot conclude whether $f_{\me}$ and/or $f_{\gc}$ match the underlying distribution ``sufficiently close." We can only assert that $f_{\me}$ or $f_{\gc}$ are almost equally good. 
% \end{example}

% % As shown in Example~\ref{example:VasicekModel-KL},  KL divergence does not provide information on how truly close, or apart,   two distributions are. 
%To address this drawback and to assess the quality of each distribution estimation separately, we use the chi-square ($\chi^2$)
%goodness-of-fit~\cite{ross2020introduction} and the  Kolmogorov-Smirnov tests~\cite{massey1951kolmogorov}.  %\efi{REFS???}


% The  Kullback-Leibler, or simply, KL
% divergence is also called relative minimum entropy and is an information measure \cite{KullbackLeibler1951,Kullback1959} that has ME as a special case. It is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% Assuming that $p(x)$ is the true (target) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% \begin{align}\label{Kullback-LeiblerDivergence}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative and $D_{KL}(P||Q)=0$ if and only if $P = Q$. As there is no pdf and nor cdf of the target distribution available, we assume that sampled distribution (indeed, kernel smoothing density approximation of sampled data) is the true (target) distribution that we would like to compare our estimated distributions with. 

% We use the predefined Matlab function \textit{ksdensity} with the default bandwidth that is the optimal for normal densities, to obtain distributions out of the sampled data.
% Tables~\ref{table:Kullback-LeiblerDivergence11} and \ref{table:Kullback-LeiblerDivergence1} shows the distances of given and  estimated functions in Example 1 and 2 using ME and GC methods, respectively. 
 
% Despite  $D_{KL}$  yields easily the distance between distributions, we can not say distances are small enough and decide that our estimations are accurate. Only in the case that we would like to compare several methods of estimations, we apply the Kulback-Leibler divergence to see which method outperform the others. To solve this issue, we apply statistical tests  chi-Square Goodness-of-Fit  and  Kolmogorov-Smirnov Goodness-of-Fit tests to see whether the sampled data follows our estimated distribution or not. These tests provide us with some statistics  for the decision-making.

% To solve this issue in our study where we are not given with the target distributions, 
% we go through sampling the random variable of interest and investigate (using statistical tools) to see whether the sampled data follows our estimated distribution or not. 
% % %%%%%%%%%%%%%%%%%%%%%%%%%

% %  To this end, we apply two statistical tests, chi-Square Goodness-of-Fit  and  Kolmogorov-Smirnov Goodness-of-Fit tests which make some statistics available for the decision-making.

% To evaluate the accuracy of an approximation we use  two statistical tests, chi-Square Goodness-of-Fit  and  Kolmogorov-Smirnov Goodness-of-Fit tests which provide us with some statistics  for the decision-making.


\paragraph{{\bf Chi-square ($\chi^2$) Goodness-of-Fit Test.}} The chi-square ($\chi^2$) goodness-of-fit test is a common statistical test to detect statistically significant differences between expected and observed frequencies~\cite{Snedecor98},  
%\footnote{\url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda35f.htm}}. 
by testing if a sample comes from a specific distribution.   We use  the $\chi^2$ goodness-of-fit test to compare $f_{\me}$ and $f_{\gc}$ with the ``true'' (sampled) empirical distribution of $x$ that is based on the sampled data, $Sample_{Data}$ (lines~5--7 of Algorithm~\ref{fig:algo}). 

We partition our $Sample_{Data}$  into~$k\in\mathbb{N}$ non-overlapping intervals $I_k$ (also called  bins), such that $Sample_{Data}=\bigcup_{i=1}^k I_i$.
%partitioning their range. 
Let 
$O_i=|I_i|$ denote the number of samples in the $i$th interval $I_i$, with  $i\in\{1,\ldots,k\}$, and let $l_i$
 and $u_i$ respectively denote the lower and upper bounds of $I_i$. As such,  $O_i$ is the \textit{observed} data frequency of $x$ for interval $I_i$.    %We compute the expected frequencies from the estimated distribution, using either the ME or GC method. 
We compute the expected frequencies\footnote{alternatively, these frequencies can also be obtained from the 
cumulative distribution function (cdf) of $x$
} in $I_i$, denoted as $E_{\me,i}$ and $E_{\gc,i}$,  from  $f_{\me}$ and $f_{\gc}$  as 
\begin{equation}\label{eq:ChiSquare:EFreqs}
\begin{array}{l}
E_{\me,i}=|Sample_{Data}|*\int_{l_i}^{u_i} f_{\me}(x) dx, \\[.5em]
E_{\gc,i}=|Sample_{Data}|*\int_{l_i}^{u_i} f_{\gc}(x) dx.
\end{array}
\end{equation}
%\lk{do we need $\E_{ME,i}(x)$ or just $\E_{ME,i}$}?\Ahmad{just $\E_{ME,i}$ is fine}
%where $N=|Sample_{Data|}$. 
%Alternatively, the frequencies $\E_{ME,i}$ and $\E_{GC,i}$ can also be 
%(or from the cdf $F$ as $N(F(u_i) - F(l_i))$), where $u_i$, $l_i$ are the upper and lower bounds of the $i$th interval and $N$ is the number of samples. \lk{check, it should be $O_i$ as number of samples, or do you refer by $N=|Sample_Data|$}\Ahmad{$N$ is the size of sampled data. i.e. $N=|sampled Data|$ and it is correct. }
%Based on the expected frequencies  $\E_{ME,i}$ and  $\E_{GC,i}$ we derive our 
The resulting chi-square goodness-of-fit test statistics are
\begin{equation}\label{eq:ChiSquare:Tests}
\begin{array}{ll}
    \chi_{\me}^2=\sum_{i=1}^k (O_i-E_{\me,i})^2/E_{\me,i},\\[.5em]
        \chi_{\gc}^2=\sum_{i=1}^k (O_i-E_{\gc,i})^2/E_{\gc,i}.\\[.5em]
\end{array}
\end{equation}
If these values exceed the chi-square critical value $CV_{\chi^2}=\chi^2_{1-\alpha,k-1}$, where $\alpha$ is the statistical significance level (parameter) and $k-1$ the degrees of freedom, the hypothesis that the ME or GC estimated distributions, respectively, are the same as the ``true'' distribution of $Sample_{Data}$ is rejected (lines~10--11 of Algorithm~\ref{fig:algo}). %assess the distributional accuracies of $f_{ME}$ and $f_{GC}$, by comparing them  Here, we only detail the setting for $f_{ME}$, the analysis of $f_{GC}$ is carried out similarly.   
Otherwise, there is not enough evidence to support the claim that the distributions differ significantly. 

%If $\chi_{ME}^2 > CV_{\chi^2}$, then we reject the {\it test  hypothesis} that the true/sampled distribution $f_{Sample}$ of $x$ and its  ME pdf approximation $f_{ME}$ are close enough; that is, in this case we conclude that our $f_{ME}$ distribution does not provide a good pdf estimate for the pdf of $x$. 
%Otherwise, we conclude that our $f_{ME}$ distribution yields an accurate distribution estimation for  the pdf of $x$, accepting thus  the aforementioned test hypothesis (lines~13--14 of Algorithm~\ref{fig:algo}). 


%
%We reject the null hypothesis that the ``true'' distribution $f_{Sample}$ of $Sample_{Data}$ and the ME/GC estimates are the same, if
%$\chi^2 > \chi^2_{1-\alpha,k-1}$,
%where $\chi^2_{1-\alpha,k-1}$ is the chi-square critical value with $k-1$ degrees of freedom and significance level~$\alpha$.

%\lk{this is implementation-specific, to be moved to Section4:  
%We use $k=15$ and $\alpha=0.05$, which gives $\chi^2_{1-\alpha,k-1} = \chi^2_{0.95,14}= 23.685$\footnote{Based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}}.
%}\Ahmad{for the next example (Example3) we need this information because %$\chi^2_{0.95,14}= 23.685$ depends on $\alpha$ and $k$. }

%Failing to reject the null hypothesis that the sampled data follow the estimated distribution, we conclude that the estimate does not statistically significantly  differ from the true underlying distribution of the program variable.


\begin{example}\label{example:VasicekModel-Chi2}
We set $k=15$ and $\alpha=0.05$, so that $CV_{\chi^2}=\chi^2_{1-\alpha,k-1}=23.685$.    Figure~\ref{fig:vasicek-histogram-ME-GC-bins}  shows observed  frequencies from $Sample_{Data}$, as well as the expected frequencies from the $f_{\me}$ and $f_{\gc}$ pdfs of Example~\ref{exactmomentsVasicek}, where $Sample_{Data}$ are collected while sampling the PP of Fig.~\ref{fig:vasicek-intro} for $e=1000$ times at the $n=100$th loop iteration.  The test statistic values of \eqref{eq:ChiSquare:Tests} are $\chi_{\me}^2=17.4018$ and $\chi_{\gc}^2=17.4017$. Since both are smaller than $CV_{\chi^2}$, we conclude that both $f_{\me}$ and $f_{\gc}$ are accurate estimates of the pdf of $r$. This result is also supported by  the close agreement of the plotted frequencies in  Fig.~\ref{fig:vasicek-histogram-ME-GC-bins}. 
    %In both cases, the test statistic is not greater than the critical value $23.685$ (for $k=15$ and $\alpha=0.05$,  $\chi^2_{1-\alpha,k-1} = \chi^2_{0.95,14}= 23.685$).
    
    
    %, thus the samples follow the estimated distributions \mm{MM: I would reduce the strength of the last sentence. You don't know if they follow the estimated distribution, it is just statistically significant.}. 
   % We conclude, that the estimated distributions are both good approximations for the underlying (true) distribution of variable $r$ of the Vasicek model and that the data generated by the Vasicek PP  follow the estimated distribution.
    
    %The test statistic for our sampled data and our estimated distribution using maximum entropy method is $\chi_{ME}^2=17.4018$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$, we can not reject the null hypothesis which means the sampled data obtained through running the prob-solvable program of Figure~\ref{fig:vasicek-intro} follow the  distribution estimated using 3 first moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 
    %For Gram-Charlier estimated distribution, the test statistic $\chi_{GC}^2=17.4017$ which is, again, not greater than the upper-tail critical value. 
    
\begin{figure}[t!]
	\centering
	%\includegraphics[width=6cm]{Figures/ChiSquareHistogramEiOi.eps}
	\includegraphics[width=8cm]{Figures/OiEiforVasicekModelUpdated.eps}
	\vspace{-5mm}
	\caption{Observed frequencies (blue) of the $Sample_{Data}$ of Figure~\ref{fig:vasicek-intro}, in alignment with the expected frequencies obtained from the $f_{\me}$ (orange) and $f_{\gc}$ (yellow) estimated distributions of the PP of Figure~\ref{fig:vasicek-intro}.}
	\label{fig:vasicek-histogram-ME-GC-bins}
\end{figure}

%\lk{please update the figure so it displays $\E_{ME,i}$ and $\E_{GC,i}$ instead of $E_i(ME)$ and $E_i(GC)$. Also, better list in this order $O_i$, $\E_{ME,i}$  $\E_{GC,i}$. Also, what is "count" in the Figure? We sample for e=1000 times, right? Finally, instead of "Number of bins" please write "$k$ number of bins"} 
% \Ahmad{Done! The figure has been updated. Count in the figure means that how many of samples. }
% \lk{if "count" is samples in the Figure, we should write "Samples" or "Sample Data". But then we should have the count/sample axis up to value 1000, as we say we use 1000 samples}\Ahmad{we have 1000 samples that are divided into 15 bins, the height of each bin shows the number of samples (how many of these 1000) is in that bin.}
\end{example}


%In order to evaluate the accuracy of estimation, as there is no pdf and nor cdf of the target distribution available, we assess it via sampling strategy. We carry out a Monte-Carlo “experiment” by executing the PP (and stopping at the fixed loop iteration (here, $n=100$)) a large number of times (here, large=1000), and compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test. Results (see Figure 7) show visually the agreement of the estimated pdf with the sampled data (indeed, with the KS density approximation of the sampled data). Numerical result of the accuracy evaluation will be presented in Section 5.

%Running the program and stopping at the fixed loop iteration (here, $n=100$), we apply the chi-square goodness-of-fit test to see if  the sampled data come from a population with \efi{this makes no sense: you compare the estimated distribution moments with the exact moments from polar! Scrap the hypotheses below}

%\bigskip

%\hspace{10mm} $\text{H}_0$:	The data follow the estimated distribution.

%\hspace{10mm} $\text{H}_a$:	The data do not follow the estimated distribution.

%\bigskip	

%For the chi-square goodness-of-fit computation, we divide the data  into $k$ bins and define the test statistic as

%where $O_i$ is the observed frequency for bin $i$ and $E_i$ is the expected frequency (with respect to the estimated distribution) for bin $i$. The expected frequency is calculated by
%$$
%E_i=N(F(Y_u)-F(Y_l)),
%$$
%where $F$ is the estimated cumulative distribution function with maximum entropy, $Y_u$ is the upper limit for bin $i$, $Y_l$ is the lower limit for class $i$, and $N$ is the sample size.





\paragraph{{\bf Kolmogorov-Smirnov (K-S) Test.}} The Kolmogorov-Smirnov (K-S) test~\cite{massey1951kolmogorov} is a goodness-of-fit test using  cumulative distribution functions (cdfs) to test whether two  distributions differ.   
%\lk{the notation is inconsistent!}
We compute the cdfs $F_{me}$ and $F_{\gc}$ of the estimated pdfs $f_{\me}$ and $f_{\gc}$, respectively. We also compute the (empirical) cdf~$F_{Sample}$ of $Sample_{Data}$. 
%To compare $F_{\me}$ and $g_{\gc}$ with $F_{Sample}$, 
%respectively compare the cdf $g_{ME}(x)$ and  of the distribution estimated using ME, or GC, respectively, to the \textit{empirical} cdf $F(X)$ computed from the sampled data, with $F(x)$ being the proportion of samples less than or equal to~$x$.
We let 
\begin{equation}\label{eq:KSTest}
    \begin{array}{l}
    D^\ast_{\me}=\max_x(|F_{\me}(x)-F_{Sample}(x)|),\\[.5em]
    D^\ast_{\gc}=\max_x(|F_{\gc}(x)-F_{Sample}(x)|)
\end{array}
\end{equation}
to denote the K-S test statistics $D^\ast_{\me}$ and  $D^\ast_{\gc}$, respectively.
To assess the distance of $F_{\me}$ and $F_{\gc}$ from $F_{Sample}(x)$ with K-S, 
we compare $D^\ast_{\me}$ and $D^\ast_{\gc}$ to the K-S test critical value  $CV_{\text{K-S}}=\sqrt{-({1}/{|Sample_{Data}|})\ln{({\alpha}/{2})}}$, where $\alpha$ is the statistical significance level. The K-S test rejects the claim that the compared distributions are the same if $D^\ast_{\cdot} < CV_{K-S}$ (lines~10--11 of Algorithm~\ref{fig:algo}). 


%\footnote{Based on statistical tables, see e.g. \cite{rohatgi2015introduction}}. 
%We reject the null hypothesis that the sampled data  follow the estimated distribution, if $D^\ast$ exceeds the critical value. 
%As in the case of the chi-squared test, we only test against estimated distributions. 
%If we cannot reject the null hypothesis, the estimated pdf is not statistically significantly different from  the true underlying distribution.

\begin{example}\label{example:VasicekModel-K-S}
We set $\alpha=0.05$, so that $CV_{\text{K-S}}=0.0608$.   We compute the \mbox{K-S} test statistics for the  ME and GC estimated distributions
 of Example~\ref{exactmomentsVasicek}, to obtain
$D^{\ast}_{\me} = 0.03602307$ and $D^{\ast}_{\gc} = 0.03602304$. Since both test statistics are smaller than the critical value, we conclude that both  $f_{\me}$ and $f_{\gc}$ are close to the underlying distribution of $r$. 
 
%
  %  \footnote{Our approach is based on the two-sample Kolmogorov-Smirnov test  if we assume $G(x)$ is the empirical cdf of a sample (of size M) generated by the ME/GC estimated distribution. In this test, the critical value is defined by  $CV$=$c(\alpha)\sqrt{({M+N})/{MN}}$ where $c(\alpha)$=$\sqrt{-({1}/{2})\ln{({\alpha}/{2})}}$ \cite{hodges1958significance}. Here, the sample sizes are the same, $M$=$N$=1000; i.e., the size of  sampled data generated by executing the PP.}
%
\end{example}



% \begin{table}[tpbh!]
%     \centering
%   \scalebox{0.9}{
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & $D^\ast$ (ME) & $D^\ast$ (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline
%     \hspace{2mm} Vasicek \hspace{2mm}&\hspace{2mm} 0.0027 \hspace{2mm} & \hspace{2mm} 0.002685\hspace{2mm} & \hspace{2mm}0.03602307  \hspace{2mm} & 0.03602301& \hspace{2mm} 17.4018 \hspace{2mm}& \hspace{2mm} 17.4017 \hspace{2mm}\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence of ME estimated distribution and sampled one), $D^\ast$ statistics (Kolmogorov–Smirnov test), $\chi^2$ statistics (Chi-Square test) for the Vasicek  probabilistic programs.}
%  \label{table:VasicekTable}
% \end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[tpbh!]
%     \centering
%   \scalebox{0.9}{
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & p-value (ME) & p-value (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline
%     \hspace{2mm} Vasicek \hspace{2mm}&\hspace{2mm} 0.0027 \hspace{2mm} & \hspace{2mm} 0.002685\hspace{2mm} & \hspace{2mm}0.15  \hspace{2mm} & 0.1456& \hspace{2mm} 17.4018 \hspace{2mm}& \hspace{2mm} 17.4017 \hspace{2mm}\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence of ME estimated distribution and sampled one), p-value (Kolmogorov–Smirnov), $\chi^2$ statistics for the Vasicek  probabilistic programs.}
%  \label{table:VasicekTable}
      
% \end{table}




% \paragraph{Precision of Higher Moments.} 
% For the last method of evaluation, we compute higher moments of estimated distributions, that is moments that have not been used for the estimation, and compare them to the exact moments. We compute both the absolute error, the difference between the estimated and exact moments, as well as the relative error, the ratio of estimated and exact moments. We also compute absolute and relative error of the higher moments from samples. 


% \lk{I do not think  paragraph on ``Precision of Higher Moments" is  needed in section 3, actually not at all. For now, it is moved to the end of the paper.}

==> Distribution Recovery (27)/preliminaries.tex <==
%!TEX root = samplepaper.tex

\section{Preliminaries}\label{section:Preliminaries}
This section reviews relevant terminology from statistics and probabilistic programs; for further details we refer to~\cite{durrett2019probability,Moosbruggeretal2022}. %\lk{check whether Silverman1998 is the best relevant works; please do not use here the book of Ross2020} ~\cite{durrett2019probability,Moosbruggeretal2022} \Ahmad{I added Durret 2019 as a reference for definitions from statistics, however, for other parts like maximum entropy and Gram Charlier  we have provided references in corresponding sections. }.
Throughout the paper, $\mathbb{N}$ denotes the set of natural numbers. To facilitate readability,  we sometimes write $\exp[t]$ to denote the exponential function $e^{t}$, where $t$ is an arbitrary expression/argument. 


\subsection{PPs and Moments of Random Variables}%Probability Theory and PPs}
{ The result of a PP is not a single output but rather multiple values  with different probabilities according to the distribution of the random variables the PP encodes. }
Different execution paths in a
PP are typically selected by draws from commonly used distributions that are fully characterized by their moments, such as the uniform or  normal. 
%whose
%properties and features have been extensively studied in probability and statistics. 
Yet, since  output values of PPs
are  results of multiple operations,  distributions arising from the random variables the PPs encode are most often not common.
%Most developments in the analysis of PPs focus on the derivation of the first moment of the outcome values,
%[3, 16, 20, 33], 
%which provides a limited account of the distribution of the random variables arising from a
%PP. 
%Bouissou et al. (2016) \cite{bouissou2016uncertainty} considered the problem of answering queries on probabilities of assertions over program variables and
%their moments; that is, of assessing the likelihood of program variables and their moments producing outputs in a
%specified range. Their approach consists of approximating program random variables with affine forms under the
%assumption that they have bounded support and all their moments are finite.

%The study of distributions  is a much explored topic in statistics. Many distributions are fully characterized by their moments and most well  known distributions fall in this category. For example, the normal, the Poisson, the uniform, etc. 
% In particular, if
% a random variable has bounded support, then the sequence of all its moments uniquely
% determines its distribution \cite{billingsley2013convergence}. Nevertheless, knowledge of all
% the moments of a random variable does not necessarily uniquely characterize its distribution.

% \begin{definition}[Moments]

% \end{definition}

% %\begin{definition}[Cumulants]

% %\end{definition}

% \begin{definition}[MGF]\cite{casella2021statistical}\label{momentgeneratingfunction}
% Let $X$ be a random variable with cdf $F_X$. The moment generating function (mgf)
%  of $X$, denoted by $M_X(t)$, is 
%  \begin{align}
%      M_X(t)=\E(e^{tX}),
%  \end{align}
% provided that the expectation exists for $t$ in some neighborhood of $0$. That is, there is an $h>0$ such that, for all $t\in(-h,h)$, $\E(e^{tX})$ exists. If the expectation does not exists in a neighborhood of $0$, we say that moment generating function does not exist.  
% \end{definition}

% If the moment generating function exists, it characterizes all moments, but characterizing the set of moments is not enough to determine a distribution uniquely as  two distinct random variables can have the same moments (see e.g.  Example~2.3.10 in \cite{casella2021statistical}). If the random variable has bounded compact support, then the infinite sequence of moments  uniquely determines its distribution (\cite{billingsley1995probability} Section~30). More generally, if the moment generating function exists in a neighborhood of $0$, then the distribution is uniquely determined. Existence of all moments is not equivalent to existence of the moment generating function. 

%\paragraph{Probabilistic programs (PPs).} Probabilistic programs are becoming widely-used tools for modeling systems with stochastic elements. Studying the properties of such systems requires knowledge of underlying distributions, i.e. the distributions of the random variables generated through the execution of the program. 


\paragraph{\bf Moments of Probabilistic Loops.}

%The recent advances in the analysis of PPs allow us to automatically compute moments of program variables in a large class of Probabilistic loops, even symbolically.

Moments of program variables of probabilistic loops can be approximated by sampling; that is, by executing the loops for an arbitrary but fixed number of iterations (see, e.g.~\cite{Hastings1970,younes2006statistical}).
Alternatively, 
for restricted classes of probabilistic loops with polynomial updates, symbolic methods from algorithmic combinatorics can be used to compute  the exact 
(higher-order) moments of random program variables $x$ by expressing these moments as closed-form expressions over loop iterations and some initial values~\cite{bartocci2019automatic,Moosbruggeretal2022}. 
That is, ~\cite{bartocci2019automatic,Moosbruggeretal2022} derive the expected value 
of the $k$th moment of variable $x$ at loop iteration $n$, denoted as $\mathbb{E}(x^k(n))$, %$\mathbb{E}(\cdot)$,
in closed form, where $x^k(n)$ specifies the value of $x^k$ at loop iteration $n$, and $k,n\in\mathbb{N}$. 
%developed automated techniques to compute moments of all orders of a program variable $x$; that is,  $\mathbb{E}(x_n^k)$ in closed-form for arbitrary $k \in \mathbb{N}$, where $n$ denotes the $n$th loop iteration, under certain restrictions on the syntax of the loops. 
%All examples in our work fall in the setting of \cite{Moosbruggeretal2022}, and we apply their methods to compute the exact closed-form of higher moments of program variables.


\iffalse
% (Miroslav and Marcel): We removed this part and replaced it with a short paragraph above. For this work the specifics of Prob-solvable loops are not relevant. The only important fact is that we can get the moments.
{\bf PPs with Prob-solvable loops:} Prob-solvable programs are generalization of $P$-solvable programs  allowing probabilistic 
assignments over random variables and distributions.
%\begin{definition}\cite{bartocci2019automatic}
    Let $m\in\mathbb{N}$ and $x_1,\dots,x_m$ denote real-valued program variables.
Prob-solvable loops  with $x_1,\dots,x_m$ variables are programs of the following form \cite{bartocci2019automatic}:
\begin{align}
    I; \text{ while (true) } \{U\},
\end{align}
where $I$ is a sequence of initial assignments over $x_1,\dots,x_m$ (i.e. $x_1:=c_1,x_2:= c_2,\dots,x_m:=c_m$, with $c_i\in \mathbb{R}$ representing a real number
drawn from a known distribution). $U$ is a sequence of $m$ random updates as the loop body. Each update is of the form:
\begin{align}\label{poly-assgmt}
 x_i := a_ix_i + P_i(x_1,\dots,x_{i-1})\; [p_i] \; b_ix_i + Q_i(x_1,\dots,x_{i-1}),   
\end{align}
where $a_i, b_i\in\mathbb{R}$ are constants and $P_i, Q_i  \in \mathbb{R}[x_1,\dots,x_{i-1}]$ are polynomials
over program variables $x_1,\dots,x_{i-1}$ and  $p_i \in [0, 1]$  is the probability
of updating $x_i$ to $a_ix_i + P_i(x_1,\dots,x_{i-1})$, whereas the probability to update $x_i$ to
$b_ix_i + Q_i(x_1,\dots,x_{i-1})$  is $1-p_i$.
%\end{definition}

Considering a Prob-solvable
program with $n\in \mathbb{N}$ denoting the loop iteration counter, \cite{bartocci2019automatic} show that variable
updates of Prob-solvable programs lead to  special recurrences in $n$, so-called moment-based
recurrences. Assume that the sequences
$x_1(n),\dots,x_m(n)$  describe relations between values of $x_i$ at
 loop iteration $n$. Then Prob-Solvable updates are expressed as 
 \begin{align}
&  x_i(n+1) := a_ix_i(n)\\\notag
& + P_i(x_1(n),\dots,x_{i-1}(n))\; [p_i] \; b_ix_i(n) + Q_i(x_1(n),\dots,x_{i-1}(n)).   
 \end{align}
 
 PPs with Prob-solvable loops: Bartocci et al. (2019) \cite{bartocci2019automatic, bartocci2020mora} calculate all moments of all generated random variables via recurrence
relations when assignments are of a specific form (see \eqref{poly-assgmt}). We focus on random variables generated in Prob-solvable loops. Our aim is to recover their distribution from their moments. 

This can be easily answered when the distributions of the random variables produced by a PP are among the known and
well studied distributions in Statistics.
When distributions are not recognized as known, the task is more difficult and is the focus of this paper.


\mm{This is a bit outdated with Polar. Important is that under some conditions moments can be obtained precisely. And given precise moments we can start reconstructing the distribution. It doesn't really matter where this moments came from (as discussed in our last meeting).}


\fi


\subsection{From Moments to Distributions}\label{section:FromMomentToDistribution}

Given a finite set of moments of a random variable $x$,  its distribution can be estimated using various statistical approaches. We focus on those we use herein.
% why are these methods used? what are their strengths/weaknesses/etc?

\paragraph{\bf Maximum Entropy (ME).}\label{section:MaximumEntropyMethod}
The Maximum Entropy (ME) distribution estimation  method is based on the maximization of constraints describing the Shannon information entropy~\cite{biswas2010function,buchen1996maximum,lebaz2016reconstruction}.  %given information in the form of constraints. 
%----------------
%lk: skipped below, unclear why the info on Shannon entrip would be needed
%Shannon's entropy is a general device for measuring the uncertainty or {entropy} in signals. ME states that one should choose a probability that maximizes the Shannon entropy, since if entropy is thought of as a measure of information, then one should choose the probability that includes the least amount of information; that is, only  the given information. %The probability that maximizes the entropy is the least informative or the most \textit{honest}.
%
Specifically, in order to estimate the unknown distribution $f$ of a PP variable $x$ in our setting, we  maximize the {Shannon entropy $H$ of $f$, defined by} 
\begin{align}\label{ShanonEntropy}
  H[f]=-\int_{l}^{u} f(x) \ln(f(x))dx,  
\end{align}
subject to its given moments $\E(x^i)=\int x^if(x)dx$ \cite{bernardo2009bayesian,Kendall2004}.
%\lk{what is H? We have a mismatch in moments-notation} \Ahmad{I changed all $\mu_i$ to $\E(x^i)$ to have a same notation} 
The ME approximation $f_{\me}(x)$ of the target 
probability density function (pdf) takes the form 
\begin{equation}\label{eq:pdf:ME}
f_{\me}(x)=\exp\left[-\sum_{j=0}^N\xi_jx^j\right],
\end{equation}
% \begin{align}
% f_{ME}(x)=\exp\Big[-\sum_{j=0}^N\xi_jx^j\Big],
% \end{align}
where the Lagrange's multipliers $\xi_j$, with $j=0,1,\dots,m$, % LK: changed $N_{\text{m}}$ to $m$, 
can be obtained from  the first $m\in\mathbb{N}$ %$N_{\text{m}}$  
moments, $\{\E(x),\E(x^2),\dots,\E(x^{m})\}$. To this end, the following system of  $m+1$ % $N_{\text{m}}+1$
nonlinear equations is solved,
\begin{align}\label{eq:nonlinearSystemME}
\bigintss_l^u x^i\exp\left[-\sum_{j=0}^{m}\xi_jx^j\right]dx=\E(x^i).   
\end{align}
%\cite{buchen1996maximum} provides details on the maximum entropy method for distribution recovery. 
% Numerically, iterative methods are used to solve the nonlinear system of equations \cite{mead1984maximum,lebaz2016reconstruction}.  Here, we use a numerical minimization algorithm, called  Levenberg–Marquardt, which was developed  to solve
% nonlinear least squares problems \cite{levenberg1944method, marquardt1963algorithm}. This algorithm is an iterative procedure  (a combination of   gradient descent and
% Gauss-Newton) with an initial choice of the Lagrange's multipliers $\xi_j$ in \eqref{eq:nonlinearSystemME} and
% a given tolerance of $10^{-6}$ for stopping the iterative process. 

% Before we move to distribution recovery in probabilistic programs where we have no information about the target pdf, we present  an  example in which the following bimodal  function on the interval $[0,1]$ are recovered via ME.  
% \begin{align}
%  f_X(x)& =\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}, \label{ex1}
% %  \\
% % g_X(x)&=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}. \label{ex2}
% \end{align}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=6cm]{Figures/reconst6moments.eps}
% 	%	\includegraphics[width=4.2cm]{Figures/MEsecondExample.eps}
% 	\caption{Maximum Entropy Method with 6 moments: Bimodal pdf in \eqref{ex1}. The Kullback-Leibler divergence  of sampled and ME estimated  distributions is $D_{KL}=0.0328 $.% (left).%, Tri-modal pdf in \eqref{ex2}.
% 	}
% 	\label{fig:MaxEntropy6Moments}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figure~\ref{fig:MaxEntropy6Moments} shows reconstructed distribution in blue compared to the true pdf in red as defined in \eqref{ex1} %and \eqref{ex2}, respectively, 
% using the first six moments. 
% \efi{the third mode is hardly observable--you should adjust the parameters. Otherwise I don't see why both examples are needed.}
% \Ahmad{I ignored the second example.}


% \efi{what is this trying to convey? These are values that do not have any reference values to compare with. I suggest the highlighted part and Table \ref{table:Kullback-LeiblerDivergence11} be dropped: We compare the accuracy of the reconstruction using the Kullback–Leibler divergence. The  Kullback-Leibler, or simply, KL
% divergence is also called relative minimum entropy and is an information measure \cite{KullbackLeibler1951,Kullback1959} that has ME as a special case. It is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% Assuming that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% \begin{align}\label{Kullback-LeiblerDivergence}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.
% % The Kullback–Leibler divergence values for the ME estimates of both target and reconstructed distributions  are given in  Table~\ref{table:Kullback-LeiblerDivergence11}. 
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %               & Example 1 & Example 2\\
% %                           \hline
% %      Maximum Entropy & 0.0328 & 0.0139\\\hline
% %     \end{tabular}
% % \vspace{5mm}
% %  \caption{Kullback-Leibler divergence $D_{KL}$ of sampled and ME estimated  distributions.}
% %       \label{table:Kullback-LeiblerDivergence11} 
% %  \end{table}
% }

% We compare the accuracy of the reconstruction using the Kullback–Leibler divergence. The  Kullback-Leibler divergence, or simply, KL
% divergence is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% Assuming that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% \begin{align}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.

% A quantitative comparison of the distributions (target and reconstructed) is also carried out. The Kullback–Leibler divergence values for the ME estimates of both functions are given in  Table~\ref{table:Kullback-LeiblerDivergence11}. 
% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|}
% \hline
%               & Example 1 & Example 2\\
%                           \hline
%      Maximum Entropy & 0.0328 & 0.0139\\\hline
%     \end{tabular}
% \vspace{5mm}
%  \caption{Kullback-Leibler divergence ($D_{KL}$ of sampled and ME estimated  distributions).}
%       \label{table:Kullback-LeiblerDivergence11} 
%  \end{table}
 
% \mm{Would be nice to see this method for a concrete PP here: (1) Get precise moments via Polar. (2) approximate distribution with Maximum Entropy.}
% \ahmad{Done for Random Walk 1D!}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Gram-Charlier Expansion}\label{section:GramCharlierExpansion}
The Gram–Charlier  series   approximates the pdf $f$ of a PP variable $x$ in terms of its cumulants {and using a known distribution $\psi$}~\cite{hald2000early,brenn2017revisit}. We let $\psi$ to be a normal/Gaussian  distribution (see Section~\ref{ssec:reconstructing-distribution}).  As an alternative to moments,  cumulants  of a distribution are defined using the {\it{cumulant-generating function}}, which equals the natural logarithm of the characteristic function, $K(t)=\ln\left(\E(e^{itx})\right)$. In what follows, we denote by $\kappa_m$ the $m$th cumulant of $f$, the unknown target distribution  to be approximated.  The relationship between  moments and cumulants can be obtained by extracting coefficients from the expansion. 
To be precise, we can express the $m$th cumulant $\kappa_m$ in terms of the first $m$ moments~\cite{broca2004cumulant} as 
\begin{equation}\label{eq:CumulantMomentRelation}
\footnotesize{
    \kappa_m=(-1)^{m+1}\det
    \begin{pmatrix}
    \E(x)& 1 & 0 & 0 & 0 & \dots & 0\\
    \E(x^2)& \E(x) & 1 & 0 & 0 & \dots & 0\\
    \E(x^3)& \E(x^2) & \binom{2}{1}\E(x) & 1 & 0 & \dots & 0\\
    \E(x^4)& \E(x^3) & \binom{3}{1}\E(x^2) & \binom{3}{2}\E(x) & 1 & \dots & 0\\
%    \E(x^5)& \E(x^4) & \binom{4}{1}\E(x^3) & \binom{4}{2}\E(x^2) &
%    \binom{4}{3}\E(x) & 1 & \dots & 0\\
    \vdots& \vdots & \vdots & \vdots & \vdots  & \ddots & \vdots\\
    \E(x^{m-1})& \E(x^{m-2}) & \dots & \dots & \dots & \ddots & 1\\
    \E(x^m)& \E(x^{m-1}) & \dots & \dots & \dots & \dots & \binom{m-1}{m-2}\E(x) \\
    \end{pmatrix},
    }
\end{equation}
where $\det(\cdot)$ stands for determinant.
The first cumulant  $\kappa_1$  of the random variable $x$ is the mean $\mu=\E(x)$; the second cumulant $\kappa_2$ of $f$ is the variance $\sigma^2$, and the third cumulant $\kappa_3$ is the same as the third central moment\footnote{The $i$th central moment of $x$ is defined as $\E\left((x-\E(x))^i\right).$}. 
Higher-order cumulants of $f$, however, are in general not equal to higher moments.  
%\todo{ Ahmad: We do not use central moments. As defined in the text  (after Equation \eqref{ShanonEntropy}), we use the  notation $\mu_i$ for the $i$th (not central) moment (i.e. $E(x^i)$). We may change the notation $\mu_i$ to $m_i$ for $i$th (not central) moment?}
%The $m$th cumulant $\kappa_m$ can however be expressed in terms of the first $m$ moments~\cite{broca2004cumulant},  % in  closed form via computing matrix determinant ($\det(\cdot)$) as follows: 
%
% where $\mu_i$ is defined in \eqref{eq:nonlinearSystemME} for all $i >0$ (see, e.g., \cite{broca2004cumulant}).
%
%
% \begin{align}\label{eq:CumulantMomentRelation}
% \footnotesize{
%     \kappa_n=(-1)^{n+1}\det
%     \begin{pmatrix}
%     \mu_1& 1 & 0 & 0 & 0 & 0 & \dots & 0\\
%     \mu_2& \mu_1 & 1 & 0 & 0 & 0 & \dots & 0\\
%     \mu_3& \mu_2 & \binom{2}{1}\mu_1 & 1 & 0 & 0 & \dots & 0\\
%     \mu_4& \mu_3 & \binom{3}{1}\mu_2 & \binom{3}{2}\mu_1 & 1 & 0 & \dots & 0\\
%     \mu_5& \mu_4 & \binom{4}{1}\mu_3 & \binom{4}{2}\mu_2 &
%     \binom{4}{3}\mu_1 & 1 & \dots & 0\\
%     \vdots& \vdots & \vdots & \vdots & \vdots & \ddots & \ddots & \vdots\\
%     \mu_{n-1}& \mu_{n-2} & \dots & \dots & \dots & \dots & \ddots & 1\\
%     \mu_{n}& \mu_{n-1} & \dots & \dots & \dots & \dots & \dots & \binom{n-1}{n-2}\mu_1 \\
%     \end{pmatrix}
%     }
% \end{align}
%
%\ms{(An alternative to the GC derivation, omitting most of the details. The question is, how much details on the derivation do we actualy need/want? I'm afraid it might take too much space to explain it in enough details so that non-mathematicians can follow it easily...)}
%LK: move this to Section 3, this is specific to what we do
%In our work, we let $\psi$ to be the normal distribution with the mean $\mu=\kappa_1$, variance $\sigma^2=\kappa_2$, and pdf  $\psi(x)=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$. 
%
% Let $\mu$,  $\sigma$ and $\psi(x)$ respectively denote the mean,  variance, and the pdf
% %\lk{pdf - is it pdf or characteristic function} \Ahmad{pdf. Here in our paper, we let known distribution to be the normal distribution, only with this assumption we can derive $f_{GC}$ as in \eqref{pdfGC}} 
% of the known distribution $\psi$.
%
%\lk{is the text below depending on normal distribution, or is it for any distribution} \Ahmad{I have updaated the formula, know is independent from normal distribution. Please check this part again. Thanks.} 
%LK: OK, resolved!
%
Using the cumulants $\kappa_m$ computed from exact moments of $x$ together with  the cumulants 
%In the sequel, we let $\gamma_i$ denote  the cumulants 
of the known distribution $\psi$, %with $i\in\mathbb{N}$. % and $\{\kappa_i\}_{i=1}^\infty$ be the cumulants of the target (unknown) distribution $f$. 
%\ms{It's a bit more general for arbitrary $\psi$ - I'm just adding it :),OK :)
%of $f$ and $\psi$, 
%properties of Fourier transform and the Gaussian distribution~$\psi$, and further simplifications, we
the pdf $f$ of a random variable $x$  can approximated by the Gram-Charlier (type-)A 
expansion $f_{\gc}(x)$, as in~\cite{KendallStuart1977} and given by 
\begin{align}\label{pdfGCGeneralC}	
f_{\gc}(x) = 
 {\psi}(x) \sum_{m=0}^{\infty}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right),
%{f}(x)=\sum_{m=0}^{\infty}B_m(0,0,\kappa_3,\dots,\kappa_m)\frac{(-D)^m}{m!}{\psi}(x),
\end{align} 
%\begin{align}\label{pdfGCGeneral}	
%f_{\gc}(x) = 
%\exp\left(\sum_{m=1}^{\infty}(\kappa_m-\gamma_m)\frac{(-D)^m}{m!}\right){\psi}(x),
%\end{align} 
%where $B_m$ are the Bell polynomials
%and $He_m$ are the Hermite polynomials~\cite{brenn2017revisit}\footnote{see Appendix~\ref{Appendix} for the full derivation of~\eqref{pdfGC}}. 
%and 
%where $D$ is the differential operator with respect to $x$.
%The Gram-Charlier A expansion can be stated without the differential operator with the use of Hermite- and Bell-polynomials.
%For the derivation of the Gram-Charlier A expansion and more details, we refer to \cite{brenn2017revisit}.
%\lk{we might not need the reference to the Appendix A at all; check in later revision }
% $${f}(x)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(-D)^m}/{m!}\big]{\psi}(x)$$
%LK:moved back to Sectoon 3.
%\lk{this paragraph should not be here, but section 3}
%\lk{moved  our GC expansion/details back to Section 3}
%\Ahmad{I think, it would be better to have a general (I mean sum to $\infty$) GC formula here (with a reference to Appendix for more detail on derivation) as our estimation formula and in section 3 we explain how we use $|S_\text{M}|$ moments to estimate our target pdf in practice. }
%The Gram-Charlier A expansion can be expressed in terms of Hermite- and Bell-polynomials. 
%We use the normal/Gaussian distribution  as the known distribution $\psi$ in the Gram-Charlier expansion with mean $\mu$ and variance $\sigma^2$. Thus, %~\eqref{pdfGCGeneral}; hence, we have 
%$\kappa_1=\mu$, $\kappa_2=\sigma^2$, and  $\psi(x)=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$. %in~\eqref{pdfGCGeneral}. 
%In addition, the cumulants $\kappa_m$ of the pdf of $x$ are computed from the moments $S_{\text{M}}$. As such, the adjusted Gram-Charlier A expansion $f_{\gc}(x)$ for the pdf of $x$ is
% \begin{align}\label{pdfGC}	f_{\gc}(x) = 
% {\psi}(x) \sum_{m=0}^{\infty}}\frac{1}{m!\sigma^m} B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right),
% \end{align} 
where $\psi$ is the normal pdf  with mean $\mu=\kappa_1$ and variance $\sigma^2=\kappa_2$, and $B_m$ and $He_m$ are respectively the Bell and  Hermite polynomials~\cite{brenn2017revisit}. Derivation details of \eqref{pdfGCGeneralC} can be found in \cite{wallace1958asymptotic}.


\iffalse
To approximate the pdf $f$, we  expand $f$ using its cumulants $\kappa_m$ in terms of a known distribution $\psi$ \todo{In terms of: the estimated distribution will be a composition of some proportion of the $\psi$, for example: $f=(1+ \alpha x + \beta x^2)\psi(x)$, it is not related to the PP}\lk{what is $\psi$, what is ``in terms of", and what is the relation to PP?}\Ahmad{we try to characterize our unknown target distribution f in terms of a known distribution $\psi$ (here in this paper, in the next paragraph,  we specify and  take $\psi$ to be normal distribution, i.e. $\psi:=\phi$)}. We denote the characteristic function of $f$ by $\hat{f}$ and let $\hat{\psi}$ and $\gamma_m$  be the characteristic function and cumulants of the known distribution $\psi$, respectively. \ms{Is this a 'standard' way of writing characteristic function (using cumulants)?} Following \cite{wallace1958asymptotic}, we set $\hat{f}(t)=\exp\big[\sum_{m=1}^{\infty}\kappa_m{(it)^m}/{m!}\big]$  and  $\hat{\psi}(t)=\exp\big[\sum_{m=1}^{\infty}\gamma_m{(it)^m}/{m!}\big]$,
% \begin{align}
% \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}\kappa_r\frac{(it)^r}{r!}\Big] \quad \text{and} \quad \hat{\psi}(t)=\exp\Big[\sum_{r=1}^{\infty}\gamma_r\frac{(it)^r}{r!}\Big],    
% \end{align}
which leads to the identity $\hat{f}(t)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(it)^m}/{m!}\big]\hat{\psi}(t)$.
% \begin{align}
%  \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(it)^r}{r!}\Big]\hat{\psi}(t).    
% \end{align}
The term $(it)^m\hat{\psi}(t)$ is the Fourier transform of  $(-1)^m[D^m(\psi)(-x)]$, where $D$ is the differential operator with respect to $x$. Thus, the expansion of $f$ in terms of the known distribution $\psi$ is ${f}(x)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(-D)^m}/{m!}\big]{\psi}(x)$.
% \begin{align}
%   {f}(x)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\psi}(x).  
% \end{align}

Here, for our work, we assume  $\psi$ to be the normal distribution with the mean $\mu=\kappa_1$, variance $\sigma^2=\kappa_2$, and pdf  $\psi(x)=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$. \lk{if $\psi(x)=\phi(x)$, why do we need $\phi(x)$?}\todo{I revised and changed all $\phi$ to $\psi$, now it is more clear.} \Ahmad{At first paragraph $\psi$ is a general known (not specific) distribution (could be normal, or binomial, etc.), but in the second paragraph: For our work... we specify and assume that $\psi$ equals to normal distribution i.e. $\phi=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$}
% \begin{align}
%   \psi(x)=\phi(x)=\frac{1}{\sqrt{2\pi}}\exp\Big[-\frac{(x-\mu)^2}{2\sigma^2}\Big], 
% \end{align} 
%\lk{to me, it is unclear what a higher cumulant vs cumulant is} \Ahmad{by higher cumulats, I mean cumulants $\kappa_i$ for $i>2$}
Since for all $m>2$, the \deleted{higher} cumulants  $\gamma_m$ of the normal distribution are zero, we obtain the expansion ${f}(x)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(-D)^m}/{m!}\big]{\psi}(x)
	= \exp\big[\sum_{m=3}^{\infty}\kappa_m{(-D)^m}/{m!}\big]{\psi}(x)$.
% \begin{align}
% 	{f}(x)&=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\phi}(x)
% 	= \exp\Big[\sum_{r=3}^{\infty}\kappa_r\frac{(-D)^r}{r!}\Big]{\phi}(x). 
% \end{align}
Expanding this exponential expression using Bell polynomials~\cite{bell1934exponential}, we obtain the \textit{Gram-Charlier A series} 
$
    {f}(x)=\sum_{m=0}^{\infty}B_m(0,0,\kappa_3,\dots,\kappa_m)\frac{(-D)^m}{m!}{\psi}(x),
$
where the $m$th derivative of the Gaussian function can be represented using  Hermite polynomials $He_m(\cdot)$ ~\cite{johnson2005univariate}, 
%\footnote{$He_n \left(x\right)= (-1)^ne^{\frac{x^2}{2}}d^n (e^{-\frac{x^2}{2}})/dx^n$ (see, e.g., \cite{johnson2005univariate}).},
so that $ D^m\psi(x)=\psi^{(m)}(x)=({(-1)^m}/{\sigma^m}) He_m\left(({x-\mu})/{\sigma}\right) \psi(x)$.
% \begin{align}
%   D^n\phi(x)=\phi^{(n)}(x)=\frac{(-1)^n}{\sigma^n} He_n\left(\frac{x-\mu}{\sigma}\right) \phi(x). 
% \end{align}
The final form of the  Gram-Charlier A expansion $f_{GC}(x)$ approximating the pdf~$f$ using its cumulants is
\begin{align}\label{pdfGC}	f_{GC}(x)={f}(x)={\psi}(x) \sum_{m=0}^{\infty}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right).
\end{align}
\fi

%We note that the $f_{GC}(x)$ expansion~\eqref{pdfGC}  of a PP variable $x$ can be computed % approximation~\eqref{pdfGC}, 
%even when the moments of PP variables are parametric, i.e. their closed-form functional representations depend on the  loop iteration $n$ and/or other symbolic values. This is especially useful in the analysis of (probabilistic) loops, as it allows us to encompass {\it all} loop iterations in a single, symbolic, GC approximation.

% In practice, the summation in \eqref{pdfGC} goes up to the order of the cumulant needed to be computed from the corresponding  moments via the cumulants-moments relation \eqref{eq:CumulantMomentRelation}. Discretizing the support of the target pdf, we are able to implement our distribution reconstruction methods numerically.   To this end, we consider $a=x_0 < x_1 <x_2 <x_3 <\cdots <x_{n}=b$, discrete points on the $x$-axis and evaluate the Hermite and Bell polynomials and  the normal pdf $\phi(x)$ at these points. 

% %\addnote{\efi{give the formula for $He_n \left(x\right)$} Done!}
% % The cumulative distribution function (CDF) is
% % \begin{align}
% % {F}(x)&=\int_{-\infty}^{x}f(u)du\\\notag
% % &={\Phi}(x)-{\phi}(x) \sum_{n=3}^{\infty}\frac{1}{n!\sigma^{n-1}}B_n(0,0,\kappa_3,\dots,\kappa_n) He_{n-1} \Big(\frac{x-\mu}{\sigma}\Big),    
% % \end{align}
% \begin{figure}[tpbh!]
% 	\centering
% 	%	\includegraphics{Figures/reconstME6Moments.pdf}
% 	\includegraphics[width=6cm]{Figures/GramCharlier1.eps}
% 	\includegraphics[width=6cm]{Figures/GramCharlier8Cumulants.eps}
% % 	\\
% % 	\includegraphics[width=4.2cm]{Figures/GramCharlier4CumulantsSecondExample.eps}
% % 	\includegraphics[width=4.2cm]{Figures/GramCharlier8CumulantsExample2.eps}
% %	\includegraphics[height=5.5cm]{Figures/recostSpline7moments.eps}
% %	\includegraphics[height=5.5cm]{Figures/reconst1Spline.eps}
% 	\caption{Estimation of distribution using Gram-Charlier expansion  with the use of 4 cumulants (left), 8 cumulants (right) for \eqref{ex1}. 
% % 	Top panel: \eqref{ex1}. Bottom panel: \eqref{ex2}.
% }
% 	\label{fig:Splinemoments}
% \end{figure}


% Figure~\ref{fig:Splinemoments} shows the estimated distributions for \eqref{ex1}
% %and \eqref{ex2} 
% using 4 and 8 cumulants. As expected, increasing the number of cumulants, equivalently moments, results in better estimation. \efi{I repeat again that in absence of an absolute measure, reporting numbers for K-L conveys no information. Use KS test instead. }The accuracy of the estimation is measured with the Kullback-Leibler distance (see Equation~\eqref{Kullback-LeiblerDivergence}) to be $D_{KL}=0.1002$ for the GC estimation using 4 cumulants while $D_{KL}=0.0148$ for estimation of distribution using 8 cumulants.
% %shown in Table~\ref{table:Kullback-LeiblerDivergence1}. 
% Examples of estimating known distributions using ME and Gram-Charlier are given in  Appendix \efi{add a label in the appendix A}. 

% % Implementation and numerical results for prob-solvable probabilistic programs will be presented in Section~\ref{Section:Implementation and Benchmark Problems} and estimation of known distribution are investigated in Appendix A.
% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|}
% \hline
%               &  GC &GC\\
%               &  (4 cumul.)&(8 cumul.)\\
%               \hline
%      Example 1&  0.1002 &0.0148\\\hline
% %     Example 2& 0.1373 & 0.0360\\\hline
% \end{tabular}
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence ($D_{KL}$ of true and estimated  distributions with  Gram-Charlier (GC)).}
%       \label{table:Kullback-LeiblerDivergence1} 
%  \end{table}


%\subsection{Statistical Methods for Evaluation}



%\lk{the GC expansion needs a bit of further revision, making it more accessible to non-experts in statistics and linking the work to the PP setting}\Ahmad{We have a set of moments, then we compute cumulants (which are real numbers), then we evaluate Bell polynomials and Hermite polynomials using these cumulants and put them is the equation \eqref{pdfGC} to obtain the pdf. }





% To approximate the pdf $f$, we  expand $f$ using its cumulants $\kappa_m$ in terms of a known distribution $\psi$ \todo{In terms of: the estimated distribution will be a composition of some proportion of the $\psi$, for example: $f=(1+ \alpha x + \beta x^2)\psi(x)$, it is not related to the PP}\lk{what is $\psi$, what is ``in terms of", and what is the relation to PP?}\Ahmad{we try to characterize our unknown target distribution f in terms of a known distribution $\psi$ (here in this paper, in the next paragraph,  we specify and  take $\psi$ to be normal distribution, i.e. $\psi:=\phi$)}. We denote the characteristic function of $f$ by $\hat{f}$ and let $\hat{\psi}$ and $\gamma_m$  be the characteristic function and cumulants of the known distribution $\psi$, respectively. \ms{Is this a 'standard' way of writing characteristic function (using cumulants)?} Following \cite{wallace1958asymptotic}, we set $\hat{f}(t)=\exp\big[\sum_{m=1}^{\infty}\kappa_m{(it)^m}/{m!}\big]$  and  $\hat{\psi}(t)=\exp\big[\sum_{m=1}^{\infty}\gamma_m{(it)^m}/{m!}\big]$,
% % \begin{align}
% % \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}\kappa_r\frac{(it)^r}{r!}\Big] \quad \text{and} \quad \hat{\psi}(t)=\exp\Big[\sum_{r=1}^{\infty}\gamma_r\frac{(it)^r}{r!}\Big],    
% % \end{align}
% which leads to the identity $\hat{f}(t)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(it)^m}/{m!}\big]\hat{\psi}(t)$.
% % \begin{align}
% %  \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(it)^r}{r!}\Big]\hat{\psi}(t).    
% % \end{align}
% The term $(it)^m\hat{\psi}(t)$ is the Fourier transform of  $(-1)^m[D^m(\psi)(-x)]$, where $D$ is the differential operator with respect to $x$. Thus, the expansion of $f$ in terms of the known distribution $\psi$ is ${f}(x)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(-D)^m}/{m!}\big]{\psi}(x)$.
% % \begin{align}
% %   {f}(x)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\psi}(x).  
% % \end{align}

% Here, for our work, we assume  $\psi$ to be the normal distribution with the mean $\mu=\kappa_1$, variance $\sigma^2=\kappa_2$, and pdf  $\psi(x)=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$. \lk{if $\psi(x)=\phi(x)$, why do we need $\phi(x)$?}\todo{I revised and changed all $\phi$ to $\psi$, now it is more clear.} \Ahmad{At first paragraph $\psi$ is a general known (not specific) distribution (could be normal, or binomial, etc.), but in the second paragraph: For our work... we specify and assume that $\psi$ equals to normal distribution i.e. $\phi=({1}/{\sqrt{2\pi}\sigma})\exp\big[-{(x-\mu)^2}/{2\sigma^2}\big]$}
% % \begin{align}
% %   \psi(x)=\phi(x)=\frac{1}{\sqrt{2\pi}}\exp\Big[-\frac{(x-\mu)^2}{2\sigma^2}\Big], 
% % \end{align} 
% \lk{to me, it is unclear what a higher cumulant vs cumulant is} \Ahmad{by higher cumulats, I mean cumulants $\kappa_i$ for $i>2$}
% Since for all $m>2$, the \deleted{higher} cumulants  $\gamma_m$ of the normal distribution are zero, we obtain the expansion ${f}(x)=\exp\big[\sum_{m=1}^{\infty}(\kappa_m-\gamma_m){(-D)^m}/{m!}\big]{\psi}(x)
% 	= \exp\big[\sum_{m=3}^{\infty}\kappa_m{(-D)^m}/{m!}\big]{\psi}(x)$.
% % \begin{align}
% % 	{f}(x)&=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\phi}(x)
% % 	= \exp\Big[\sum_{r=3}^{\infty}\kappa_r\frac{(-D)^r}{r!}\Big]{\phi}(x). 
% % \end{align}
% Expanding this exponential expression using Bell polynomials~\cite{bell1934exponential}, we obtain the \textit{Gram-Charlier A series} 
% $
%     {f}(x)=\sum_{m=0}^{\infty}B_m(0,0,\kappa_3,\dots,\kappa_m)\frac{(-D)^m}{m!}{\psi}(x),
% $
% where the $m$th derivative of the Gaussian function can be represented using  Hermite polynomials $He_m(\cdot)$ ~\cite{johnson2005univariate}, 
% %\footnote{$He_n \left(x\right)= (-1)^ne^{\frac{x^2}{2}}d^n (e^{-\frac{x^2}{2}})/dx^n$ (see, e.g., \cite{johnson2005univariate}).},
% so that $ D^m\psi(x)=\psi^{(m)}(x)=({(-1)^m}/{\sigma^m}) He_m\left(({x-\mu})/{\sigma}\right) \psi(x)$.
% % \begin{align}
% %   D^n\phi(x)=\phi^{(n)}(x)=\frac{(-1)^n}{\sigma^n} He_n\left(\frac{x-\mu}{\sigma}\right) \phi(x). 
% % \end{align}
% The final form of the  Gram-Charlier A expansion $f_{GC}(x)$ approximating the pdf~$f$ using its cumulants is
% \begin{align}\label{pdfGC}	f_{GC}(x)={f}(x)={\psi}(x) \sum_{m=0}^{\infty}\frac{1}{m!\sigma^m}B_m(0,0,\kappa_3,\dots,\kappa_m) He_m \left(\frac{x-\mu}{\sigma}\right).
% \end{align}
% Notice, that even when the moments of program variables are parametric, i.e. their closed forms depend on the loop iteration $n$ or other symbolic values, we can still compute the cumulants as well as the final Gram-Charlier approximation~\eqref{pdfGC}. This is especially useful to analyze (probabilistic) loops, as we can address all loop iterations with a single, symbolic, GC approximation.
% % In practice, the summation in \eqref{pdfGC} goes up to the order of the cumulant needed to be computed from the corresponding  moments via the cumulants-moments relation \eqref{eq:CumulantMomentRelation}. Discretizing the support of the target pdf, we are able to implement our distribution reconstruction methods numerically.   To this end, we consider $a=x_0 < x_1 <x_2 <x_3 <\cdots <x_{n}=b$, discrete points on the $x$-axis and evaluate the Hermite and Bell polynomials and  the normal pdf $\phi(x)$ at these points. 


==> OldVersion.tex <==



% \section{Introduction}

% \textcolor{red}{To do: 
%  \bigskip 
% \begin{itemize}
%     \item Finding several benchmarks in PPs for which we should do distribution recovery.
%     \mm{Check out Github of polar and the paper draft for the polar tool. Also related work cited in the polar paper draft.}
%     \bigskip 
%     \item What is the gain of this distribution recovery. In particular, what we can do having this estimated distribution that we can not do without it (in the context of verification and program analysis)? Sensitivity Analysis? Add some reasoning and justification.
%     \mm{I would say answer questions of the form $\mathbb{P}(a \leq x \leq b)$: What's the probability that some program variable of interest is in some interval.}
%      \Ahmad{We take advantage of the reconstructed pdf  for different queries, such as to compute the probability of assertions and to answer questions of the form $\mathbb{P}(a \leq x \leq b)$: What's the probability that some program variable of interest is in some interval. Calculating  expectations, performing inference,  quantifying the loss of precision would be the other advantages of the distribution recovery for probabilistic programs with the help of their moments and without executing of the programs themselves (which is of essential premises in the field of  program analysis and verification).}
%         \bigskip 
%      \item How good are our distribution estimations? If we have the true distribution (for example in Square)? and If we do not have the true distribution? For latter, we do sampling and assess our estimated distribution and sampled one. For this, we have done with statistical tests (Chi-squared and Kolmogorov-Smirnov goodness of fit test) and using Kullback-Leibler Divergence in Section~\ref{Section:Implementation and Benchmark Problems}.
%      \ms{There should be quite a few known distributions we can encode as loops and compare exactly (there may be a bias, and the performance would be, potentially, better than for arbitrary distribution). %something to mention in the evaluation section
%      Another way, potentially, would be to only use some moments for reconstruction and a few more to test. E.g. use first 6 moments to get an approximate distribution and compare it's 7th, 8th moments to 7th and 8th precise moments (computed by Polar). }
%       \bigskip 
%       \item Writing what we have and we have done in a proper story. Adding a section on Prob-solvable programs that we can calculate exact moments. Then,...?, Adding from Polar? 
%       \ms{We can differentiate between \textit{moment computation} and \textit{distribution recovery}, both being somewhat separate problems in a wider problem of analysing probabilistic programs/loops.}
% \end{itemize}
% }

% Probabilistic programs are ordinary programs whose execution is based  on the outcome of
% random experiments.  Running a probabilistic program (repeatedly) on a \efi{single
% input} generally produces probability distributions over outputs.

% Almost all machine or statistical learning involves probabilistic algorithms
% (programs) for representing and updating the beliefs of an artificially intelligent system about the world in
% light of data; i.e., inferring plausible models to explain observed data. We aim to derive the probability
% distribution of the random variables generated by a PP. Quantifying and modelling the uncertainty in probabilistic programs
% will bring together computer programming, statistics and machine learning. 



% Computing invariant properties is of importance in probabilistic programs analysis as they summarize loop behaviors. \cite{bartocci2019automatic} presented fully automated approaches  to generate invariants over higher-order moments of program variables, without any user guidance. In the way to recover the full probabilistic program behavior, in this paper, we present numerical methods to reconstruct distributions of program variables using their moments. This procedure would help us to efficiently estimate posterior distributions of different variable directly without any use of sampling or running of the program itself, which is an essential requirement  in the verification of computer programs. 



% In this paper, we go through several approaches to reconstruct distributions for different variables involving in the probabilistic programs: characterization of distributions associated with prob-solvable probabilistic programs,  reconstruction of distribution from the scratch using numerical methods, and extracting properties of distribution using concentration inequalities. Our reconstruction methods will be tested on benchmarks. 


% \bigskip
% \bigskip


% % \section{Characterization of  Distributions Associated with Prob-Solvable Probabilistic Programs}
% % % \deleted{ The outcome values of a probabilistic program are
% % % realizations of random variables representing program expressions that are not deterministic. }

% % % \mm{"outcome values" is not a common terminology. "non-determinism" is very common but in CS means something different than probabilistic. Suggestion: The result of a PP is not a single value but rather different values with different probabilities according to the distribution the PP encodes.} \ahmad{Done!}

% % { The result of a PP is not a single value but rather different values with different probabilities according to the distribution the PP encodes. }
% % Different paths in a
% % PP are typically selected by draws from commonly used distributions such as the uniform or the normal, whose
% % properties and features have been extensively studied in probability and statistics. Yet, since a PP’s output values
% % are the result of multiple operations, their distributions are most often non common ones.
% % %Most developments in the analysis of PPs focus on the derivation of the first moment of the outcome values,
% % %[3, 16, 20, 33], 
% % %which provides a limited account of the distribution of the random variables arising from a
% % %PP. 
% % %Bouissou et al. (2016) \cite{bouissou2016uncertainty} considered the problem of answering queries on probabilities of assertions over program variables and
% % %their moments; that is, of assessing the likelihood of program variables and their moments producing outputs in a
% % %specified range. Their approach consists of approximating program random variables with affine forms under the
% % %assumption that they have bounded support and all their moments are finite.

% % The study of distributions and their characteristics is a much explored topic in statistics. Many distributions are fully characterized by their moments. Many of well known known distributions fall in this category. For example, the normal, the Poisson, the uniform, etc. 
% % % In particular, if
% % % a random variable has bounded support, then the sequence of all its moments uniquely
% % % determines its distribution \cite{billingsley2013convergence}. Nevertheless, knowledge of all
% % % the moments of a random variable does not necessarily uniquely characterize its distribution.

% % \begin{definition}\cite{casella2021statistical}\label{momentgeneratingfunction}
% % Let $X$ be a random variable with cdf $F_X$. The moment generating function (mgf)
% %  of $X$, denoted by $M_X(t)$, is 
% %  \begin{align}
% %      M_X(t)=E(e^{tX}),
% %  \end{align}
% % provided that the expectation exists for $t$ in some neighborhood of $0$. That is, there is an $h>0$ such that, for all $t\in(-h,h)$, $E(e^{tX})$ exists. If the expectation does not exists in a neighborhood of $0$, we say that moment generating function does not exist.  
% % \end{definition}

% % If the moment generating function exists, it characterizes all moments, but characterizing the set of moments is not enough to determine a distribution uniquely as  two distinct random variables can have the same moments (see e.g.  Example~2.3.10 in \cite{casella2021statistical}). If the random variable has bounded compact support, then the infinite sequence of moments  uniquely determines its distribution (\cite{billingsley1995probability} Section~30). More generally, if the moment generating function exists in a neighborhood of $0$, then the distribution is uniquely determined. Existence of all moments is not equivalent to existence of the moment generating function. 


% % % \efi{this has to do with the definition and existence of the moment generating function. See for example Casella and Berger's book}.  

% % % %The main approaches for characterizing distributions rely on moments of order statistics or conditional expectations \cite{bairamov2007characterization,su2000characterizations}.

% % % \efi{These paragraphs try to say what wrt our problem???}

% % % \textcolor{blue}{Carleman's condition guarantees that a probability distribution is uniquely determined by its moments.
% % % Let $\{\mu_k\}$ be the moment sequence of random variable $X \geq 0$, and let
% % % $$\sum_{k=1}^{\infty}\mu_k^{-1/(2k)}=\infty \qquad \text{(Carleman’s condition)},$$
% % % then   the  cumulative distribution function (cdf) $X$ is uniquely determined by the moments
% % % $\{\mu_k\}$. \cite{yarovaya2020conditions} study the relationship between the well-known Carleman's condition and some easily checkable conditions on the rate of growth of the moments. In the Stieltjes problem of moments, the pdf of a non-negative  random variable $X$ is determinable depends on the rate of growth of the moments. Let the moments $\{\mu_k\}$ follow a quadratic rate of growth, that is, 
% % % $$\frac{\mu_{k+1}}{\mu_k} = {\mathcal{O}}\big((k+1)^2\big) \quad as \quad k\rightarrow \infty.$$
% % % Then the random variable $X$ is uniquely determined by the moments \cite{lin2015moment}.
% % % As an extension, assume that
% % % $$\frac{\mu_{k+1}}{\mu_k} = {\mathcal{O}}\big((k+1)^2q^2(k+1)\big) \quad  as  \quad k\rightarrow \infty$$
% % % for the moment sequence $\{\mu_k\}$ of the random variable  $X$, where $q(k) > 0, n = 1,2,\dots$, is a function satisfying the condition 
% % % $$\sum_{k=1}^{\infty}\frac{1}{kq(k)}=\infty.$$
% % % \cite{yarovaya2020conditions} show that the moments $\{\mu_k\}$ satisfy Carleman’s condition, and these
% % % moments uniquely determine the random variable $X$.}




% % % %Also, if the moment generating function of a random variable $X$,
% % %$M_X(t)=E(e^{tX})$, exists in an open neighborhood of 0, then its distribution is uniquely determined %regardless of
% % %its support \cite{casella2021statistical}. Unfortunately, ascertaining this condition requires prior knowledge of the
% % %distribution of $X$.
% % %The main approaches for characterizing distributions rely on moments of order statistics or conditional expectations \cite{bairamov2007characterization,su2000characterizations}.
% % %Conditional moments of order statistics are extensively used in characterizing the parent probability distribution. 

% % %[51] obtained the explicit expression of the cumulative distribution function F(x) of a random variable
% % %X starting from $E(X|x\leq X\leq y) =
% % %\int_{x}^{y}tdF (t)/(F(y)-F(x))$ and define the relationship with order
% % %statistics as
% % %
% % %$$...$$





% % % \begin{comment}
% % % \bigskip
% % % \bigskip
% % % \textit{
% % % ... We have to  identify the class of PPs that admit closed form solutions for the distributions and those
% % % 	that do not. For the latter, the probability distributions will be approximated via simulations.}


% % % \bigskip
% % % \bigskip
% % % \textit{
% % % ... We should  identify the class of PPs that admit closed-form distribution(s)
% % % of the underlying random variables and characterize their distributions via higher order moments. When PPs do not
% % % generate variables whose distribution is characterized by moments, we will explore other statistical approaches,
% % % such as those based on order statistics \cite{balakrishnan1988recurrence} and conditional expectations, for distribution characterization.}

% % % \bigskip
% % % \bigskip

% % % \textit{
% % % ...We will characterize the distributions of
% % % continuous random variables in Prob-solvable and non Prob-solvable programs using distribution theory and results
% % % on moments of order statistics and/or conditional expectations. We will explore computer algebra packages
% % % that support the symbolic computation of probability and cumulative density functions for continuous random
% % % variables.}
% % % \end{comment}






% \section{Distribution Reconstruction via Their Moments and Cumulants}
% The reconstruction  of a probability density function (PDF) from  a finite number of its moments is
% known as the finite-moment problem which  arises in different  applications, such as physics, engineering, computer science, verification and cyber-physical systems \cite{gavriliadis2009moment, john2007techniques}. 

% Generally, the finite-moment problem is ill-posed and  there is no well-established algorithm available to solve this problem \cite{de2010reconstruction}. Depending on the specific problem and underlying field of study, 
%  several methods  add constraints on the domain and
% on the range of density function due to the underlying physics of the
% application, and try to reconstruct distributions from available finite number of moments. A typical example in the literature  is the reconstruction of particle
% size distributions (PSD) when considering particulate processes
% like crystallization in chemical engineering. Among existing  methods for physic-based finite-moment problem are for example: A kernel density estimation method \cite{athanassoulis2002truncated}, spline-based methods \cite{john2007techniques,de2010reconstruction}, and  Maximum Entropy \cite{biswas2010function, lebaz2016reconstruction} to reconstruct distributions from moments. 
% % We focus on nonparametric density estimation (e.g. kernel-based or spline-based methods) and Maximum Entropy. 
% Kernel density estimation together with a constrained minimization problem  is proposed by  \cite{athanassoulis2002truncated} for the Hausdorff moment problem and is extended in \cite{gavriliadis2009moment} for the Stieltjes moment problem.  In this method, the target pdf at a point is approximated by a sum of weights. The weight is typically modeled by a symmetric density, such as the standard normal. The optimal weights are computed through  minimizing the distance between the set of given moments and those estimated via the kernel density estimator. However, this nonparametric estimation method requires constant tuning  of the bandwidth parameters which increase with the number of moments and is seen to often perform poorly \cite{lebaz2016reconstruction}.


% The spline-based nonparametric density estimation (see, e.g., \cite{john2007techniques}) uses a piecewise polynomial function to recover  the target distribution.  This method is improved by \cite{de2010reconstruction} to be an adaptive algorithm to have better performance in non-smooth and multi-modal distributions.  As shown in \cite{mortier2014comparison,lebaz2016reconstruction}, the spline-based algorithm is highly sensitive to the negative tolerances leading to different reconstructions for the same target probability density function. This method assumes a smooth transition at the boundaries of sub-intervals and these conditions need to be changed during the reconstruction process.   

% Maximum Entropy is based on the maximization of the Shannon entropy (\cite{mead1984maximum}, \cite{tagliani1999hausdorff,tagliani2001numerical}, \cite{biswas2010function}). Its main advantage is the low computational cost  
% %there is no need to {\it a priori} information on the shape of target distribution and  
% (\cite{lebaz2016reconstruction}: Tables~2, 3) and has received increasing interest over the last two decades.

% Recovery of (posterior) distribution given some evidences is a common task in probabilistic inference. Existing  approaches for probabilistic inference  include: 
% \textit{exact symbolic} approaches (see e.g. \cite{sanner2012symbolic,bhat2013deriving,gehr2016psi}) and \textit{approximate symbolic} approaches (\cite{?, ?, ?}).  
% In \cite{gehr2016psi}, a symbolic
% analysis system, called \textit{PSI (Probabilistic Symbolic Inference)}, is presented  for automating exact inference in PPs via program analysis. PSI  automatically  computes the exact pdf of the random variable(s) of interest represented by that program. 
% As exact inference is theoretically expensive,  
% probabilistic inference systems may exploit  approximate
%   techniques and implement algorithms that calculate numerical approximations \cite{?,?,?,?}. 
% % These methods trade precision for better performance \cite{gehr2016psi}.

% Distribution recovery from moments  has not been much explored in the context of probabilistic programs, verification and cyber-physical systems.
% Note that non of above-mentioned works (nor existing symbolic-based methods, neither approximation-based methods) recover an unknown distribution form its moments. A quantitative analysis of PPs is presented in \cite{sankaranarayanan2020quantitative} using only expectation and concentration inequalities, but recovering distribution numerically using higher order moments in the context of (prob-solvable) probabilistic programs has not been well studied so far. Since exact inference is theoretically expensive, we exploit approximate
% inference techniques for  probabilistic inference. 
% % Although there is no accuracy guarantee in approximation approaches, they still worth to focus on them ad they  provide us with an  insight on the problem.   



% \addnote[id=ahmad]{Are you aware of any work in this context, Marcel and Miroslav?}
% \mm{A relevant work could be the tool PSI (from ETH) (https://psisolver.org/). The can reconstruct the exact distribution for some (loop-free) PPs. PSI could also serve as a comparison. For programs PSI can recover the distribution approximate it with some moments and compare it to the exact distribution given by PSI.}
% \todo{Effie: a description and comparison, or at the very least, why it is not directly comparable, should be given.}

% %\efi{Previous attempts to estimate distributions from their moments in the context ??? of PP are KDE and splines???, maximum entropy etc}

% % Here we focus on maximum entropy because there is no need to {\it a priori} information on the shape of target distribution and  the computational cost is low (\cite{lebaz2016reconstruction}).


% % \subsection{Spline-based Methods}
% % Splines can be applied for the reconstruction of a function for which a finite number of moments is given. Let $x_1 <x_2 <x_3 <\cdots
% % <x_{n+1}$ be discrete points on the $x$-axis. A spline  $s(x)$ is a piecewise polynomial of degree $q$. When $q= 1, 2$, or 3, the spline is called linear, quadratic, or cubic, respectively. Here, we use the cubic splines and  generate a linear system of equations. Let $[a, b]$ be a given
% % interval and $a=x_1 <x_2 <x_3 <\cdots
% % <x_{n+1}=b$. The ansatz is
% % $$s_i(x) =
% % \sum_{j=0}^3
% % s_{ij} (x-x_i)^j, \qquad x\in[x_i, x_{i+1}],\quad i= 1,\dots,n.$$
% % There are $4n$ unknown coefficients $s_{ij}$ to determine. The function $f(x)$ which should be reconstructed is a probability
% % density function. We assume that $f(x)$ vanishes everywhere
% % outside $[x_1, x_{n+1}]$ and   the transition
% % at the boundaries of the interval is smooth.
% % This means for the left boundary 
% % $$s_1(x_1) = 0, \quad s'_1(x_1) = 0, \quad s''_1 (x_1) = 0.$$ 
% % Inserting these conditions into the ansatz gives the following
% % three equations:
% % $$s_1(x_1) = s_{10} = 0, \quad  s'_1(x_1) = s_{11} = 0, \quad s''_1 (x_1) = 2s_{12}= 0.$$
% % Analogously, the right boundary corresponds to
% % $$s_n(x_{n+1}) = 0, \quad s'_n(x_{n+1}) = 0, \quad s''_n (x_{n+1}) = 0.$$ 
% % which gives the following three equations:
% % \begin{equation*}
% % \begin{pmatrix}
% % 1&x_{n+1}-x_n &(x_{n+1}-x_n)^2 &(x_{n+1}-x_n)^2 \\
% % 0 &1     &  2(x_{n+1}-x_n)  &  3(x_{n+1}-x_n)^2\\
% % 0 & 0     & 2     &  6(x_{n+1}-x_n)
% % \end{pmatrix}
% % \begin{pmatrix}
% % 	s_{n0}\\
% % 	s_{n1}\\
% % 	s_{n2}\\
% % 	s_{n3}
% % \end{pmatrix}
% % =
% % \begin{pmatrix}
% % 0\\
% % 0\\
% % 0
% % \end{pmatrix}
% % \end{equation*}
% % For continuity of the estimator at $x_{i+1} \;\;  (i=1,\dots,n-1)$ we include $s_i(x_{i+1})=s_{i+1}(x_{i+1})$ which give us $n-1$ equations of the form 
% % \begin{equation*}
% % 	\begin{pmatrix}
% % 		1&x_{i+1}-x_i &(x_{i+1}-x_n)^2 &(x_{i+1}-x_i)^2 & -1
% % 	\end{pmatrix}
% % 	\begin{pmatrix}
% % 		s_{i0}\\
% % 		s_{i1}\\
% % 		s_{i2}\\
% % 		s_{i3}\\
% % 		s_{(i+1)0}
% % 	\end{pmatrix}
% % 	= 0.
% % \end{equation*}
% % For smoothness of the spline estimator, we include the continuity of the first derivative of cubic spline. To this end, we set $s'_i(x_{i+1})=s'_{i+1}(x_{i+1})$ for all $i=1,\dots,n-1$. This leads to $n-1$ equations of the form 
% % \begin{equation*}
% % 	\begin{pmatrix}
% % 		1&2(x_{i+1}-x_i) &3(x_{i+1}-x_i)^2  & -1
% % 	\end{pmatrix}
% % 	\begin{pmatrix}
% % 		s_{i1}\\
% % 		s_{i2}\\
% % 		s_{i3}\\
% % 		s_{(i+1)1}
% % 	\end{pmatrix}
% % 	= 0.
% % \end{equation*}
% % Also we should include the continuity of the second derivative of the cubic spline at $x_{i+1} \;\;  (i=1,\dots,n-1)$,  $s''_i(x_{i+1})=s''_{i+1}(x_{i+1})$ which add $n-1$ equations of following form to our system:  
% % \begin{equation*}
% % 	\begin{pmatrix}
% % 		2 &6(x_{i+1}-x_i)  & -1
% % 	\end{pmatrix}
% % 	\begin{pmatrix}
% % 		s_{i2}\\
% % 		s_{i3}\\
% % 		s_{(i+1)2}
% % 	\end{pmatrix}
% % 	= 0.
% % \end{equation*}
% % We need $n-3$ more equations for the system of equations to be solvable. These equations derive from the known moments. The $k$th moment of the cubic spline $s(x)$, $k\in\mathbb{N}$,
% % \begin{align*}
% % 	\mu_k=\int_{a}^{b}x^k s(x) dx = \sum_{i=1}^{n}\int_{x_i}^{x_{i+1}}x^k s_i(x)dx=\sum_{i=1}^{n}\sum_{j=0}^{3}s_{ij}\int_{x_i}^{x_{i+1}} x^k (x-x_i)^jdx. 
% % \end{align*}
% % The straightforward calculations and setting 
% % \begin{align*}
% % I_1=\frac{x_{i+1}^{k+1}-x_i^{k+1}}{k+1}, \qquad I_2=\frac{x_{i+i}^{k+2}-x_i^{k+2}}{k+2}, \qquad I_3=\frac{x_{i+i}^{k+3}-x_i^{k+3}}{k+3},  \qquad I_4=\frac{x_{i+i}^{k+4}-x_i^{k+4}}{k+4},
% % \end{align*}
% % leads to 
% % \begin{align*}
% % 	\mu_k&=\int_{a}^{b}x^k s(x) dx \\
% % 	&= \sum_{i=1}^{n} \big[I_1s_{i0} + (I_2-x_iI_1)s_{i1} + (I_3-2x_iI_2+x_i^2I_1)s_{i2} + (I_4 - 3x_iI_3 + 3x_i^2I_2 -x_i^3I_1)s_{i3}\big]. 
% % \end{align*}
% % Now, a $4n\times4n$ linear system of equations has been obtained
% % and can be solved. The simplifications corresponding to linear
% % and quadratic splines are straightforward. 

% % Figure~\ref{fig:SplinemomentsQuad} shows numerical results of implementation of quadratic spline for two different examples.  A finite number of  moments for each distribution are given. In the first example,the true distribution is assumed to be \begin{align}\label{pdf1}
% %  f_X(x)&=\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}  
% % \end{align} whose  support in $[0,1]$. The first 6 moments of  $f$ are calculated separately and are used to approximate the pdf $f$ via quadratic spline method.  The same strategy is applied for the second example with probability density function 
% % \begin{align}\label{pdf2}
% %  g_X(x)&=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}.
% % \end{align} 

% % \efi{Recompute the right panel of  Figure~\ref{fig:SplinemomentsQuad} and verify \eqref{pdf2} is a proper density}

% % You should approximate the following distributions
% % \begin{itemize}
% %     \item Normal mixture: $f(x)=\alpha N(\mu_1,\sigma_1)+(1-\alpha) N(\mu_2,\sigma_2)$, $\alpha \in (0,1)$.
% %     \item check distributions from \url{https://en.wikipedia.org/wiki/List_of_probability_distributions}. Specifically, the Cauchy, truncated normal, gamma, the Gompertz distribution, the half-normal distribution, Hotelling's T-squared distribution, F-distribution, Weibull, Gumbel, Generalized extreme value distribution.
% % \end{itemize}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	%	\includegraphics{Figures/reconstME6Moments.pdf}
% % 	\includegraphics[height=5cm]{Figures/reconstSpline6moments.eps}
% % 	\includegraphics[height=5cm]{Figures/SplineQsecondExample.eps}
% % 	%\includegraphics[height=3.7cm]{Figures/recostSpline7moments.eps}
% % 	%\includegraphics[height=3.7cm]{Figures/reconst1Spline.eps}
% % 	\caption{Quadratic Spline Method with 6 moments: Example 1 (left), Example 2 (right).}
% % 	\label{fig:SplinemomentsQuad}
% % \end{figure}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % %\begin{figure}[tpbh!]
% % %	\centering
% % %	%	\includegraphics{Figures/reconstME6Moments.pdf}
% % %	\includegraphics[height=3.7cm]{Figures/SplineQsecondExample.eps}
% % %	\caption{Quadratic Spline Method Example 2 with 5 moments }
% % %	\label{fig:Splinemoments}
% % %\end{figure}
% % %\newpage

% % %\newpage
% %\newpage

% \todo{Effie: no discussion about cumulant-based methods in this preamble. Needs to be added.}

% In this paper, the Maximum Entropy and Gram-Charlier expansion methods will be used. 

% \iffalse

% \subsection{Maximum Entropy}\label{section:MaximumEntropyMethod}

% The Maximum Entropy (ME) method is based on the maximization of the Shannon entropy  from information theory. In order to estimate the unknown distribution $f$, we  maximize $H[f]$ given by \cite{bernardo2009bayesian,o2004kendall}
% \begin{align}
%   H[f]=-\int_{a}^{b} f(x) \ln(f(x))dx,  
% \end{align}
% subject to its given moments $\mu_i=\int x^if(x)dx$. The explicit representation of the ME approximation $f_M(x)$ of the target PDF takes the form
% \begin{align}
% f_M(x)=\exp\Big[-\sum_{j=0}^N\xi_jx^j\Big],    
% \end{align}
% where the Lagrange's multipliers $\xi_j\;\; j=0,1,\dots,N$ can be obtained from given moments. To this end, the following system of $N+1$ nonlinear equations is solved,
% \begin{align}\label{eq:nonlinearSystemME}
% \int_a^b x^i\exp\Big[-\sum_{j=0}^N\xi_jx^j\Big]dx=\mu_i.   
% \end{align}
% For more details on the maximum entropy method for distribution recovery, we refer to \cite{buchen1996maximum}. Numerically, iterative methods are used to solve the nonlinear system of equations \cite{mead1984maximum,lebaz2016reconstruction}.  Here, we use a numerical minimization algorithm, called  Levenberg–Marquardt which was developed  to solve
% nonlinear least squares problems \cite{levenberg1944method, marquardt1963algorithm}. This algorithm is an iterative procedure  (a combination of   gradient descent and
% Gauss-Newton) with an initial choice of the Lagrange's multipliers $\xi_j$ in \eqref{eq:nonlinearSystemME} and
% a given tolerance of $10^{-6}$ for stopping the iterative process. 

% Before we move to distribution recovery in probabilistic programs where we have no information about the target PDF, we present  two  examples in which the following bimodal and tri-modal functions on the interval $[0,1]$ are recovered via ME.  
% \begin{itemize}
%     \item Example 1, $f_X(x)=\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}$,
%     \item Example 2, $g_X(x)=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}$. 
% \end{itemize}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/reconst6moments.eps}
% 		\includegraphics[width=4.2cm]{Figures/MEsecondExample.eps}
% 	\caption{Maximum Entropy Method with 6 moments: Example 1 (left), Example 2 (right).}
% 	\label{fig:MaxEntropy6Moments}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figure~\ref{fig:MaxEntropy6Moments} shows reconstructed distributions compared to the given ones in Example 1 and 2. 
% We compare the accuracy of the reconstruction using the Kullback–Leibler divergence. The  Kullback-Leibler divergence, or simply, KL
% divergence is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% Assuming that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% \begin{align}\label{Kullback-LeiblerDivergence}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.

% A quantitative comparison of the distributions (target and reconstructed) is also carried out. The Kullback–Leibler divergence values for the ME estimates of both functions are given in  Table~\ref{table:Kullback-LeiblerDivergence11}. 
% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|}
% \hline
%               & Example 1 & Example 2\\
%                           \hline
%      Maximum Entropy & 0.0328 & 0.0139\\\hline
%     \end{tabular}
% \vspace{5mm}
%  \caption{Kullback-Leibler divergence ($D_{KL}$ of sampled and ME estimated  distributions).}
%       \label{table:Kullback-LeiblerDivergence11} 
%  \end{table}


% % We compare the accuracy of the reconstruction using the Kullback–Leibler divergence. The  Kullback-Leibler divergence, or simply, KL
% % divergence is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$.
% % Assuming that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$, the continuous version of KL divergence is defined to be
% % \begin{align}
% %     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% % \end{align}
% % $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.

% % A quantitative comparison of the distributions (target and reconstructed) is also carried out. The Kullback–Leibler divergence values for the ME estimates of both functions are given in  Table~\ref{table:Kullback-LeiblerDivergence11}. 
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %               & Example 1 & Example 2\\
% %                           \hline
% %      Maximum Entropy & 0.0328 & 0.0139\\\hline
% %     \end{tabular}
% % \vspace{5mm}
% %  \caption{Kullback-Leibler divergence ($D_{KL}$ of sampled and ME estimated  distributions).}
% %       \label{table:Kullback-LeiblerDivergence11} 
% %  \end{table}
 
% % \mm{Would be nice to see this method for a concrete PP here: (1) Get precise moments via Polar. (2) approximate distribution with Maximum Entropy.}
% % \ahmad{Done for Random Walk 1D!}

% Next, we apply  Maximum Entropy to estimate distributions of a random variable generated in the probabilistic program  \textit{Random Walk 1D} using its calculated moments via moment-based invariant generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. The target distribution is unknown and  only moments of the random variable of interest, expressed as a function of loop iteration, are available (Equations~(\ref{eq:ExactmomentsofRandomWalk1}-\ref{eq:ExactmomentsofRandomWalk3})). \textcolor{blue}{In order to reconstruct the distribution of random variable $x$ in the probabilistic program Random Walk 1D, we fix the loop iteration to be $n=100$ and use the first three exact moments of $x$, i.e. $E[x(100)], E[x^2(100)]$ and $E[x^3(100)]$. Applying ME method to the given moments, we recover the pdf and the cdf of $x$ which is shown with red color in Figure~\ref{fig:pdfRandomwalk1DME1} (Middle and Right).}  
 







% In order to assess accuracy of distribution estimation, we carry out a Monte Carlo ``experiment'' by executing  the PP a \textit{large} number of times (here, large=1000), and  compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test. Results (see Figure~\ref{fig:pdfRandomwalk1DME1}) show visually the agreement of the estimated pdf and cdf with the sampled data (indeed, with the KS density approximation of the sampled data). Details and numerical result of the accuracy evaluation will be presented in Section~\ref{section:Evaluation}.

% % Here, we apply the Maximum Entropy method  to estimate distributions of a random variable of probabilistic program  Random Walk 1D  using its calculated moments via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. Note that the target distribution is unknown and we have only moments of the random variable of interest presented as a function of loop iteration. With the help of  statistical tools, we also confirm the agreement of our estimated distributions with the ones generated during the execution of these probabilistic programs. 


% \todo{The following is not a correct statement: We assess the agreement or accuracy  of the estimated distributions with the ones generated during the execution of the probabilistic programs.}

% What you do is the following: 

% \begin{enumerate}
%     \item You estimate the distribution using ME and the exact moments provided by the recurrence-based algorithm in \cite{bartocci2020mora,bartocci2019automatic}
%     \item Assess accuracy of ME estimation of moments and the true moments with plots only (so far)!
%     \item To assess accuracy of distribution estimation, you carry out a monte carlo ``experiment,'' as follows: You repeat the PP a \textit{large} number of times (here, large=1000), and then compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test.   
% \end{enumerate}

% \fi



 
% % \bigskip

% % \noindent{\bf Random Walk 1D} 
% % \begin{align}
% % &v:=0\\\notag
% % &x:=0\\\notag
% % &\text{while true:}\\\notag
% % &\quad v:=\text{uniform}(0,1)\\\notag
% % &\quad x:=x+v\;\;[7/10]\;\;x-v
% % \end{align}
% % Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~1 of  \cite{bartocci2019automatic}: 
% % \begin{align}\label{eq:ExactmomentsofRandomWalk1}
% % &E[x(n)] = n/5\\\label{eq:ExactmomentsofRandomWalk2}
% % &E[x^2(n)] = n^2/25 + 22n/75\\\label{eq:ExactmomentsofRandomWalk3}
% % &E[x^3(n)] = n^3/125 + n^222/125 - n21/250
% % \end{align}
% % Figure~\ref{fig:SampledEXforRandomWalk1Sample1000loop1} show the agreement of sampled data and exact expected value of random variable $x$ per each loop iteration. One easily can see that the uncertainty propagates through probabilistic loop and remains around the exact expected value of the variable $x$. Figure~\ref{fig:SampledEXforRandomWalk1000Sample1000loop1} shows that the mean value and the second moment for a sample of size 1000 agrees the exact expected values for each loop iteration $n$. This shows the strength  of the moment-based invariant generator in which on can calculate moments of random variables of a PP without running the program.  
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% % % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% % 	\caption{$x$-axis: iteration, $y$-axis: sampled values of the random variable. In red is the Mora generated $E(x)$, and in blue are the sampled values of the random variable in \textit{Random Walk 1D}.}
% % 	\label{fig:SampledEXforRandomWalk1Sample1000loop1}
% % \end{figure}

% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1000loop1000Sample.eps}
% % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ $E(x)$ and $E(x^2)$ for Random Walk 1D using 1000 sample for each iteration of loop.}
% % 	\label{fig:SampledEXforRandomWalk1000Sample1000loop1}
% % \end{figure}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=10cm]{Figures/absoluteErrorExRandomWalk1D.eps}\\
% % 	\includegraphics[width=10cm]{Figures/relativeErrorExRandomWalk1D.eps}
% % 	\caption{ Absolute and relative errors $E(x)$ and $E(x^2)$ for Random Walk 1D: \\
% % 	Absolute Error of $E(x)= |{E(x)}_{sample}-{E(x)}_{exact}|$\\
% % 	Absolute Error of $E(x^2)= |{E(x^2)}_{sample}-{E(x^2)}_{exact}|$\\
% %     Relative Error=$\frac{\text{Absolute Error}}{\text{Exact Value}}$}
% % 	\label{fig:AbsoluteandRelativeErrorsRandomWalk1D}
% % \end{figure}








% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=3.8cm]{Figures/histogramRandomwalk1D.eps}
% % 	\includegraphics[width=3.8cm]{Figures/pdfRandomwalk1DME.eps}
% % 	\includegraphics[width=3.8cm]{Figures/cdfRandomwalk1DME.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Random Walk 1D. Estimation of Distribution using Maximum Entropy method with 3 moments.}
% % 	\label{fig:pdfRandomwalk1DME1}
% % \end{figure}

 
 
% %  In order to evaluate our estimation, as there is no pdf and nor cdf of the target distribution available, we assess it via sampling strategy. Running the program itself and stopping at the fixed loop iteration (here, $n=100$), we apply Chi-Square Goodness-of-Fit Test to see if  our sampled data came from a population with the ME estimated distribution. To this end,  we consider following hypothesis:

% % \bigskip

% % \hspace{10mm} $\text{H}_0$:	The data follow the estimated distribution.

% % \hspace{10mm} $\text{H}_a$:	The data do not follow the estimated distribution.

% % \bigskip	

% % For the chi-square goodness-of-fit computation, we divide the data  into $k$ bins and define the test statistic as
% % \begin{equation}
% %     \chi^2=\sum\limits_{i=1}^k(O_i-E_i)^2/E_i,
% % \end{equation}
% % where $O_i$ is the observed frequency for bin $i$ and $E_i$ is the expected frequency (with respect to the estimated distribution) for bin $i$. The expected frequency is calculated by
% % $$
% % E_i=N(F(Y_u)-F(Y_l)),
% % $$
% % where $F$ is the estimated cumulative distribution function with maximum entropy, $Y_u$ is the upper limit for bin $i$, $Y_l$ is the lower limit for class $i$, and $N$ is the sample size.
% % The $\text{H}_0$ hypothesis (the data are from a population with the estimated distribution) is rejected if
% % \begin{equation}
% %     \chi^2 > \chi^2_{1-\alpha,k-1}
% % \end{equation}
% % where $\chi^2_{1-\alpha,k-1}$ is the chi-square critical value with $k-1$ degrees of freedom and significance level $\alpha$. Here, we set $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and our estimated distribution using maximum entropy method  is $\chi^2=11.3721$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we can not reject the null hypothesis which means the sampled data obtained through running the prob-solvable program Random Walk 1D  follow the  distribution estimated using  3 first moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 
% % % We have the same $\chi^2$ goodness-of-fit test result for the same sampled data and estimated distribution using Gram-Charlier expansion in which the test statistic $\chi^2=11.5346$.

% % % \bigskip


% % % Another goodness-of-fit test is the Kolmogorov-Smirnov which is  used for continuous distributions. The two-sample Kolmogorov-Smirnov test is a  hypothesis test that evaluates the difference between the cdfs of the distributions of the two sample data vectors over the range of $x$ in each data set. The test uses the maximum absolute difference between the cdfs of the distributions of the two data vectors. The test statistic is 
% % %  $$D^\ast=\max_x(|{G}(x)-{F}(x)|),$$
% % % where ${G}(x)$ is the empirical cdf (of the sampled data obtained by running of prob-solvable programs) and F(x) is the cdf of the hypothesized distribution (estimated distribution by moments).

% % % Here we reject the null hypothesis by comparing the $p$-value $p$ with the significance level $\alpha=0.05$, If the $p$-value is very small ($p\text{-value} <\alpha$), then either the null hypothesis is false or something unlikely has occurred.

% % % \begin{table}[tpbh!]
% % %     \centering
% % %  \begin{tabular}{|c|c|c|}
% % % \hline
% % %           {\bf Random Walk 1D}   & $D_{KL}$ &  p-value (KS) \qquad\\
% % %                          \hline
% % %      Maximum Entropy&0.0045 &0.6418\\\hline
% % %      Gram-Charlier& 0.0045&0.6423\\\hline
% % % \end{tabular}
% % %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Random Walk 1D probabilistic program.}
% % %     \label{tableRandomwalk}
        
% % % \end{table}

% % % Table~\ref{tableRandomwalk} shows the  Kullback-Leibler distances between sampled distribution and the estimated distribution  (using 3 first moments by maximum entropy and Gram-Charlier expansion) and also p-values for Kolmogorov–Smirnov goodness-of-fit test for Random Walk 1D probabilistic program. As $p$-values are not smaller than the significance level $\alpha=0.05$, we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of prob-solvable probabilistic program Random Walk 1D follow the  distributions estimated using moments. 




% \iffalse 

% \subsection{Gram-Charlier Expansion}\label{section:GramCharlierExpansion}
% The Gram–Charlier A series  approximates a probability distribution in terms of its cumulants \cite{hald2000early,brenn2017revisit}.  Cumulants $\kappa_n$  (an alternative to the moments) of the distribution are defined using the {\it{cumulant-generating function}} $K(t)=\ln(\text{E}[e^{itX}])$, i.e. the natural logarithm of the characteristic function. The relationship between the  moments and cumulants can be obtained 
% by extracting coefficients from the expansion. The first cumulant, $\kappa_1$, is the mean, $\mu_1$, the second cumulant, $\kappa_2$ is the variance, $\sigma^2$, and the third cumulant is the same as the third central moment. But fourth and higher-order cumulants are not equal to central moments. \todo{Effie: Define central moments $\mu_i$--before they first show up in the paper.}
% The $n$th cumulant can be expressed in terms of the first $n$ moments in a closed form via the determinant of following matrix \cite{broca2004cumulant},
% \begin{align}\label{eq:CumulantMomentRelation}
%     \kappa_n=(-1)^{n+1}\det
%     \begin{pmatrix}
%     \mu_1& 1 & 0 & 0 & 0 & 0 & \dots & 0\\
%     \mu_2& \mu_1 & 1 & 0 & 0 & 0 & \dots & 0\\
%     \mu_3& \mu_2 & \binom{2}{1}\mu_1 & 1 & 0 & 0 & \dots & 0\\
%     \mu_4& \mu_3 & \binom{3}{1}\mu_2 & \binom{3}{2}\mu_1 & 1 & 0 & \dots & 0\\
%     \mu_5& \mu_4 & \binom{4}{1}\mu_3 & \binom{4}{2}\mu_2 &
%     \binom{4}{3}\mu_1 & 1 & \dots & 0\\
%     \vdots& \vdots & \vdots & \vdots & \vdots & \ddots & \ddots & \vdots\\
%     \mu_{n-1}& \mu_{n-2} & \dots & \dots & \dots & \dots & \ddots & 1\\
%     \mu_{n}& \mu_{n-1} & \dots & \dots & \dots & \dots & \dots & \binom{n-1}{n-2}\mu_1 \\
%     \end{pmatrix}
% \end{align}
% Gram-Charlier is similar to the Edgeworth expansion (see, e.g., \cite{Kolassa2006}). Both write the characteristic function of the distribution whose probability density function $f$ is to be approximated in terms of the characteristic function of a known distribution, and recover $f$ through the inverse Fourier transform. They differ as to the arrangement of terms, which may affect the accuracy of truncating the series. As in  the cases we consider here, both perform roughly the same, we focus on the Gram-Charlier expansion. 

% Assume that $f$ is an unknown pdf and we would like to expand $f$ using its cumulants $\kappa_r$ in terms of a known distribution $\psi$. We denote the characteristic function of $f$ by $\hat{f}$ and assume $\hat{\psi}$ and $\gamma_r$ to be the characteristic function and cumulants of the known distribution $\psi$, respectively. Following \cite{wallace1958asymptotic}, 
% \begin{align}
% \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}\kappa_r\frac{(it)^r}{r!}\Big] \quad \text{and} \quad \hat{\psi}(t)=\exp\Big[\sum_{r=1}^{\infty}\gamma_r\frac{(it)^r}{r!}\Big],    
% \end{align}
% which leads to the identity 
% \begin{align}
%  \hat{f}(t)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(it)^r}{r!}\Big]\hat{\psi}(t).    
% \end{align}
% The term $(it)^r\hat{\psi}(t)$ is exactly the Fourier transform of the term  $(-1)^r[D^r(\psi)(-x)]$, where $D$ is the differential operator with respect to $x$. Thus, the expansion of $f$ in terms of the known distribution $\psi$ is
% \begin{align}
%   {f}(x)=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\psi}(x).  
% \end{align}
% Suppose $\psi(x)$ is the normal  density with  mean $\mu=\kappa_1$, variance $\sigma^2=\kappa_2$, and pdf
% \begin{align}
%   \psi(x)=\phi(x)=\frac{1}{\sqrt{2\pi}}\exp\Big[-\frac{(x-\mu)^2}{2\sigma^2}\Big], 
% \end{align}
% Since for all $r>2$, the  higher cumulants $\gamma_r$ of the normal distribution are zero, we obtain the expansion
% \begin{align}
% 	{f}(x)&=\exp\Big[\sum_{r=1}^{\infty}(\kappa_r-\gamma_r)\frac{(-D)^r}{r!}\Big]{\phi}(x)
% 	= \exp\Big[\sum_{r=3}^{\infty}\kappa_r\frac{(-D)^r}{r!}\Big]{\phi}(x). 
% \end{align}
% Expanding the exponential term using Bell polynomials, we find the \textit{Gram-Charlier A series}, which can be written as
% \begin{align}
%     {f}(x)=\sum_{n=0}^{\infty}B_n(0,0,\kappa_3,\dots,\kappa_n)\frac{(-D)^n}{n!}{\phi}(x),
% \end{align}
% where the $n$-th derivative of the Gaussian function can be presented using Hermite polynomials\footnote{$He_n \left(x\right)$ stands for  the probabilist's Hermite polynomials \cite{johnson2005univariate} which is defined by $He_n \left(x\right)= (-1)^ne^{\frac{x^2}{2}}\frac{d^n}{dx^n}e^{-\frac{x^2}{2}}$}  and the function $\phi$ itself, 
% \begin{align}
%   D^n\phi(x)=\phi^{(n)}(x)=\frac{(-1)^n}{\sigma^n} He_n(\frac{x-\mu}{\sigma}) \phi(x). 
% \end{align}
% The  Gram-Charlier A expansion of the unknown probability density $f$ using its cumulants is
% \begin{align}\label{pdfGC}	{f}(x)={\phi}(x) \sum_{n=0}^{\infty}\frac{1}{n!\sigma^n}B_n(0,0,\kappa_3,\dots,\kappa_n) He_n \left(\frac{x-\mu}{\sigma}\right).
% \end{align}
% %\addnote{\efi{give the formula for $He_n \left(x\right)$} Done!}
% % The cumulative distribution function (CDF) is
% % \begin{align}
% % {F}(x)&=\int_{-\infty}^{x}f(u)du\\\notag
% % &={\Phi}(x)-{\phi}(x) \sum_{n=3}^{\infty}\frac{1}{n!\sigma^{n-1}}B_n(0,0,\kappa_3,\dots,\kappa_n) He_{n-1} \Big(\frac{x-\mu}{\sigma}\Big),    
% % \end{align}
% \begin{figure}[tpbh!]
% 	\centering
% 	%	\includegraphics{Figures/reconstME6Moments.pdf}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier1.eps}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier8Cumulants.eps}\\
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier4CumulantsSecondExample.eps}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlier8CumulantsExample2.eps}
% %	\includegraphics[height=5.5cm]{Figures/recostSpline7moments.eps}
% %	\includegraphics[height=5.5cm]{Figures/reconst1Spline.eps}
% 	\caption{Estimation of distribution using Gram-Charlier expansion  with the use of 4 cumulants (left), 8 cumulants (right). Top: $f_X(x)=\frac{1}{0.3}e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}$. \\Bottom: $g_X(x)=e^{- 80(x-0.3)^2}+\frac{1}{0.6}e^{-80(x-0.6)^2}+e^{-50(x-0.8)^2}$.}
% 	\label{fig:Splinemoments}
% \end{figure}

% In practice, the summation in \eqref{pdfGC} goes up to the order of the cumulant needed to be computed from the corresponding first moments via the cumulants-moments relation \eqref{eq:CumulantMomentRelation}. Discretizing the support of target PDF, we are able to implement our distribution reconstruction methods numerically.   To this end, we consider $a=x_0 < x_1 <x_2 <x_3 <\cdots <x_{n}=b$, discrete points on the $x$-axis and evaluate the Hermite and Bell polynomials and  $\phi(x)$ at these points. 

% \fi








% % Figure~\ref{fig:Splinemoments} shows the estimated distributions for Examples 1 and 2 using 4 and 8 cumulants. The accuracy of the estimation is measured with  the Kullback-Leibler distance (see Equation~\eqref{Kullback-LeiblerDivergence}), shown in Table~\ref{table:Kullback-LeiblerDivergence1}. Examples of estimating known distributions using ME and GC are given in  Appendix A. 

% % % Implementation and numerical results for prob-solvable probabilistic programs will be presented in Section~\ref{Section:Implementation and Benchmark Problems} and estimation of known distribution are investigated in Appendix A.
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %               &  GC &GC\\
% %               &  (4 cumul.)&(8 cumul.)\\
% %               \hline
% %      Example 1&  0.1002 &0.0148\\\hline
% %      Example 2& 0.1373 & 0.0360\\\hline
% % \end{tabular}
% % \vspace{2mm}
% %  \caption{Kullback-Leibler divergence ($D_{KL}$ of true and estimated  distributions with  Gram-Charlier (GC)).}
% %       \label{table:Kullback-LeiblerDivergence1} 
% %  \end{table}

% %%% Moved to the Evaluation Section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % For probabilistic program Random Walk 1D, we have almost the same $\chi^2$ goodness-of-fit test result for the same sampled data and estimated distribution using Gram-Charlier expansion in which the test statistic $\chi^2=11.5346$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ which shows  
% % the sampled data follow the estimated distribution.  

% % Another goodness-of-fit test is the Kolmogorov-Smirnov which is  used for continuous distributions. The two-sample Kolmogorov-Smirnov test is a  hypothesis test that evaluates the difference between the cdfs of the distributions of the two sample data vectors over the range of $x$ in each data set. The test uses the maximum absolute difference between the cdfs of the distributions of the two data vectors. The test statistic is 
% %  $$D^\ast=\max_x(|{G}(x)-{F}(x)|),$$
% % where ${G}(x)$ is the empirical cdf (of the sampled data obtained by running of prob-solvable programs) and F(x) is the cdf of the hypothesized distribution (estimated distribution by moments).
% % %%% Here we reject the null hypothesis by comparing the $p$-value $p$ with the %%%significance level $\alpha=0.05$, If the $p$-value is very small ($p\text{-value} %%%<\alpha$), then either the null hypothesis is false or something unlikely has occurred.
% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Random Walk 1D}   & $D_{KL}$ &  p-value (KS) \qquad\\
% %                          \hline
% %      Maximum Entropy&0.0045 &0.6418\\\hline
% %      Gram-Charlier& 0.0045&0.6423\\\hline
% % \end{tabular}
% % \vspace{2mm}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Random Walk 1D probabilistic program.}
% %  \label{tableRandomwalk}
      
% % \end{table}

% % Table~\ref{tableRandomwalk} shows the  Kullback-Leibler distances between sampled distribution and the estimated distribution  (using 3 first moments by maximum entropy and Gram-Charlier expansion) and also p-values for Kolmogorov–Smirnov goodness-of-fit test for Random Walk 1D probabilistic program. As $p$-values are not smaller than the significance level $\alpha=0.05$, we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of prob-solvable probabilistic program Random Walk 1D follow the  distributions estimated using moments. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % \newpage
% % \ahmad{I am going to ignore this sub-section because I did not use it for the simulations.} {\bf The Edgeworth Series:}  Similar to Gram-Charlier expansion, Edgeworth series \cite{hall2013bootstrap} is also used to  approximate a probability distribution in terms of its cumulants. The series are the
% % same but, they differ in the ordering of their terms \cite{benhamou2018gram}. Let $Z_i$ be a sequence of i.i.d. random variables with mean $\mu$ and variance $\sigma^2$, and let $X_n$ be their standardized sums
% % $$X_n=\frac{1}{\sqrt{n}}\sum_{i=1}^{n}\frac{Z_i-\mu}{\sigma}.$$
% % Using the central limit theorem \cite{fischer2010history}, one can see that  the normalized sum $X_n$ tends toward a normal distribution. That is, if $F_n$ be the cumulative distributions of $X_n$, then 
% % $$\lim_{n\rightarrow\infty}F_n(x)=\Phi(x)\equiv\int_{-\infty}^{x}\frac{1}{\sqrt{2\pi}}e^{-\frac{1}{2}q^2}dq$$ 
% % for every $x$, as long as the mean and variance are finite. Assume that random variables $Z_i$ have also higher cumulants $\kappa_r$. Cumulants of $X_n$ can be calculated in terms of cumulants of $Z_i$
% % $$\kappa_r^{F_n}=\frac{n\kappa_r}{\sigma^rn^{r/2}} = \frac{\lambda_r}{n^{r/2-1}} \quad \text{where} \quad \lambda_r=\frac{\kappa_r}{\sigma^r} \quad \text{and}\quad r\geq2.$$
% % The Gram-Charlier A series for the density function $X_n$ would change to 
% % $$	{f}_n(x)={\phi}(x) \sum_{r=0}^{\infty}\frac{1}{r!}B_r\Big(0,0,\frac{\lambda_3}{n^{1/2}},\dots,\frac{\lambda_r}{n^{r/2-1}}\Big) He_r(x).$$
% % In the Edgeworth series the terms are collected according to powers of $n$. To this end, the coefficient of $n^{-m/2}$ term is obtained by collecting monomials of the Bell polynomials corresponding to the integer parts of $m$. Therefore, the characteristic function of unknown distribution would be as
% % $$\hat{f}_n(t)=\Big[1+\sum_{j=1}^{\infty}\frac{P_j(it)}{n^{j/2}}\Big]\exp(-t^2/2), $$
% % where $P_j(x)$ is a polynomial of degree $3j$ with coefficients depending on the cumulants of orders $3$ to $j+2$. Inverse Fourier transform leads us to the pdf  $f_n$ as follows \cite{wallace1958asymptotic} 
% % $${f}_n(x)=\phi(x)+\sum_{j=1}^{\infty}\frac{P_j(-D)}{n^{j/2}}\phi(x). $$ 
% % The first few terms of the Edgeworth expansion are 
% % $${f}_n(x)=\phi(x)-\frac{\lambda_3\phi^{(3)}(x)}{6\sqrt{n}} + \frac{1}{n}\Big(\frac{\lambda_4\phi^{(4)}(x)}{24} + \frac{\lambda_3^2\phi^{(6)}(x)}{72}\Big) + \cdots.$$ 
% % \cite{cramer1928composition} proved that such a series is valid uniformly in $x$. 

% % \efi{What is the connection between Edgeworth and G-C? Since the results look the same?}


% %\subsection{Polynomial Chaos Expansion} 
% %Polynomial Chaos Expansion (PCE) provides a way to represent a random variable $Y$ with finite variance  as a function of an $M$-dimensional random vector $X$, using a polynomial basis that is orthogonal to the distribution of this random vector. 




% % \bigskip
% % \bigskip

% % \newpage
% % \section{Numerical Inversion of Characteristic Functions}

% % For a univariate random variable $X$, with cumulative  distribution
% % function $F$, the characteristic function $\varphi:\mathbb{R}\rightarrow\mathbb{C}$ is defined
% % by
% % $$\varphi(\omega) := E\Big[e^{i\omega X}\Big]= \int_{-\infty}^{\infty} e^{i\omega x} dF(x), $$
% % which is the Fourier transform of the probability distribution function. For any random variable, the characteristic function always
% % exists and it uniquely determines the distribution.  
% % If $F(x)$
% % has a density $f(x)$ then $\varphi(\omega)$ can be written in terms of $f$
% % $$\varphi(\omega) = \int_{-\infty}^{\infty} e^{i\omega x} f(x)dx. $$
% % If we have the characteristic function $\varphi(\omega)$, we can obtain $F(x)$ and $f(x)$ using inversion \cite{bohman1975numerical,mccullagh1994does,waller1995does,waller1995obtaining, witkovsky2016numerical,witkovsky2017computing}. 

% % Having moments (or cumulants) of an unknown distribution, the idea for reconstruction is that we approximate characteristic function of the unknown distribution using function approximation methods, then we will apply numerical inversion of characteristic function to recover PDF and/or CDF of the distribution of interest. Bohman \cite{bohman1975numerical} presented an approximation for inversion of characteristic function to obtsin cumulative distribution function where $E(x)=0$ and $\text{var}(x)=1$ as follows,
% % $$F_X(x)=\frac{1}{2}+\frac{\eta x}{2\pi} - \sum_{\nu=1-H}^{H-1} \frac{\varphi(\eta\nu)}{2\pi i \nu}e^{-i\eta\nu x} \qquad {\nu\neq0},$$
% % where $\eta$ and $H$ are parameters. Waller \cite{waller1995does} showed that even though two random variables have quite similar moments, the characteristic functions are distinct enough to numerically approximate two different cdf's. He applied McCullagh's example \cite{mccullagh1994does} to illustrate how characteristic function can distinguish distribution functions while the moment generating functions are very similar. More details and discussion on Bohman's inversion method are presented in \cite{waller1995obtaining}.
% % %Witkovsky \cite{witkovsky2016numerical,witkovsky2001computing} presented numerical methods to derive PDF/CDF from characteristic function.
% % \bigskip
% % \bigskip

% % \todo{to do /////}
% % \newpage
% % \section{Uncertainty Propagation in Prob-Solvable Probabilistic Programs}
% % Concentration of measure is a well-studied phenomenon with a wealth of results that under suitable conditions
% % provide an upper bound on the probability of deviations from the expected value of a random
% % quantity. References for concentration inequalities for distribution recovery \cite{bouissou2016uncertainty,sankaranarayanan2020quantitative,chakarov2013probabilistic}.

% % Let $X_1,\dots,X_n$ be independent random variables bounded by the interval $[0,1]$. The empirical mean of these variables is defined by
% % $$ {\overline {X}}={\frac{1}{n}}(X_{1}+\cdots +X_{n}).$$
% % Hoefding's inequality states that 
% % $$P\Big(\overline{X}-E\Big[\overline{X}\Big]\geq \delta \Big)\leq e^{-2n\delta^2},$$
% % where $\delta\geq0$.
% % As a  generalization of the Hoeffding's inequality is  that when $X_i$ are strictly bounded by the intervals $[a_i, b_i]$:
% % $$P\Big(\Big|\overline{X}-E\Big[\overline{X}\Big]\Big|\geq \delta \Big)\leq 2\exp{\Big(-\frac{2n\delta^2}{\sum_{i=1}^n (b_i-a_i)^2}\Big)}.$$
% % $E\Big[\overline{X}\Big]$ is the expected value of $\overline{X}.$

% % Here, we would like to analyse the uncertainty propagation through prob-solvable probabilistic programs. We would like to find an upper  bound  on  the  probability  of deviation of a random variable   from  its expected  value that we are able to compute symbolically using Mora tool. We are not going to run the program itself to see what happens to a random variable, say $X$, after a fixed number of loop iterations being executed, but using calculated $E(X)$  by Mora, we are able to quantify how far a realization of $X$ could be from $E(X)$ before we run the loop.  Consider  Random Walk 1D probabilistic program:  
% % \begin{align*}
% % &v:=0\\
% % &x:=0\\
% % &\text{while true:}\\
% % &\quad v:=\text{uniform}(0,1)\\
% % &\quad x:=x+v\;\;[7/10]\;\;x-v
% % \end{align*}  
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% % % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% % 	\caption{Mora generated $E(x)$ compared to the sampled $x$  in  Random Walk 1D stopping at each iteration of loop.}
% % 	%\label{fig:SampledEXforRandomWalk1Sample1000loop}
% % \end{figure}
% % Without running the program, Mora computes moments of random variable $X$ for each iteration of loop as $E(X)=\frac{n}{5}$ and $E(X^2)=\frac{n^2}{25} + \frac{22n}{75}$ where $n$ is the number of loop iteration.  
% % Applying the generalization of the Hoefding's inequality, 
% % $$P\Big({X}-E\Big[{X}\Big]\geq \delta \Big)\leq \exp{\Big(-\frac{2\delta^2}{(b-a)^2}\Big)}.$$
% % where $a=-n$ and $b= n$ are lower and upper bounds for $X$, respectively,  with $P(a\leq X\leq b)=1$. If we take $n$ number of loop iterations to be, for example 1000, then the probability of being bigger than  $E(X)=200$ as $\delta$ is at maximum $\exp(-\frac{2\delta^2}{2000^2})$.
% % %\begin{figure}[tpbh!]
% % %	\centering
% % %	\includegraphics[height=5.5cm]{Figures/ConcentrationIneqBounds.eps}
% % %		\caption{Hoefding's and Bernstein's Upper Bounds for Random Walk 1D.}
% % %	\label{fig:ConcentrationIneqBounds}
% % %\end{figure}
    


% % Bernstein inequality is another concentration inequality  that provides
% % sharper bounds on distances between a realization  and the expectation of the random variable. If $P(|X_i|\leq c)=1$ and $E(X_i)=\mu$ then, for any $\delta>0$, 
% % $$P\Big(\Big|{\overline{X}}-\mu\Big|\geq \delta \Big)\leq 2\exp{\Big(-\frac{n\delta^2}{2\sigma^2 + 2c\delta/3}\Big)},$$
% % where $\sigma^2=\frac{1}{n}\sum_{i=1}^{n}\text{Var}(X_i).$


% \subsection{PPs with Prob-solvable loops}

% Prob-solvable programs are generalization of $P$-solvable programs  allowing probabilistic 
% assignments over random variables and distributions.
% %\begin{definition}\cite{bartocci2019automatic}
%     Let $m\in\mathbb{N}$ and $x_1,\dots,x_m$ denote real-valued program variables.
% Prob-solvable loops  with $x_1,\dots,x_m$ variables are programs of the following form \cite{bartocci2019automatic}:
% \begin{align}
%     I; \text{ while (true) } \{U\},
% \end{align}
% where $I$ is a sequence of initial assignments over $x_1,\dots,x_m$ (i.e. $x_1:=c_1,x_2:= c_2,\dots,x_m:=c_m$, with $c_i\in \mathbb{R}$ representing a real number
% drawn from a known distribution). $U$ is a sequence of $m$ random updates as the loop body. Each update is of the form:
% \begin{align}\label{poly-assgmt}
%  x_i := a_ix_i + P_i(x_1,\dots,x_{i-1})\; [p_i] \; b_ix_i + Q_i(x_1,\dots,x_{i-1}),   
% \end{align}
% where $a_i, b_i\in\mathbb{R}$ are constants and $P_i, Q_i  \in \mathbb{R}[x_1,\dots,x_{i-1}]$ are polynomials
% over program variables $x_1,\dots,x_{i-1}$ and  $p_i \in [0, 1]$  is the probability
% of updating $x_i$ to $a_ix_i + P_i(x_1,\dots,x_{i-1})$, whereas the probability to update $x_i$ to
% $b_ix_i + Q_i(x_1,\dots,x_{i-1})$  is $1-p_i$.
% %\end{definition}

% Considering a Prob-solvable
% program with $n\in \mathbb{N}$ denoting the loop iteration counter, \cite{bartocci2019automatic} show that variable
% updates of Prob-solvable programs lead to  special recurrences in $n$, so-called moment-based
% recurrences. Assume that the sequences
% $x_1(n),\dots,x_m(n)$  describe relations between values of $x_i$ at
%  loop iteration $n$. Then Prob-Solvable updates are expressed as 
%  \begin{align}
% &  x_i(n+1) := a_ix_i(n)\\\notag
% & + P_i(x_1(n),\dots,x_{i-1}(n))\; [p_i] \; b_ix_i(n) + Q_i(x_1(n),\dots,x_{i-1}(n)).   
%  \end{align}
 
%  PPs with Prob-solvable loops: Bartocci et al. (2019) \cite{bartocci2019automatic, bartocci2020mora} calculate all moments of all generated random variables via recurrence
% relations when assignments are of a specific form (see \eqref{poly-assgmt}). We focus on random variables generated in Prob-solvable loops. Our aim is to recover their distribution from their moments. 

% This can be easily answered when the distributions of the random variables produced by a PP are among the known and
% well studied distributions in Statistics. %One approach is to study recurrence relations that characterize variable updates that result in known distributions.
% When distributions are not recognized as known, the task is more difficult and is the focus of this paper.
% %we should use or adapt the approaches based on conditional expectation  to analyze the discrete and/or continuous random variables produced by prob-solvable PPs \cite{kotz1980some,su2000characterizations,zoroa1990characterization}. 


% % We investigate  recurrence relations that characterize variable updates that result in known distributions. We should identify the class of PPs that admit closed-form distribution(s) of the underlying random variables and reconstruct  their distributions via higher order moments.

% \mm{This is a bit outdated with Polar. Important is that under some conditions moments can be obtained precisely. And given precise moments we can start reconstructing the distribution. It doesn't really matter where this moments came from (as discussed in our last meeting).}


% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %\newpage
% \section{Implementation and Benchmark Problems: Distribution Reconstruction in Probabilistic Programs}\label{Section:Implementation and Benchmark Problems}
% In this section, we apply the approaches in Sections \ref{section:MaximumEntropyMethod} and \ref{section:GramCharlierExpansion} to estimate distributions of the random variables of probabilistic programs in \cite{bartocci2019automatic} using their calculated moments via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora} without executing programs. With the help of  statistical tools, we also confirm the agreement of our estimated distributions with the ones generated during the execution of these probabilistic programs. We refer to Section~\ref{section:Evaluation} for evaluation of estimations for the benchmark programs.  We  do our assessment for the Random Walk 1D and the  selected probabilistic programs (see Table~\ref{table:BenchmarkPrograms}) for which the exact calculated moments are available on in Table~\ref{Table:Benchmarks}. 

% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|clc|clc|clc|}
% \hline
%       \multirow{3}{*}{} 
%       &&&&& &&&\\
% \hspace{2mm}&{\bf StutteringP}&\hspace{2mm}&\hspace{3mm}& {\bf Square} & \hspace{2mm}&\hspace{3mm}&  {\bf Binomial($p$)} \hspace{10mm} & \hspace{2mm}\\
% &&&&&&&&\\
% &$f:=0$&&& $x:=0$ &&& $x:=0$ &\\
% &$x:=-1$&&& $y:=1$ &&&$\text{while true:}$&\\
% &$y:=1$&&& $\text{while true:}$ &&&$\quad x:=x+1\;\;[\;p\;]\;\;x$ &\\
% &$s:=0$&&& $\quad x:=x+2\;\;[1/2]\;\;x$  &&&&\\
% &$\text{while true:}$&&& $\quad y:=x^2$ &&&&\\
% &$\quad f:=1\;\;[\;{ p }\;]\;\;0$&&&  &&&&\\
% &$\quad x:=x+f*\text{uniform}(0,2)$&&&  &&&&\\
% &$\quad y:=y+f*\text{uniform}(0,4)$&&&  &&&&\\
% &$\quad s:=x+y$&&&&  &&&\\
% &&&&&  &&&\\
%                          \hline
                         
% &&&&& &&&\\
% \hspace{2mm}&{\bf Sum Rand. Series}  &\hspace{2mm}&\hspace{3mm}& {\bf Prod. Dep. Vars.}  & \hspace{2mm}&\hspace{3mm}& {\bf Bimodal}  & \hspace{2mm}\\
% &&&&& &&&\\
% &$n:=0$&&& $f:=0$ &&& $....$ &\\
% &$x:=0$&&& $x:=0$ &&& $....$ &\\
% &$\text{while true:}$&&& $y:=0$ &&& $....$ &\\
% &$\quad n:= n + 1$&&& $p:=0$ &&& $....$ &\\
% &$\quad x:=x+n\;\;[1/2]\;\;x$&&& $\text{while true:}$ &&& $....$ &\\
% &  &&& $\quad f:=0\;\;[1/2]\;\;1$ &&& $....$ &\\
% &  &&& $\quad x:=x+f$ &&& $....$ &\\
% &  &&& $\quad y:=y+1-f$ &&& $....$ &\\
% &  &&& $\quad p:=x \ast y$ &&& $....$ &\\
% &&&&& &&&\\
%                          \hline
                         
%                          &&&&& &&&\\
% \hspace{2mm}&{\bf ..... }&\hspace{2mm}&\hspace{3mm}& {\bf ..... } & \hspace{2mm}&\hspace{3mm}& {\bf .... } & \hspace{2mm}\\
% &&&&& &&&\\

% &&&&& &&&\\
%                          \hline
    
% \end{tabular}
% \vspace{2mm}
%  \caption{Benchmark Programs.}
%     \label{table:BenchmarkPrograms}
        
% \end{table}



% % \addnote{Explain why I did choose these 3 programs. Any other suggestion Marcel and Miroslav?}
% \mm{See my comment above. Also you could again take (loop-free) programs from PSI and try to approximate the distribution with just the moments.}




% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|l|}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
 
 
%  \multirow{3}{*}{StutteringP}&1& $E[s(n)] = 3np $ \\\cline{2-3}
%     &2& $E[s^2(n)] = 9n^2p^2 - 9np^2+\frac{32}{3}np$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{} $E[s^3(n)] = 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
%       & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
%       & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
%       & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
%       & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
%     \\\hline
%         \hline
   
% \multirow{3}{*}{Square}&1& $E[y(n)] = n^2+n$  \\\cline{2-3}
%     &2&$E[y^2(n)] = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
%     &3&$E[y^3(n)] = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
%         \hline
        
% \multirow{3}{*}{Binomial($p$)}&1&$E[x(n)] = np$  \\\cline{2-3}
%     &2& $E[x^2(n)] = n^2p^2 + np(1-p)$  \\\cline{2-3}
%     &3&$E[x^3(n)] = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
%         \hline        

% \multirow{3}{*}{Sum Rand. Series}&1&$E[x(n)] = n^2/4 + n/4$  \\\cline{2-3}
%     &2& $E[x^2(n)] = n^4/16 + 5n^3/24 + 3n^2/16 + n/24$  \\\cline{2-3}
%     &3&$E[x^3(n)] = n^6/64 + 7n^5/64 + 13n^4/64 + 9n^3/64 + n^2/32$    \\\hline
%         \hline        
 
% \multirow{3}{*}{Prod. Dep. Var.}&1&$E[p(n)] = n^2/4 - n/4$  \\\cline{2-3}
%     &2& $E[p^2(n)] = n^4/16 - n^3/8 + 3n^2/16 - n/8$  \\\cline{2-3}
%     &3& \multirow{3}{*}{}$E[x^3(n)] = n^6/64 - 3n^5/64 + 9n^4/64 - 21n^3/64$ \\
%     & &+ $15n^2/32 -n/4$    \\\hline
%         \hline        
        
% \multirow{3}{*}{Bimodal}&1& .  \\\cline{2-3}
%     &2&.  \\\cline{2-3}
%     &3&.   \\\hline
%         \hline   
        
% \multirow{3}{*}{Loop free PPs}&1& .  \\\cline{2-3}
%     &2&.  \\\cline{2-3}
%     &3&.   \\\hline
%         \hline   
% \end{tabular}
% \vspace{2mm}
%  \caption{Benchmarks}
%  \label{Table:Benchmarks}
% \end{table}



% % \subsection{Random Walk 1D} 

% % \begin{align}
% % &v:=0\\\notag
% % &x:=0\\\notag
% % &\text{while true:}\\\notag
% % &\quad v:=\text{uniform}(0,1)\\\notag
% % &\quad x:=x+v\;\;[7/10]\;\;x-v
% % \end{align}
% % Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~1 of  \cite{bartocci2019automatic}: 
% % \begin{align}
% % &E[x(n)] = n/5\\
% % &E[x^2(n)] = n^2/25 + 22n/75\\
% % &E[x^3(n)] = n^3/125 + n^222/125 - n21/250
% % \end{align}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% % % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% % 	\caption{Mora generated $E(x)$ compared to the sampled $x$  in  Random Walk 1D stopping at each iteration of loop.}
% % 	\label{fig:SampledEXforRandomWalk1Sample1000loop}
% % \end{figure}

% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4cm]{Figures/ExSampledandMora1000loop1000Sample.eps}
% % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ $E(x)$ and $E(x^2)$ for Random Walk 1D using 1000 sample for each iteration of loop.}
% % 	\label{fig:SampledEXforRandomWalk1000Sample1000loop}
% % \end{figure}


% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=3.8cm]{Figures/histogramRandomwalk1D.eps}
% % 	\includegraphics[width=3.8cm]{Figures/pdfRandomwalk1DME.eps}
% % 	\includegraphics[width=3.8cm]{Figures/cdfRandomwalk1DME.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Random Walk 1D. Estimation of Distribution using Maximum Entropy method with 3 moments.}
% % 	\label{fig:pdfRandomwalk1DME}
% % \end{figure}


% % We apply Chi-Square Goodness-of-Fit Test to see if  our sampled data came from a population with the estimated distribution. To this end,  we consider following hypothesis:

% % \bigskip

% % \hspace{10mm} $\text{H}_0$:	The data follow the estimated distribution.

% % \hspace{10mm} $\text{H}_a$:	The data do not follow the estimated distribution.

% % \bigskip	

% % For the chi-square goodness-of-fit computation, we divide the data  into $k$ bins and define the test statistic as
% % \begin{equation}
% %     \chi^2=\sum\limits_{i=1}^k(O_i-E_i)^2/E_i,
% % \end{equation}
% % where $O_i$ is the observed frequency for bin $i$ and $E_i$ is the expected frequency (with respect to the estimated distribution) for bin $i$. The expected frequency is calculated by
% % $$
% % E_i=N(F(Y_u)-F(Y_l)),
% % $$
% % where $F$ is the estimated cumulative distribution function with maximum entropy, $Y_u$ is the upper limit for bin $i$, $Y_l$ is the lower limit for class $i$, and $N$ is the sample size.
% % The $\text{H}_0$ hypothesis (the data are from a population with the estimated distribution) is rejected if
% % \begin{equation}
% %     \chi^2 > \chi^2_{1-\alpha,k-1}
% % \end{equation}
% % where $\chi^2_{1-\alpha,k-1}$ is the chi-square critical value with $k-1$ degrees of freedom and significance level $\alpha$. Here, we set $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and our estimated distribution using maximum entropy method  is $\chi^2=11.3721$ which is not  greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we can not reject the null hypothesis which means the sampled data obtained through running the prob-solvable program Random Walk 1D  follow the  distribution estimated using  3 first moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 
% % We have the same $\chi^2$ goodness-of-fit test result for the same sampled data and estimated distribution using Gram-Charlier expansion in which the test statistic $\chi^2=11.5346$.

% % \bigskip


% % Another goodness-of-fit test is the Kolmogorov-Smirnov which is  used for continuous distributions. The two-sample Kolmogorov-Smirnov test is a  hypothesis test that evaluates the difference between the cdfs of the distributions of the two sample data vectors over the range of $x$ in each data set. The test uses the maximum absolute difference between the cdfs of the distributions of the two data vectors. The test statistic is 
% %  $$D^\ast=\max_x(|{G}(x)-{F}(x)|),$$
% % where ${G}(x)$ is the empirical cdf (of the sampled data obtained by running of prob-solvable programs) and F(x) is the cdf of the hypothesized distribution (estimated distribution by moments).

% % Here we reject the null hypothesis by comparing the $p$-value $p$ with the significance level $\alpha=0.05$, If the $p$-value is very small ($p\text{-value} <\alpha$), then either the null hypothesis is false or something unlikely has occurred.

% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Random Walk 1D}   & $D_{KL}$ &  p-value (KS) \qquad\\
% %                          \hline
% %      Maximum Entropy&0.0045 &0.6418\\\hline
% %      Gram-Charlier& 0.0045&0.6423\\\hline
% % \end{tabular}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Random Walk 1D probabilistic program.}
% %     \label{tableRandomwalk}
        
% % \end{table}

% % Table~\ref{tableRandomwalk} shows the  Kullback-Leibler distances between sampled distribution and the estimated distribution  (using 3 first moments by maximum entropy and Gram-Charlier expansion) and also p-values for Kolmogorov–Smirnov goodness-of-fit test for Random Walk 1D probabilistic program. As $p$-values are not smaller than the significance level $\alpha=0.05$, we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of prob-solvable probabilistic program Random Walk 1D follow the  distributions estimated using moments. 





% % % %\newpage
% % \subsection{StutteringP}\label{subsectionStutteringP} 

% % \begin{align*}
% % &f:=0\\
% % &x:=-1\\
% % &y:=1\\
% % &s:=0\\
% % &\text{while true:}\\
% % &\quad f:=1\;\;[\text{ p }]\;\;0\\
% % &\quad x:=x+f*\text{uniform}(0,2)\\
% % &\quad y:=y+f*\text{uniform}(0,4)\\
% % &\quad s:=x+y\\
% % \end{align*}

% Exact moments of the output  random variable of each probabilistic program are computed as functions of $n$, iteration of the loop are available in Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}: Table~1)\footnote{The second moment $E[s^2(n)]$ here differs from the one mentioned in \cite{bartocci2019automatic} as it did not agree with the simulations. The Calculations are presented in Appendix B.}. 
% % \begin{align}
% % &E[s(n)] = 3np \label{1st}\\
% % &E[s^2(n)] = 9n^2p^2 - 9np^2+\frac{32}{3}np\label{2nd}\\
% % &E[s^3(n)] = 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3) \notag\\
% % &+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)\notag\\ &+3np(4p^2-3p+3)+3np(8p^2-12p+9) \notag \\
% % &+ np(p^2-3p(-p-1)-3p+2)/2\notag \\
% % &+2np(2p^2 -6p(-p+2)-6p+13) +6 \label{3rd}
% % \end{align}

% % % \newpage
% % % \includepdf[pages=-]{deriveSecondmoment.pdf}

% % In order to assess the our estimations, we set the number of loop in the StutteringP program to be 100 and we take 1000 sample for the output $s$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments.   To perform the $\chi^2$ goodness-of-fit test for the StutteringP benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the maximum entropy estimated distribution  is $\chi^2=15.1544$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program StutteringP follow the  distribution estimated using  moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 


% % For the Kolmogorov-Smirnov goodness-of-fit test, we set again the significance level $\alpha=0.05$.  The test result is reported in Table~\ref{tableStutteringP}. In this test $p$-value is greater than the significance level $\alpha$, therefore we can not reject the $\text{H}_0$.

% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Square}   & $D_{KL}$ &  p-value (KS) \qquad\\
% %                          \hline
% %      Maximum Entropy& 0.00425 & 0.4494\\\hline
% % \end{tabular}
% % \vspace{2mm}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for the StutteringP probabilistic program. As p-value is greater than the  significance  level $\alpha=0.05$, the $\text{H}_0$ is not rejected which states that the sampled data obtained by the StutteringP program follow the maximum entropy estimated distribution. }
% %  \label{tableStutteringP}
% % \end{table}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/ExSampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex2SampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex3SampledandMora1000sample1000loopSttuteringP.eps}
% 	\caption{ $E(S)$, $E(S^2)$ and $E(S^2)$ for Stuttering P using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora1000loop1000sampleStutteringP}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/histogramStutteringP100loop1000sample.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfStutteringP100loop1000sampleME.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfStutteringP100loop1000SampleME.eps}
% 	\caption{ Left: histogram of sampled data by executing the StutteringP program (number of samples is 1000 and number of loop iteration in SutteringP is 100). Middle: pdf of sampled (kernel density estimation) and maximum entropy estimated Distribution for SutteringP. Right: cdf of sampled distribution and Maximum Entropy Estimation  for random varible $S$ in SutteringP.  }
% 	\label{fig:StutteringP100loop1000sample}
% \end{figure}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[height=5.5cm]{Figures/MEforStutterinP.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled and Estimated Distribution for Stuttering P. Estimation of Distribution using Maximum Entropy with 2 cumulants.}
% % 	\label{fig:MEforStutterinP}
% % \end{figure}

% %\newpage
% % \subsection{The Square Probabilistic Program} 
% % Square is a prob-solvable probabilistic program with polynomial assignment \cite{bartocci2019automatic}. The exact moments are available in Table~\ref{Table:Benchmarks}.
% % \begin{align*}
% % &x:=0\\
% % &y:=1\\
% % &\text{while true:}\\
% % &\quad x:=x+2\;\;[1/2]\;\;x\\
% % &\quad y:=x^2\\
% % \end{align*}
% % Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop (\cite{bartocci2019automatic}: Table~1): 
% % \begin{align*}
% % &E[y(n)] = n^2+n\\
% % &E[y^2(n)] = n^4+6n^3+3n^2-2n\\
% % &E[y^3(n)] = n^6+15n^5+45n^4-15n^3-30n^2+16n
% % \end{align*}
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4.2cm]{Figures/ExSampledandMora100loop1sampleSquare.eps}
% % % 	\includegraphics[width=4.2cm]{Figures/Ex2SampledandMora100loop1sampleSquare1.eps}
% % 	\caption{Mora generated  $E(Y)$ compared to the sampled $y$ in  Square probabilistic program stopped at each iteration of loop.}
% % 	\label{fig:ExSampledandMora100loop1sampleSquare}
% % \end{figure}
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/ExSampledandMora100loop1000sampleSquare.eps}
% 	\includegraphics[width=4.2cm]{Figures/Ex2SampledandMora100loop1000sampleSquare.eps}
% 	\caption{ $E(Y)$ and $E(Y^2)$ for Square using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora100loop1000sampleSquare}
% \end{figure}

% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[height=5.5cm]{Figures/pdfSampledandMoraSquare.eps}
% % 	\includegraphics[height=5.5cm]{Figures/cdfSampledandMoraSquare.eps}
% % 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% % 	\caption{ Sampled (kernel density estimation) and Gram-Charlier Estimated Distribution for Square. Estimation of Distribution using Gram-Charlier Expansion with 3 cumulants.}
% % 	\label{fig:GramCharlierforSquare}
% % \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/HistogramSquare1000Sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfSquare1000sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfSquare1000sample1000loop.eps}
% 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% 	\caption{Left: histogram of sampled data by executing the Square program (number of samples is 1000 and number of loop iteration in Square is 1000). Middle: pdf of sampled (kernel density estimation) and Gram-Charlier Estimated Distribution for Square. Estimation of Distribution using Gram-Charlier Expansion with 3 cumulants. Right: cdf of sampled distribution and Gram-Charlier estimation.}
% 	\label{fig:GramCharlierforSquare}
% \end{figure}



% \todo{explain about figures}



% {\bf Programs with Known Distribution:} Variable $x$ and $y$ in the Square program are inherently discrete random variables. Consider a Bernoulli process as a sequence of independent random variables $t_1, t_2, t_3 , \dots$ such that for each $i=1,2,3,\dots$, the variable $t_i$ is 0 or 1, and for all $i$, $P(t_i=1)=p$. In our special case, $p=1/2$. Using Bernoulli process we can rewrite the Square program as follows:
% \begin{align*}
% &x:=0\\
% &y:=1\\
% &\text{while true:}\\
% &\quad t:=1\;\;[ p ]\;\;0\\
% &\quad x:=x+2*t\\
% &\quad y:=x^2\\
% \end{align*}
% Note that $x$ and $y$ are somehow sum of Bernoulli variables which have Binomial distributions. In a more general case, we can use $x:=x+f(t)$ to update variable $x$, where  $f:\{0,1\}\rightarrow \mathbb{R}$ is a function for which $f(0)\neq f(1)$. In this case again we have Binomial distribution.   



% \bigskip
% \bigskip
% \bigskip



% % In order to assess the our estimations, we fix the number of loop in the Square program to be 1000 and we take 1000 sample for the output, i.e. the variable $y$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments (cumulants).   To perform the $\chi^2$ goodness-of-fit test for the Square benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the Gram-Charlier estimated distribution  is $\chi^2=9.9100$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program Square  follow the  distribution estimated using  moments (cumulants) calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 

% % Table~\ref{tableSquare} shows the result for the Kolmogorov–Smirnov goodness-of-fit test as well as the Kullback-Leibler between sampled and estimated distributions. As $p$-value is greater than the  significance  level $\alpha=0.05$, the $\text{H}_0$ is not rejected which states that the sampled data obtained by Square program follow the Gram-Charlier estimated distribution.

% % \begin{table}[tpbh!]
% %     \centering
% %  \begin{tabular}{|c|c|c|}
% % \hline
% %           {\bf Square}   & $D_{KL}$ &  p-value (Kolmogorov–Smirnov) \qquad\\
% %                          \hline
% %      Gram-Charlier& 0.0025 & 0.0886\\\hline
% % \end{tabular}
% %  \caption{Kullback-Leibler divergence and p-value (Kolmogorov–Smirnov) for Square probabilistic program.  }
% %   \label{tableSquare}
% % \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \newpage
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %  \multirow{3}{*}{Random Walk 1D}&1& 20 & $9.20\times 10^{-2}$  &$2.37 \times 10^{-5}$&$1.88\times 10^{-6}$\\\cline{2-6}
% %     &2& $4.2933 \times 10^2 $ &  $4.23 \times 10^{0}$ &$5.25\times 10^{-4}$& $6.63 \times 10^{-5}$\\\cline{2-6}
% %     &3& $9.7516 \times 10^3$  & $1.45 \times 10^{2} $ &$1.04\times 10^{-2}$& $3.56 \times 10^{-3}$\\\cline{2-6}
% %     &4&   & &   &  \\\cline{2-6}
% %     &5&   & &   &  \\\cline{2-6}
% %     &6&   & &   &  \\\cline{2-6}
% %     &7&   & &   &  \\\cline{2-6}
% %     &8&   & &   &  
% %     \\\hline
% %         \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In Table~\ref{table:AbsoluteandRelativeErrors}, we compare  errors of sample moments and estimated ones. Here, we first use 3 exact moments of each benchmark program and estimate the target distribution using these moments. Having the distribution for the variable of interest, we compute moments of order 4 to 10 and we call them estimated moments. Comparing first 10 moments of the underlying variable yields absolute estimate errors as \textit{absolute error of }$E(x^i)= |{E(x^i)}_{estimate}-{E(x^i)}_{exact}|$. Normalizing obtained errors with the exact moments we reach the \textit{relative estimate errors}. The same process is done for the \textit{absolute and relative sample errors}, but instead of estimated moments we compare  sample moments to the exact ones. Comparing two columns of sample error and estimate error shows the importance of the distribution recovery as the errors (absolute and relative) of moments obtained by estimated distribution are less than the errors of moments calculated by sampled data. 
% \begin{table}[tpbh!]\label{table:AbsoluteandRelativeErrors}
%     \centering
%  \begin{tabular}{|c|c|c|c|c|}
% \hline
%   {\bf Program}   & Moment &   Exact Value$^{1}$  & Absol. sample error$^{2}$   &Absol. estimate error$^{3}$  \\
%     &  & & (relative error$^\ast$)&  (relative error$^\ast$) \\
%                          \hline
%                          \hline
 
%  \multirow{3}{*}{RandomWalk1D}&1& 20 & $9.20\times 10^{-2} (0.5\%)$  &$1.88\times 10^{-6} (0.00001\%)$\\\cline{2-5}
%     &2& $4.2933 \times 10^2 $ &  $4.23 \times 10^{0} (1.0\%)$& $6.63 \times 10^{-5} (0.000015\%)$\\\cline{2-5}
%     &3& $9.7516 \times 10^3$  & $1.45 \times 10^{2} (1.5\%) $& $3.56 \times 10^{-3} (0.000037\%)$\\\cline{2-5}
%     &4&   & &     \\\cline{2-5}
%     &5&   & &    \\\cline{2-5}
%     &6&   & &    \\\cline{2-5}
%     &7&   & &    \\\cline{2-5}
%     &8&   & &    
%     \\\hline
%         \hline

%  \multirow{3}{*}{StutteringP}&1& 210 & $2.29\times 10^{-1} (0.1\%)$  &$8.11\times 10^{-5} (0.000038\%)$\\\cline{2-5}
%     &2& $4.4405 \times 10^4 $ &  $8.16 \times 10^{1} (0.2\%)$& $1.76 \times 10^{-2} (0.000039\%)$\\\cline{2-5}
%     &3& $9.3823 \times 10^6$  & $5.01 \times 10^{4} (0.5\%) $& $7.12 \times 10^{4} (0.75\%)$\\\cline{2-5}
%     &4&   & &     \\\cline{2-5}
%     &5&   & &    \\\cline{2-5}
%     &6&   & &    \\\cline{2-5}
%     &7&   & &    \\\cline{2-5}
%     &8&   & &    
%     \\\hline
%         \hline

%  \multirow{3}{*}{Square}&1& 10100 & $1.024\times 10^1 (0.1\%)$  &  $1.1063\times 10^{0} (0.01\%)$   \\\cline{2-5}
%     &2& $1.060298 \times 10^8$ & $6.78\times 10^5 (0.6\%)$ & $2.3037\times 10^3 (0.002\%)$    \\\cline{2-5}
%     &3& $1.1545\times 10^{12}$  &$1.93\times 10^{10} (1.7\%)$  &  $1.2681\times 10^7 (0.001\%)$  \\\cline{2-5}
%     &4&   & &     \\\cline{2-5}
%     &5&   & &     \\\cline{2-5}
%     &6&   & &     \\\cline{2-5}
%     &7&   & &     \\\cline{2-5}
%     &8&   & &     
         
%     \\\hline
%         \hline



% %  \multirow{3}{*}{StutteringP}&1& $E[s(n)] = 3np $ \\\cline{2-3}
% %     &2& $E[s^2(n)] = 9n^2p^2 - 9np^2+\frac{32}{3}np$  \\\cline{2-3}
% %     &3&  \multirow{3}{*}{} $E[s^3(n)] = 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
% %       & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
% %       & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
% %       & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
% %       & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
% %     \\\hline
% %         \hline
   
% % \multirow{3}{*}{Square}&1& $E[y(n)] = n^2+n$  \\\cline{2-3}
% %     &2&$E[y^2(n)] = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
% %     &3&$E[y^3(n)] = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
% %         \hline
        
% % \multirow{3}{*}{Binomial(p)}&1&$E[x(n)] = np$  \\\cline{2-3}
% %     &2& $E[x^2(n)] = n^2p^2 + np(1-p)$  \\\cline{2-3}
% %     &3&$E[x^3(n)] = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
% %         \hline        

% % \multirow{3}{*}{Sum Rand. Series}&1&$E[x(n)] = n^2/4 + n/4$  \\\cline{2-3}
% %     &2& $E[x^2(n)] = n^4/16 + 5n^3/24 + 3n^2/16 + n/24$  \\\cline{2-3}
% %     &3&$E[x^3(n)] = n^6/64 + 7n^5/64 + 13n^4/64 + 9n^3/64 + n^2/32$    \\\hline
% %         \hline        
 
% % \multirow{3}{*}{Prod. Dep. Var.}&1&$E[p(n)] = n^2/4 - n/4$  \\\cline{2-3}
% %     &2& $E[p^2(n)] = n^4/16 - n^3/8 + 3n^2/16 - n/8$  \\\cline{2-3}
% %     &3&$E[x^3(n)] = n^6/64 - 3n^5/64 + 9n^4/64 - 21n^3/64 + 15n^2/32 -n/4$    \\\hline
% %         \hline        
        
% % \multirow{3}{*}{Bimodal}&1& .  \\\cline{2-3}
% %     &2&.  \\\cline{2-3}
% %     &3&.   \\\hline
% %         \hline   
        
% % \multirow{3}{*}{Loop free PPs}&1& .  \\\cline{2-3}
% %     &2&.  \\\cline{2-3}
% %     &3&.   \\\hline
% %         \hline   
% \end{tabular}
% \vspace{2mm} 
%  \caption{Error for Benchmarks:\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Table ~\ref{Table:Benchmarks})\\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$}
%  \label{Table:ErrorforBenchmarks}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \bibliographystyle{splncs04}
% \bibliography{refs1}
%
% \begin{thebibliography}{8}
% \bibitem{ref_article1}
% Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

% \bibitem{ref_lncs1}
% Author, F., Author, S.: Title of a proceedings paper. In: Editor,
% F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
% Springer, Heidelberg (2016). \doi{10.10007/1234567890}

% \bibitem{ref_book1}
% Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
% Location (1999)

% \bibitem{ref_proc1}
% Author, A.-B.: Contribution title. In: 9th International Proceedings
% on Proceedings, pp. 1--2. Publisher, Location (2010)

% \bibitem{ref_url1}
% LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
% Oct 2017
% \end{thebibliography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \newpage

% \section{Appendix A: Estimation of Known Distributions}

% % \subsection{Cauchy Distribution}

% % \todo{explain more!!!}


% % The Cauchy distribution has the probability density function 
% % \begin{align*}
% %     f(x)=\frac{1}{\pi\gamma\Big[1+\Big(\frac{x-x_0}{\gamma}\Big)^2\Big]}
% % \end{align*}
% % where $x_0$   is the location parameter specifies location of the peak of the distribution, and  the scale parameter $\gamma$   specifies half the width of the PDF at half the maximum height.

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4.2cm]{Figures/MEforCauchyDist6moments.eps}
% % 	\caption{Maximum Entropy with 6 moments: Standard Cauchy Distribution.}
% % 	\label{fig:MEforChauchyDist6moments}
% % \end{figure}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[tpbh!]
% % 	\centering
% % 	\includegraphics[width=4.2cm]{Figures/GramCharlierCauchyDist4Cumulants.eps}
% % 	\includegraphics[width=4.2cm]{Figures/GramCharlierCauchyDist8Cumulants.eps}
% % 	\caption{Gram-Charlier for Standard Cauchy Distribution: with 4 cumulants (left), with 8 cumulants (right)}
% % 	\label{fig:GramCharlierforChauchyDist6moments}
% % \end{figure}

% % \bigskip
% % %\newpage
% \subsection{Normal Mixture Distribution}

% \addnote{explain more!!!}

% Normal mixture: $f(x)=\alpha N(\mu_1,\sigma_1)+(1-\alpha) N(\mu_2,\sigma_2)$, $\alpha \in (0,1)$.
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/MEforNormalMixture.eps}
% 	\includegraphics[width=3.8cm]{Figures/MEforNormalMixturealph05.eps}
% 	\includegraphics[width=3.8cm]{Figures/MEforNormalMixturealpha018.eps}
% 	\caption{Maximum Entropy for Normal Mixture with $\mu_1=-2, \sigma_1=1, \mu_2=1, \sigma_2=1$:   $\alpha=0.85$ (left),  $\alpha=0.5$ (middle), $\alpha=0.19$ (right).}
% 	\label{fig:MEforNormalMixtureDist6moments}
% \end{figure}


% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture4cumulantsalpha085.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture4cumulantsalpha05.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture4cumulantsalpha019.eps}\\
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture8cumulantsalpha0850.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture8cumulantsalpha05.eps}
% 	\includegraphics[width=3.8cm]{Figures/GramCharlierforNormalMixture8cumulantsalpha019.eps}
% 	\caption{Maximum Entropy for Normal Mixture with $\mu_1=-2, \sigma_1=1, \mu_2=1, \sigma_2=1$: (top: 4 cumulants, bottom: 8 cumulants);  $\alpha=0.85$ (left),  $\alpha=0.5$ (middle), $\alpha=0.19$ (right).}
% 	\label{fig:GramCharlierforNormalMixtureDist}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \bigskip
% % \newpage
% % \subsection{Gamma Distribution}

% % \subsection{Gompertz Distribution}
% % .
% % \bigskip
% \subsection{Weibull Distribution}

% \addnote{explain more!!!}

% The PDF of Weibull random variable is 
% \begin{align*}
%     f(x;\lambda,k)=\Big\{
%     \begin{matrix}
%          \frac{k}{\lambda}(\frac{x}{\lambda})^{k-1}e^{-(x/\lambda)^k}& & x\geq 0, \\
%           0& &  x<0,\\
%     \end{matrix}
% \end{align*}
% where $k>0$ is the shape parameter and $\lambda>0$ is the scale parameter of the distribution.
% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/MEforWeibull.eps}
% 		\caption{Maximum Entropy for Weibull Distribution  with $k=1.5, \lambda=1$.}
% 	\label{fig:MEforWeibull6moments}
% \end{figure}


% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/GramCharlierforWeibull4cumulants05.eps}
% 	\includegraphics[width=4.2cm]{Figures/GramCharlierforWeibull8cumulants05.eps}
% 	\caption{Gram-Charlier for Weibull Distribution  with $k=1.5, \lambda=1$:   4 cumulants (left),  8 cumulants (right).}
% 	\label{fig:GramCharlierforWeibull}
% \end{figure}

% % \subsection{Hotelling's T-squared Distribution}

% % \subsection{Truncated Normal Distribution}

% % \subsection{Half-normal Distribution}

% % \subsection{F-distribution}

% % \subsection{Generalized Extreme Value Distribution}

% % \subsection{Gumbel Distribution}
% %\newpage

% \subsection{Numerical Results}
% % \begin{itemize}
% % \item The {\bf Hellinger Distance} is used to quantify the similarity between two probability distributions.  Let $p(x)$ and $q(x)$ are pdfs of true and estimated distributions, respectively.  The square of the Hellinger distance is defined as follows: 
% % \begin{align*}
% %     H^2(P,Q)&=\frac{1}{2}\int\Big(\sqrt{p(x)} - \sqrt{q(x)}\Big)^2dx \\
% %     &= 1-\int\sqrt{p(x)q(x)} dx.
% % \end{align*}
% % Note that $0\leq H(P,Q) \leq 1$.

% % \item 
% {\bf Kullback–Leibler Divergence},  $D_{\text{KL}}$ quantifies how much one probability distribution differs from another probability distribution.
% To measure the difference between two probability distributions over the same
% variable $X$,  the Kullback-Leibler divergence, or simply, the KL
% divergence, has been popularly used in the data mining literature and it is a non-symmetric measure of the difference between two probability distributions $p(x)$ and $q(x)$. Here we assume that $p(x)$ is the true (known) distribution and $q(x)$ is an approximation of $p(x)$.  The continuous version of KL divergence is 
% \begin{align}
%     D_{KL}(P||Q) = \int_{-\infty}^{\infty} p(x)\ln\frac{p(x)}{q(x)}dx.
% \end{align}
% $D_{KL}(P||Q)$ is non-negative  and $D_{KL}(P||Q)=0$ if and only if $P = Q$.


% %\end{itemize}

% \bigskip
% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|c|}
% \hline
%               & ME& GC &GC\\
%               & (6 mom.)& (4 cumul.)&(8 cumul.)\\
%               \hline
%     %  Example 1& 0.0328& 0.1002 &0.0148\\\hline
%     %  Example 2& 0.0139&0.1373 & 0.0360\\\hline
%      Cauchy & 0.8516& 0.3684& 0.2990\\\hline
%      Normal Mixture& 0.0236 & 0.0399 &0.0012\\\hline
%      Weibull& 0.0105 & 0.0614 & 0.0407\\\hline
     
% \end{tabular}
%  \caption{Kullback-Leibler divergence ($D_{KL}$ of true and estimated  distributions with Maximum Entropy (ME) and Gram-Charlier (GC)).}
%      \label{table:Kullback-LeiblerDivergence} 
        
% \end{table}

% %\todo{to do /////}


% \bigskip
% \bigskip



% \newpage
% \section{Appendix B: Second Moment of StutteringP}

% \addnote{Type the calculation!}

% With a closer look at the StutteringP probabilistic program in Table~\ref{table:BenchmarkPrograms} we can see that \begin{align}
%     & E[f(n+1)]= p E[1] + (1-p) E[0],\\
%     & E[x(n+1)]= E[x(n)+ f(n+1)\cdot rand(0,2)],\label{eq:firstmomentStutteringPCalculations-1}\\
%     & E[y(n+1)]= E[y(n)+ f(n+1)\cdot rand(0,4)],\label{eq:firstmomentStutteringPCalculations-2}\\
%     &  E[s(n+1)]= E[x(n+1)+ y(n+1)].
% \end{align}
% which leads to 
% \begin{align}
%     & E[f(n+1)]= p,\\
%     & E[x(n+1)]= E[x(n)]+ E[f(n+1)]\cdot E[rand(0,2)],\\
%     & E[y(n+1)]= E[y(n)]+ E[f(n+1)]\cdot E[rand(0,4)],\\
%     &  E[s(n+1)]= E[x(n+1)]+E[y(n+1)].
% \end{align}
% Then we can write the recurrence relations. Solving this recurrences leads us to the close form of first moments, i.e. expectation, of each involved variables. 
% \begin{align}
%     & E[f(n)]= p,\label{eq:firstmomentStutteringPCalculations1}\\
%     & E[x(n+1)]= E[x(n)]+ p \;\Longrightarrow \; E[x(n)]=np-1 \; \text{ as } \; x(0)=-1,\label{eq:firstmomentStutteringPCalculations2}\\
%     & E[y(n+1)]= E[y(n)]+ 2p \;\Longrightarrow \; E[y(n)]=2np+1 \; \text{ as } \; y(0)=1,\label{eq:firstmomentStutteringPCalculations3}\\
%     &  E[s(n)]= E[x(n)]+E[y(n)]= np-1+2np+1 \;\Longrightarrow \; E[s(n)]=3np. 
% \end{align}

% Now we calculate recurrences and closed forms for the second moments of involved variables. As  $E[f(n+1)^2]=p E[1^2] + (1-p) E[0^2] = p$, we conclude that 
% \begin{align}
%     E[f(n)^2]=p.
% \end{align}
% For other variables
% \begin{align}
%   E[x(n+1)^2] & = E[\big(x(n)+ f(n+1)\cdot rand(0,2)\big)^2]\notag\\
%              & = E[x(n)^2]+ 2E[x(n)] E[f(n+1)]E[rand(0,2)] \notag\\
%              & \hspace{2.8cm}+ E[f(n+1)^2] E[rand(0,2)^2]\notag\\
%              & = E[x(n)^2]+ 2E[x(n)] E[f(n+1)] + E[f(n+1)^2] \frac{4}{3}\notag\\
%              & = E[x(n)^2]+ 2E[x(n)] E[f(n+1)] + E[f(n+1)^2] \frac{4}{3}
% \end{align}
% Considering Equations~\eqref{eq:firstmomentStutteringPCalculations1} and \eqref{eq:firstmomentStutteringPCalculations2} we have following recurrence for the second moment of random variable $x$:
% \begin{align}
%   E[x(n+1)^2] = E[x(n)^2]+ 2(np-1)p +  \frac{4}{3}p.
% \end{align}
% To solve this recurrence we have
% \begin{align*}
%   E[x(n)^2] &= E[x(0)^2]+ \sum_{i=0}^{n-1}\Big(2(ip-1)p +  \frac{4}{3}p\Big)\\
%   & = E[x(0)^2]+ 2p^2\Big(\sum_{i=0}^{n-1} i\Big)+ n(-2p+\frac{4}{3}p)\\
%   &=1+ 2p^2\Big(\frac{(n-1)(n)}{2}-\frac{2np}{3},
% \end{align*}
% which leads us to the closed form for second moment of $x$ in StutteringP:
% \begin{align}
%   E[x(n)^2] &= n^2p^2 - np^2 -\frac{2}{3}np+1.
% \end{align}
% The same calculations and considering Equations ~\eqref{eq:firstmomentStutteringPCalculations1} and \eqref{eq:firstmomentStutteringPCalculations3}, we reach 
% \begin{align}
%   E[y(n)^2] &= 4n^2p^2 - 4np^2 -\frac{28}{3}np+1.
% \end{align}
% To obtain recurrence relation for random variable $s$ we consider 
% \begin{align*}
%   E[s(n+1)^2]&=E[\Big(x(n+1)+y(n+1)\Big)^2]\\
%               &= E[x(n+1)^2] + 2E[(xy)(n+1)]  + E[y(n+1)^2] 
% \end{align*}
% in which $E[(xy)(n+1)]$ can be represented as a recurrence by multiplication of recurrences of $E[x(n+1)]$ and $E[y(n+1)]$ in \eqref{eq:firstmomentStutteringPCalculations-1} and \ref{eq:firstmomentStutteringPCalculations-2}:
% \begin{align*}
%   E[(xy)(n+1)]&= E[(xy)(n)] + 2 E[x(n)] E[f(n+1)] + E[y(n)] E[f(n+1)]+ 2E[f(n+1)^2] \\
%   &= E[(xy)(n)] + 2(np-1)p + (2np+1)p +2p
% \end{align*}
% Solving this recurrence we obtain
% \begin{align*}
%   E[(xy)(n)]&= E[(xy)(0)] + \sum_{i=0}^{n-1}\Big(2ip^2-2p+2ip^2+p+2p\Big)\\
%   &=2n^2p^2 -2np^2+np-1.
% \end{align*}
% Finally we obtain a closed form  for the second moment of random variable $s$:
% \begin{align*}
%   E[s(n)^2]&=E[\big(x(n)+y(n)\big)^2]\\
%               &= E[x(n)^2] + 2E[(xy)(n)]  + E[y(n)^2]\\
%               &=(n^2p^2 - np^2 -\frac{2}{3}np+1)+2(2n^2p^2 -2np^2+np-1)+(4n^2p^2 - 4np^2 -\frac{28}{3}np+1)\\
%               & = 9n^2p^2 - 9np^2+ 32np.
% \end{align*}




==> Precision_Vasicek.tex <==

\begin{example}
    %We have previously estimated the distribution  using ME and GC  from the first two moments of $r$. 
We  compute the first 8 exact moments of $r$ of the Vasicek model using Mora/Polar. We also compute these moments for the ME/GC estimated distributions and for $Sample_{Data}$. Resulting errors, absolute and relative, are listed in  Table~\ref{Table:ErrorforBenchmarksVasicek}. 
The error rates of the  ME and GC estimated pdfs are much smaller than the errors from sampling. Furthermore, ME performs marginally better than GC. Running times for distribution reconstruction using different number of moments for the Vasicek PP are shown in Table~\ref{table:TimeVasicekTable}. The running time for both methods increases with the number of higher moments used for estimation, with  ME being faster than GC.
    %The results show that, in this case, error for the moments from samples are a few orders of magnitude larger than in the case of estimating the distribution using ME or GC method.  \mm{MM: The last sentence is a bit hard to parse.}
\end{example}

%\vspace{5mm}


\begin{table}[tpbh!]\label{table:AbsoluteandRelativeErrorsVasicek}
\centering
\scalebox{0.8}{
\begin{tabular}{c|c|c|c|c}
\hline
  Moment & \;\;  Exact \;\;  & Absol. sample error$^{2}$   &Absol. ME estimate error$^{3}$  &Absol. GC estimate error$^{3}$ \\
    &Value$^{1}$ & (relative error$^\ast$)&  (relative error$^\ast$)&  (relative error$^\ast$) \\
                         \hline
                         \hline
 
1& 0.20 & $2.16\times 10^{-3} (1.08\%)$  &$6.63\times 10^{-11} (3.32\times 10^{-8}\%)$ &$1.40 \times 10^{-8} (7.00\times 10^{-6}\%)$\\%\cline{2-6}
    2& $0.0933$ &  $5.91 \times 10^{-3} (6.33\%)$& $9.67\times 10^{-11} (1.04\times 10^{-7}\%)$ &$2.15 \times 10^{-8} (2.31\times 10^{-5}\%)$ \\%\cline{2-6}
    3& 0.0400  & $3.13 \times 10^{-3} (7.83\%) $& $2.00 \times 10^{-8} (5.00\times 10^{-5}\%)$& $3.32 \times 10^{-8} (8.30\times 10^{-5}\%)$\\%\cline{2-6}
    4& 0.0229 & $ 2.54\times 10^{-3} (11.09\%) $ &   $4.02 \times 10^{-8} (1.75\times 10^{-4}\%)$ & $5.11\times 10^{-8} (2.23\times 10^{-4}\%)$ \\%\cline{2-6}
    5& 0.0131  & $ 1.83\times 10^{-3} (13.93\%) $ &   $7.11 \times 10^{-8} (5.42\times 10^{-4}\%)$ & $7.89\times 10^{-8} (6.01\times 10^{-4}\%)$\\%\cline{2-6}
    6& 0.0087& $ 1.61\times 10^{-3} (18.46\%) $&  $1.15 \times 10^{-7} (1.32\times 10^{-3}\%)$ & $1.22\times 10^{-7} (1.39\times 10^{-3}\%)$\\%\cline{2-6}
    7& 0.0059  &$ 1.40\times 10^{-3} (23.49\%) $ &   $1.83 \times 10^{-7} (3.07\times 10^{-3}\%)$ & $1.88\times 10^{-7} (3.16\times 10^{-3}\%)$\\%\cline{2-6}
    8&  0.0044 & $ 1.33\times 10^{-3} (29.86\%) $&   $2.86 \times 10^{-7} (6.43\times 10^{-3}\%)$ & $2.91\times 10^{-7} (6.53\times 10^{-3}\%)$
    \\\hline
      %  \hline
\end{tabular}
}
\vspace{2mm}
\caption{Error of moments (sample error and estimate error) for Vasicek model:\\
 $^{1}$ Exact value of moments at the iteration loop $n=100$ \\
 $^{2}$ Error of exact moments and sample moments\\
 $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
 $^\ast$ Relative error ($\%$)=$100 \times (\text{Absolute Error}/\text{Exact Value})$}
 \label{Table:ErrorforBenchmarksVasicek}
\end{table}
%\vspace{-15mm}

\begin{table}[tpbh!]
\centering
     %\scalebox{0.95}{
 %\footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength\abovecaptionskip{8pt}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}ccccccc@{}}
 %\begin{tabular}{c|c|c|c|c|c|c}
\toprule
& & \multicolumn{5}{c}{\# moments for estimation}\\
   & & 2 & 3 & 4 & 5 & 6 \\
  \cline{3-7}
  \multirow{2}{*}{Time $(s)$ }& Gram-Charlier & 1.55 & 1.73 & 1.88 & 2.11 & 2.28 \\
 % &&&&&&\\
  %\cline{2-7}
   %&&&&&&\\
   & Maximum Entropy & 0.63 & 0.71 & 0.89 & 1.14 & 1.67\\
  %&&&&&&\\
    \bottomrule
\end{tabular}
%}
%\vspace{2mm}
 \caption{Running times for distribution reconstruction vs. number of moments used for the Vasicek PP.
 %\ms{Maybe only address computation times in the to Evaluation section?}\Ahmad{All results of Vasicek are presented here. I think we keep this table here as well.}
 }
 \label{table:TimeVasicekTable}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%


==> benchmarks.tex <==
%!TEX root = samplepaper.tex
%\newpage
\section{Benchmarks}\label{section:Benchmarks}
%\subsection{Programs with Unknown Target Distribution} 
We evaluate our approach in Section~\ref{section:Evaluation}
% Sections \ref{section:MaximumEntropyMethod} and \ref{section:GramCharlierExpansion} 
on several benchmarks selected from \cite{bartocci2019automatic,Moosbruggeretal2022}. These benchmarks include {\bf StutteringP}, {\bf Square}, {\bf Binomial}, {\bf Random Walk 1D}, and {\bf Uniform}. We refer to Table~\ref{table:BenchmarkPrograms} in Appendix~\ref{Appendix} for the description of benchmarks.  We estimate the distributions of the random variables in these probabilistic programs  using their exact moments. The selected benchmarks are prob-solvable loops and their  exact moments can be calculated  via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora} without executing the programs. Exact moments of the output  random variable for selected benchmarks  are available,  as functions of loop iteration $n$, in Appendix~\ref{Appendix}: Table~\ref{Table:Benchmarks}.

\efi{what is this???  are available in Appendix~\ref{Appendix}:  Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}).}



% We  do our assessment for different probabilistic programs (see Table~\ref{table:BenchmarkPrograms}) for which the exact calculated moments are available on in Table~\ref{Table:Benchmarks}. Exact moments of the output  random variable of each probabilistic program are computed as functions of $n$, iteration of the loop are available in Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}:






% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.6}{
%  \begin{tabular}{|clc|clc|clc|clc|}
% \hline
%       \multirow{3}{*}{} 
%       &&&&& &&&& &&\\
% \hspace{2mm}&{\bf StutteringP}&\hspace{2mm}&\hspace{3mm}& {\bf Square} & \hspace{2mm}&\hspace{3mm}&  {\bf Binomial($p$)} \hspace{10mm} & \hspace{2mm}&\hspace{3mm}& {\bf Random Walk 1D } & \hspace{2mm}\\
% &&&&&&&&&&&\\
% &$f:=0$&&& $x:=0$ &&& $x:=0$ && & $v:=0$&\\
% &$x:=-1$&&& $y:=1$ &&&$\text{while true:}$&& & $x:=0$&\\
% &$y:=1$&&& $\text{while true:}$ &&&$\quad x:=x+1\;\;[\;p\;]\;\;x$ && & $\text{while true:}$&\\
% &$s:=0$&&& $\quad x:=x+2\;\;[1/2]\;\;x$  &&&&& &$\quad v:=\text{uniform}(0,1)$&\\
% &$\text{while true:}$&&& $\quad y:=x^2$ &&&&& &$\quad x:=x+v\;\;[7/10]\;\;x-v$&\\
% &$\quad f:=1\;\;[\;{ p }\;]\;\;0$&&&  &&&&& &&\\
% &$\quad x:=x+f*\text{uniform}(0,2)$&&&  &&&&& &&\\
% &$\quad y:=y+f*\text{uniform}(0,4)$&&&  &&&&& &&\\
% &$\quad s:=x+y$&&&&  &&&& &&\\
% &&&&&  &&&& &&\\
%                          \hline
% &&&&& &&&& &&\\
% \hspace{2mm}&{\bf Sum Rand. Series}  &\hspace{2mm}&\hspace{3mm}& {\bf Prod. Dep. Vars.}  & \hspace{2mm}&\hspace{3mm}& {\bf Bimodal}  & \hspace{2mm}&  &{\bf Uniform}&\hspace{2mm}\\
% &&&&& &&&& &&\\
% &$n:=0$&&& $f:=0$ &&& $x := 0$ && &$x := 1/2$&\\
% &$x:=0$&&& $x:=0$ &&& $xlow := 0$ && &$u := 0$ &\\
% &$\text{while true:}$&&& $y:=0$ &&& $xup := 0$ && &$\text{while true:}$&\\
% &$\quad n:= n + 1$&&& $p:=0$ &&& $\text{while true:}$ && &$\quad u:=u\;\;[1/2]\;\;u+x$&\\
% &$\quad x:=x+n\;\;[1/2]\;\;x$&&& $\text{while true:}$ &&& $\quad d := \text{Bernoulli}(1/3)$ && &$\quad  x := x/2$ &\\
% &  &&& $\quad f:=0\;\;[1/2]\;\;1$ &&& $\quad \text{if } d :== 0:$ && &&\\
% &  &&& $\quad x:=x+f$ &&& $\quad \quad step := \text{Normal}(3/4, 1)$ && &&\\
% &  &&& $\quad y:=y+1-f$ &&& $\quad \quad xlow := xlow - step$ && &&\\
% &  &&& $\quad p:=x \ast y$ &&& $\quad \quad x := xlow$ && &&\\
% &&&&& &&$\quad \text{else:}$&& &&\\
% &&&&& &&$\quad \quad step := \text{Normal}(3/4, 1)$&& &&\\
% &&&&& &&$\quad \quad xup := xup + step$&& &&\\
% &&&&& &&$\quad \quad x := xup$&& &&\\
% &&&&& && $\quad \text{end}$&& &&\\
% &&&&& &&&& &&\\
%                          \hline
% %                         &&&&& &&&& &&\\
% % \hspace{2mm}&{\bf Random Walk 1D }&\hspace{2mm}&\hspace{3mm}& {\bf Uniform } & \hspace{2mm}&\hspace{3mm}& {\bf .... } & \hspace{2mm}\\
% % &&&&  &&&&\\
% % &$v:=0$&&& $x := 1/2$ &&&&\\
% % &$x:=0$&&& $u := 0$ &&&&\\
% % &$\text{while true:}$&&& $\text{while true:}$  &&&&\\
% % &$\quad v:=\text{uniform}(0,1)$&&& $\quad u:=u\;\;[1/2]\;\;u+x$&&&&\\
% % &$\quad x:=x+v\;\;[7/10]\;\;x-v$&&& $\quad  x := x/2$ &&&&\\
% % &&&&& &&&\\
% %                         \hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Benchmark Programs.}
%     \label{table:BenchmarkPrograms}
% \end{table}
% % \addnote{Explain why I did choose these 3 programs. Any other suggestion Marcel and Miroslav?}
% % \mm{See my comment above. Also you could again take (loop-free) programs from PSI and try to approximate the distribution with just the moments.}
% \end{singlespace}
% \begin{singlespace}
% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.7}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
%  \multirow{3}{*}{StutteringP}&1& $\E(s(n)) = 3np $ \\\cline{2-3}
%     &2& $\E(s^2(n)) = 9n^2p^2 - 9np^2+\frac{32}{3}np$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{} $\E(s^3(n)) = 3np(9n^2p^2 - 27np^2 + 32np + 18p^2 - 32p + 14)$
%     % 27n^3p^3 -3n^2p^3 + 3n^2p^2(-6p+3)$\\ 
%     %   & & $+ 12n^2p^2(-3*p+3) +12n^2p^2(-2p+3)$\\
%     %   & & $+3np(4p^2-3p+3)+3np(8p^2-12p+9)$\\ 
%     %   & & $+ np(p^2-3p(-p-1)-3p+2)/2$\\
%     %   & &$+2np(2p^2 -6p(-p+2)-6p+13) +6$ 
%     \\\hline
%         \hline
   
% \multirow{3}{*}{Square}&1& $\E(y(n)) = n^2+n$  \\\cline{2-3}
%     &2&$\E(y^2(n)) = n^4+6n^3+3n^2-2n$ \\\cline{2-3}
%     &3&$\E(y^3(n)) = n^6+15n^5+45n^4-15n^3-30n^2+16n$     \\\hline
%         \hline
        
% \multirow{3}{*}{Binomial($p$)}&1&$\E(x(n)) = np$  \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^2p^2 + np(1-p)$  \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^3p^3 -3n^2p^3 + 3n^2p^2 + 2np^3 - 3np^2 + np$    \\\hline
%         \hline 
                
% \multirow{3}{*}{Random Walk 1D}&1&$\E(x(n)) =  n/5$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^2/25 + 22n/75$   \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^3/125 + n^222/125 - n21/250$   \\\hline
%         \hline   

% \multirow{3}{*}{Uniform(0,1)}&1& $\E(u(n))=2^{-n}(2^n - 1)/2$ \\\cline{2-3}
%     &2&$\E(u^2(n))=2^{-3n}(2^{3n+1} + 2^n - (3)4^n)/6$  \\\cline{2-3}
%     &3&$\E(u^3(n))=2^{-3n}(-2^{2n+1} + 2^n + 8^n)/4$  \\\hline
%   %      \hline           
% % \multirow{3}{*}{Loop free PPs}&1& .  \\\cline{2-3}
% %     &2&.  \\\cline{2-3}
% %     &3&.   \\\hline
% %         \hline   
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Exact moments of Benchmarks calculated by Mora/Polar.}
%  \label{Table:Benchmarks}
% \end{table}
% \end{singlespace}
% Exact moments of the output  random variable of each probabilistic program are computed as functions of $n$, iteration of the loop are available in Table~\ref{Table:Benchmarks} (cf. \cite{bartocci2019automatic}: Table~1).%\footnote{The second moment $\E(s^2(n))$ here differs from the one mentioned in \cite{bartocci2019automatic} as it did not agree with the simulations. Calculations are presented in Appendix B.}. 

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/ExSampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex2SampledandMora1000sample1000loopSttuteringP.eps}
% 	\includegraphics[width=3.8cm]{Figures/Ex3SampledandMora1000sample1000loopSttuteringP.eps}
% 	\caption{ $E(S)$, $E(S^2)$ and $E(S^2)$ for Stuttering P using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora1000loop1000sampleStutteringP}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/histogramStutteringP100loop1000sample.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfStutteringP100loop1000sampleME.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfStutteringP100loop1000SampleME.eps}
% 	\caption{ Left: histogram of sampled data by executing the StutteringP program (number of samples is 1000 and number of loop iteration in SutteringP is 100). Middle: pdf of sampled (kernel density estimation) and maximum entropy estimated Distribution for SutteringP. Right: cdf of sampled distribution and Maximum Entropy Estimation  for random varible $S$ in SutteringP.  }
% 	\label{fig:StutteringP100loop1000sample}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=4.2cm]{Figures/ExSampledandMora100loop1000sampleSquare.eps}
% 	\includegraphics[width=4.2cm]{Figures/Ex2SampledandMora100loop1000sampleSquare.eps}
% 	\caption{ $E(Y)$ and $E(Y^2)$ for Square using 1000 sample for each iteration of loop.}
% 	\label{fig:ExSampledandMora100loop1000sampleSquare}
% \end{figure}



% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.8cm]{Figures/HistogramSquare1000Sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/pdfSquare1000sample1000loop.eps}
% 	\includegraphics[width=3.8cm]{Figures/cdfSquare1000sample1000loop.eps}
% 	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
% 	\caption{Left: histogram of sampled data by executing the Square program (number of samples is 1000 and number of loop iteration in Square is 1000). Middle: pdf of sampled (kernel density estimation) and Gram-Charlier Estimated Distribution for Square. Estimation of Distribution using Gram-Charlier Expansion with 3 cumulants. Right: cdf of sampled distribution and Gram-Charlier estimation.}
% 	\label{fig:GramCharlierforSquare}
% \end{figure}






% \newpage
% \subsection{Programs with Known Distribution} 
% Variable $x$ and $y$ in the Square program are inherently discrete random variables. Consider a Bernoulli process as a sequence of independent random variables $t_1, t_2, t_3 , \dots$ such that for each $i=1,2,3,\dots$, the variable $t_i$ is 0 or 1, and for all $i$, $P(t_i=1)=p$. In our special case, $p=1/2$. Using Bernoulli process we can rewrite the Square program as follows:
% \begin{align*}
% &x:=0\\
% &y:=1\\
% &\text{while true:}\\
% &\quad t:=1\;\;[ p ]\;\;0\\
% &\quad x:=x+2*t\\
% &\quad y:=x^2
% \end{align*}
% Note that $x$ and $y$ are somehow sum of Bernoulli variables which have Binomial distributions. In a more general case, we can use $x:=x+f(t)$ to update variable $x$, where  $f:\{0,1\}\rightarrow \mathbb{R}$ is a function for which $f(0)\neq f(1)$. In this case again we have Binomial distribution.  

% For a fixed loop iteration, say $n$, a trajectory of random variable $\{y(i)\}_{i=0}^{n}$ could be a sequence of $\{x(i)^2\}$ where $x(i)=2b(i)$. In other word, $\{y(i)\}$ is the sequence of \textit{even-squared} numbers between 0 and $(2n)^2$. Here $b(i)=i$ where $i=0,1,2,\dots,n$. Random variable $b$ has  binomial distribution.    

% \begin{align}
%   P\Big[y=\text{even-squared}(i)\Big]&=p\Big[y=(2b(i))^2\Big]\notag\\
%   &=p\Big[x=2b(i)\Big]\notag\\
%   &=p\Big[b=i\Big]={n \choose
% i} p^i(1-p)^n-i \qquad i=0,1,2,\dots,n  
% \end{align}




% \newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \multirow{3}{*}{Random Walk 1D}&1& 20 & $9.20\times 10^{-2}$  &$2.37 \times 10^{-5}$&$1.88\times 10^{-6}$\\\cline{2-6}
%     &2& $4.2933 \times 10^2 $ &  $4.23 \times 10^{0}$ &$5.25\times 10^{-4}$& $6.63 \times 10^{-5}$\\\cline{2-6}
%     &3& $9.7516 \times 10^3$  & $1.45 \times 10^{2} $ &$1.04\times 10^{-2}$& $3.56 \times 10^{-3}$\\\cline{2-6}
%     &4&   & &   &  \\\cline{2-6}
%     &5&   & &   &  \\\cline{2-6}
%     &6&   & &   &  \\\cline{2-6}
%     &7&   & &   &  \\\cline{2-6}
%     &8&   & &   &  
%     \\\hline
%         \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%\subsection{A Real-life Application}


% {\bf Vasicek Model in Finance:}
% In finance, the Vasicek model is a mathematical model describing the evolution of interest rates. 
% %It is a type of one-factor short-rate model as it describes interest rate movements as driven by only one source of market risk.
% Following stochastic differential equation describes the Vasicek model: 
% \begin{align}
%  dr_{t}=a(b-r_{t})\,dt+\sigma \,dW_{t}   
% \end{align}
% where $W_t$ is a Wiener process under  modeling the continuous inflow of randomness into the system. $\sigma$ is the standard deviation factor which shows the amplitude of the instantaneous randomness inflow. $b$ is the long term mean level which paths  will evolve around it in a long term. $a$ is the speed of reversion specifying  the velocity at which such trajectories will regroup around $b$ in time.

% \bigskip
% \bigskip

% The Vasicek model of interest rate can be represented as a prob-solvable  probabilistic program as follows:
% \iffalse
% \begin{align}
% &a:=0.5\\\notag
% &b:=0.2\\\notag
% &\sigma:=0.2\\\notag
% &w:=0\\\notag
% %&dt:=1\\\notag
% &r:=2\\\notag
% &\text{while true:}\\\notag
% &\quad w:=\text{Normal}(0,1)\\\notag
% &\quad r:=(1-a)r + a\ast b + \sigma\ast w
% \end{align}
% \fi
% \begin{algorithmic}
%     \STATE $a:=0.5$
%     \STATE $b:=0.2$
%     \STATE $\sigma:=0.2$
%     \STATE $w:=0$
%     \STATE $r:=2$
%     \WHILE{true} 
%         \STATE $w:=\text{Normal}(0,1)$
%         \STATE $r:=(1-a)\ast r + a\ast b + \sigma\ast w$
%     \ENDWHILE
% \end{algorithmic}

% \bigskip

% % The expected value and variance of the random variable $r(t)$ given $r(0)$ are:
% % \begin{align}\label{eq:firstmomentVasicek}
% % &E\big(r(t)\big) = r(0) e^{-at}\,+\, b\big(1-e^{-at}\big)\\\label{eq:secondmomentVasicek}
% % &Var\big(r(t)\big) =\frac{\sigma^2}{2a} \big(1-e^{-2at}\big)
% % \end{align}



% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|l|}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
 
 
%  \multirow{3}{*}{Vasicek}&1& $\E(r(n)) = 2^{-n}(2^n + 9)/5 $ \\\cline{2-3}
%     &2& $\E(r^2(n)) = 7/75 + (18)2^{-n}/25 + (239)2^{-2*n}/75$  \\\cline{2-3}
%     &3&  \multirow{3}{*}{}$\E(r^3(n)) = 8^{-n}((239)2^n + (63)4^n + (5)8^n + 693)/125 $
%     \\\hline
%         \hline
% \end{tabular}
% \vspace{2mm}
%  \caption{Moments for Vasicek Model calculated by Polar\cite{}}
%  \label{Table:VasicekMomentsfromPolar}
% \end{table}

% %\newpage

% \begin{figure}[tpbh!]
% 	\centering
% % 	\includegraphics[width=10cm,  height=6cm]{Figures/AbsoluteErrorVasicek1000loop1000sample.eps}\\
% % 	\includegraphics[width=10cm,  height=6cm]{Figures/RelativeErrorVasicek.eps}\\
% \includegraphics[width=10cm,  height=6cm]{Figures/abserrorvasicekmodeln100sigma02.eps}\\
% 	\includegraphics[width=10cm,  height=6cm]{Figures/relerrorvasicekmodeln100sigma02.eps}\\
% 	\caption{Absolute and relative error of $E(r)$ and $E(r^2)$ in  \textit{Vasicek} model of interest rate.}
% 	\label{fig:AbsoluteandRelativeErrorsVasicekModel}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% % 	\includegraphics[width=3.9cm]{Figures/HistogramVasicek100loop1000sample.eps}
% % 	\includegraphics[width=3.9cm]{Figures/pdfVasicekME.eps}
% %      \includegraphics[width=3.9cm]{Figures/cdfVasicekModelME.eps}
% \includegraphics[width=3.9cm]{Figures/histogramvasicekmodeln100sigma02.eps}
% 	\includegraphics[width=3.9cm]{Figures/pdfvasicekmodeln100sigma02.eps}
%      \includegraphics[width=3.9cm]{Figures/cdfvasicekmodeln100sigma02.eps}
% 	\caption{Left: histogram of sampled data of random variable $r$ in Vasicek PP (sample size=1000 and loop iteration=100). Middle: PDF of ME estimate distribution in comparison with the K-S density of sampled data. Right: CDF (ME estimate and the K-S density).}
% 	\label{fig:HistogramPDFCDFofVasicekME}
% \end{figure}

% \begin{table}[tpbh!]
%     \centering
%   \scalebox{0.9}{
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & p-value (ME) & p-value (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline
%     \hspace{2mm} Vasicek \hspace{2mm}&\hspace{2mm} 0.0027 \hspace{2mm} & \hspace{2mm} 0.002685\hspace{2mm} & \hspace{2mm}0.15  \hspace{2mm} & 0.1456& \hspace{2mm} 17.4018 \hspace{2mm}& \hspace{2mm} 17.4017 \hspace{2mm}\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence of ME estimated distribution and sampled one), p-value (Kolmogorov–Smirnov), $\chi^2$ statistics for the Vasicek  probabilistic programs.}
%  \label{table:VasicekTable}
      
% \end{table}

% \begin{table}[tpbh!]\label{table:AbsoluteandRelativeErrorsVasicek}
%     \centering
%      \scalebox{0.7}{
%  \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%   {\bf Program}   & Moment &   Exact Value$^{1}$  & Absol. sample error$^{2}$   &Absol. ME estimate error$^{3}$  &Absol. GC estimate error$^{3}$ \\
%     &  & & (relative error$^\ast$)&  (relative error$^\ast$)&  (relative error$^\ast$) \\
%                          \hline
%                          \hline
 
%  \multirow{3}{*}{Vasicek}&1& 0.200000000000000 & $2.16\times 10^{-3} (1.08\%)$  &$6.63\times 10^{-11} (3.32\times 10^{-8}\%)$ &$1.40 \times 10^{-8} (7.00\times 10^{-6}\%)$\\\cline{2-6}
%     &2& $0.093333333333333$ &  $5.91 \times 10^{-3} (6.33\%)$& $9.67\times 10^{-11} (1.04\times 10^{-7}\%)$ &$2.15 \times 10^{-8} (2.31\times 10^{-5}\%)$ \\\cline{2-6}
%     &3& 0.0400000000000000  & $3.13 \times 10^{-3} (7.83\%) $& $2.00 \times 10^{-8} (5.00\times 10^{-5}\%)$& $3.32 \times 10^{-8} (8.30\times 10^{-5}\%)$\\\cline{2-6}
%     &4& 0.0229333333333333  & $ 2.54\times 10^{-3} (11.09\%) $ &   $4.02 \times 10^{-8} (1.75\times 10^{-4}\%)$ & $5.11\times 10^{-8} (2.23\times 10^{-4}\%)$ \\\cline{2-6}
%     &5& 0.0131200000000000  & $ 1.83\times 10^{-3} (13.93\%) $ &   $7.11 \times 10^{-8} (5.42\times 10^{-4}\%)$ & $7.89\times 10^{-8} (6.01\times 10^{-4}\%)$\\\cline{2-6}
%     &6& 0.00873955555555556  & $ 1.61\times 10^{-3} (18.46\%) $&  $1.15 \times 10^{-7} (1.32\times 10^{-3}\%)$ & $1.22\times 10^{-7} (1.39\times 10^{-3}\%)$\\\cline{2-6}
%     &7& 0.00594631111111111  &$ 1.40\times 10^{-3} (23.49\%) $ &   $1.83 \times 10^{-7} (3.07\times 10^{-3}\%)$ & $1.88\times 10^{-7} (3.16\times 10^{-3}\%)$\\\cline{2-6}
%     &8&  0.00445202962962963 & $ 1.33\times 10^{-3} (29.86\%) $&   $2.86 \times 10^{-7} (6.43\times 10^{-3}\%)$ & $2.91\times 10^{-7} (6.53\times 10^{-3}\%)$
%     \\\hline
%         \hline
 
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Error of moments (sample error and estimate error):\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ \\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$}
%  \label{Table:ErrorforBenchmarksVasicek}
% \end{table}


% \begin{table}[tpbh!]
%     \centering
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \hspace{2mm}{Vasicek}\hspace{2mm} & \# moments for estimation  & 2 & 3 & 4 & 5 & 6 \\
%                          \hline
%                           &&&&&&\\
%   \multirow{3}{*}{\hspace{2mm}Time \hspace{2mm}}& \hspace{2mm}Gram-Charlier\hspace{2mm} & 1.55 & 1.73 & 1.88 & 2.11 & 2.28 \\
%   &&&&&&\\\cline{2-7}
%   &&&&&&\\
%   $([s])$ & \hspace{2mm}Maximum Entropy \hspace{2mm}& \hspace{2mm}0.63\hspace{2mm} &\hspace{2mm} 0.71\hspace{2mm} &\hspace{2mm} 0.89\hspace{2mm} &\hspace{2mm} 1.14\hspace{2mm} &\hspace{2mm} 1.67 \hspace{2mm}\\
%   &&&&&&\\
%     \hline
% \end{tabular}
% \vspace{2mm}
%  \caption{Time of distribution reconstruction vs. number of moments applied for the reconstruction for Vasicek probabilistic program.}
%  \label{table:TimeVasicekTable}
      
% \end{table}

% \bigskip
% \bigskip
%\newpage

We also present, for the first time, 
a gene circuit  model in biology as a probabilistic program. As the resulting PP is prob-solvable, Mora/Polar calculate exact moments which are used to estimate the distribution of protein and mRNA levels  of a gene, the random variables of this model.  


\paragraph{A Piecewise-deterministic process (PDP) Model for Gene  Circuits: }
%As another real life  example, we present, for the first time, a piecewise-deterministic process (PDP) model  in biology as a prob-solvable probabilistic program. 
This  model is used to represent gene networks. 
We consider the simple model of
a single constitutive gene controlled by a two state (ON/OFF) promoter (see \cite{innocentini2018time}).

The continuous
variables are the protein ($x$) and and mRNA ($y$)  levels of the
gene. The discrete variable is a two-value variable
$s\in\{0, 1\}$ representing the promoter states (0 stands for OFF
and 1 stands for ON). 
The transition rates between ON and OFF are $f$ and $h$, thus $s$ can be modelled using a Markov chain. %f from ON to OFF, h from OFF to ON
The transcription initiation rates in states 0 and 1 are $k_0$ and $k_1$, respectively. The translation rate is $b$, $\rho$ is the mRNA and $a$ the protein degradation rate.
The protein and mRNA concentrations follow the ODEs
\begin{align}\label{PDP}
&\frac{dy}{dt}=\begin{cases}
k_0-\rho y & \text{if} \quad s=0\\
k_1-\rho y &  \text{if} \quad  s=1\\
\end{cases}\notag\\
&\frac{dx}{dt}=by-ax
\end{align}
We modify  the model by setting $dt=1$ in order to induce discrete-time recurrences, and translate the PDP model \eqref{PDP} for gene circuits to the prob-solvable probabilistic program in Figure~\ref{table:PDPmodelPPandMoments} (left).  The first- and second-order moments of the random variable $x$ as functions of loop iteration calculated by Polar \cite{Moosbruggeretal2022} are available in Appendix~\ref{Appendix}: Table~\ref{Table:Benchmarks}.
\begin{singlespace}
\begin{table}[tpbh!]
    \centering
    %\scalebox{0.6}{
    \begin{minipage}{0.48\textwidth}
\begin{algorithmic}
    \STATE $k_1:=4$, $k_2:=40$, $y:=0$
    % \STATE $k_2:=40$
    %  \STATE $y:=0$%, $x:=0$
    % \STATE $x:=0$
    % % \STATE $a:=0.2$
    % \STATE $a:=0.2$ 
    \STATE $x:=0$, $a:=0.2$, $b:=4$ 
    \STATE $s:=0$, $h:=0.6$, $f:=0.1$
    \STATE $\rho:=0.5$
    % \STATE $f:=0.1$
    % \STATE $h:=0.6$
    % % %\STATE $p:=0.5$
    % % \STATE $f:=0.1$, $h:=0.6$
    %   \STATE  $\rho:=0.5$
    % % %\STATE $\epsilon:=0.5$
    \WHILE{$true$}
        %\STATE $k:= k_1 \;[\;p\;] \;k_2$
        \IF{$s=0$}
            \STATE $s = 1 \;[\;f\;]\; 0$
        \ELSE
            \STATE $s = 0 \;[\;h\;]\; 1$
        \ENDIF
        \STATE $k:= k_2 * s + k_1 * (1-s)$
        % \STATE s:= 1 \;[\;p\;]\; 0
        % \STATE if s= 0 
        % \STATE    k=k0
        % \STATE else
        % \STATE    k=k1
        % \STATE end\\\notag
        \STATE $y:=(1-\rho)y+k$
        \STATE $x:=(1-a)x+by$
    \ENDWHILE
\end{algorithmic}
\end{minipage}
\begin{minipage}{0.58\textwidth}

\end{minipage}
\vspace{5mm}
\caption{The Prob-solvable loop expressing the PDP model \eqref{PDP} for gene circuits (left).} 
\label{table:PDPmodelPPandMoments}
%}
\end{table}
\end{singlespace}
% \begin{table}%[tpbh!]
%      \scalebox{0.7}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
%  \multirow{4}{*}{PDPModel} \hspace{2mm} &1& $\E(x(n)) = 1000^{-n}\big((24960)10^{3n} - (1944)300^n + (13720)500^n - (36736)800^n\big)/21$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = (2.62144\times 10^{27})^{-n}\big(-51514624000*(1.048576\times 10^{27})^n $\\
%     &&$+ 31603353600*(1.31072\times 10^{27})^n   + 59761049600(1.6777216\times 10^{27})^n  $\\
%     &&$- 84619591680(2.097152\times 10^{27})^n  + 30050150400*  (2.62144\times 10^{27})^n $\\ 
%     &&$- 413683200*  (3.93216\times 10^{26})^n  + 2326579200* (6.291456\times 10^{26})^n $\\
%     &&$- 2546790400*  (6.5536\times 10^{26})^n  + 15353556480*  (7.86432\times 10^{26})^n \big)/20349$ \\
%     \hline
%      %   \hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Moments for PDP  Model for Gene Circuits calculated by Polar \cite{polar}}
%  \label{Table:PDPModel}
% \end{table}


% \begin{algorithmic}
%     \STATE $k_1:=4$  
%     \STATE $k_2:=40$
%     \STATE $y:=0$
%     \STATE $x:=0$
%     \STATE $a:=0.2$
%     \STATE $b:=4$
%     \STATE $f:=0.1$
%     \STATE $h:=0.6$
%     %\STATE $p:=0.5$
%     \STATE $\rho:=0.5$
%     %\STATE $\epsilon:=0.5$
%     \WHILE{$true$}
%         %\STATE $k:= k_1 \;[\;p\;] \;k_2$
%         \IF{$s=0$}
%             \STATE $s = 1 \;[\;f\;]\; 0$
%         \ELSE
%             \STATE $s = 0 \;[\;h\;]\; 1$
%         \ENDIF
%         \STATE $k:= k_2 * s + k_1 * (1-s)$
%         % \STATE s:= 1 \;[\;p\;]\; 0
%         % \STATE if s= 0 
%         % \STATE    k=k0
%         % \STATE else
%         % \STATE    k=k1
%         % \STATE end\\\notag
%         \STATE $y:=(1-\rho)y+k$
%         \STATE $x:=(1-a)x+by$
%     \ENDWHILE
% \end{algorithmic}
% \ms{I updated the $s$ in the PDP to come form a MC. To do: update results in Tab 10-12 and Fig 14, 15, if necessary}
% \Ahmad{I need first 10 moments as functions of loop iteration (also evaluated in n=100), I appreciate it if I can have them to update the results.}

% \begin{table}[tpbh!]
%     \centering
%      \scalebox{0.7}{
%  \begin{tabular}{c|c|l}
% \hline
%   {\bf Program}   & Moment &  Computed Moment-based Invariants \\
%                          \hline
%                          \hline
 
 
%  \multirow{4}{*}{PDPModel} \hspace{2mm} &1& $\E(x(n)) = -4400(4/5)^n/3 + 880 + (1760)2^{-n}/3$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = 17920000(16/25)^n/9 - 13760000(2/5)^n/9$ \\
%     & & $- 7744000(4/5)^n/3 + 819200 + (2406400)4^{-n}/9$ \\
%     & & $+ (3097600)2^{-n}/3$ 
%     % \\
%     % \cline{2-3}
%     % &3&  \multirow{3}{*}{}$\E(x^3(n)) = 15769600000(16/25)^n/3 $\\
%     % &&$- 12108800000(2/5)^n/3 - 3604480000(4/5)^n $\\
%     % &&$- 66176000000(64/125)^n/27 + 23936000000(8/25)^n/9 $\\
%     % &&$+ 799744000 + (1802240000)8^{-n}/27 - (7546880000)5^{-n}/9 $\\
%     % &&$+ (2117632000)4^{-n}/3 + (1441792000)2^{-n}$
%     \\\hline
%      %   \hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Moments for PDP  Model for Gene Circuits calculated by Polar \cite{polar}}
%  \label{Table:PDPModel}
% \end{table}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=10cm,  height=4cm]{Figures/absErrorPDPmodeln100simoltain.eps}\\
% 	\includegraphics[width=10cm,  height=4cm]{Figures/relErrorPDPmodeln100simoltain.eps}\\
% % 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
% 	\caption{Absolute and relative error of $\E(x)$ and $\E(x^2)$ in  {PDP} model for Gene Circuits.}
% 	\label{fig:AbsoluteandRelativeErrorsPDPModeln10}
% \end{figure}

% \begin{figure}[tpbh!]
% 	\centering
% 	\includegraphics[width=3.3cm]{Figures/histogramPDPmodeln100simoltain.eps}
% 	\includegraphics[width=3.3cm]{Figures/pdfPDPmodeln100simoltain.eps}
%     %  \includegraphics[width=3.9cm]{Figures/cdfPDPmodeln100simoltain.eps}
% 	\caption{Left: histogram of sampled data of random variable $x$ in the PDP model for Gene Circuits  (sample size=1000 and loop iteration=100). Right: PDF of ME estimate distribution in comparison with the kernel smoothing density approximation  of sampled data. %Right: CDF (ME estimate and the K-S density).
% 	}
% 	\label{fig:HistogramPDFCDFofPDPmodeln10ME}
% \end{figure}

%\Ahmad{Results moved to the Evaluation section. }
% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.8}{
%  \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & $D^\ast$ (ME) & $D^\ast$ (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
%                          \hline
%     \hspace{2mm} PDP Model \hspace{2mm}&\hspace{2mm} 0.00439 \hspace{2mm} & \hspace{2mm}0.00415 \hspace{2mm} & \hspace{2mm}- \hspace{2mm}& - &16.4081   & 14.7861\\\hline
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Kullback-Leibler divergence of ME estimated distribution and sampled one), $D^\ast$ statistics (Kolmogorov–Smirnov test), $\chi^2$ statistics (Chi-Square test) for the PDP model for Gene Circuits (maximum loop iteration $n=100$).}
%  \label{table:PDPmodeln10}
      
% \end{table}

% \begin{table}[tpbh!]
%     \centering
%      \scalebox{0.7}{
%  \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%   {\bf Program}   & Moment &   Exact Value$^{1}$  & Absol. sample error$^{2}$   &Absol. ME estimate error$^{3}$ & Absol. GC estimate error$^{3}$ \\
%     &  & & (relative error$^\ast$)&  (relative error$^\ast$) &  (relative error$^\ast$)\\
%                          \hline
%                          \hline
 
%  \multirow{3}{*}{PDP Model}&1& 879.999999701235 & $3.89 \; (0.44\%)$  &$3.42 (0.39\%)$  &$0.012 (0.0014\%)$ \\\cline{2-6}
%     &2& 819199.999474173 &  $8.95\times 10^{3} (1.09\%)$& $3.61\times 10^{3} (0.44\%)$ &$2.362\times 10^{1} (0.0029\%)$ \\\cline{2-6}
%     &3& 799743999.265754  & $1.63 \times 10^{7} (2.04\%)$& $1.70\times 10^{6}(0.21\%)$ & $4.35\times 10^{4} (0.0054\%)$\\\cline{2-6}
%      &4& 813327753935.119 & $2.70\times 10^{10}(3.32\%)$ &  $2.40\times 10^{9}$ (0.29\%)  & $4.67\times 10^{8} (0.0573\%)$\\\cline{2-6}
%      &5& 857115541104823  &$4.22\times 10^{13}(4.92\%)$  & $ 9.61\times 10^{12}$ (1.11\%) & $2.26\times 10^{12} (0.2630\%)$\\\cline{2-6}
%      &6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\\cline{2-6}
%      &7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\\cline{2-6}
%      &8& $1.19415322490998\times 10^{24}$
%   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
%     & $2.95\times 10^{22} (2.4119\%)$\\\hline
%         \hline
 
% \end{tabular}
% }
% \vspace{2mm}
%  \caption{Error of moments (sample error and estimate error):\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ \\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$}
%  \label{Table:ErrorforBenchmarksPDPmodeln100}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
Our approach for distribution estimation using moments is not limited to prob-solvable loops. Once  moments of a  probabilistic program, either exact or approximated, are available, we can estimate the distribution of any random variable. As an example, we also represent a stochastic differential equation (SDE) as a probabilistic program that is not prob-solvable next, and estimate the distribution of its random variable. 


%\newpage
\paragraph{General Loops in Probabilistic Programs: }

We consider the  stochastic differential equation,
\begin{align}\label{eq:SDE2}
    dX(t)= -\frac{1}{4}X^3(t) dt -\frac{1}{2}X^2(t) dW(t) \qquad \text{with} \qquad X(0)=2,
\end{align}
where $W$ denotes the Wiener process (standard Brownian motion) \cite{morters2010brownian}. Eqn. \eqref{eq:SDE2} can be represented as a probabilistic program which is shown  in Figure~\ref{fig:HistogramPDFCDFofGeneralLoopEx1}.
\begin{figure}[tpbh!]
	\centering
	\begin{minipage}{0.42\textwidth}
	\begin{align*}
&x:=2\\\notag
&w:=0\\\notag
&dt:=1\\\notag
&\sigma:=0.1\\\notag
&\text{\bf while } true \text{ \bf do}\\\notag
&\quad w:=\text{Normal}(0,1)\\\notag
&\quad x:=x-\frac{1}{4}x^3\ast dt -\frac{1}{2}x^2\ast \sigma\ast w\\
& \text{\bf end while }
\end{align*}
	\end{minipage}
	\begin{minipage}{0.56\textwidth}
	\includegraphics[width=\textwidth]{Figures/pdfGeneralSDEusingGC.eps}
% 	\includegraphics[width=5.5cm,height=3cm]{Figures/HistogramGeneralLoopExample1Loop1000Sample1000.eps}\\
% 	\includegraphics[width=5.5cm,height=3cm]{Figures/PDFGeneralLoopExample1.eps}
    %  \includegraphics[width=3.9cm]{Figures/CDFGeneralLoopExample1.eps}
	\end{minipage}
	\caption{Left: Probabilistic program of the SDE in \eqref{eq:SDE2} (left).  Sampled data from $x$ from executing the PP (sample size=1000 and loop iteration=1000) and the GC estimate of underlying distribution compared to the kernel density estimate of the sampled data (right). The first 6 empirical moments are used for estimation. %Right: CDF (GC estimate and the sampled distribution).
	}
	\label{fig:HistogramPDFCDFofGeneralLoopEx1}
\end{figure}



% \begin{align}
% &x:=2\\\notag
% &w:=0\\\notag
% &dt:=1\\\notag
% &\sigma:=0.1\\\notag
% &\text{while true:}\\\notag
% &\quad w:=\text{Normal}(0,1)\\\notag
% &\quad x:=x-\frac{1}{4}x^3\ast dt -\frac{1}{2}x^2\ast \sigma\ast w
% \end{align}
Currently,  we are not able to theoretically compute moments of the probabilistic program. We can, nevertheless, approximate them by carrying out a Monte-Carlo experiment (i.e. running the program   and stopping at a fix loop iteration) in order to obtain empirical moments from sampled data. For  the specific value  of  $\sigma=0.1$,
% \Ahmad{parameter $\sigma=0.1$} \efi{which parameters?}, 
the program generates data whose histogram in the left panel of Figure \ref{fig:HistogramPDFCDFofGeneralLoopEx1} indicates the distribution for the output random variable $x$ is bimodal. Here we use the first 6 (empirical) moments  and apply the Gram-Charlier expansion  to reconstruct the target distribution. The estimated pdf as well as the sampled data and their kernel density estimate are presented in Figure~\ref{eq:SDE2} (right panel). 


\efi{what does this sentence say? With the help of  statistical tools, we  evaluate   our estimations to see if  the probabilistic programs generate data with the estimated distributions. We refer to Section~\ref{section:Evaluation} for evaluation of estimations for the benchmark programs.}  













% \multirow{3}{*}{Sum Rand. Series}&1&$\E(x(n)) = n^2/4 + n/4$  \\\cline{2-3}
%     &2& $\E(x^2(n)) = n^4/16 + 5n^3/24 + 3n^2/16 + n/24$  \\\cline{2-3}
%     &3&$\E(x^3(n)) = n^6/64 + 7n^5/64 + 13n^4/64 + 9n^3/64 + n^2/32$    \\\hline
%         \hline        
 
% \multirow{3}{*}{Prod. Dep. Var.}&1&$\E(p(n)) = n^2/4 - n/4$  \\\cline{2-3}
%     &2& $\E(p^2(n)) = n^4/16 - n^3/8 + 3n^2/16 - n/8$  \\\cline{2-3}
%     &3& \multirow{3}{*}{}$\E(p^3(n)) = n^6/64 - 3n^5/64 + 9n^4/64 - 21n^3/64$ \\
%     & &+ $15n^2/32 -n/4$    \\\hline
%         \hline        
        
% \multirow{3}{*}{Bimodal}&1&$\E(x(n)) =  - n/4$ \\\cline{2-3}
%     &2& $\E(x^2(n)) = 3n^2/16 + 67n/72 + 4/9$   \\\cline{2-3}
%     &3&$\E(x^3(n)) = -5n^3/64 - 37n^2/48 - 3n/8 + 1/3$   \\\hline
%         \hline   

        

==> data/Vasicek2.tex <==


a := 0.5
b := 0.2
σ := 0.2
w := 0
r := 2
while true:
  w := Normal(0, 1)
  r := (1 − a)r + a*b + σ*w


-------------------
- Analysis Result -
-------------------

E(r) = 2; 2**(-n)*(2**n + 9)/5
Solution is exact
E(r | n=100) = 253530120045645880299340641077/1267650600228229401496703205376 ≅ 0.200000000000000

E(r**2) = 4; 7/75 + 18*2**(-n)/25 + 239*2**(-2*n)/75
Solution is exact
E(r**2 | n=100) = 149980884130839092383916461952754551334236604588804957602669/1606938044258990275541962092341162602522202993782792835301376 ≅ 0.0933333333333333

E(r**3) = 8; 8**(-n)*(239*2**n + 63*4**n + 5*8**n + 693)/125
Solution is exact
E(r**3 | n=100) = 81481439053379443450737827537185023216365266845510598919987987673794078674015657532856473/2037035976334486086268445688409378161051468393665936250636140449354381299763336706183397376 ≅ 0.0400000000000000

E(r**4) = 16; 2**(-4*n)*(43*2**(4*n) + 540*2**(3*n) + 3346*2**(2*n) + 8316*2**n + 17755)/1875
Solution is exact
E(r**4 | n=100) = 59219597204126436989442413011855738679145584841728838252514556454886256672408394853108933389625452502820767086708240601/2582249878086908589655919172003011874329705792829223512830659356540647622016841194629645353280137831435903171972747493376 ≅ 0.0229333333333333

E(r**5) = 32; 2**(-5*n)*(123*2**(5*n) + 1935*2**(4*n) + 11950*2**(3*n) + 48510*2**(2*n) + 88775*2**n + 148707)/9375
Solution is exact
E(r**5 | n=100) = 42946884775597381334573048822911077251919481576989991755124800942140761042733912071887585838142022029768983929394608421699637813635503080332355671357/3273390607896141870013189696827599152216642046043064789483291368096133796404674554883270092325904157150886684127560071009217256545885393053328527589376 ≅ 0.0131200000000000

E(r**6) = 64; 2**(-6*n)*(1229*2**(6*n) + 19926*2**(5*n) + 154155*2**(4*n) + 623700*2**(3*n) + 1864275*2**(2*n) + 2676726*2**n + 3659989)/140625
Solution is exact
E(r**6 | n=100) = 36264921842878153571639105881185156521580337367664624127957672288901956281099069362776500776899554565851166879332188330544999827221389308132321888632909870492299823163071732165189/4149515568880992958512407863691161151012446232242436899995657329690652811412908146399707048947103794288197886611300789182395151075411775307886874834113963687061181803401509523685376 ≅ 0.00873955555555556

E(r**7) = 128; 2**(-7*n)*(4181*2**(7*n) + 77427*2**(6*n) + 617337*2**(5*n) + 3128895*2**(4*n) + 9321375*2**(3*n) + 21859929*2**(2*n) + 25619923*2**n + 29370933)/703125
Solution is exact
E(r**7 | n=100) = 31278404557331555034701623040914634656167423086083456156766362702659579153171254629832650079870748091303698134448546411992295494282693334866367516710555464058758582123882604560113739560579007664916682138937633/5260135901548373507240989882880128665550339802823173859498280903068732154297080822113666536277588451226982968856178217713019432250183803863127814770651880849955223671128444598191663757884322717271293251735781376 ≅ 0.00594631111111111

E(r**8) = 256; 2**(-8*n)*(46955*2**(8*n) + 903096*2**(7*n) + 8224468*2**(6*n) + 42960456*2**(5*n) + 160327650*2**(4*n) + 374741640*2**(3*n) + 717357844*2**(2*n) + 704902392*2**n + 690535499)/10546875
Solution is exact
E(r**8 | n=100) = 29686197825979122483144954390572284923930250139993009936185830000520152338839023081641180484786642282433946112372019741643745567514422084630227190246209822387957001403434044596220966652898047036100720692016431132255698829984912102724515761/6668014432879854274079851790721257797144758322315908160396257811764037237817632071521432200871554290742929910593433240445888801654119365080363356052330830046095157579514014558463078285911814024728965016135886601981690748037476461291163877376 ≅ 0.00445202962962963

E(r**9) = 512; 2**(-9*n)*(20083*2**(9*n) + 422595*2**(8*n) + 3997036*2**(7*n) + 23847516*2**(6*n) + 91722330*2**(5*n) + 268564842*2**(4*n) + 512398460*2**(3*n) + 822386124*2**(2*n) + 690535499*2**n + 586105515)/5859375
Solution is exact
E(r**9 | n=100) = 28971660817196551215770391622053942220586843408638230430695122534651023736937175953318538441972273492466562962635319988358915515574566103043159448389609991936435689058349888480144827004813194240325030545689885603381082801013465370689821514002448419952380726545067749957/8452712498170643941637436558664265704301557216577944354047371344426782440907597751590676094202515006314790319892114058862117560952042968596008623655407033230534186943984081346699704282822823056848387726531379014466368452684024987821414350380272583623832617294363807973376 ≅ 0.00342749866666667

E(r**10) = 1024; 2**(-10*n)*(248069*2**(10*n) + 5422410*2**(9*n) + 56111225*2**(8*n) + 347691960*2**(7*n) + 1527462650*2**(6*n) + 4609322172*2**(5*n) + 11016566890*2**(4*n) + 17622559800*2**(3*n) + 24168742465*2**(2*n) + 17583165450*2**n + 13062706909)/87890625
Solution is exact
E(r**10 | n=100) = 30243051369368479065924818887093930259555860295286037811428443049326984815308826250630029488486876242907115877511165375938365244482659680813374744284381961810350034679590221740546855862357410930250928086911333845150303793313754208581573881355989648252003025109644410242401807502359866531233537969949/10715086071862673209484250490600018105614048117055336074437503883703510511249361224931983788156958581275946729175531468251871452856923140435984577574698574803934567774824230985421074605062371141877954182153046474983581941267398767559165543946077062914571196477686542167660429831652624386837205668069376 ≅ 0.00282247395555556





==> evaluation.tex <==
%!TEX root = samplepaper.tex


%vs exact, psi, sampling; some moms; (measure: #moms b4 close match?)
%exact - limited complexity, arbitrary iteration
%psi - more complex, limited # iterations
%sampling - not precise,
%witheld moms - 'ability to generalize' within the class of distributions (PP encodable) 
%\newpage
\section{Evaluation}\label{section:Evaluation}

We evaluate how well do the two approaches estimate distributions of random variables involved in  probabilistic programs (and probabilistic loops in particular) using their given exact moments.

% We evaluate against a few sets of benchmarks:
% (1) against loops encoding a known distribution; 
% (2) against loop-free programs, with fully characterized distributions; %PSI
% (3a) against complex programs encoding a distribution that cannot be easily characterized - using sampling;
% (3b) against complex programs encoding a distribution that cannot be easily characterized - against exact moments. %only use subset of computed moments to approximate a distribution, use the remaining moments to check accuracy
% For each set of benchmarks we also give a detailed case study of one of the benchmarks - we discuss the underlying probabilistic program, distribution it encodes, how we measure the goodness of fit. 



%\paragraph{KL Divergence.} 
Table~\ref{table:DKL-Chi2-K-SforBenchmarks} provides us with the Kulback-Leibler distance for benchmark programs in which $D_{KL}$ is the distance between sampled distributions (as the target distribution are not known) and the estimated ones using either ME or GC methods. For the benchmark programs, Table~\ref{table:DKL-Chi2-K-SforBenchmarks}  also includes  $D^\ast$ statistics  for Kolmogorov–Smirnov goodness-of-fit test as well as $\chi^2$ statistics for Chi-Square goodness-of-fit test. In Kolmogorov-Smirnov test, We reject the null hypothesis, that sampled data follow the estimated distribution, if $D^\ast$ is greater than $CV_{\text{K-S}}=0.0608$, the critical value with respect to the significance level $\alpha=0.05$ and sample size 1000. For Chi-Square test: we reject the null hypothesis, that the sampled data follow the estimated distribution, if  $\chi^2$ is greater than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$, where $k=15$ is the number of bins that the sample data belongs to, and  $\alpha=0.05$ is the significance level. 

 

% , we can not reject the null hypothesis $\text{H}_0$, which states the sampled data as outputs of  probabilistic programs  follow the  distributions estimated using moments. 



% In order to assess the our estimations, we set the number of loop in the StutteringP program to be 100 and we take 1000 sample for the output $s$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments.   To perform the $\chi^2$ goodness-of-fit test for the StutteringP benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the maximum entropy estimated distribution  is $\chi^2=15.1544$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program StutteringP follow the  distribution estimated using  moments calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 


% %%%% Square Chi2 Evaluation 
% In order to assess the our estimations, we fix the number of loop in the Square program to be 1000 and we take 1000 sample for the output, i.e. the variable $y$ by running the program 1000 times. We would like to see if the data comes from the  estimated distribution with the use of moments (cumulants).   To perform the $\chi^2$ goodness-of-fit test for the Square benchmark problem, we set  again $k=15$ and $\alpha=0.05$. The test statistic for our sampled data and the Gram-Charlier estimated distribution  is $\chi^2=9.9100$ which is not larger than the upper-tail critical value $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,14}=23.685$ (based on \url{https://www.itl.nist.gov/div898/handbook/eda/section3/eda3674.htm}), we  can not reject the null hypothesis. Therefore,   the sampled data obtained through running the prob-solvable program Square  follow the  distribution estimated using  moments (cumulants) calculated by Mora \cite{bartocci2019automatic,bartocci2020mora}. 




% \bigskip
% \bigskip




\begin{table}[tpbh!]
    \centering
     \scalebox{0.8}{
 \begin{tabular}{c|l|l|l|l|l|l}
\hline
          {\bf Program}   & $D_{KL}$ (ME) &  $D_{KL}$ (GC) & $D^\ast$ (ME) & $D^\ast$ (GC)& $\chi^2$ (ME) &$\chi^2$ (GC)\qquad\\
                         \hline\hline
     StutteringP& 0.005858 & 0.005831& 0.0181 \cmark & 0.0213 \cmark & 18.6432 \cmark& 16.7943 \cmark\\%\hline
     Square & 0.005116 & 0.007204 & 0.0586 \cmark & 0.0566 \cmark& 36.9009 \xmark& 39.1309 \xmark \\%\hline
     Binomial & 0.003779 & 0.003844 & 0.0598 \cmark &  0.0597 \cmark & 27.4661 \xmark& 27.4574 \xmark\\%\hline
     \hspace{2mm} Random Walk 1D \hspace{2mm}& 0.006410 \hspace{2mm} & 0.006710 \hspace{2mm}&  0.0264 \cmark \hspace{2mm}&  0.0263 \cmark \hspace{2mm}& 18.6709 \cmark \hspace{2mm}& 18.7068 \cmark \hspace{2mm}\\%\hline
    Uniform (Cont.) & 0.062240 & 0.007650 & 0.0214 \cmark & 0.0658 \xmark & 16.3485 \cmark& 105.276 \xmark\\%\hline
     PDP Model & 0.006180 & 0.009348 & 0.0403 \cmark & 0.0393 \cmark & 64.4182 \cmark $^{\ast\ast}$& 65.9500 \cmark $^{\ast\ast}$\\\hline
\end{tabular}
}
\vspace{2mm}
 \caption{Kullback-Leibler distance, $D^\ast$  (Kolmogorov–Smirnov statistics) and $\chi^2$ (Chi-Square statistics) for the benchmark probabilistic programs.  \xmark \; means that the null hypothesis of the underlying test is rejected while \cmark states that we can not reject the null hypothesis which means there is no evidence against null hypothesis. \\
 $^{\ast\ast}$ Chi-Square test accepts null hypothesis when the number of bins $k$ is at least 50, for which $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,49}=66.339$. }
 \label{table:DKL-Chi2-K-SforBenchmarks}
      
\end{table}
Based on Table~\ref{table:DKL-Chi2-K-SforBenchmarks}, one can see that our distribution estimation methods work very well for continuous random variables and goodness of fit tests accept the null hypothesis that sampled data (generated by executing of PP) follow the estimated distributions. For discrete random variables (e.g. in Square and Binomial PPs), Chi-Square goodness of fit test rejects the null hypothesis while Kolmogorov-Smirnov accepts it.

We note that  Chi-Square test is sensitive to the choice of bins while Kolmogorov–Smirnov is independent of this issue. In PDP model The test rejects the null hypothesis for the $\alpha=0.05$ and  $k=15$, while Kolmogorov–Smirnov accept the null hypothesis. Increasing the number of bins to $k=50$, Chi-Square test accepts the null hypothesis as the test statistics $\chi^2$ for both ME and GC methods are below $\chi^2_{1-\alpha,k-1}=\chi^2_{0.95,49}=66.339$. 

\bigskip



%%%%%%%%%%%%%%%%%%%%%%
We further investigate the precision of higher moments.  As explained in \ref{ssec:methods-of-evaluation},  we first use 2 exact moments of each benchmark program and estimate the target distribution using these moments. Having the distribution for the variable of interest, we compute moments of order 3 to 8 and we call them estimated moments.  Table~\ref{table:AbsoluteandRelativeErrors}, shows absolute  (and relative) sample errors, absolute (and relative) estimate errors for Maximum Entropy method, as well as  absolute (and relative) estimate errors for Gram-Charlier method. Results expose practical evidence of the high accuracy of our methods for estimating distributions of probabilistic loop outputs.  Comparing  columns of sample error and estimate error shows the importance of the distribution recovery as the errors (absolute and relative) of moments obtained by estimated distribution are less than the errors of moments calculated by sampled data. However, Gram-Charlier method fail to estimate Uniform distribution as the relative estimate errors for this method are rather high comparing to the sample errors and ME estimate errors.
Maximum Entropy estimates the Uniform distribution in a high accuracy level.



% As shown in the Tables~\ref{table:DKL-Chi2-K-SforBenchmarks} and \ref{table:AbsoluteandRelativeErrors}, the relative estimate errors for Gram-Charlier method are rather high comparing to the sample errors and ME estimate errors. Therefore, Gram-Charlier method fail to estimate Uniform distribution using its moments while Maximum Entropy estimates the distribution in a high accuracy level. 
 


% Comparing first 8 moments of the underlying variable yields absolute estimate errors as \textit{absolute error of }$\E(x^i)= |{\E(x^i)}_{estimate}-{\E(x^i)}_{exact}|$. Normalizing obtained errors with the exact moments we reach the \textit{relative estimate errors}\footnote{Moments above 5 for the Square benchmark could not be computed within ~30 minutes.}. The same process is done for the \textit{absolute} and \textit{relative sample errors}, but instead of estimated moments we compare  sample moments to the exact ones. 

In complex PPs, calculating exact higher moments is (time) expensive. For example, for Square probabilistic program and PDP model for gene circuits, calculating moments higher than fifth order is not possible within $\sim30$ minutes. Using our methods of estimation one can approximate higher moments of complex PPs much faster as it only needs to estimate distribution using the first few moments (which takes few seconds).  
 
\begin{table}[tpbh!]
    \centering
    \scalebox{0.7}{
 \begin{tabular}{c|c|c|l|l|l|l}
\hline
  {\bf Program}  &\#Mom. & Moment &   Exact Value$^{1}$  &Absol. sample error$^{2}$   & Absol. ME est. error$^{3}$ & Absol. GC est. error$^{3}$  \\
    & for est.& & & (relative error$^\ast$)&  (relative error$^\ast$) &  (relative error$^\ast$)\\
                         \hline
                         \hline
 


 \multirow{3}{*}{StutteringP}&&1& 210 & $5.69\times 10^{-2} (0.027\%)$  &$8.08\times 10^{-5} (0.00003\%)$&$4.71\times 10^{-5} (0.00002\%)$\\%\cline{2-6}
    &2&2& $4.4405 \times 10^4 $ &  $2.39 \times 10^{1} (0.053\%)$& $1.75 \times 10^{-2} (0.00003\%)$&$1.75 \times 10^{-2} (0.00003\%)$\\%\cline{2-6}
    &&3& $9.4536\times 10^6$  & $6.78 \times 10^{3} (0.0.072\%)$ & $9.21 \times 10^{1} (0.000974\%)$ & $9.25 \times 10^{1} (0.000978\%)$\\%\cline{2-6}
    &&4& $2.0260\times 10^9$  & $1.48 \times 10^{6} (0.073\%)$& $7.38 \times 10^{4} (0.00364\%)$   & $7.42 \times 10^{4} (0.00366\%)$\\%\cline{2-6}
    &&5& $4.3705\times 10^{11}$  & $2.17 \times 10^{8} (0.050\%)$ & $3.82 \times 10^{7} (0.00873\%)$ & $3.83 \times 10^{7} (0.00876\%)$ \\%\cline{2-6}
    &&6&  $9.4884\times 10^{13}$ & $5.51 \times 10^{9} (0.0058\%)$ & $1.60 \times 10^{10} (0.0168\%)$  & $1.60 \times 10^{10} (0.0168\%)$\\%\cline{2-6}
    &&7& $2.0729\times 10^{16}$  & $2.10 \times 10^{13} (0.101\%)$& $5.88 \times 10^{12} (0.0284\%)$  & $5.90 \times 10^{12} (0.0285\%)$\\%\cline{2-6}
    &&8& $4.5570\times 10^{18}$  &$1.12 \times 10^{16} (0.245\%)$ &  $1.99 \times 10^{15} (0.0438\%)$  & $2.00 \times 10^{15} (0.0439\%)$
    \\\hline
        \hline

 \multirow{3}{*}{Square$^{\ast\ast}$}&&1& 10100 & $1.66\times 10^1 (0.16\%)$  &  $1.11\times 10^{0} (0.011\%)$  & $7.97\times 10^{-3} (0.00007\%)$ \\%\cline{2-6}
    &2&2& $1.0602 \times 10^8$ & $2.31\times 10^5 (0.22\%)$ & $2.30\times 10^3 (0.00217\%)$   & $1.64\times 10^{2} (0.00015\%)$ \\%\cline{2-6}
    &&3& $1.1544\times 10^{12}$  &$1.27\times 10^{9} (0.11\%)$  &  $1.26\times 10^7 (0.0011\%)$  &$2.39\times 10^{9} (0.2072\%)$\\%\cline{2-6}
    &&4& $1.3012\times 10^{16}$  & $2.98\times 10^{13} (0.23\%)$& $1.99\times 10^{12} (0.0153\%)$   &$9.79\times 10^{13} (0.7581\%)$ \\%\cline{2-6}
    &&5& $1.5157\times 10^{20}$  & $1.32\times 10^{18} (0.87\%)$& $8.83\times 10^{16} (0.0583\%)$    &$2.61\times 10^{18} (1.7505\%)$
    \\\hline
        \hline

\multirow{3}{*}{Binomial}&&1& 50 & $2.95\times 10^{-1} (0.59\%)$  &  $5.19\times 10^{-5} (0.000051\%)$ & $3.16\times 10^{-3} (0.0063\%)$\\%\cline{2-6}
    &2&2&   2525  & $2.82\times 10^{1} (1.12\%)$ & $2.74\times 10^{-3} (0.000108\%)$  & $1.87\times 10^{-1} (0.0074\%)$ \\%\cline{2-6}
    &&3& 128750  & $2.04\times 10^{3} (1.59\%)$ & $1.43\times 10^{-1} (0.000111\%)$  & $1.22\times 10^{1} (0.0095\%)$ \\%\cline{2-6}
    &&4&  $6.6268\times 10^{6}$  &$1.32\times 10^{5} (2.00\%)$ & $3.66\times 10^{0} (0.000055\%)$  & $8.22\times 10^{2} (0.0125\%)$ \\%\cline{2-6}
    &&5&  $3.4421\times 10^{8}$ &$8.08\times 10^{6} (2.35\%)$ &  $5.52\times 10^{2} (0.000160\%)$ & $5.53\times 10^{4} (0.0161\%)$ \\%\cline{2-6}
    &&6& $1.8038\times 10^{10}$ & $4.67\times 10^{8} (2.64\%)$& $1.20\times 10^{5} (0.000664\%)$   & $3.66\times 10^{6} (0.0203\%)$\\%\cline{2-6}
    &&7&  $9.5354\times 10^{11}$ &$2.74\times 10^{10} (2.87\%)$ &  $1.51\times 10^{7} (0.001587\%)$  & $2.38\times 10^{8} (0.0250\%)$\\%\cline{2-6}
    &&8&  $5.0830\times 10^{13}$ &$1.54\times 10^{12} (3.04\%)$ &  $1.54\times 10^{9} (0.0030363\%)$   & $1.51\times 10^{10} (0.0298\%)$
         \\\hline
        \hline



 \multirow{3}{*}{RandomWalk1D}&&1& 20 & $1.57\times 10^{-1} (0.79\%)$  &$1.83\times 10^{-6} (0.000009\%)$ & $4.44\times 10^{-3} (0.022\%)$\\%\cline{2-6}
    &2&2& $4.2933\times 10^{2} $ &  $6.78 \times 10^{0} (1.58\%)$& $6.76 \times 10^{-5} (0.00001\%)$ & $1.90\times 10^{-1} (0.0044\%)$\\%\cline{2-6}
    &&3& $9.7516\times 10^{3}$  & $2.45 \times 10^{2} (2.51\%) $& $8.40 \times 10^{0} (0.09\%)$  & $5.61\times 10^{-1} (0.0057\%)$\\%\cline{2-6}
    &&4&  $2.3230\times 10^{5}$ & $8.38\times 10^{3} (3.61\%)$&  $6.48\times 10^{2} (0.28\%)$  & $3.54\times 10^{2} (0.15\%)$\\%\cline{2-6}
    &&5& $5.7681\times 10^{6}$  & $2.79\times 10^{5} (4.48\%)$&  $3.37\times 10^{4} (0.58\%)$ &$2.32\times 10^{4} (0.40\%)$ \\%\cline{2-6}
    &&6&  $1.4858\times 10^{8}$ & $9.19\times 10^{6} (6.19\%)$&  $1.48\times 10^{6} (0.98\%)$ & $1.12\times 10^{6} (0.75\%)$ \\%\cline{2-6}
    &&7& $3.9565\times 10^{9}$  & $3.03\times 10^{8} (7.66\%)$& $5.94\times 10^{7} (1.48\%)$  & $4.72\times 10^{7} (1.18\%)$ \\%\cline{2-6}
    &&8& $1.0857\times 10^{11}$  & $1.01\times 10^{10} (9.26\%)$&  $2.26\times 10^{9} (2.04\%)$  & $1.85\times 10^{9} (1.67\%)$
    \\\hline
        \hline

 \multirow{3}{*}{Uniform (Cont.)}&&1& 0.5 & $5.92\times 10^{-3} (1.18\%)$  & $1.47\times 10^{-9} (3\times 10^{-7}\%)$ & $3.28\times 10^{-2} (7.03\%)$\\%\cline{2-6}
    &6&2& 0.333333 & $4.94\times 10^{-3} (1.48\%)$ &   $1.66\times 10^{-5} (0.00499\%)$& $3.40\times 10^{-2} (11.36\%)$\\%\cline{2-6}
    &&3& 0.25  & $4.57\times 10^{-3} (1.83\%)$ & $2.50\times 10^{-5} (0.00998\%)$  & $3.46\times 10^{-2} (16.06\%)$ \\%\cline{2-6}
    &&4&  0.20  &$4.57\times 10^{-3} (2.28\%)$ &  $3.33\times 10^{-5} (0.0166\%)$  & $3.43\times 10^{-2} (20.69\%)$\\%\cline{2-6}
    &&5&  0.166667  & $4.66\times 10^{-3} (2.80\%)$&   $4.18\times 10^{-5} (0.0249\%)$ &$3.35\times 10^{-2} (25.18\%)$ \\%\cline{2-6}
    &&6&  0.142857 &$4.74\times 10^{-3} (3.32\%)$ &   $4.99\times 10^{-5} (0.0349\%)$ & $3.25\times 10^{-2} (29.51\%)$\\%\cline{2-6}
    &&7&  0.125 &$4.76\times 10^{-3} (3.81\%)$ &     $5.82\times 10^{-5} (0.00465\%)$ &$3.15\times 10^{-2} (33.65\%)$\\%\cline{2-6}
    &&8&  0.1111111 &$4.73\times 10^{-3} (4.25\%)$ &  $6.66\times 10^{-5} (0.00599\%)$ &  $3.04\times 10^{-2} (37.60\%)$
         
    \\\hline
        \hline

 
 \multirow{3}{*}{PDP Model$^{\ast\ast}$}&&1& $1.1885\times 10^{3}$ & $1.60\times 10^{1}  (1.35\%)$  &$2.84\times 10^{-1}  (0.024\%)$ &$5.74\times 10^{0}  (0.48\%)$ \\%\cline{2-6}
    &3&2& $1.4767\times 10^{6}$ &  $3.93\times 10^{4} (2.66\%)$& $3.95\times 10^{2} (0.027\%)$ &$1.16\times 10^{4} (0.78\%)$ \\%\cline{2-6}
    &&3& $1.8981\times 10^{9}$  & $7.37 \times 10^{7} (3.88\%)$& $3.19\times 10^{6}(0.168\%)$ & $2.35\times 10^{7} (1.23\%)$\\%\cline{2-6}
     &&4& $2.5058\times 10^{12}$ & $1.28\times 10^{11}(5.01\%)$ &  $1.64\times 10^{10}$ (0.650\%)  & $4.85\times 10^{10} (1.90\%)$\\%\cline{2-6}
     &&5& $3.3804\times 10^{15}$  &$2.04\times 10^{14}(6.03\%)$  & $ 4.97\times 10^{13}$ (1.450\%) & $1.00\times 10^{14} (2.87\%)$\\%\cline{2-6}
%      &&6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\%\cline{2-6}
%      &&7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\%\cline{2-6}
%      &&8& $1.19415322490998\times 10^{24}$
%   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
%     & $2.95\times 10^{22} (2.4119\%)$\\\hline
        \hline


\end{tabular}
}
\vspace{2mm} 
 \caption{Error for Benchmarks:\\
 $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Appendix~\ref{Appendix}: Table ~\ref{Table:Benchmarks})\\
 $^{2}$ Error of exact moments and sample moments\\
 $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
 $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$\\
 $^{\ast\ast}$Moments of order above 5  could not be computed within ~30 minutes
 }
%  \label{Table:ErrorforBenchmarks}
\label{table:AbsoluteandRelativeErrors}
\end{table}



















%%%%backup last version

% \begin{table}[tpbh!]
%     \centering
%     \scalebox{0.7}{
%  \begin{tabular}{c|c|c|l|l|l|l}
% \hline
%   {\bf Program}  &\#Mom. & Moment &   Exact Value$^{1}$  &Absol. sample error$^{2}$   & Absol. ME est. error$^{3}$ & Absol. GC est. error$^{3}$  \\
%     & for est.& & & (relative error$^\ast$)&  (relative error$^\ast$) &  (relative error$^\ast$)\\
%                          \hline
%                          \hline
 


%  \multirow{3}{*}{StutteringP}&&1& 210 & $5.69\times 10^{-2} (0.027\%)$  &$8.08\times 10^{-5} (0.00003\%)$&$4.71\times 10^{-5} (0.00002\%)$\\%\cline{2-6}
%     &2&2& $4.4405 \times 10^4 $ &  $2.39 \times 10^{1} (0.053\%)$& $1.75 \times 10^{-2} (0.00003\%)$&$1.75 \times 10^{-2} (0.00003\%)$\\%\cline{2-6}
%     &&3& $9.453658199999997\times 10^6$  & $6.78 \times 10^{3} (0.0.072\%)$ & $9.21 \times 10^{1} (0.000974\%)$ & $9.25 \times 10^{1} (0.000978\%)$\\%\cline{2-6}
%     &&4& $2.026042602406666\times 10^9$  & $1.48 \times 10^{6} (0.073\%)$& $7.38 \times 10^{4} (0.00364\%)$   & $7.42 \times 10^{4} (0.00366\%)$\\%\cline{2-6}
%     &&5& $4.370501248066238\times 10^{11}$  & $2.17 \times 10^{8} (0.050\%)$ & $3.82 \times 10^{7} (0.00873\%)$ & $3.83 \times 10^{7} (0.00876\%)$ \\%\cline{2-6}
%     &&6&  $9.488480678476714\times 10^{13}$ & $5.51 \times 10^{9} (0.0058\%)$ & $1.60 \times 10^{10} (0.0168\%)$  & $1.60 \times 10^{10} (0.0168\%)$\\%\cline{2-6}
%     &&7& $2.072981561969703\times 10^{16}$  & $2.10 \times 10^{13} (0.101\%)$& $5.88 \times 10^{12} (0.0284\%)$  & $5.90 \times 10^{12} (0.0285\%)$\\%\cline{2-6}
%     &&8& $4.557008480549055\times 10^{18}$  &$1.12 \times 10^{16} (0.245\%)$ &  $1.99 \times 10^{15} (0.0438\%)$  & $2.00 \times 10^{15} (0.0439\%)$
%     \\\hline
%         \hline

%  \multirow{3}{*}{Square}&&1& 10100 & $1.66\times 10^1 (0.16\%)$  &  $1.11\times 10^{0} (0.011\%)$  & $7.97\times 10^{-3} (0.000078\%)$ \\%\cline{2-6}
%     &2&2& $1.060298 \times 10^8$ & $2.31\times 10^5 (0.22\%)$ & $2.30\times 10^3 (0.00217\%)$   & $1.64\times 10^{2} (0.000155\%)$ \\%\cline{2-6}
%     &&3& $1.1544847016\times 10^{12}$  &$1.27\times 10^{9} (0.11\%)$  &  $1.26\times 10^7 (0.0011\%)$  &$2.39\times 10^{9} (0.2072\%)$\\%\cline{2-6}
%     &&4& $1.301272653385280\times 10^{16}$  & $2.98\times 10^{13} (0.23\%)$& $1.99\times 10^{12} (0.0153\%)$   &$9.79\times 10^{13} (0.7581\%)$ \\%\cline{2-6}
%     &&5& $1.515712810699512\times 10^{20}$  & $1.32\times 10^{18} (0.87\%)$& $8.83\times 10^{16} (0.0583\%)$    &$2.61\times 10^{18} (1.7505\%)$
%     \\\hline
%         \hline

% \multirow{3}{*}{Binomial}&&1& 50 & $2.95\times 10^{-1} (0.59\%)$  &  $5.19\times 10^{-5} (0.000051\%)$ & $3.16\times 10^{-3} (0.0063\%)$\\%\cline{2-6}
%     &2&2&   2525  & $2.82\times 10^{1} (1.12\%)$ & $2.74\times 10^{-3} (0.000108\%)$  & $1.87\times 10^{-1} (0.0074\%)$ \\%\cline{2-6}
%     &&3& 128750  & $2.04\times 10^{3} (1.59\%)$ & $1.43\times 10^{-1} (0.000111\%)$  & $1.22\times 10^{1} (0.0095\%)$ \\%\cline{2-6}
%     &&4&  $6.6268625\times 10^{6}$  &$1.32\times 10^{5} (2.00\%)$ & $3.66\times 10^{0} (0.000055\%)$  & $8.22\times 10^{2} (0.0125\%)$ \\%\cline{2-6}
%     &&5&  $3.44215625\times 10^{8}$ &$8.08\times 10^{6} (2.35\%)$ &  $5.52\times 10^{2} (0.000160\%)$ & $5.53\times 10^{4} (0.0161\%)$ \\%\cline{2-6}
%     &&6& $1.803882346250000\times 10^{10}$ & $4.67\times 10^{8} (2.64\%)$& $1.20\times 10^{5} (0.000664\%)$   & $3.66\times 10^{6} (0.0203\%)$\\%\cline{2-6}
%     &&7&  $9.535413368750000\times 10^{11}$ &$2.74\times 10^{10} (2.87\%)$ &  $1.51\times 10^{7} (0.001587\%)$  & $2.38\times 10^{8} (0.0250\%)$\\%\cline{2-6}
%     &&8&  $5.083096302286250\times 10^{13}$ &$1.54\times 10^{12} (3.04\%)$ &  $1.54\times 10^{9} (0.0030363\%)$   & $1.51\times 10^{10} (0.0298\%)$
%          \\\hline
%         \hline



%  \multirow{3}{*}{RandomWalk1D}&&1& 20 & $1.57\times 10^{-1} (0.79\%)$  &$1.83\times 10^{-6} (0.000009\%)$ & $4.44\times 10^{-3} (0.022\%)$\\%\cline{2-6}
%     &2&2& $429.333333333333 $ &  $6.78 \times 10^{0} (1.58\%)$& $6.76 \times 10^{-5} (0.00001\%)$ & $1.90\times 10^{-1} (0.0044\%)$\\%\cline{2-6}
%     &&3& $9751.60000000000$  & $2.45 \times 10^{2} (2.51\%) $& $8.40 \times 10^{0} (0.09\%)$  & $5.61\times 10^{-1} (0.0057\%)$\\%\cline{2-6}
%     &&4&  232303.040000000 & $8.38\times 10^{3} (3.61\%)$&  $6.48\times 10^{2} (0.28\%)$  & $3.54\times 10^{2} (0.15\%)$\\%\cline{2-6}
%     &&5& 5768119.43466667  & $2.79\times 10^{5} (4.48\%)$&  $3.37\times 10^{4} (0.58\%)$ &$2.32\times 10^{4} (0.40\%)$ \\%\cline{2-6}
%     &&6&  148588624.477714 & $9.19\times 10^{6} (6.19\%)$&  $1.48\times 10^{6} (0.98\%)$ & $1.12\times 10^{6} (0.75\%)$ \\%\cline{2-6}
%     &&7& 3956546143.08960  & $3.03\times 10^{8} (7.66\%)$& $5.94\times 10^{7} (1.48\%)$  & $4.72\times 10^{7} (1.18\%)$ \\%\cline{2-6}
%     &&8& 108576810406.772  & $1.01\times 10^{10} (9.26\%)$&  $2.26\times 10^{9} (2.04\%)$  & $1.85\times 10^{9} (1.67\%)$
%     \\\hline
%         \hline

%  \multirow{3}{*}{Uniform (Cont.)$^{\ast\ast}$}&&1& 0.5 & $5.92\times 10^{-3} (1.18\%)$  & $1.47\times 10^{-9} (3\times 10^{-7}\%)$ & $3.28\times 10^{-2} (7.03\%)$\\%\cline{2-6}
%     &6&2& 0.333333 & $4.94\times 10^{-3} (1.48\%)$ &   $1.66\times 10^{-5} (0.00499\%)$& $3.40\times 10^{-2} (11.36\%)$\\%\cline{2-6}
%     &&3& 0.25  & $4.57\times 10^{-3} (1.83\%)$ & $2.50\times 10^{-5} (0.00998\%)$  & $3.46\times 10^{-2} (16.06\%)$ \\%\cline{2-6}
%     &&4&  0.20  &$4.57\times 10^{-3} (2.28\%)$ &  $3.33\times 10^{-5} (0.0166\%)$  & $3.43\times 10^{-2} (20.69\%)$\\%\cline{2-6}
%     &&5&  0.166667  & $4.66\times 10^{-3} (2.80\%)$&   $4.18\times 10^{-5} (0.0249\%)$ &$3.35\times 10^{-2} (25.18\%)$ \\%\cline{2-6}
%     &&6&  0.142857 &$4.74\times 10^{-3} (3.32\%)$ &   $4.99\times 10^{-5} (0.0349\%)$ & $3.25\times 10^{-2} (29.51\%)$\\%\cline{2-6}
%     &&7&  0.125 &$4.76\times 10^{-3} (3.81\%)$ &     $5.82\times 10^{-5} (0.00465\%)$ &$3.15\times 10^{-2} (33.65\%)$\\%\cline{2-6}
%     &&8&  0.1111111 &$4.73\times 10^{-3} (4.25\%)$ &  $6.66\times 10^{-5} (0.00599\%)$ &  $3.04\times 10^{-2} (37.60\%)$
         
%     \\\hline
%         \hline

 
%  \multirow{3}{*}{PDP Model$^{\ast\ast\ast}$}&&1& $1.18857142821508\times 10^{3}$ & $1.60\times 10^{1}  (1.35\%)$  &$2.84\times 10^{-1}  (0.024\%)$ &$0.012 (0.0014\%)$ \\%\cline{2-6}
%     &3&2& $1.47673843347401\times 10^{6}$ &  $3.93\times 10^{4} (2.66\%)$& $3.95\times 10^{2} (0.027\%)$ &$2.362\times 10^{1} (0.0029\%)$ \\%\cline{2-6}
%     &&3& $1.89812214743201\times 10^{9}$  & $7.37 \times 10^{7} (3.88\%)$& $3.19\times 10^{6}(0.168\%)$ & $4.35\times 10^{4} (0.0054\%)$\\%\cline{2-6}
%      &&4& $2.50589193271731\times 10^{12}$ & $1.28\times 10^{11}(5.01\%)$ &  $1.64\times 10^{10}$ (0.650\%)  & $4.67\times 10^{8} (0.0573\%)$\\%\cline{2-6}
%      &&5& $3.38043447836444\times 10^{15}$  &$2.04\times 10^{14}(6.03\%)$  & $ 4.97\times 10^{13}$ (1.450\%) & $2.26\times 10^{12} (0.2630\%)$\\%\cline{2-6}
% %      &&6& $9.31994079132823\times 10^{17}$  & $6.33\times 10^{16}(6.79\%)$& $2.16\times 10^{16}$ (2.27\%)   & $6.42\times 10^{15} (0.6842\%)$ \\%\cline{2-6}
% %      &&7& $1.04195827518657\times 10^{21}$  & $9.27\times 10^{19}(8.90\%)$&  $4.11\times 10^{19}$ (3.79\%)  & $1.46\times 10^{19} (1.3837\%)$ \\%\cline{2-6}
% %      &&8& $1.19415322490998\times 10^{24}$
% %   & $1.33\times 10^{23}(11.18\%)$& $7.23\times 10^{22}$ (5.71\%)   
% %     & $2.95\times 10^{22} (2.4119\%)$\\\hline
%         \hline


% \end{tabular}
% }
% \vspace{2mm} 
%  \caption{Error for Benchmarks:\\
%  $^{1}$ Exact value of moments at the iteration loop $n=100$ (See Table ~\ref{Table:Benchmarks})\\
%  $^{2}$ Error of exact moments and sample moments\\
%  $^{3}$ Error of exact moments and the ones calculated by the  estimated distribution\\
%  $^\ast$ Relative error ($\%$)=$\frac{\text{Absolute Error}}{\text{Exact Value}}\times 100$\\
%  $^{\ast\ast}$ Distributions are estimated using 6 moments.
%  }
% %  \label{Table:ErrorforBenchmarks}
% \label{table:AbsoluteandRelativeErrors}
% \end{table}







 %  Sum Rand. Series & -- & -- & & & & \\\hline
    %  Prod. Rand. Var. & -- & -- & & & & \\\hline
    % Bimodal & -- & -- & & & & \\\hline

% \multirow{3}{*}{Sum Rand. Series}&&1& 0.5 &   &   &\\\cline{2-6}
%     &&2&     &  &   & \\\cline{2-6}
%     &&3&   &  &   & \\\cline{2-6}
%     &&4&    & &    & \\\cline{2-6}
%     &&5&    & &    & \\\cline{2-6}
%     &&6&   & &    & \\\cline{2-6}
%     &&7&   & &    & \\\cline{2-6}
%     &&8&   & &     &
         
%     \\\hline
%         \hline
        
%         \multirow{3}{*}{Prod. Rand. Var}&&1& 0.5 &   &   &\\\cline{2-6}
%     &&2&     &  &   & \\\cline{2-6}
%     &&3&   &  &   & \\\cline{2-6}
%     &&4&    & &    & \\\cline{2-6}
%     &&5&    & &    & \\\cline{2-6}
%     &&6&   & &    & \\\cline{2-6}
%     &&7&   & &    & \\\cline{2-6}
%     &&8&   & &    & 
         
%     \\\hline
%         \hline
        
%         \multirow{3}{*}{Bimodal}&1& 0.5 &   &  & \\\cline{2-6}
%     &&2&     &  &   & \\\cline{2-6}
%     &&3&   &  &   & \\\cline{2-6}
%     &&4&    & &    & \\\cline{2-6}
%     &&5&    & &    & \\\cline{2-6}
%     &&6&   & &    & \\\cline{2-6}
%     &&7&   & &    & \\\cline{2-6}
%     &&8&   & &     &
         
%     \\\hline
%         \hline



% , however, $D_{KL}$ is a small number in these cases. Therefore,  Kullback-Leibler distance would not be a proper tool to decide on the quality of  estimations in probabilistic programs. 

==> methodology.tex <==
%!TEX root = samplepaper.tex
\section{Methodology}\label{section:Methodology}
Maximum Entropy is applied to estimate the distribution of the random variable generated in the probabilistic program  \textit{Random Walk 1D} using its calculated moments via moment-based invariant generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. The target distribution is unknown and  only moments of the random variable of interest, expressed as a function of loop iteration, are available (Equations~(\ref{eq:ExactmomentsofRandomWalk1}-\ref{eq:ExactmomentsofRandomWalk3})). 

In order to reconstruct the distribution of random variable $x$ in the probabilistic program Random Walk 1D, we fix the loop iteration to be $n=100$ and use the first three exact moments of $x$, i.e. $E[x(100)], E[x^2(100)]$ and $E[x^3(100)]$. Applying ME method to the given moments, we recover the pdf and the cdf of $x$ which is shown with red color in Figure~\ref{fig:pdfRandomwalk1DME1} (Middle and Right).  


In order to assess accuracy of distribution estimation, we carry out a Monte Carlo ``experiment'' by executing  the PP a \textit{large} number of times (here, large=1000), and  compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test. Results (see Figure~\ref{fig:pdfRandomwalk1DME1}) show visually the agreement of the estimated pdf and cdf with the sampled data (indeed, with the KS density approximation of the sampled data). Details and numerical result of the accuracy evaluation will be presented in Section~\ref{section:Evaluation}.

% Here, we apply the Maximum Entropy method  to estimate distributions of a random variable of probabilistic program  Random Walk 1D  using its calculated moments via moment-based invariants generator for prob-solvable loops \cite{bartocci2019automatic,bartocci2020mora}. Note that the target distribution is unknown and we have only moments of the random variable of interest presented as a function of loop iteration. With the help of  statistical tools, we also confirm the agreement of our estimated distributions with the ones generated during the execution of these probabilistic programs. 


% \todo{The following is not a correct statement: We assess the agreement or accuracy  of the estimated distributions with the ones generated during the execution of the probabilistic programs.}

% What you do is the following: 

% \begin{enumerate}
%     \item You estimate the distribution using ME and the exact moments provided by the recurrence-based algorithm in \cite{bartocci2020mora,bartocci2019automatic}
%     \item Assess accuracy of ME estimation of moments and the true moments with plots only (so far)!
%     \item To assess accuracy of distribution estimation, you carry out a monte carlo ``experiment,'' as follows: You repeat the PP a \textit{large} number of times (here, large=1000), and then compare the agreement of the sampled data with the estimated distribution via the chi-square test and Kolmogorov-Smirnov test.   
% \end{enumerate}

\efi{What about multivariate distribution approximation? That is, in a Prob PP, multiple random variables can be generated that are dependent so they have a joint distribution. I believe ME applies also in multivariate distribution estimation.}


\bigskip

\noindent{\bf Random Walk 1D} 
\begin{align}
&v:=0\\\notag
&x:=0\\\notag
&\text{while true:}\\\notag
&\quad v:=\text{uniform}(0,1)\\\notag
&\quad x:=x+v\;\;[7/10]\;\;x-v
\end{align}
Moments of the random variable $x$ are computed as functions of $n$, iteration of the loop and are available in Table~1 of  \cite{bartocci2019automatic}: 
\begin{align}\label{eq:ExactmomentsofRandomWalk1}
&E[x(n)] = n/5\\\label{eq:ExactmomentsofRandomWalk2}
&E[x^2(n)] = n^2/25 + 22n/75\\\label{eq:ExactmomentsofRandomWalk3}
&E[x^3(n)] = n^3/125 + n^222/125 - n21/250
\end{align}
Figure~\ref{fig:SampledEXforRandomWalk1Sample1000loop1} shows the agreement of sampled data and exact expected value of random variable $x$ per each loop iteration. One easily can see that the uncertainty propagates through probabilistic loop and remains around the exact expected value of the variable $x$. Figure~\ref{fig:SampledEXforRandomWalk1000Sample1000loop1} shows that the mean value and the second moment for a sample of size 1000 agrees the exact expected values for each loop iteration $n$. This shows the strength  of the moment-based invariant generator in which on can calculate moments of random variables of a PP without running the program.  
\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=4cm]{Figures/ExSampledandMora1Sample1000loop.eps}
% 	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1Sample1000loop1.eps}
	\caption{$x$-axis: iteration, $y$-axis: sampled values of the random variable. In red is the Mora generated $E(x)$, and in blue are the sampled values of the random variable in \textit{Random Walk 1D}.}
	\label{fig:SampledEXforRandomWalk1Sample1000loop1}
\end{figure}

\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=4cm]{Figures/ExSampledandMora1000loop1000Sample.eps}
	\includegraphics[width=4cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
	\caption{ $E(x)$ and $E(x^2)$ for Random Walk 1D using 1000 sample for each iteration of loop.}
	\label{fig:SampledEXforRandomWalk1000Sample1000loop1}
\end{figure}
\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=10cm,height=6cm]{Figures/absoluteErrorExRandomWalk1D.eps}\\
	\includegraphics[width=10cm,height=6cm]{Figures/relativeErrorExRandomWalk1D.eps}
	\caption{ Absolute and relative errors $E(x)$ and $E(x^2)$ for Random Walk 1D: \\
	Absolute Error of $E(x)= |{E(x)}_{sample}-{E(x)}_{exact}|$\\
	Absolute Error of $E(x^2)= |{E(x^2)}_{sample}-{E(x^2)}_{exact}|$\\
    Relative Error=$\frac{\text{Absolute Error}}{\text{Exact Value}}$}
	\label{fig:AbsoluteandRelativeErrorsRandomWalk1D}
\end{figure}








\begin{figure}[tpbh!]
	\centering
	\includegraphics[width=3.8cm]{Figures/histogramRandomwalk1D.eps}
	\includegraphics[width=3.8cm]{Figures/pdfRandomwalk1DME.eps}
	\includegraphics[width=3.8cm]{Figures/cdfRandomwalk1DME.eps}
	%\includegraphics[height=5.5cm]{Figures/Ex2SampledandMora1000loop1000Sample.eps}
	\caption{ Sampled (kernel density estimation) and Maximum Entropy Estimated Distribution for Random Walk 1D. Estimation of Distribution using Maximum Entropy method with 3 moments.}
	\label{fig:pdfRandomwalk1DME1}
\end{figure}

 







